Efficient nonparametric estimation of the covariate-adjusted threshold-response function, a support-restricted stochastic intervention

Identifying a biomarker or treatment-dose threshold that marks a specified level of risk is an important problem, especially in clinical trials. This risk, viewed as a function of thresholds and possibly adjusted for covariates, we call the threshold-response function. Extending the work of Donovan, Hudgens and Gilbert (2019), we propose a nonparametric efficient estimator for the covariate-adjusted threshold-response function, which utilizes machine learning and Targeted Minimum-Loss Estimation (TMLE). We additionally propose a more general estimator, based on sequential regression, that also applies when there is outcome missingness. We show that the threshold-response for a given threshold may be viewed as the expected outcome under a stochastic intervention where all participants are given a treatment dose above the threshold. We prove the estimator is efficient and characterize its asymptotic distribution. A method to construct simultaneous 95% confidence bands for the threshold-response function and its inverse is given. Furthermore, we discuss how to adjust our estimator when the treatment or biomarker is missing-at-random, as is the case in clinical trials with biased sampling designs, using inverse-probability-weighting. The methods are assessed in a diverse set of simulation settings with rare outcomes and cumulative case-control sampling. The methods are employed to estimate neutralizing antibody thresholds for virologically confirmed dengue risk in the CYD14 and CYD15 dengue vaccine trials.

==> bib.tex <==







@article{FrangakisRubin1999,
  title={Addressing complications of intention-to-treat analysis in the combined presence of all-or-none treatment-noncompliance and subsequent missing outcomes},
  author={Frangakis, Constantine E and Rubin, Donald B},
  journal={Biometrika},
  volume={86},
  number={2},
  pages={365--379},
  year={1999},
  publisher={Oxford University Press}
}

@article{Giorgietal2020,
author={Giorgi, Elena E and Li, Hui and Bhattacharya, T and Shaw, George M and Korber, Bette},
title={Estimating the timing of early SHIV infections: 
a comparison between Poisson Fitter and BEAST},
year={2020},
journal={submitted}
}


@article{wang2017identification,
  title={Identification and estimation of causal effects with outcomes truncated by death},
  author={Wang, Linbo and Zhou, Xiao-Hua and Richardson, Thomas S},
  journal={Biometrika},
  volume={104},
  number={3},
  pages={597--612},
  year={2017},
  publisher={Oxford University Press}
}

@article{McMichaeletal2009,
  title={The immune response during acute {HIV-1} infection: clues for vaccine development},
  author={McMichael, Andrew J and Borrow, Persephone and Tomaras, Georgia D and Goonetilleke, Nilu and Haynes, Barton F},
  journal={Nature Reviews Immunology},
  volume={10},
  number={1},
  pages={11--26},
  year={2009},
  publisher={Nature Publishing Group},
  note={PMCID: PMC3119211}
}

@article{HuangZhangetal2020,
author={Huang, Y and Zhang, Y and Bailer, R and Grunenberg, N and
 Carpp, LN and Seaton, K and Mayer, KH and Ledgerwood, J and
 Corey, L and Mascola, J and Montefiori, D and Gilbert, PB},
title={Prediction of serum {HIV-1} neutralization titers after 
passive administration of {VRC01}},
journal={Journal of AIDS},  
year={in press}
}

@article{Julienetal2019,
  title={Antibodies against Plasmodium falciparum malaria at the molecular level},
  author={Julien, Jean-Philippe and Wardemann, Hedda},
  journal={Nature Reviews Immunology},
  pages={1--15},
  year={2019},
  publisher={Nature Publishing Group}
}

@article{Seamanetal2019,
  title={Adjusting for time-varying confounders in survival analysis using structural nested cumulative survival time models},
  author={Seaman, Shaun and Dukes, Oliver and Keogh, Ruth and Vansteelandt, Stijn},
  journal={Biometrics},
  year={2019},
  publisher={Wiley Online Library}
}

@article{JoStuart2009,
  title={On the use of propensity scores in principal causal effect estimation},
  author={Jo, Booil and Stuart, Elizabeth A},
  journal={Statistics in Medicine},
  volume={28},
  number={23},
  pages={2857--2875},
  year={2009},
  publisher={Wiley Online Library}
}

@article{StuartJo2015,
  title={Assessing the sensitivity of methods for estimating principal causal effects},
  author={Stuart, Elizabeth A and Jo, Booil},
  journal={Statistical Methods in Medical Research},
  volume={24},
  number={6},
  pages={657--674},
  year={2015},
  publisher={SAGE Publications Sage UK: London, England}
}	

@article{DingLu2017,
  title={Principal stratification analysis using principal scores},
  author={Ding, Peng and Lu, Jiannan},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={79},
  number={3},
  pages={757--777},
  year={2017},
  publisher={Wiley Online Library}
}





@article{Benkeseretal2017,
  
title={Doubly robust nonparametric inference on the average treatment effect},
  
author={Benkeser, David and Carone, Marco and Laan, MJ Van Der and Gilbert, PB},
  
journal={Biometrika},
  volume={104},
  number={4},
  pages={863--880},
  
year={2017},
  publisher={Oxford University Press}
}

@article{HuangChoFong2019,
  title={Threshold-based subgroup testing in logistic regression models},
  author={Huang, Y and Cho, J and Fong, Y},
  journal={},
  volume={},
  number={},
  pages={},
  year={Submitted}
}


@article{Hanetal2017,
  title={Mark-specific additive hazards regression with continuous marks},
  author={Han, Dongxiao and Sun, Liuquan and Sun, Yanqing and Qi, Li},
  journal={Lifetime Data Analysis},
  volume={23},
  number={3},
  pages={467--494},
  year={2017},
  publisher={Springer},
  note={PMCID: PMC5319915}
}

@article{fiore2017sievesifter,
  title={{SieveSifter}: a web-based tool for visualizing the sieve analyses of {HIV-1} vaccine efficacy trials},
  author={Fiore-Gartland, Andrew and Kullman, Nicholas and Decamp, Allan C and Clenaghan, Graham and Yang, Wayne and Magaret, Craig A and Edlefsen, Paul T and Gilbert, Peter B},
  journal={Bioinformatics},
  volume={33},
  number={15},
  pages={2386--2388},
  year={2017},
  publisher={Oxford University Press},
  note={PMCID: PMC5860116}
}

@article{SpiekerHuang2017,
  title={A method to address between-subject heterogeneity for identification of principal surrogate markers in repeated low-dose challenge {HIV} vaccine studies},
  author={Spieker, AJ and Huang, Y}, 
  journal={Statistics in Medicine},
  volume={36},
  number={25},
  pages={4071--4080},
  year={2017},
  note={PMCID: PMC5669638}
}

@article{Qietal2019,
  title={Weighted estimators for additive risks models with missing covariates},
  author={Qi, L and Zhang, X and Sun, Y and Wang, L and Zhao, Y}, 
  journal={Annals of the Institute of Statistical Mathematics},
  volume={71},
  number={},
  pages={365--387},
  year={2019}
}

@article{Pilcheretal2019,
  title={A generalizable method for estimating duration of {HIV} infections using clinical testing history and {HIV} test results},
  author={Pilcher, Christopher D and Porco, Travis C and Facente, Shelley N and Grebe, Eduard and Delaney, Kevin P and Masciotra, Silvina and Kassanjee, Reshma and Busch, Michael P and Murphy, Gary and Owen, S Michele and {Alex Welte, on behalf of the Consortium for the Evaluation and Performance of HIV Incidence Assays (CEPHIA)}},
  journal={AIDS},
  volume={33},
  number={7},
  pages={1231--1240},
  year={2019},
  publisher={LWW},
  note={PMCID:
    PMC6561657
    [Delayed release (embargo): Available on 2020-06-01]}
}

@article{Grebeetal2018,
  title={Interpreting Diagnostic Histories into {HIV} Infection Time Estimates: Framework and Online Tool},
  author={Grebe, Eduard and Facente, Shelley N and Bingham, Jeremy and Pilcher, Christopher D and Powrie, Andrew and Gerber, Jarryd and Priede, Gareth and Chibawara, Trust and Busch, Michael P and Murphy, Gary and Kassanjee, Reshma and {Alex Welte, on behalf of the Consortium for the Evaluation and Performance of HIV Incidence Assays (CEPHIA)}},
  journal={},
  pages={},
  year={},
  publisher={Cold Spring Harbor Laboratory},
  note={doi: https://doi.org/10.1101/323808. [Preprint] 18 May, 2018. Cited 3 Sep, 2019. Available from https://www.biorxiv.org/content/10.1101/323808v1.full}
}


@article{LeDelletal2016,
  title={{AUC}-maximizing ensembles through metalearning},
  author={LeDell, Erin and van der Laan, Mark J and Petersen, Maya},
  journal={The International Journal of Biostatistics},
  volume={12},
  number={1},
  pages={203--218},
  year={2016},
  publisher={De Gruyter},
  note={PMCID:
    PMC4912128 }
}


@article{Janesetal2019,
  title={Taking stock of the present and looking to the future: Envisioning challenges in the design of future {HIV} prevention efficacy trials},
  author={Janes, HE and Donnell, D and Gilbert, Peter B and Brown, ER and Nason, M},
  journal={Lancet HIV},
  volume={},
  number={},
  url={},
  pages={11--26},
  year={2019},
  note={PMCID:
    PMC6612578
    [Delayed release (embargo): Available on 2020-07-01]}
}



@inproceedings{ling2003auc,
  title={{AUC}: a statistically consistent and more discriminating measure than accuracy},
  author={Ling, Charles X and Huang, Jin and Zhang, Harry},
  booktitle={IJCAI},
  volume={3},
  pages={519--524},
  year={2003}
}

@article{bradley1997use,
  title={The use of the area under the {ROC} curve in the evaluation of machine learning algorithms},
  author={Bradley, Andrew P},
  journal={Pattern Recognition},
  volume={30},
  number={7},
  pages={1145--1159},
  year={1997},
  publisher={Elsevier}
}

@article{Neidichetal2019,
  title={Antibody Fc effector functions and IgG3 associate with decreased HIV-1 risk},
  author={Neidich, Scott D and Fong, Youyi and Li, Shuying S and Geraghty, Daniel E and Williamson, Brian D and Young, William Chad and Goodman, Derrick and Seaton, Kelly E and Shen, Xiaoying and Sawant, Sheetal and others},
  journal={Journal of Clinical Investigation},
  volume={129},
  number={11},
  pages={4838--4849},
  year={2019},
  publisher={Am Soc Clin Investig}
}
 
@article{ledell2015computationally,
  title={Computationally efficient confidence intervals for cross-validated area under the {ROC} curve estimates},
  author={LeDell, Erin and Petersen, Maya and van der Laan, Mark},
  journal={Electronic Journal of Statistics},
  volume={9},
  number={1},
  pages={1583},
  year={2015},
  publisher={NIH Public Access},
  note={PMCID:
    PMC4533123}
}

@article{breiman1996stacked,
  title={Stacked regressions},
  author={Breiman, Leo},
  journal={Machine Learning},
  volume={24},
  number={1},
  pages={49--64},
  year={1996},
  publisher={Springer}
}, 

@article{GilbertHuang2016,
  title={Predicting overall vaccine efficacy in a new setting by re-calibrating baseline covariate and intermediate response endpoint effect modifiers of type-specific vaccine efficacy},
  author={Gilbert, Peter B and Huang, Ying},
  journal={Epidemiologic Methods},
  volume={5},
  number={1},
  pages={93--112},
  year={2016},
  publisher={De Gruyter},
  note={PMCID:
    PMC5279575}
}

@article{FongGilbert2015,
  title={Calibration weighted estimation of semiparametric transformation models for two-phase sampling},
  author={Fong, Youyi and Gilbert, Peter},
  journal={Statistics in Medicine},
  volume={34},
  number={10},
  pages={1695--1707},
  year={2015},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC4390487}
}

@article{fong2017chngpt,
  title={chngpt: threshold regression model estimation and inference},
  author={Fong, Youyi and Huang, Ying and Gilbert, Peter B and Permar, Sallie R},
  journal={BMC Bioinformatics},
  volume={18},
  number={1},
  pages={454},
  year={2017},
  publisher={BioMed Central},
  note={PMCID: PMC5644082}
}

@article{FongDietal2017,
  title={Model-robust inference for continuous threshold regression models},
  author={Fong, Youyi and Di, Chongzhi and Huang, Ying and Gilbert, Peter B},
  journal={Biometrics},
  volume={73},
  number={2},
  pages={452--462},
  year={2017},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC5435560}
}

@article{Qiuetal2019,
  title={Smoothed Rank Regression for the Accelerated Failure Time Competing Risks Model with Missing Cause of Failure},
  author={Qiu, Z and Wan, ATK and Zhou, Y and Gilbert, Peter B},
  journal={Statistica Sinica},
  volume={29},
  number={1},
  pages={23--46},
  year={2019},
  note={PMCID:
    PMC6364751
    [Delayed release (embargo): Available on 2020-01-01]}
}

@Manual{JuraskaRpackage2018,
    title = {pssmooth: Flexible and Efficient Evaluation of Principal Surrogates/Treatment Effect Modifiers},
    author = {Michal Juraska},
    year = {2018},
    note = {R package version 1.0.1},
  }


@article{Dunningetal2015,
  title={Some extensions in continuous models for immunological correlates of protection},
  author={Dunning, Andrew J and Kensler, Jennifer and Coudeville, Laurent and Bailleux, Fabrice},
  journal={BMC Medical Research Methodology},
  volume={15},
  number={1},
  pages={107},
  year={2015},
  publisher={BioMed Central}
}


@article{Dunningetal2016,
  title={Correlates of protection against influenza in the elderly: results from an influenza vaccine efficacy trial},
  author={Dunning, Andrew J and DiazGranados, Carlos A and Voloshen, Timothy and Hu, Branda and Landolfi, Victoria A and Talbot, H Keipp},
  journal={Clinical and Vaccine Immunology},
  pages={CVI--00604},
  year={2016},
  publisher={Am Soc Microbiol}
}

@article{PearlBareinboim2014,
author={Pearl, J and Bareinboim, E},
title={External validity: From {D}o-calculus to transportability across populations},
journal={Statistical Science},
volume={29},
number={4},
year={2014},
pages={579--595}
}

@article{HuangFong2014,
  title={Identifying optimal biomarker combinations for treatment selection via a robust kernel method},
  author={Huang, Ying and Fong, Youyi},
  journal={Biometrics},
  volume={70},
  number={4},
  pages={891--901},
  year={2014},
  publisher={Wiley Online Library},
  note={PMCID: PMC4277554}
}

@article{FongHuangetal2017,
author={Fong, Y and Huang, Y and Gilbert, Peter B and Permar, S},
title={chngpt: {T}hreshold regression model estimation and inference},
journal={BMC Bioinformatics},
volume={18},
number={454},
year={2017},
note={PMCID:
    PMC5644082}
}

@article{SunQianShouGilbert2017,
author={Sun, Y and Qian, X and Shou, Q and Gilbert, Peter B},
title ={Analysis of two-phase sampling data with semiparametric additive hazards models},
journal={Lifetime Data Analysis},
year={2017},
volume={23},
number={3},
pages={377--399},
note={PMCID:
    PMC5309201}
}

@misc{lee1990u,
  title={U-statistics, volume 110 of Statistics: Textbooks and Monographs},
  author={Lee, Alan J},
  year={1990},
  publisher={Marcel Dekker Inc., New York. Theory and practice}
}

@article{LeeSunScheikeGilbert2018,
author={Lee, U and Sun, Y and Scheike, T and Gilbert, Peter B},
title ={Analysis of generalized semiparametric regression models for cumulative incidence functions with missing covariates},
journal={Computational Statistics and Data Analysis},
year={2018},
volume={122},
number={},
pages={59--79},
note={PMCID: PMC5993453}
}	  


@article{Montoetal2015JID,
  title={Antibody to influenza virus neuraminidase: an independent correlate of protection},
  author={Monto, Arnold S and Petrie, Joshua G and Cross, Rachel T and Johnson, Emileigh and Liu, Merry and Zhong, Weimin and Levine, Min and Katz, Jacqueline M and Ohmit, Suzanne E},
  journal={Journal of Infectious Diseases},
  pages={jiv195},
  year={2015},
  publisher={Oxford University Press}
}

@article{Zambonellietal2016,
title={Generation and Characterization of a Bivalent {HIV-1} Subtype {C} gp120 Protein Boost for Proof-of-Concept {HIV} Vaccine Efficacy Trials in {S}outhern {A}frica},
author={Carlo Zambonelli , Antu K. Dey  , Susan Hilt, Samuel Stephenson, Eden P. Go, Daniel F. Clark, Mark Wininger, Celia Labranche, David Montefiori, Hua-Xin Liao, Ronald I. Swanstrom, Heather Desaire, Barton F. Haynes, Andrea Carfi , Susan W. Barnett},
journal={PLoS One},
year={2016}
}

@article{PrenticePyke1979,
  title={Logistic disease incidence models and case-control studies},
  author={Prentice, RL and Pyke, R},
  journal={Biometrika},
  volume={66},
  pages={403--411},
  year={1979}
}


@article{Montoetal2009NEJM,
  title={Comparative efficacy of inactivated and live attenuated influenza vaccines},
  author={Monto, Arnold S and Ohmit, Suzanne E and Petrie, Joshua G and Johnson, Emileigh and Truscon, Rachel and Teich, Esther and Rotthoff, Judy and Boulton, Matthew and Victor, John C},
  journal={New England Journal of Medicine},
  volume={361},
  number={13},
  pages={1260--1267},
  year={2009},
  publisher={Mass Medical Soc}
}

@article{DonovanHudgensGilbert2017,
  title={Non-parametric statistical methods for immune
response thresholds of risk},
  author={Donovan, KM and Hudgens, MG and Gilbert, Peter B},
  journal={submitted},
  volume={},
  number={},
  pages={},
  year={2018}
}

@article{zhuangetal2019simultaneous,
  title={Simultaneous Inference of Treatment Effect Modification by Intermediate Response Endpoint Principal Strata with Application to Vaccine Trials},
  author={Zhuang, Yingying and Huang, Ying and Gilbert, Peter B},
  journal={The International Journal of Biostatistics},
  year={2019},
  publisher={De Gruyter}
}

@article{DonovanHudgensGilbert2019,
  title={Nonparametric inference for immune response thresholds of risk in vaccine studies},
  author={Donovan, KM and Hudgens, MG and Gilbert, Peter B},
  journal={Annals of Applied Statistics},
volume={13},
  number={2},
  pages={1147--1165},
  year={2019},
  publisher={Institute of Mathematical Statistics},
  note={PMCID:
    PMC6613658
    [Delayed release (embargo): Available on 2020-06-01]}}


@article{StewartJonesetal2016,
  title={Trimeric {HIV}-1-{E}nv structures define glycan shields from clades {A}, {B}, and {G}},
  author={Stewart-Jones, Guillaume BE and Soto, Cinque and Lemmin, Thomas and Chuang, Gwo-Yu and Druz, Aliaksandr and Kong, Rui and Thomas, Paul V, and et al.},
  journal={Cell},
  volume={165},
  number={},
  pages={813--826},
  year={2016}
}

@article{GilbertZhangRudnickiHuang2019,
  title={Assessing pharmacokinetic marker correlates of outcome, with application to antibody prevention efficacy trials},
  author={Gilbert, Peter B and Zhang, Yuanyuan and Rudnicki, Erika and Huang, Yunda},
  journal={Statistics in Medicine},
  year={2019},
  publisher={Wiley Online Library},
  doi={https://doi.org/10.1002/sim.8310},
  note={In Press. doi: 10.1002/sim.8310. PubMed PMID: 31313349, NIHMSID: NIHMS1037312.}
}

@article{GabrielFollmann2016,
  title={Augmented trial designs for evaluation of principal surrogates},
  author={Gabriel, E and Follmann, D},
  journal={Biostatistics},
  volume={},
  number={},
  pages={453--467},
  year={2016}
}

@article{Pearl2013,
  title={Discussion on ``{S}urrogate {M}easures and {C}onsistent {S}urrogates"},
  author={Pearl, Judea},
  journal={Biometrics},
  volume={69},
  number={3},
  pages={573--577},
  year={2013},
  publisher={Wiley Online Library}
}

@article{Joffe2013,
  title={Discussion on ``{S}urrogate {M}easures and {C}onsistent {S}urrogates"},
  author={Joffe, M},
  year={2013},
  journal={Biometrics},
  volume={69},
  pages={572--575}
}


@article{Capedingetal2014,
  title={Clinical efficacy and safety of a novel tetravalent dengue vaccine in healthy children in {Asia}: a phase 3, randomised, observer-masked, placebo-controlled trial},
  author={Capeding, Maria Rosario and Tran, Ngoc Huu and Hadinegoro, Sri Rezeki S and Ismail, Hussain Imam HJ Muhammad and Chotpitayasunondh, Tawee and Chua, Mary Noreen and Luong, Chan Quang and Rusmil, Kusnandi and Wirawan, Dewa Nyoman and Nallusamy, Revathy and Pitisuttithum, Punnee and Thisyakorn, Usa and Yoon, In-Kyu and van der Vliet, Diane and Langevin, Edith and Laot, Thelma and Hutagalung, Yanee and Frago, Carina and Boaz, Mark and Wartel, T Anh and Tornieporth, Nadia G and Saville, Melanie and Bouckenooghe, Alain and the CYD14 Study Group,},
  journal={The Lancet},
  volume={384},
  number={9951},
  pages={1358--1365},
  year={2014},
  publisher={Elsevier}
}

@article{Sridharetal2018,
  title={Effect of Dengue Serostatus on Dengue Vaccine Safety and Efficacy},
  author={Sridhar, Saranya and Luedtke, Alexander and Langevin, Edith and Zhu, Ming and Bonaparte, Matthew and Machabert, Tifany and Savarino, Stephen and Zambrano, Betzana and Moureau, Annick and Khromava, Alena and Moodie, Zoe and Westling, Ted and Mascare{\~n}as, Cesar and Frago, Carina and Cort\'es, Margarita and Chansinghakul, Danaya and Noriega, Fernando and Bouckenooghe, Alain and Chen, Josh and Ng, Su-Peing and Gilbert, Peter B and Gurunathan, Sanjay and DiazGranados, Carlos A},
  journal={New England Journal of Medicine},
  year={2018},
  publisher={Mass Medical Soc},
  note={DOI:
    10.1056/NEJMoa1800820}
}


@article{Hadinegoroetal2015,
  title={Efficacy and long-term safety of a dengue vaccine in regions of endemic disease},
  author={Hadinegoro, Sri Rezeki and Arredondo-Garc{\'\i}a, Jose Luis and Capeding, Maria Rosario and Deseda, Carmen and Chotpitayasunondh, Tawee and Dietze, Reynaldo and Hj Muhammad Ismail, HI and Reynales, Humberto and Limkittikul, Kriengsak and Rivera-Medina, Doris Maribel and others},
  journal={New England Journal of Medicine},
  volume={373},
  number={13},
  pages={1195--1206},
  year={2015},
  publisher={Mass Medical Soc}
}

@article{Capedingetal2014short,
  title={Clinical efficacy and safety of a novel tetravalent dengue vaccine in healthy children in {Asia}: a phase 3, randomised, observer-masked, placebo-controlled trial},
  author={Capeding, Maria Rosario and Tran, Ngoc Huu and Hadinegoro, Sri Rezeki S  and Ismail, Hussain Imam HJ Muhammad and Chotpitayasunondh, Tawee and Chua, Mary Noreen and others},
  journal={The Lancet},
  volume={384},
  number={9951},
  pages={1358--1365},
  year={2014},
  publisher={Elsevier}
}

@article{Villaretal2015,
  title={Efficacy of a tetravalent dengue vaccine in children in {L}atin {A}merica},
  author={Villar, Luis and Dayan, Gustavo Horacio and Arredondo-Garc{\'\i}a, Jos{\'e} Luis and Rivera, Doris Maribel and Cunha, Rivaldo and Deseda, Carmen and Reynales, Humberto and Costa, Maria Selma and Morales-Ram{\'\i}rez, Javier Osvaldo and Carrasquilla, Gabriel and Rey, Luis Carlos and Dietze, Reynaldo and Luz, Kleber and Rivas, Enrique and Montoya, Maria Consuelo Miranda and Supelano, Margarita Cort\'es and Zambrano, Betzana and Langevin, Edith and Boaz, Mark and Tornieporth, Nadia and Saville, Melanie and {Fernando Noriega for the CYD15 Study Group}},
  journal={New England Journal of Medicine},
  year={2015},
  volume={372},
  pages={113-123},
  publisher={Mass Medical Soc},
  note={DOI:
    10.1056/NEJMoa1411037}
}

@article{Villaretal2015short,
  title={Efficacy of a tetravalent dengue vaccine in children in {Latin America}},
  author={Villar, Luis and Dayan, Gustavo Horacio and Arredondo-Garc{\'\i}a, Jos{\'e} Luis and Rivera, Doris Maribel and Cunha, Rivaldo and Deseda, Carmen and others},
  journal={New England Journal of Medicine},
  year={2015},
  volume={372},
  pages={113-123},
  publisher={Mass Medical Soc}
}

@article{KobayashiKuroki2014,
  title={A new proportion measure of the treatment effect captured by candidate surrogate endpoints},
  author={Kobayashi, Fumiaki and Kuroki, Manabu},
  journal={Statistics in Medicine},
  year={2014},
  volume={33},
  pages={3338-3353},
  publisher={Wiley Online Library}
}


@article{MurphyvanderVaart2000,
  title={On profile likelihood},
  author={Murphy, SA and Van der Vaart, AW},
  journal={Journal of the American Statistical Association},
  year={2000},
  volume={95},
  number={450},
  pages={449-465}
}


@article{little2012prevention,
  title={The prevention and treatment of missing data in clinical trials},
  author={Little, Roderick J and D'Agostino, Ralph and Cohen, Michael L and Dickersin, Kay and Emerson, Scott S and Farrar, John T and Frangakis, Constantine and Hogan, Joseph W and Molenberghs, Geert and Murphy, Susan A and others},
  journal={New England Journal of Medicine},
  volume={367},
  number={14},
  pages={1355--1360},
  year={2012},
  publisher={Mass Medical Soc}
}

@article{LendleSubbaramanvanderLaan2013,
  title={Identification and Efficient Estimation of the Natural Direct Effect among the Untreated},
  author={Lendle, SD and Subbaraman, MS and van der Laan, MJ},
  journal={Biometrics},
  volume={69},
  number={2},
  pages={310--317},
  year={2013} 
}

@article{Parketal2011,
  title={Designing a genome-based {HIV} incidence assay with high sensitivity and specificity},
  author={Park, Sung Yong and Love, Tanzy MT and Nelson, Jeremy and Thurston, Sally W and Perelson, Alan S and Lee, Ha Youn},
  journal={AIDS (London, England)},
  volume={25},
  number={16},
  pages={F13--F19},
  year={2011},
  publisher={NIH Public Access},
note = {PMCID: PMC3319025}

}

@article{Giorgietal2010,
  title={Estimating time since infection in early homogeneous {HIV-1} samples using a poisson model},
  author={Giorgi, Elena and Funkhouser, Bob and Athreya, Gayathri and Perelson, Alan and Korber, Bette and Bhattacharya, Tanmoy},
  journal={BMC Bioinformatics},
  volume={11},
  number={1},
  pages={532},
  year={2010},
  publisher={BioMed Central Ltd},
  note={PMCID: PMC2975664}
}

@article{Giorgietal2012,
  title={A note on two-sample tests for comparing intra-individual genetic sequence diversity between populations},
  author={Giorgi, EE and Bhattacharya, T},
  journal={Biometrics},
  volume={68},
  number={4},
  pages={1323--1326},
  year={2012},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC3652673
}
}


@article{coudeville2016estimation,
  title={Estimation of parameters related to vaccine efficacy and dengue transmission from two large phase {III} studies},
  author={Coudeville, Laurent and Baurin, Nicolas and Vergu, Elisabeta},
  journal={Vaccine},
  volume={34},
  number={50},
  pages={6417--6425},
  year={2016},
  publisher={Elsevier},
  note={DOI:
    10.1016/j.vaccine.2015.11.023}
}

@article{Koffetal2013,
  title={Accelerating next-generation vaccine development for global disease prevention.},
  author={Koff, WC and Burton, DR and Johnson, PR and Walker, BD and King, CR and Nabel, GJ and Ahmed, R and Bhan, MK and Plotkin, SA},
  journal={Science},
  volume={340},
  number={1},
  pages={},
  year={2013},
  note={PMCID:
    PMC4026248}
}

@Book{WandJones1995,
  author =          {Wand, MP and Jones, MC},
  ALTeditor =          {},
  title =          {Kernel Smoothing},
  publisher =          {Chapman \& Hall Ltd },
  year =          {1995},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {London; New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Book{vanderVaartWellner,
  author =          {van der Vaart, A and Wellner, JA},
  ALTeditor =          {},
  title =          {Weak Convergence and Empirical Processes},
  publisher =          {Springer},
  year =          {1996},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}




@incollection{PlotkinGilbert2018,
  author       = {Plotkin, S and Gilbert, Peter B}, 
  title        = {Correlates of protection},
  booktitle    = {Vaccines, Seventh Edition},
  publisher    = {Elsevier Inc.},
  year         = {2018},
  editor       = {Plotkin, S and Orenstein, Walter and Offit, Paul  and Edwards, Kathryn},
  volume       = {},
  series       = {},
  chapter      = {},
  pages        = {35--40},
  address      = {New York},
  edition      = {},
  month        = {},
  note         = {}
}

@Book{WandJones1995,
  author =          {Wand, MP and Jones, MC},
  ALTeditor =          {},
  title =          {Kernel Smoothing},
  publisher =          {Chapman \& Hall Ltd },
  year =          {1995},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {London; New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Book{Carrolletal2006,
  author =          {Carroll, RJ and Ruppert, D and Stefanski, LA and Crainiceanu, C},
  ALTeditor =          {},
  title =          {{Measurement Error in Nonlinear Models: A Modern Perspective, Second Edition}},
  publisher =          {Chapman and Hall},
  year =          {2006},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {London},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@article{Grayetal2011,
  title={Safety and efficacy of the {HVTN 503/Phambili study} of a clade-{B}-based {HIV-1} vaccine in South Africa: a double-blind, randomised, placebo-controlled test-of-concept phase {2b} study},
  author={Gray, Glenda E and Allen, Mary and Moodie, Zoe and Churchyard, Gavin and Bekker, Linda-Gail and Nchabeleng, Maphoshane and Mlisana, Koleka and Metch, Barbara and de Bruyn, Guy and Latka, Mary H and others},
  journal={The Lancet Infectious Diseases},
  volume={11},
  number={7},
  pages={507--515},
  year={2011},
  publisher={Elsevier},
  note={PMCID: PMC3417349}
}

@article{Fukazawaetal2012,
  title={Lymph node {T} cell responses predict the efficacy of live attenuated {SIV} vaccines},
  author={Fukazawa, Yoshinori and Park, Haesun and Cameron, Mark J and Lefebvre, Francois and Lum, Richard and Coombes, Noel and Mahyari, Eisa and Hagen, Shoko I and Bae, Jin Young and Reyes III, Marcelo Delos and Swanson,	 T and Legasse, Alfred W and Sylwester,	A and Hansen, Scott G and Smith, Andrew T	and Stafova, Petra and Shoemaker, Rebecca and Li, Yuan and Oswald, Kelli and Axthelm, Michael K and McDermott, Adrian and Ferrari, Guido and Montefiori, David C and Edlefsen,	 Paul T and Piatak Jr, Michael and Lifson, Jeffrey D and Sekaly, Rafick P and Picker, LJ},
  journal={Nature Medicine},
  volume={18},
  number={11},
  pages={1673--1681},
  year={2012},
  note={PMCID: PMC3493820}
}

@article{Hansenetal2013,
  title={Immune clearance of highly pathogenic {SIV} infection},
  author={Hansen, Scott G and Piatak Jr, Michael and Ventura, Abigail B and Hughes, Colette M and Gilbride, Roxanne M and Ford, Julia C and Oswald, Kelli and Shoemaker, Rebecca and Li, Yuan and Lewis, Matthew S and Gilliam, Awbrey N and Xu, Guangwu and	 Whizin, Nathan and Burwitz, Benjamin J and Planer, Shannon L and Turner, John M and Legasse,	 Alfred W and Axthelm, Michael K  and Nelson, Jay A and Fruh, Klaus and Sacha, Jonah B and Estes,	 Jacob D and Keele,	Brandon F and Edlefsen, Paul T and	Lifson, Jeffrey D and Picker, Louis LJ},
  journal={Nature},
  volume={502},
  number={7469},
  pages={100--104},
  year={2013},
  note={PMCID: NIHMS512106}
}

@article{Hansenetal2013cytomegalovirus,
  title={Cytomegalovirus vectors violate {CD8+} {T} cell epitope recognition paradigms},
  author={Hansen, Scott G and Sacha, Jonah B and Hughes, Colette M and Ford, Julia C and Burwitz, Benjamin J and Scholz, Isabel and Gilbride, Roxanne M and Lewis, Matthew S and Gilliam, Awbrey N and Ventura, Abigail B and Malouli, Daniel and Xu, Guangwu and Richards, Rebecca and Whizin, Nathan and Reed, Jason S and Hammond, Katherine B and Fischer, Miranda and Turner, John M and Legasse, Alfred W and Axthelm, Michael K and Edlefsen, Paul T and Nelson, Jay A and Lifson, Jeffrey D and Fruh, Klaus and Picker, LJ},
  journal={Science},
  volume={340},
  number={6135},
  year={2013},
  publisher={American Association for the Advancement of Science},
  note={PMCID: NIHMS493094}
}

@article{Flatzetal2012,
  title={Gene-based vaccination with a mismatched envelope protects against simian immunodeficiency virus infection in nonhuman primates},
  author={Flatz, Lukas and Cheng, Cheng and Wang, Lingshu and Foulds, Kathryn E and Ko, Sung-Youl and Kong, Wing-Pui and Roychoudhuri, Rahul and Shi, Wei and Bao, Saran and Todd, John-Paul and et., al and Mascola, JR and Roederer, M and Nabel, GJ},
  journal={Journal of Virology},
  volume={86},
  number={15},
  pages={7760--7770},
  year={2012},
  publisher={Am Soc Microbiol},
  note={PMCID: PMC3421661}
}


@Book{Nelsen1999,
  author =          {Nelson, RB},
  ALTeditor =          {},
  title =          {An Introduction to Copulas},
  publisher =          {Springer},
  year =          {1999},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Book{Pearl2000,
  author =          {Pearl, J},
  ALTeditor =          {},
  title =          {Causality: models, reasoning, and inference}, 
  publisher =          {Cambridge University Press }, 
  year =          {2000},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {London},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Book{Pearl2009,
  author =          {Pearl, J},
  ALTeditor =          {},
  title =          {Causality: {M}odels, {R}easoning, and {I}nference, {Second} {E}dition},
  publisher =          {Cambridge University Press },
  year =          {2009},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {London},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@article{FlemingPowers2012,
  title={Biomarkers and surrogate endpoints in clinical trials},
  author={Fleming, Thomas R and Powers, John H},
  journal={Statistics in medicine},
  volume={31},
  number={25},
  pages={2973--2984},
  year={2012},
  publisher={Wiley Online Library}
}


@Book{FlemingHarrington1991,
  author =          {Fleming, TR and Harrington, DP},
  ALTeditor =          {},
  title =          {Counting processes and survival analysis},
  publisher =          {John Wiley \& Sons},
  year =          {1991},
  OPTkey =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}




@Article{Robins1995,
  author =          {Robins, JM},
  title =          {An analytic method for randomized trials with informative censoring: {P}art $\mbox{I}$},
  journal =          {Lifetime Data Analysis},
  year =          {1995},
  OPTkey =          {},
  volume =          {1},
  OPTnumber =          {},
  pages =          {241--254},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Article{Tianetal2012,
  author =          {Tian, L and Cai, T and Zhao, L and Wei, LJ},
  title =          {On the covariate adjustment for an overall treatment difference with data from a randomized comparative clinical trial},
  journal =          {Biostatistics},
  year =          {2012},
  OPTkey =          {},
  volume =          {13},
  OPTnumber =          {},
  pages =          {256-273},
  note={PMCID: PMC3297822}
}

@Article{VittinghoffBauer2006,
  author =          {Vittinghoff, E and Bauer, DC},
  title =          {Case-only analysis of treatment-covariate interactions in
clinical trials},
  journal =          {Biometrics},
  year =          {2006},
  OPTkey =          {},
  volume =          {62},
  OPTnumber =          {},
  pages =          {769--776}
}

@Article{Daietal2012,
  author =          {Dai, JY and Logsdon, BA and Huang, Y and Hsu, L and Reiner, AP and Prentice, RL and Kooperberg, C},
  title =          {Simultaneously testing for marginal genetic association and gene-environment interaction},
  journal =          {American Journal of Epidemiology},
  year =          {2012},
  OPTkey =          {},
  volume =          {176},
  OPTnumber =          {},
  pages =          {164--173},
  note={PMCID: PMC3499112}
}


@Article{LongHudgensbiom2013,
  author =          {Long, DM and Hudgens, MG},
  title =          {Sharpening bounds on principal effects with covariates},
  journal =          {Biometrics},
  year =          {2013},
  OPTkey =          {},
  volume =          {69},
  OPTnumber =          {},
  pages =          {812--819},
  note={PMCID: PMC4086842}
}

@Article{SunQianShouGilbert2013,
  author =          {Sun, Y and Qian, X and Shou, Q and Gilbert, Peter B}, 
  title =          {Semiparametric additive
hazards regression models for case-cohort/two- phase sampling designs},
  journal =          {Scandinavian Journal of Statistics, Under Revision},
  year =          {2013},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {},
  note={PMCID: PMC}
}


@Article{Laietal2011,
  author =          {Lai, L and Kwa, S and Kozlowski, PA and Montefiori, DC and Ferrari, G and Johnson, WE and Hirsch, V and Villinger, F and Chennareddi, L and Earl, PL and Moss, B and Amara, RR and Robinson, HL},
  title =          {Prevention of infection by a granulocyte-macrophage colony-stimulating factor co-expressing {DNA}/modified vaccinia {Ankara} simian immunodeficiency virus vaccine},
  journal =          {The Journal of Infectious Diseases},
  year =          {2011},
  OPTkey =          {},
  volume =          {204},
  OPTnumber =          {},
  pages =          {164--173},
  note={PMCID: PMC3143670}
}

@article{lee2008semiparametric,
  title={Semiparametric estimation of a binary response model with a change-point due to a covariate threshold},
  author={Lee, Sokbae and Seo, Myung Hwan},
  journal={Journal of Econometrics},
  volume={144},
  number={2},
  pages={492--499},
  year={2008},
  publisher={Elsevier}
}

@article{zhong2008bias,
  title={Bias-reduced estimators and confidence intervals for odds ratios in genome-wide association studies},
  author={Zhong, Hua and Prentice, Ross L},
  journal={Biostatistics},
  volume={9},
  number={4},
  pages={621--634},
  year={2008},
  publisher={Biometrika Trust},
  note={PMCID: PMC2536726}
}




@article{Laietal2012,
  title={{SIVmac239 MVA} vaccine with and without a {DNA} prime, similar prevention of infection by a repeated dose {SIVsmE660} challenge despite different immune responses},
  author={Lai, Lilin and Kwa, Sue-Fen and Kozlowski, Pamela A and Montefiori, David C and Nolen, Tracy L and Hudgens, Michael G and Johnson, Welkin E and Ferrari, Guido and Hirsch, Vanessa M and Felber, Barbara K and others},
  journal={Vaccine},
  volume={30},
  number={9},
  pages={1737--1745},
  year={2012},
  publisher={Elsevier},
  note={PMCID: PMC3278564}
}

@article{Winstoneetal2011,
  title={Enhanced control of pathogenic {Simian} immunodeficiency virus {SIVmac239} replication in macaques immunized with an interleukin-12 plasmid and a {DNA} prime-viral vector boost vaccine regimen},
  author={Winstone, Nicola and Wilson, Aaron J and Morrow, Gavin and Boggiano, Cesar and Chiuchiolo, Maria J and Lopez, Mary and Kemelman, Marina and Ginsberg, Arielle A and Mullen, Karl and Coleman, John W and Hudgens, MG and others},
  journal={Journal of Virology},
  volume={85},
  number={18},
  pages={9578--9587},
  year={2011},
  publisher={Am Soc Microbiol},
  note={PMCID: PMC3165762}
}


@article{LiSun2016,
  title={Semiparametric random effects models for longitudinal data with informative observation times},
  author={Li, Yang and Sun, Yanqing},
  journal={Statistics and its interface},
  volume={9},
  number={3},
  pages={333},
  year={2016},
  publisher={NIH Public Access}
}

@Article{Jiangetal2013,
  author =          {Jiang, J and Ghosh, L and Sun, Y and Zhou, H}, 
  title =          {Failure time regression
with continuous informative auxiliary covariates},
  journal =          {under revision},
  year =          {2013},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {}
}



@Article{TherneauLi1999,
  author =          {Therneau, T and Li, H},
  title =          {Computing the $\mbox{Cox}$ model for case-cohort designs.},
  journal =          {Lifetime Data Analysis},
  year =          {1999},
  OPTkey =          {},
  volume =          {5},
  OPTnumber =          {},
  pages =          {99--112}
}

@Article{Borganetal2000,
  author =          {Borgan, L and Langholz, B and Samuelson, S and Pogoda, J},
  title =          {Exposure stratified case-cohort designs},
  journal =          {Lifetime Data Analysis},
  year =          {2000},
  OPTkey =          {},
  volume =          {6},
  OPTnumber =          {},
  pages =          {39--58}
}

@Article{Haynesetal2012,
  author =          {Haynes, BF and  Gilbert, Peter B and McElrath, MJ and et al.},
  title =          {Immune correlates analysis of the $\mbox{ALVAC-AIDSVAX 
HIV-1}$ vaccine efficacy trial},
  journal =          {New England Journal of Medicine},
  year =          {2012},
  OPTkey =          {},
  volume =          {366},
  OPTnumber =          {},
  pages =          {1275--1286}
}
%  note = {PMCID: PMC3371689}

@Article{LiParnesChan2013,
  author =          {Li, S and Parnes, M and Chan, ISF},
  title =          {Determining the cutoff based on a continuous variable to define two populations with application to vaccines},
  journal =          {Journal of Biopharmaceutical Statistics},
  year =          {2013},
  OPTkey =          {},
  volume =          {23},
  OPTnumber =          {},
  pages =          {662--680}
}


@Article{Liaoetal2013,
  author =          {Liao, H-X and Bonsignori, M and Alam, SM and et al.},
  title =          {Vaccine Induction of Antibodies against a Structurally Heterogeneous Site of Immune Pressure within $\mbox{HIV-1}$ Envelope Protein Variable Regions 1 and 2.},
  journal =          {Immunity},
  year =          {2013},
  OPTkey =          {},
  volume =          {38},
  OPTnumber =          {},
  pages =          {176--186}
}
%  note={PMCID: PMC3569735}

@article{Rollandetal2011,
  title={Genetic impact of vaccination on breakthrough $\mbox{HIV-1 sequences from the STEP trial}$.},
  author={Rolland, M and Tovanabutra, S and deCamp, A and Frahm, N and Gilbert, Peter B and Sanders-Buell, E and 
Heath, L and Magaret, CA and Bose, M and Bradfield, A and
O'Sullivan, A and Crossler, J and Jones, T and Nau, M and Wong, K and Zhao, H and Raugi, DN and Sorensen, S and
 Stoddard, JN and Maust, BS and Deng, W and Hural, J and Dubey, S and Michael, NL and Shiver, J and Corey, L and
 Li, F and Self, SG and Kim, J and Buchbinder, S and Casimiro, DR and Robertson, MN and Duerr, A and
 McElrath, MJ and McCutchan, FE and Mullins, JI},
  journal={Nature Medicine},
  volume={17},
  number={3},
  pages={366--371},
  year={2011},
  publisher={Nature Publishing Group},
  note={PMCID: PMC3053571}
}

@article{Rollandetal2011short,
  title={Genetic impact of vaccination on breakthrough $\mbox{HIV-1 sequences from the STEP trial}$.},
  author={Rolland, M and Tovanabutra, S and deCamp, A and Frahm, N and Gilbert, Peter B and Sanders-Buell, E and et al.},
  journal={Nature Medicine},
  volume={17},
  number={3},
  pages={366--371},
  year={2011},
  publisher={Nature Publishing Group},
  note={PMCID: PMC3053571}
}

@Article{RollandGilbert2012,
  author =          {Rolland, M and Gilbert, Peter B}, 
  title =          {Evaluating immune correlates in {HIV} type 1 vaccine efficacy trials: what {RV144} may provide},
  journal =          {AIDS Research and Human Retroviruses},
  year =          {2012},
  OPTkey =          {},
  volume =          {28},
  OPTnumber =          {},
  pages =          {400--404},
  note={PMCID: PMC3316118}
}

@Article{RollandEdlefsenetal2012,
  author =          {Rolland$^*$, M and Edlefsen$^*$, PT and Larsen, BB and Tovanabutra, S and Sanders-Buell, E and 
Hertz, T and DeCamp, AC and Carrico, C and Menis, S and Magaret, CA and Ahmed, H and Juraska, M and Chen, L and Konopa, P and Nariya, S and 
 Stoddard, JN and Wong, K and Zhao, H and Deng, W and Maust, BS and Bose, M and Howell, S and Bates, A and Lazzaro, M and O'Sullivan, A and Lei, E and 
 Bradfield, A and Ibitamuno, G and Assawadarachai, V and O'Connell, RJ and deSouza, MS and Nitayaphan, S and Rerks-Ngarm, S and Robb, ML and 
 McLellan, JS and Georgiev, I and Kwong, PD and Carlson, JM and Michael, NL and Schief, WR and Gilbert$^*$, PB and Mullins$^*$, JI and Kim$^*$, JH.},
  title =          {Increased $\mbox{HIV-1}$ vaccine efficacy against viruses with genetic signatures in $\mbox{Env V2}$.},
  journal =          {Nature},
  year =          {2012},
  OPTkey =          {},
  volume =          {490},
  OPTnumber =          {},
  pages =          {417--420},
note={$^*$Contributed equally. PMCID: PMC3551291}}
%

@Article{RollandEdlefsenetal2012med,
  author =          {Rolland$^*$, M and Edlefsen$^*$, PT and Larsen, BB and 
Kwong, PD and Carlson, JM and Michael, NL and Schief, WR and Gilbert$^*$, PB and Mullins$^*$, JI and Kim$^*$, JH.},
  title =          {Increased $\mbox{HIV-1}$ vaccine efficacy against viruses with genetic signatures in $\mbox{Env V2}$.},
  journal =          {Nature},
  year =          {2012},
  OPTkey =          {},
  volume =          {490},
  OPTnumber =          {},
  pages =          {417--420},
  note={PMCID: PMC3551291. $^*$Contributed equally}
}


@Article{RollandEdlefsenetal2012short,
  author =          {Rolland$^*$, M and Edlefsen$^*$, PT and Larsen, BB and et al.},
  title =          {Increased $\mbox{HIV-1}$ vaccine efficacy against viruses with genetic signatures in $\mbox{Env V2}$.},
  journal =          {Nature},
  year =          {2012},
  OPTkey =          {},
  volume =          {490},
  OPTnumber =          {},
  pages =          {417--420},
  note={$^*$Contributed equally}
}
%note={PMCID: PMC3551291. $^*$Contributed equally}



@Article{SunLiGilbert2013,
  author =          {Sun, Y and Li, M and Gilbert, Peter B},
  title =          {Mark-specific proportional hazards model with multivariate continuous marks and its application to $\mbox{HIV}$ vaccine efficacy trials},
  journal =          {Biostatistics},
  year =          {2013},
  OPTkey =          {},
  volume =          {14},
  OPTnumber =          {},
  pages =          {60--74},
  note={PMCID: PMC3520499}
}

@Article{JuraskaGilbert2013,
  author =          {Juraska, M and Gilbert, Peter B},
  title =          {Mark-specific hazard ratio model with multivariate continuous marks: {An} application to vaccine efficacy},
  journal =          {Biometrics},
  year =          {2013},
  OPTkey =          {},
  volume =          {69},
  OPTnumber =          {},
  pages =          {328--337},
  note={PMCID: PMC3940058} 
}

@Article{JuraskaGilbert2014,
  author =          {Juraska, M and Gilbert, Peter B},
  title =          {Mark-specific hazard ratio model with missing multivariate marks},
  journal =          {under review},
  year =          {2014},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {}
}

@article{Gartlandetal2014,
  title={Analysis of {HLA A*} 02 association with vaccine efficacy in the {RV144 HIV-1} vaccine trial},
  author={Gartland, Andrew J and Li, Sue and McNevin, John and Tomaras, Georgia D and Gottardo, Raphael and Janes, Holly and Fong, Youyi and Morris, Daryl and Geraghty, Daniel E and Kijak, Gustavo H and Edlefsen, Paul T and Frahm, Nicole and Larsen, Brendan B and Tovanabutra, Sodsai and Sanders-Buell, Eric and deCamp, Allan C and Magaret, Craig A and Ahmed, Hasan and Goodridge, Jodie P and Chen, Lennie and Konopa, Philip and Nariya, Snehal and Stoddard, Julia N and Wong, Kim and Zhao, Hong and Deng, Wenjie and Maust, Brandon S and Bose, Meera and Howell, Shana and Bates, Adam and Lazzaro, Michelle and O’Sullivan, Annemarie and Lei, Esther and Bradfield, Andrea and Ibitamuno, Grace and Assawadarachai, Vatcharain and O'Connell, Robert J and deSouza, Mark S and Nitayaphan, Sorachai and Rerks-Ngarm, Supachai and Robb, Merlin L and Sidney, John and Sette, Alessandro and Zolla-Pazner, Susan and Montefiori, David and McElrath, M. Juliana and Mullins, James I and Kim, Jerome H and Gilbert, Peter B and Hertz, Tomer },
  journal={Journal of Virology},
  volume={88},
  number={15},
  pages={8242--8255},
  year={2014},
  publisher={Am Soc Microbiol},
  note={PMCID: PMC4135964}
}

@Article{Vansteelandtetal2006,
  author =          {Vansteelandt, S and Goetghebeur, E and Kenward, MG and Molenberghs, G},
  title =          {Ignorance and uncertainty regions as inferential tools in a sensitivity analysis},
  journal =          {Statistica Sinica},
  year =          {2006},
  OPTkey =          {},
  volume =          {16},
  OPTnumber =          {},
  pages =          {953--979}
}


@Article{GilbertShepherdHudgens2013,
  author =          {Gilbert, Peter B and Shepherd, BE and Hudgens, MG}, 
  title =          {Sensitivity analysis of per-protocol time-to-event treatment efficacy in randomized trials},
  journal =          {Journal of the American Statistical Association},
  year =          {2013},
  OPTkey =          {},
  volume =          {108},
  OPTnumber =          {},
  pages =          {789-800},
  note={PMCID: PMC3811958}
}

@Article{Efron2014,
  author =          {Efron, B},
  title =          {Estimation and accuracy after model selection}, 
  journal =          {Journal of the American Statistical Association, In Press},
  year =          {2014},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {},
  note={PMCID: (in process)}
}


@Article{GilbertGroveetal2011,
  author =          {Gilbert, Peter B and Grove, D and Gabriel, E and Huang, Y and Gray, G and Hammer, SM and Buchbinder, SP and Kublin, J and Corey, L and Self, SG},
  title =          {A sequential {Phase 2b} trial design for evaluating vaccine efficacy and immune correlates for multiple {HIV} vaccine regimens.},
  journal =          {Statistical Communications in Infectious Diseases},
  year =          {2011},
  OPTkey =          {},
  volume =          {3, Issue 1},
  OPTnumber =          {},
  pages =          {Article 4}
}
%note={PMCID: PMC3502884}

@Article{GilbertBergeretal2011,
  author =          {Gilbert, Peter B and Berger, JO and Stablein, D and Becker, S and Essex, M and Hammer, SM and
 Kim, JH and Degruttola, VG},
  title =          {Statistical interpretation of the $\mbox{RV144 HIV}$ vaccine efficacy trial in $\mbox{Thailand}$: A case study for statistical issues in efficacy trials.},
  journal =          {Journal of Infectious Diseases},
  year =          {2011},
  OPTkey =          {},
  volume =          {203},
  OPTnumber =          {},
  pages =          {969--975},
  note={PMCID: PMC3068028}
}

@Article{rolland2019,
  author =          {Rolland, M},
  title =          {{Molecular dating and viral load growth rates suggested an eclipse phase of a week in HIV-1 infected adults in East Africa and Thailand.}},
  journal =          {PLoS Pathogens}, 
  year =          {under review},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {}
}

@inproceedings{McCalletal2018,
  title={Correlating efficacy and immunogenicity in malaria vaccine trials},
  author={McCall, Matthew BB and Kremsner, Peter G and Mordm{\"u}ller, Benjamin},
  booktitle={Seminars in immunology},
  year={2018},
  organization={Elsevier}
}


@Article{EdlefsenGilbertRolland2013,
  author =          {Edlefsen, PT and Gilbert, Peter B and Rolland, M},
  title =          {Sieve analysis in {HIV-1} vaccine efficacy trials.},
  journal =          {Current Opinion in {HIV} and {AIDS}}, 
  year =          {2013},
  OPTkey =          {},
  volume =          {8},
  OPTnumber =          {},
  pages =          {431--435},
  note={PMCID:  (in process)}
}


@Article{SunWangGilbert2012,
  author =          {Sun, YQ and Wang, HJ and Gilbert, Peter B},
  title =          {Quantile Regression for Competing Risks Data with Missing Cause of Failure},
  journal =          {Statistica Sinica},
  year =          {2012},
  OPTkey =          {},
  volume =          {22},
  OPTnumber =          {},
  pages =          {703--728},
  note={PMCID: PMC3742132}
}

@Article{SunSunZhou2013,
  author =          {Sun, Y and Sun, L and Zhou, J},
  title =          {Profile local linear estimation of generalized semiparametric regression model for longitudinal data}, 
  journal =          {Lifetime Data Analysis},
  year =          {2013},
  OPTkey =          {},
  volume =          {19},
  OPTnumber =          {},
  pages =          {317--349},
  note={PMCID: PMC3710313}
}

@Article{SunLee2011,
  author =          {Sun, Y and Lee, J},
  title =          {Testing independent censoring for longitudinal data},
  journal =          {Statistica Sinica},
  year =          {2011},
  OPTkey =          {},
  volume =          {21},
  OPTnumber =          {},
  pages =          {1315--1339},
  note={PMCID: PMC3749084}
}



@Article{Sun2010,
  author =          {Sun, Y},
  title =          {Estimation of semiparametric regression model with longitudinal data},
  journal =          {Lifetime Data Analysis},
  year =          {2010},
  OPTkey =          {},
  volume =          {16},
  OPTnumber =          {},
  pages =          {271--298},
  note={PMCID: PMC3043558}
}



@Article{Hudgensetal2009,
  author =          {Hudgens, MG and Gilbert, Peter B and Mascola, JR and Wu, CD and Barouch, DH and Self, SG},
  title =          {Power to detect the effects of HIV vaccination in repeated low-dose challenge experiments},
  journal =          {Journal of Infectious Diseases},
  year =          {2009},
  OPTkey =          {},
  volume =          {200},
  OPTnumber =          {},
  pages =          {609--613},
  note={PMCID: PMC2754821}
}

@Article{Edlefsen2013,
author =          {Edlefsen, PT},
title =          {Failure avoidance models to evaluate the dependence of an intervention's efficacy on a categorical mark},
journal =          {Submitted},
year =          {2013},
volume =          {},
pages =          {}
}


@Article{Letvinetal2011,
  author =          {Letvin, NL and Rao, SS and Montefiori, DC and Seaman, MS and Sun, Y and Lim, SY and Yeh, WW and Asmal, M and Gelman, RS and Shen, L and Whitney, JB and Seoighe, C and Lacerda, M and Keating, S and Norris, PJ and Hudgens, MG and Gilbert, Peter B and Buzby, AP and Mach, LV and Zhang, J and Balachandran, H and Shaw, GM and Schmidt, SD and Todd, JP and Dodson, A and Mascola, JR and Nabel, GJ},
  title =          {Immune and Genetic Correlates of Vaccine Protection Against Mucosal Infection by $\mbox{SIV}$ in Monkeys},
  journal =          {Science Translational Medicine},
  year =          {2011},
  OPTkey =          {},
  volume =          {3},
  OPTnumber =          {},
  pages =          {81ra36},
  note={PMCID: PMC3718279}
}


@Article{Daietal2013, 
  author =          {Dai, JY and Gilbert, Peter B and Hughes, JP and Brown, ER},
  title =          {Estimating the efficacy of preexposure prophylaxis for {HIV} prevention among participants with a threshold level of drug concentration},
  journal =          {American Journal of Epidemiology},
  year =          {2013},
  OPTkey =          {},
  volume =          {177},
  OPTnumber =          {},
  pages =          {256--263},
  note={PMCID: PMC3577049}
}

@article{Billingsetal2011,
   author = {Billings, E. A. and Karasavvas, N. and de Souza, M. S. and Currier, J. and Pitisuttithum, P. and Kaewkunwal, J. and Nitayaphan, S. and Gilbert, P. B. and Tomaras, G. D. and Zolla-Pazner, S. B. and Haynes, B. F. and Michael, N. L. and Rerks-Ngarm, S. and Kim, J. H. and Rao, M.},
   title = {Surface plasmon resonance analysis of anti-gp120 {V2-specific IgG} antibodies generated in the {RV144 Thai Trial}},
   journal = {AIDS Research and Human Retroviruses},
   volume = {27},
   number = {10},
   pages = {A21-A22},
   year = {2011}
}

@article{Karasavvasetal2012,
   author = {Karasavvas, N. and Billings, E. and Rao, M. and Williams, C. and Zolla-Pazner, S. and Bailer, R. T. and Koup, R. A. and Madnote, S. and Arworn, D. and Shen, X. and Tomaras, G. D. and Currier, J. R. and Jiang, M. and Magaret, C. and Andrews, C. and Gottardo, R. and Gilbert, P.B. and Cardozo, T. J. and Rerks-Ngarm, S. and Nitayaphan, S. and Pitisuttithum, P. and Kaewkungwal, J. and Paris, R. and Greene, K. and Gao, H. and Gurunathan, S. and Tartaglia, J. and Sinangil, F. and Korber, B. T. and Montefiori, D. C. and Mascola, J. R. and Robb, M. L. and Haynes, B. F. and Ngauy, V. and Michael, N. L. and Kim, J. H. and de Souza, M.S., for the {MOPH TAVEG Collaboration}},
   title = {{The Thai Phase III HIV Type 1 Vaccine Trial (RV144) Regimen Induces Antibodies That Target Conserved Regions Within the V2 Loop of gp120}},
   journal = {AIDS Res Hum Retroviruses},
   volume = {28},
   number = {11},
   pages = {1444-57},
   year = {2012},
  note={PMCID: PMC3484815}
}

@article{yang2012antiviral,
  title={Antiviral inhibitory capacity of {CD8+ T} cells predicts the rate of {CD4+ T-cell} decline in {HIV-1} infection},
  author={Yang, Hongbing and Wu, Hao and Hancock, Gemma and Clutton, Genevieve and Sande, Nellia and Xu, Xiaoning and Yan, Huiping and Huang, Xiaojie and Angus, Brian and Kuldanek, Kristin and others},
  journal={Journal of Infectious Diseases},
  volume={206},
  number={4},
  pages={552--561},
  year={2012},
  publisher={Oxford University Press}
}



@article{MontefioriKarnasutaetal2012,
   author = {Montefiori, D. C. and Karnasuta, C. and Huang, Y. and Ahmed, H. and Gilbert, P.B. and de Souza, M. S. and McLinden, R. and Tovanabutra, S. and Laurence-Chenine, A. and Sanders-Buell, E. and Moody, M. A. and Bonsignori, M. and Ochsenbauer, C. and Kappes, J. and Tang, H. and Greene, K. and Gao, H. and LaBranche, C. C. and Andrews, C. and Polonis, V. R. and Rerks-Ngarm, S. and Pitisuttithum, P. and Nitayaphan, S. and Kaewkungwal, J. and Self, S. G. and Berman, P. W. and Francis, D. and Sinangil, F. and Lee, C. and Tartaglia, J. and Robb, M. L. and Haynes, B. F. and Michael, N. L. and Kim, J. H.},
   title = {Magnitude and breadth of the neutralizing antibody response in the {RV144 and Vax003 HIV-1} vaccine efficacy trials},
   journal = {Journal of Infectious Diseases},
   volume = {206},
   number = {3},
   pages = {431-41},
   year = {2012},
  note={PMCID: PMC3392187}
}

@article{Liuetal2013,
   author = {Liu, P. and Yates, N. L. and Shen, X. and Bonsignori, M. and Moody, M. A. and Liao, H. X. and Fong, Y. and Alam, S. M. and Overman, R. G. and Denny, T. and Ferrari, G. and Ochsenbauer, C. and Kappes, J. C. and Polonis, V. R. and Pitisuttithum, P. and Kaewkungwal, J. and Nitayaphan, S. and Rerks-Ngarm, S. and Montefiori, D. C. and Gilbert, P.B. and Michael, N. L. and Kim, J. H. and Haynes, B. F. and Tomaras, G. D.},
   title = {Infectious virion capture by {HIV-1 gp120-specific IgG from RV144} vaccinees},
   journal = {Journal of Virology},
   volume = {87},
   number = {14},
   pages = {7828-36},
   year = {2013},
  note={PMCID: PMC3700223}
}

@article{Tomarasetal2013,
   author = {Tomaras, G. D. and Ferrari, G. and Shen, X. and Alam, S. M. and Liao, H. X. and Pollara, J. and Bonsignori, M. and Moody, M. A. and Fong, Y. and Chen, X. and Poling, B. and Nicholson, C. O. and Zhang, R. and Lu, X. and Parks, R. and Kaewkungwal, J. and Nitayaphan, S. and Pitisuttithum, P. and Rerks-Ngarm, S. and Gilbert, P. B. and Kim, J. H. and Michael, N. L. and Montefiori, D. C. and Haynes, B. F.},
   title = {Vaccine-induced plasma {IgA} specific for the {C1} region of the {HIV-1} envelope blocks binding and effector function of {IgG}},
   journal = {Proceedings of the National Academy of Sciences USA},
   volume = {110},
   number = {22},
   pages = {9019-24},
   year = {2013},
  note={PMCID: PMC3670311}
}

@article{ZollaPazneretal2013,
   author = {Zolla-Pazner, S. and DeCamp, A. C. and Cardozo, T. and Karasavvas, N. and Gottardo, R. and Williams, C. and Morris, D. E. and Tomaras, G. and Rao, M. and Billings, E. and Berman, P. and Shen, X. and Andrews, C. and O'Connell, R. J. and Ngauy, V. and Nitayaphan, S. and de Souza, M. and Korber, B. and Koup, R. and Bailer, R. T. and Mascola, J. R. and Pinter, A. and Montefiori, D. and Haynes, B. F. and Robb, M. L. and Rerks-Ngarm, S. and Michael, N. L. and Gilbert, P. B. and Kim, J. H.},
   title = {Analysis of {V2} antibody responses induced in vaccinees in the {ALVAC/AIDSVAX HIV-1} vaccine efficacy trial.},
   journal = {PLoS One},
   volume = {8},
   number = {1},
   pages = {e53629},
   year = {2013},
  note={PMCID: PMC3547933}
}

@Article{Janesetal2013,
  author =          {Janes, HE and Gilbert, Peter B and Buchbinder, S and Kublin, J and Sobieszczyk, ME and Hammer, SM},
  title =          {In pursuit of an {HIV} vaccine: {Designing} efficacy trials in the context of partially effective non-vaccine prevention modalities.},
  journal =          {AIDS Research and Human Retroviruses},
  year =          {2013},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {},
  note={PMCID: (in process)}
}



@Article{GilbertYuRotnitzky2014,
  author =          {Gilbert, Peter B and Yu, X and Rotnitzky, A},
  title =          {Optimal auxiliary-covariate-based two-phase sampling design for semiparametric efficient estimation of a mean or mean difference, with application to clinical trials},
  journal =          {Statistics in Medicine},
  year =          {2014},
  OPTkey =          {},
  volume =          {33},
  OPTnumber =          {},
  pages =          {901--917},
  note={PMCID: (in process)}
}


@Article{Richardsonetal2014,
  author =          {Richardson, A and Hudgens, MG and Gilbert, Peter B and Fine, JP},
  title =          {Nonparametric bounds and sensitivity analysis of treatment effects},
  journal =          {Statistical Science},
  year =          {2014},
  OPTkey =          {},
  volume =          {29},
  OPTnumber =          {},
  pages =          {596--618}
}
%note={PMCID: PMC4317325}

@Article{KangHuang2013,
  author =          {Kang, C and Huang, Y},
  title =          {A discrete time survival model with random effect for designing and analyzing repeated low-dose challenge experiment},
  journal =          {Biometrics, Submitted},
  year =          {2013},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {}
}

@article{stitelman2011general,
  title={A general implementation of tmle for longitudinal data applied to causal inference in survival analysis},
  author={Stitelman, Ori M and De Gruttola, Victor and van der Laan, Mark J},
  year={2011},
  journal={U.C. Berkeley Division of Biostatistics Working Paper Series},
  volume={Working Paper 281}, 
  publisher={bepress}
}

@article{vanderLaanDudoit2003,
  title={Unified cross-validation 
methodology for selection among estimators and a general cross-validated 
adaptive epsilon-net estimator: {Finite} sample oracle inequalities and examples},
  author={Van Der Laan, MJ and Dudoit, S},
  year={2003},
  journal={U.C. Berkeley Division of Biostatistics Working Paper Series},
  volume={Working Paper 130}, 
  publisher={bepress}
}

@article{Vaart2006,
  title={Oracle inequalities for multi-fold cross validation},
  author={Vaart, AW and Dudoit, S and van der Laan, MJ},
  year={2006},
  journal={Statistics and Decisions},
  volume={24},
  number={3}, 
  pages={351--371}
}


@Article{Qureshietal2012,
  author =          {Qureshi, H and Ma, ZM and Huang, Y and Hodge, G and Thomas, MA and DiPasquale, J and
 DeSilva, V and Fritts, L and Bett, AJ and Casimiro, DR and Shiver, JW and Robert-Guroff, M and
 Robertson, MN and McChesney, MB and Gilbert, Peter B and Miller, CJ},
  title =          {Low-dose penile {SIVmac251} exposure of rhesus macaques infected with adenovirus type 5 ({Ad5}) and then immunized with a replication-defective {Ad5-based SIV gag/pol/nef} vaccine recapitulates the results of the Phase {IIb} {Step} trial of a similar {HIV-1} vaccine.},
  journal =          {Journal of Virology},
  year =          {2012},
  OPTkey =          {},
  volume =          {86},
  OPTnumber =          {},
  pages =          {2239--2250},
  note={PMCID: PMC3302390}
}


@Article{Janesetal2012,
  author =          {Janes, H and Frahm, N and DeCamp, A and Rolland, M and Gabriel, E and Wolfson, J and
 Hertz, T and Kallas, E and Goepfert, P and Friedrich, DP and Corey, L and Mullins, JI and McElrath, MJ and Gilbert, Peter B}, 
  title =          {$\mbox{MRKAd5 HIV-1 Gag/Pol/Nef}$ vaccine-induced $\mbox{T-cell}$ responses inadequately predict distance of breakthrough $\mbox{HIV-1}$ sequences to the vaccine or viral load},
  journal =          {PLoS One},
  year =          {2012},
  OPTkey =          {},
  volume =          {7},
  OPTnumber =          {},
  pages =          {e43396},
  note={PMCID: PMC3428369}
}


@Article{Scottetal2013,
  author =          {Scott, J and deCamp, A and Juraska, M and Fay, MP and Gilbert, Peter B},
  title =          {Corrected {GEE} for Valid Inferences of Population Average Treatment Effects in Stepped Wedge and Parallel Cluster Randomized Trials},
  journal =          {Biometrics, Submitted},
  year =          {2013},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {}
}





@Article{KangSchafer2007,
  author =          {Kang, JDY and Schafer, JL}, 
  title =          {A comparison of alternative strategies for estimating a population mean from incomplete data},
  journal =          {Statistical Science},
  year =          {2007},
  OPTkey =          {},
  volume =          {22},
  OPTnumber =          {},
  pages =          {523--539}
}

@Article{vanderLaanGruber2010,
  author =          {van der Laan, MJ and Gruber, S},
  title =          {Collaborative double robust targeted maximum likelihood estimation},
  journal =          {International Journal of Biostatistics},
  year =          {2010},
  OPTkey =          {},
  volume =          {6},
  OPTnumber =          {},
  pages =          {Article 17},
  note={PMCID: PMC2898626}
}

@Article{Gilbert2010,
  author =          {Gilbert, Peter B},
  title =          {Some design issues in {Phase 2b versus Phase 3} prevention trials for testing efficacy of products or concepts},
  journal =          {Statistics in Medicine},
  year =          {2010},
  OPTkey =          {},
  volume =          {29},
  OPTnumber =          {},
  pages =          {1061--1071},
  note={PMCID: PMC2929839}
}




@Article{Oxmanetal2005,
  author =          {Oxman, MN and Levin, MJ and Johnson, GR et al.},
  title =          {A vaccine to prevent herpes zoster and postherpetic neuralgia in older adults},
  journal =          {New England Journal of Medicine},
  year =          {2005},
  OPTkey =          {},
  volume =          {352},
  OPTnumber =          {},
  pages =          {2271--2284},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{Dunning2006,
  author =          {Dunning, AJ},
  title =          {A model for immunological correlates of protection},
  journal =          {Statistics in Medicine},
  year =          {2006},
  OPTkey =          {},
  volume =          {25},
  OPTnumber =          {},
  pages =          {1485--1497},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Article{SalkMenkeFrancis1943,
  author =          {Salk, JE and Menke, WJ Jr and Francis, T Jr},
  title =          {A clinical, epidemiological and immunological evaluation of vaccination against epidemic influenza},
  journal =          {American Journal of Hygiene},
  year =          {1943},
  OPTkey =          {},
  volume =          {42}, 
  OPTnumber =          {},
  pages =          {57--93},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}





@Article{Heckermanetal2007,
  author =          {Heckerman, D and Kadie, C and Listgarten, J},
  title =          {Leveraging information across $\mbox{HLA}$ alleles/supertypes improves epitope prediction},
  journal =          {Journal of Computational Biology},
  year =          {2007},
  OPTkey =          {},
  volume =          {14},
  OPTnumber =          {},
  pages =          {736-746},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}

@Article{Edwardsetal1994,
  author =          {Edwards, KM and Dupont, WD and Westrich, MK and Plummer, WD Jr and Palmer, PS and Wright, PF},
  title =          {A randomized controlled trial of cold-adapted and inactivated vaccines for the prevention of influenza {A} disease},
  journal =          {Journal of Infectious Diseases},
  year =          {1994},
  OPTkey =          {},
  volume =          {169},
  OPTnumber =          {},
  pages =          {68--76},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}

@Article{Keiteletal1997,
  author =          {Keitel, WA and Cate, TR and Nino, D and Huggins, LL and Six, HR and Quarles, JM and Couch, RB},
  title =          {Immunization against influenza: comparison of various topical and parenteral regimens containing inactivated and/or live attenuated vaccines in healthy adults},
  journal =          {Journal of Infectious Diseases},
  year =          {1997},
  OPTkey =          {},
  volume =          {183},
  OPTnumber =          {},
  pages =          {329--332},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}

@Article{Nielsenetal2005,
  author =          {Nielsen, M and Lundegaard, C and Lund, O and Kesmir, C},
  title =          {The role of the proteasome in generating cytotoxic
$\mbox{T-cell}$ epitopes: insights obtained from improved
predictions of proteasomal cleavage.},
  journal =          {Immunogenetics},
  year =          {2005},
  OPTkey =          {},
  volume =          {57},
  OPTnumber =          {},
  pages =          {33--41},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}


@Article{HyunSun2007,
  author =          {Hyun, S and Sun, Y},
  title =          {Hypotheses tests of strain-specific vaccine efficacy adjusted for covariate effects.},
  journal =          {Journal of Applied Statistics},
  year =          {2007},
  OPTkey =          {},
  volume =          {34},
  OPTnumber =          {},
  pages =          {1065--1073},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Article{HyunLeeSun2012,
  author =          {Hyun, S and Lee, J and Sun, Y},
  title =          {Proportional hazards model for competing risks data with missing cause of failure.},
  journal =          {Journal of Statistical Planning and Inference},
  year =          {2012},
  OPTkey =          {},
  volume =          {142},
  OPTnumber =          {},
  pages =          {1767--1779},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: PMC3314432}
}


@Article{SunHyunGilbert2008,
  author =          {Sun, Y and Hyun, S and Gilbert, Peter B},
  title =          {Testing and estimation of time-varying cause-specific hazard ratios with covariate adjustment.},
  journal =          {Biometrics},
  year =          {2008},
  OPTkey =          {},
  volume =          {64},
  OPTnumber =          {},
  pages =          {1070--1079},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}





@article{Nebojsaetal2006,
author = {Nebojsa Jojic and Manuel Reyes-Gomez and David Heckerman and Carl Kadie and Ora Schueler-Furman}, 
journal = {Bioinformatics},
title = {Learning $\mbox{MHC}$ I--peptide binding},
abstract = {MOTIVATION AND RESULTS: Motivated by the ability of a simple threading approach to predict $\mbox{MHC}$ I--peptide binding, we developed a new and improved structure-based model for which parameters can be estimated from additional sources of data about $\mbox{MHC}$-peptide binding. In addition to the known 3D structures of a small number of $\mbox{MHC}$-peptide complexes that were used in the original threading approach, we included three other sources of information on peptide-$\mbox{MHC}$ binding: (1) $\mbox{MHC}$ class $\mbox{I}$ sequences; (2) known binding energies for a large number of $\mbox{MHC}$-peptide complexes; and (3) an even larger binary dataset that contains information about strong binders (epitopes) and non-binders (peptides that have a low affinity for a particular $\mbox{MHC}$ molecule). Our model significantly outperforms the standard threading approach in binding energy prediction. In our approach, which we call adaptive double threading, the parameters of the threading model are learnable, and both $\mbox{MHC}$ and peptide sequences can be threaded onto structures of other alleles. These two properties make our model appropriate for predicting binding for alleles for which very little data (if any) is available beyond just their sequence, including prediction for alleles for which 3D structures are not available. The ability of our model to generalize beyond the $\mbox{MHC}$ types for which training data is available also separates our approach from epitope prediction methods which treat $\mbox{MHC}$ alleles as symbolic types, rather than biological sequences. We used the trained binding energy predictor to study viral infections in 246 $\mbox{HIV}$ patients from the West Australian cohort, and over 1000 sequences in $\mbox{HIV}$ clade B from Los Alamos National Laboratory database, capturing the course of $\mbox{HIV}$ evolution over the last 20 years. Finally, we illustrate short-, medium-, and long-term adaptation of $\mbox{HIV}$ to the human immune system. AVAILABILITY: http://www.research.microsoft.com/~jojic/hlaBinding.html.},
affiliation = {Microsoft Research, Redmond, WA 98052, USA. jojic@microsoft.com},
number = {14},
pages = {e227--35},
volume = {22},
year = {2006},
month = {Jul},
language = {eng},
keywords = {Peptides, Molecular Sequence Data, Pattern Recognition: Automated, Models: Chemical, Sequence Alignment, Binding Sites, Artificial Intelligence, Amino Acid Sequence, Software, Histocompatibility Antigens Class $\mbox{I}$, Protein Binding, Computer Simulation, Models: Molecular, Sequence Analysis: Protein, Protein Conformation, Algorithms}, 
date-added = {2009-04-21 15:59:38 -0700},
date-modified = {2009-04-21 16:00:34 -0700},
doi = {10.1093/bioinformatics/btl255},
pii = {22/14/e227},
pmid = {16873476},
URL = {http://bioinformatics.oxfordjournals.org/cgi/reprint/22/14/e227},
local-url = {file://localhost/Users/thertz/Documents/Papers/2006/Jojic/Bioinformatics%202006%20Jojic-2.pdf},
uri = {papers://A465BBE6-F53C-492D-99AA-EDED51208D16/Paper/p4801},
read = {Yes},
rating = {0},
  note={PMCID: }
}

@article{Gottardoetal2013,
  title={Plasma $\mbox{IgG}$ to Linear Epitopes in the $\mbox{V2 and V3}$ Regions of $\mbox{HIV-1 gp120}$ 
 Correlate with a Reduced Risk of Infection in the $\mbox{RV144}$ Vaccine Efficacy Trial},
  author={Gottardo, Raphael and Bailer, Robert T and Korber, Bette T and Gnanakaran, S and Phillips, Joshua and Shen, Xiaoying and Tomaras, Georgia D and Turk, Ellen and Imholte, Gregory and Eckler, Larry and Wenschuh, Holger and Zerweck, Johannes and Greene, Kelli and Gao, Hongmei and Berman, Phillip W and Francis, Donald and Sinangil, Faruk and Lee, Carter and Nitayaphan, Sorachai and Rerks-Ngarm, Supachai and Kaewkungwal, Jaranit and Pitisuttithum, Punnee and Tartaglia, James and Robb, Merlin L and Michael, Nelson L and Kim, Jerome H and Zolla-Pazner, Susan and Haynes, Barton F and Mascola, John R and Self, Steve and Gilbert, Peter and Montefiori, David C},
  journal={PLoS One},
  volume={8},
  number={9},
  pages={e75665},
  year={2013},
  publisher={Public Library of Science},
note={PMCID: PMC3784573}}
%




@InProceedings{deCamp2009HVTN,
  author =          {deCamp, A and Gilbert, P and Rolland, M and Margaret, C and Heath, L and
Geraghty, D and McElrath, J and Mullins, J},
  title =          {Sieve analysis of Step $\mbox{HIV}$ sequences.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {Annual HVTN Meeting 2009},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Seattle WA, November 2009},
  OPTpublisher = {},
  OPTannote =          {},
  note={PMCID: }
}

@article{ZhangLundegaardNielsen2009,
author = {Hao Zhang and Claus Lundegaard and Morten Nielsen}, 
journal = {Bioinformatics},
title = {Pan-specific $\mbox{MHC}$ class $\mbox{I}$ predictors: a benchmark of $\mbox{HLA}$ class $\mbox{I}$ pan-specific prediction methods},
abstract = {MOTIVATION: $\mbox{MHC}$:peptide binding plays a central role in activating the immune surveillance. Computational approaches to determine $\mbox{T-cell}$ epitopes restricted to any given major histocompatibility complex ($\mbox{MHC}$) molecule are of special practical value in the development of for instance vaccines with broad population coverage against emerging pathogens. Methods have recently been published that are able to predict peptide binding to any human $\mbox{MHC}$ class $\mbox{I}$ molecule. In contrast to conventional allele-specific methods, these methods do allow for extrapolation to uncharacterized $\mbox{MHC}$ molecules. These pan-specific human lymphocyte antigen ($\mbox{HLA}$) predictors have not previously been compared using independent evaluation sets. RESULT: A diverse set of quantitative peptide binding affinity measurements was collected from Immune Epitope database (IEDB), together with a large set of $\mbox{HLA}$ class $\mbox{I}$ ligands from the SYFPEITHI database. Based on these datasets, three different pan-specific $\mbox{HLA}$ web-accessible predictors $\mbox{Net}$$\mbox{MHC}$pan, adaptive double threading (ADT) and kernel-based inter-allele peptide binding prediction system (KISS) were evaluated. The performance of the pan-specific predictors was also compared with a well performing allele-specific $\mbox{MHC}$ class $\mbox{I}$ predictor, $\mbox{Net}$$\mbox{MHC}$, as well as a consensus approach integrating the predictions from the $\mbox{Net}$$\mbox{MHC}$ and $\mbox{Net}$$\mbox{MHC}$pan methods. Conclusions: The benchmark demonstrated that pan-specific methods do provide accurate predictions also for previously uncharacterized $\mbox{MHC}$ molecules. The $\mbox{Net}$$\mbox{MHC}$pan method trained to predict actual binding affinities was consistently top ranking both on quantitative (affinity) and binary (ligand) data. However, the KISS method trained to predict binary data was one of the best performing methods when benchmarked on binary data. Finally, a consensus method integrating predictions from the two best performing methods was shown to improve the prediction accuracy.},
affiliation = {Center for Biological Sequence Analysis, Department of Systems Biology, Technical University of Denmark, Lyngby 2800, Denmark.},
number = {1},
pages = {83--9},
volume = {25},
year = {2009},
month = {Jan},
language = {eng},
keywords = {Statistics: Nonparametric, Protein Binding, Databases: Protein, Humans, Ligands, $\mbox{HLA}$ Antigens, Alleles, Peptides, Histocompatibility Antigens Class $\mbox{I}$, Area Under Curve, Computational Biology}, 
date-added = {2009-04-19 15:05:18 -0700},
date-modified = {2009-04-19 15:09:43 -0700},
doi = {10.1093/bioinformatics/btn579},
pii = {btn579},
pmid = {18996943},
URL = {http://bioinformatics.oxfordjournals.org/cgi/content/full/25/1/83},
local-url = {file://localhost/Users/thertz/Documents/Papers/2009/Zhang/Bioinformatics%202009%20Zhang.pdf},
uri = {papers://A465BBE6-F53C-492D-99AA-EDED51208D16/Paper/p3266},
rating = {0},
  note={PMCID: PMC2638932}
}


@Article{Korberetal2007,
  author =          {Korber, BTM and Brander, C and Haynes, BF and Koup, R and Moore, JP and Walker, BD and Watkins, DI},
  title =          {$\mbox{HIV}$ Molecular Immunology 2006/2007.},
  publisher =          {Los Alamos National Laboratory, Theoretical Biology and Biophysics, Los Alamos, New Mexico},
  year =          {2007},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}


@Article{Cuzick1982,
  author =          {Cuzick, J},
  title =          {The efficiency of the proportions test and the logrank test for censored survival data},
  journal =          {Biometrics},
  year =          {1982},
  OPTkey =          {},
  volume =          {38},
  OPTnumber =          {},
  pages =          {1033-1039},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}

@Article{FlemingRichardson2004,
  author =          {Fleming, TR and Richardson, BA},
  title =          {Some design issues in trials of microbicides for the prevention of $\mbox{HIV}$ infection},
  journal =          {The Journal of Infectious Diseases},
  year =          {2004},
  OPTkey =          {},
  volume =          {190},
  OPTnumber =          {},
  pages =          {666-674},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}




@Article{Catanzaro2006,
  author =          {Catanzaro, AT and Koup, RA and Roederer, M and et al.},
  title =          {Safety and immunogenicity evaluation of a multiclade $\mbox{HIV-1}$ candidate vaccine delivered by a replication-defective recombinant adenovirus vector},
  journal =          {Journal of Infectious Diseases},
  year =          {2006},
  OPTkey =          {},
  volume =          {194},
  OPTnumber =          {},
  pages =          {1638--1649},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}
% Whole author list:
Andrew T. Catanzaro, Richard A. Koup, Mario Roederer, Robert T. Bailer, Mary E. Enama, Zoe Moodie, Lin Gu, Julie E. Martin, Laura Novik, Bimal K. Chakrabarti, Bryan T. Butman, Jason G. D. Gall, C. Richter King, Charla A. Andrews, Rebecca Sheets, Phillip L. Gomez, John R. Mascola, Gary J. Nabel, Barney S. Graham, and Vaccine Research Center 006 Study Team



 

@Article{HoganHammer2001,
  author =          {Hogan, CM and Hammer, SM},
  title =          {Host determinants in $\mbox{HIV}$ infection
                and disease Part $\mbox{II}$:
                Genetic factors and implications for antiretroviral
                therapeutics},
  journal =          {Annals of Internal Medicine},
  year =          {2001},
  OPTkey =          {},
  volume =          {134},
  OPTnumber =          {},
  pages =          {978--96},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}



@Article{CzeschinskiBindingWitting2000,
  author =          {Czeschinski, PA and Binding, N and Witting, U},
  title =          {Hepatitis $\mbox{A}$ and hepatitis $\mbox{B}$ vaccinations: immunogenicity of combined vaccine and of simultaneously or separately applied single vaccines},
  journal =          {Vaccine},
  year =          {2000},
  OPTkey =          {},
  volume =          {18},
  OPTnumber =          {},
  pages =          {1074--1080},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}


@Article{Louis1982,
  author =          {Louis, TA},
  title =          {Finding the observed information matrix when using the EM algorithm},
  journal =          {Journal of the Royal Statistics Society Series B},
  year =          {1982},
  OPTkey =          {},
  volume =          {44},
  OPTnumber =          {},
  pages =          {226--233},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {},
  note={PMCID: }
}


@Article{WeirWalley2006,
  author =          {Weir, CJ and Walley, RJ},
  title =          {Statistical evaluation of biomarkers as surrogate endpoints: a literature review},
  journal =          {Statistics in Medicine},
  year =          {2006},
  OPTkey =          {},
  volume =          {25},
  pages =          {183--203},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{Freedman1992,
  author =          {Freedman, LS and Graubard, BI and Schatzkin, A},
  title =          {Statistical validation of intermediate endpoints for chronic diseases},
  journal =          {Statistics in Medicine},
  year =          {1992},
  OPTkey =          {},
  volume =          {11},
  OPTnumber =          {},
  pages =          {167--178},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{WangTaylor2002,
  author =          {Wang, Y and Taylor, JMG},
  title =          {A measure of the proportion of treatment effect explained by a surrogate marker},
  journal =          {Biometrics},
  year =          {2002},
  OPTkey =          {},
  volume =          {58},
  OPTnumber =          {},
  pages =          {803--812},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{TaylorWangThiebaut2005,
  author =          {Taylor, JMG and Wang, Y and Thibaut, R},
  title =          {Counterfactual links to the proportion of treatment effect explained by a surrogate marker},
  journal =          {Biometrics},
  year =          {2005},
  OPTkey =          {},
  volume =          {61},
  OPTnumber =          {},
  pages =          {1102--1111},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{Aalen1978,
  author =          {Aalen, O},
  title =          {Nonparametric inference for a family of counting processes.},
  journal =          {Annals of Statistics},
  year =          {1978},
  volume =          {6},
  pages =          {701--726}
}

@Article{Gilbert2000AOS,
  author =          {Gilbert, P},
  title =          {Large sample theory of maximum likelihood estimates in semiparametric biased sampling models.},
  journal = {Annals of Statistics}, 
  year = {2000},
  volume = {28},
  pages = {151--194}
}


                        processes.},
  journal =          {Annals of Statistics},
  year =          {1978},
  volume =          {6},
  pages =          {701-726},
}

@Book{Andersen1993,
  author =          {Andersen, PK and Borgan, O and Gill, RD and
Keiding, N},
  title =          {Statistical models based
                        on counting processes.},
  publisher =          {New York:  Springer-Verlag},
  year =          {1993},
}

 

@Article{Cai2002,
  author =          {Cai, T and Hyndman, RJ and Wand,  MP},
  title =          {Mixed model-based hazard estimation},
  journal =          {Journal of Computational and Graphical Statistics},
  year =          {2002},
  Volume = 11,
  Pages = {784--798},
}

 

@article{LindseyRyan1998,
         Author = {Lindsey, JC and Ryan, LM},
         Title = {Methods for Interval-censored Data},
         Year = 1998,
         Journal = {Stat. In Med.},
         Volume = 17,
         Pages = {219--238},
         Keywords = {Survival analysis}
     }

 

@Article{ChengWang2001,
  author =          {Cheng, S-S and Wang, N},
  title =          {Linear transformation models for failure time
                data with covariate measurement error.},
  journal =          {Journal of the American Statistical Association},
  year =          {2001},
  volume =          {96},
  pages =          {706-716}
}

 

 

@Article{ClementsMann1998,
  author =          {Clements-Mann, ML},
  title =          {Lessons for $\mbox{AIDS}$ vaccine development from
        non-$\mbox{AIDS}$ vaccines.},
  journal =          {AIDS Research and Human Retroviruses},
  year =          {1998},
  volume =          {14},
  note =          {Suppl 3:S197-S203}
}

 

@Article{Durhametal1998,
  author =          {Durham, LK  and Longini , IM and Halloran,  ME and
                Clemens , JD and Nizam , A and Rao , M},
  title =          {Estimation of vaccine efficacy in the
        presence of waning: application to cholera vaccines},
  journal =          {American Journal of Epidemiology},
  year =          {1998},
  volume =          {147},
  pages =          {948-959}
}

@Article{Clemensetal1990,
  author =          {Clemens, JD and Sack, DA and Harris, JR and Van Loon, F and Chakraborty, J and
Ahmed, F and Rao, MR and Khan, MR and Yunus, MD and Huda, N and Stanton, BF and Kay,
BA and Walter, S and Eeckels, R and
Svennerholm, A-M and Holmgren, J},
  title =          {Field trial
of oral cholera vaccines in $\mbox{Bangladesh}$: results from
three-year follow-up.},
  journal =          {Lancet},
  year =          {1990},
  volume =          {335},
  pages =          {270-273}
}


@Article{Efron1988,
  author =          {Efron , B},
  title =          {Logistic regression and survival analysis and the
Kaplan-Meier curve.},
  journal =          {Journal of the American Statistical Association},
  year =          {1988},
  volume =          {83},
  pages =          {414-425}
}

@Article{HsiehLavori1998,
  author =          {Hsieh, FY and Lavori, P},
  title =          {Sample size calculations for the $\mbox{Cox}$ proportional hazards regression model with nonbinary covariates.},
  journal =          {Controlled Clinical Trials},
  year =          {1998},
  volume =          {21},
  pages =          {552-560}
}

@Article{KohbergerJemioloNoriega2008,
  author =          {Kohberger, RC and Jemiolo, D and Noriega, F},
  title =          {Prediction of pertussis vaccine efficacy using a correlates of protection model.},
  journal =          {Vaccine},
  year =          {2008},
  volume =          {26},
  pages =          {3518-3521}
}

@Article{Gilbertetal2009,
  author =          {Gilbert, Peter B and Sato, A and Sun, X and Mehrotra, DV},
  title =          {Efficient and robust method for comparing the immunogenicity of candidate vaccines in randomized clinical trials.},
  journal =          {Vaccine},
  year =          {2009},
  volume =          {27},
  pages =          {396--401},
  note={PMCID: PMC2653280}
}




@Article{Jodaretal2003,
  author =          {Jodar, L and Butler, J and Carlone, G and Dagan, R and Goldblatt, D and K�yhty, H and Klugman, K and Plikaytis, B and Siber, G and Kohberger, R and Chang, I and Cherian, T},
  title =          {Serological criteria for evaluation and licensure of new pneumococcal conjugate vaccine formulations for use in infants.},
  journal =          {Vaccine},
  year =          {2003},
  volume =          {21},
  pages =          {3265-3272}
}
 

 

@Article{Francis1998,
  author =          {Francis ,DP and Gregory ,T and McElrath, MJ and
Belshe, RB
                and Gorse ,GJ and Migasena, S and Kitayaporn, D and
                Pitisutithum, P and Matthews, T and Schwartz, DH and
                Berman, PW},
  title =          {Advancing $\mbox{AIDSVAX}$ to phase 3: safety,
        immunogenicity, and plans for phase 3. },
  journal =          {AIDS Research and Human Retroviruses},
  year =          {1998},
  volume =          {14},
  pages =          {Suppl 3:S325-S331}
}

 

 

@Article{GilbertWeiKosorokClemens2002,
  author =          {Gilbert, Peter B and Wei, L J and Kosorok, MR and
Clemens, JD},
  title =          {Simultaneous inferences on the contrast of
                  two hazard functions with censored observations.},
  journal =          {Biometrics},
  year =          {2002},
  volume =       {58},
  pages =        {773--80}
}

@Article{Siberetal2007,
  author =          {Siber, GR and Chang, I and Baker, S and Fernsten, P and O'Brien, KL and Santosham, M and Klugman, KP and Madhi, SA and Paradiso, P and Kohberger, R},
  title =          {Estimating the protective concentration of anti-pneumococcal capsular polysaccharide antibodies.},
  journal =          {Vaccine},
  year =          {2007},
  volume =       {25},
  pages =        {3816--3826}
}


@Article{FayGraubard2001,
  author =          {Fay, MP and Graubard, BI},
  title =          {Small-sample adjustments for Wald-type tests using sandwich estimators.},
  journal =          {Biometrics},
  year =          {2001},
  volume =          {57},
  pages =          {1198--1206}
}

@Article{LachinFoulkes1986,
  author =          {Lachin, JM and Foulkes, M},
  title =          {Evaluation of sample size and power for analyses of survival with allowance for nonuniform patient entry, losses to follow-up, non-compliance, and stratification.},
  journal =          {Biometrics},
  year =          {1986},
  volume =          {42},
  pages =          {507--519}
}


@Article{ManclDeRouen2001,
  author =          {Mancl, LA and DeRouen, TA},
  title =          {A covariance estimator for {GEE} with improved small
sample properties.},
  journal =          {Biometrics},
  year =          {2001},
  volume =          {57},
  pages =          {126--134}
}

%Jim
@Article{Feng2001,
  author =          {Feng, Z and Diehr, P and Peterson, A and McLerran, D},
  title =          {Selected statistical issues in group randomized
trials.},
  journal =          {Annual Review of Public Health},
  year =          {2001},
  volume =          {22},
  pages =          {167--187}
}

@Article{Abu-Raddad2007,
  author =          {Abu-Raddad, L and Boily, MC and Self, S and Longini, IM},
  title =          {Analytic insights into the population level impact
of imperfect prophylactic $\mbox{HIV}$ vaccines.},
  journal =          {Journal of Acquired Immune Deficiency Syndromes},
  year =          {2007},
  volume =          {45},
  pages =          {454--467}
}

 
%Jim
@Article{HalloranStruchinerLongini1997,
  author =          {Halloran, ME and Struchiner, CJ and Longini, IM},
  title =          {Study designs for evaluating different efficacy
                and effectiveness aspects of vaccines.},
  journal =          {American Journal of Epidemiology},
  year =          {1997},
  volume =          {146},
  pages =          {789-803}
}

 

 

@Article{Hayes1998,
  author =          {Hayes, R},
  title =          {Design of human immunodeficiency virus intervention
trials
                in developing countries.},
  journal =          {Journal of the Royal Statistical Society, Series A},
  year =          { 1998},
  volume =          { 161},
  pages =          {251-263}
}

@Article{LangholzJiao2007,
  author =          {Langholz, B and Jiao, J},
  title =          {Computational methods for case-cohort studies.},
  journal =          {Computational Statistics and Data Analysis},
  year =          { 2007},
  volume =          {51},
  pages =          {3737-3748},
  note={PMCID: }
}
 
@Article{LangholzThomas1991,
  author =          {Langholz, B and Thomas, D},
  title =          {Efficiency of cohort sampling designs: Some surprising results.},
  journal =          {Biometrics},
  year =          { 1991},
  volume =          {47},
  pages =          {1563-1571}
}

@Article{Lakatos1988,
  author =          {Lakatos, E},
  title =          {Sample size based on the log-rank statistic in complex clinical trials.},
  journal =          {Biometrics},
  year =          { 1988},
  volume =          {44},
  pages =          {229-241}
}

@Article{Lietal2002,
  author =          {Li, S and Chan, ISF and Matthews, H and Heyse, JF and Chan, CY and Kutler, BJ and Kaplan, KM and Vessey, SJR and Sadoff, JC},
  title =          {Childhood vaccination against varicella: inverse relationship between 6-Week postvaccination varicella antibody response and likelihood of long-term breakthrough infection.},
  journal =          {Pediatric Infectious Disease Journal},
  year =          {2002},
  volume =          {21},
  pages =          {337-342}
}


@Article{HuTsiatisDavidian1998,
  author =          {Hu ,P and Tsiatis, AA and Davidian, M},
  title =          {Estimating the parameters in the $\mbox{Cox}$
        model when covariate variables are measured with error},
  journal =          {Biometrics},
  year =          {1998},
  volume =          {54},
  pages =          {1407-1419}
}

@Article{Molenberghsetal2008,
  author =          {Molenberghs, G and Burzykowski, T and Alonso, A and Assam, P and Tilahum, A and Buyse, M},
  title =          {The meta-analytic framework for the evaluation of surrogate endpoints in clinical trials.},
  journal =          {Journal of Statistical Planning and Inference},
  year =          {2008},
  volume =          {138},
  pages =          {432--449}
}


@Article{Alonso2004,
  author =          {Alonso, A and Molenberghs, G and Burzykowski, T and et al.},
  title =          {Prentice's approach and the meta-analytic paradigm: a reflection on the role of statistics in the evaluation of surrogate endpoints.},
  journal =          {Biometrics},
  year =          {2004},
  volume =          {60},
  pages =          {724--728}
}



@Article{McCormacketal2008,
  author =          {McCormack, S and Stohr, W and Barber, T and Bart, P-A and Harari, A and Moog, C and
Ciuffreda, D and Cellerai, C and Cowen, M and Gamboni, R and Burnet, S and Legg, K and Brodnicki, E and Wolf, H and Wagner, R and Heeney, J and Frachette, M-J and Tartaglia, J and Babiker, A and Pantaleo, G and Weber, J},
  title =          {$\mbox{EV02}$: A $\mbox{Phase I}$ trial to compare the safety and immunogenicity of $\mbox{HIV DNA-C prime-NYVAC-C boost to NYVAC-C alone}$.},
  journal =          {Vaccine},
  year =          {2008},
  volume =          {26},
  pages =          {3162--3174}
}
 

@Article{Hughes1993,
  author =          {Hughes, MD},
  title =          {Regression dilution in the proportional hazards model.},
  journal =          {Biometrics},
  year =          { 1993},
  volume =          {49},
  pages =          {1056-1066}
}

 

@Article{LonginiSusmitaHalloran1996,
  author =          {Longini ,IM and Susmita, D and Halloran, ME},
  title =          {Measuring vaccine efficacy for both susceptibility
        to infection and reduction in infectiousness for
        prophylactic $\mbox{HIV}$-1 vaccines},
  journal =          {Journal of Acquired Immune Deficiency
                Syndromes and Human Retrovirology},
  year =          {1996},
  volume =          {13},
  pages =          {440--447}
}

 

@Article{Mellors1996,
  author =          {Mellors ,JW and Rinaldo CR Jr. and Gupta, P and et
al.},
  title =          {Prognosis in $\mbox{HIV}$-1 infection predicted by the
                quantity of virus in plasma.},
  journal =          {Science},
  year =          {1996},
  volume =          {272},
  pages =          {1167-1170}
}

 

@Article{Mellors1997,
  author =          {Mellors ,JW and Munoz, A and Giorgi, JV and et al. },
  title =          {Plasma viral load and $\mbox{CD4}$ + lymphocytes
                as prognostic markers of $\mbox{HIV}$-1 infection.},
  journal =          {Annals of Internal Medicine},
  year =          {1997},
  volume =          {126},
  pages =          {946-954}
}

 

@Article{Nelson1972,
  author =          {Nelson, W },
  title =          {Theory and applications of hazard plotting for censored
                        failure time data.},
  journal =          {Technometrics},
  year =          {1972},
  volume =          {14},
  pages =          {945-966}
}

@article{BreslowClayton1993,
         Author = {Breslow, NE and Clayton, DG},
         Title = {Approximate Inference in Generalized Linear Mixed Models},
         Year = 1993,
         Journal = {Journal of the American Statistical Association},
         Volume = 88,
         Pages = {9--25},
         Keywords = {Overdispersion; Penalized likelihood; Variance
component}
     }


@Article{PepeSelfPrentice1989,
  author =          {Pepe, MS and Self ,SG and Prentice, RL},
  title =          {Further results on covariate
measurement errors in cohort studies with time to response data.},
  journal =          {Statistics in Medicine},
  year =          {1989},
  volume =          {8},
  pages =          {1167-1178}
}

@article{BreslowHolubkov1997,
  title={Maximum Likelihood Estimation of Logistic Regression Parameters under Two-phase, Outcome-dependent Sampling},
  author={Breslow, Norman E and Holubkov, Richard},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={59},
  number={2},
  pages={447--461},
  year={1997},
  publisher={Wiley Online Library}
}

@Article{Breslowetal2009a,
  author =          {Breslow, NE and Lumley, T and Ballantyne, CM and Chambless, LE and Kulich, M},
  title =          {Using the whole cohort in the analysis of case-cohort data.},
  journal =          {American Journal of Epidemiology},
  year =          {2009},
  volume =          {169},
  pages =          {1398--1405}
}
%note={PMCID: PMC2768499}

@Article{Breslowetal2009b,
  author =          {Breslow, NE and Lumley, T and Ballantyne, CM and Chambless, LE and Kulich, M},
  title =          {Improved {Horvitz-Thompson} Estimation of Model Parameters from Two-phase Stratified Samples: Applications in Epidemiology},
  journal =          {Statistical Biosciences},
  year =          {2009},
  volume =          {1},
  pages =          {32--49}
}

@article{WellnerSaegusa13,
    AUTHOR={Saegusa, T. and Wellner, Jon A.},
    TITLE ={Weighted likelihood estimation under two-phase sampling},
    JOURNAL={Annals of Statistics},
    VOLUME={41}, 
    YEAR={2013},
    PAGES={269--295}
 }
 
@Article{HorvitzThompson1952,
  author =          {Horvitz, DG and Thompson, DJ},
  title =          {A generalization of sampling without replacement from a finite universe.},
  journal =          {Journal of the American Statistical Association},
  year =          {1952},
  volume =          {47},
  pages =          {663--685}
}





@Article{Prentice1982,
  author =          {Prentice, RL},
  title =          {Covariate measurement errors and parameter estimation
in a failure time regression model.},
  journal =          {Biometrika},
  year =          {1982},
  volume =          {69},
  pages =          {331-342}
}


@Article{Prentice1978,
  author =          {Prentice, RL and Kalbfleisch ,JD and Peterson, AV and
                Fluornoy, N and Farewell, VT and Breslow, NE},
  title =          {The analysis of failure time in the presence of
competing risk.},
  journal =          {Biometrics},
  year =          {1978},
  volume =          {34},
  pages =          {541-554}
}

 

@Article{Quinn2000,
  author =          {Quinn, TC and Wawer ,MJ and Sewankambo, N and et al.},
  title =          {Viral load and
heterosexual transmission of human immunodeficiency virus type 1},
  journal =          {New England Journal of Medicine},
  year =          {2000},
  volume =          {342},
  pages =          {921-929}
}

 
@Article{Ramlau-Hansen1983,
  author =          {Ramlau-Hansen, H},
  title =          {Smoothing counting process intensities by means of
                kernel functions.},
  journal =         {Annals of Statistics},
  year =          {1983},
  volume =          {11},
  pages =          {453-66}
}

@Article{Rosenbaum1984,
  author =          {Rosenbaum, PR},
  title =          {The consequence of adjustment for a concomitant variable that has been affected by the treatment.},
  journal =          {Journal of the Royal Statistical Society, Series A},
  year =          {1984},
  volume =          {147},
  pages =          {656-666}
}

@Article{RobinsGreenland1992,
  author =          {Robins, JM and Greenland, S},
  title =          {Identifiability and exchangeability
of direct and indirect effects.},
  journal =          {Epidemiology},
  year =          {1992},
  volume =          {3},
  pages =          {143-155}
}

 


@Article{RiceRosenblatt1976,
  author =          {Rice, J and Rosenblatt, M},
  title =          {Estimation of the log survivor function and
hazard function. },
  journal =          {Sankhy$\bar{a}$, Series A},
  year =          {1976},
  volume =          {38},
  pages =          {60-78}
}

 

@Article{ShenSiliciano2000,
  author =          {Shen, X and Siliciano, RF},
  title =          {$\mbox{AIDS}$: Preventing $\mbox{AIDS}$ but not
$\mbox{HIV}$-1 infection with a $\mbox{DNA}$ vaccine.},
  journal =          {Science},
  year =          {2000},
  volume =          {290},
  pages =          {463-465}
}

 

@Article{Wang1997,
  author =          {Wang, CY and Hsu ,L and Feng ,ZD and Prentice, RL},
  title =          {Regression calibration in
failure time regression.},
  journal =          {Biometrics},
  year =          {1997},
  volume =          {52},
  pages =          {131-145}
}


@Article{WangTaylor2001,
  author =          {Wang ,Y and Taylor, JMG},
  title =          {Jointly modeling longitudinal and event time
data with application to acquired immunodeficiency syndrome. },
  journal =          {Journal of the American Statistical Association},
  year =          {2001},
  volume =          {96},
  pages =          {895-905}
}

 

@Article{Yandell1983,
  author =          {Yandell, BS},
  title =          {Nonparametric inference for rates with censored survival data.},
  journal =          {Annals of Statistics},
  year =          {1983},
  volume =          {11},
  pages =          {1119--1135}
}

 

@Article{ZhouPepe1995,
  author =          {Zhou, H and Pepe, MS},
  title =          {Auxiliary covariate data in failure time
regression. },
  journal =          {Biometrika},
  year =          {1995},
  volume =          {82},
  pages =          {139-149}
}

 

@InProceedings{Pitisutithum2004,
  author =          {Pitisutithum, P},
  title =          {Efficacy of $\mbox{AIDSVAX}$ $\mbox{B/E}$ vaccines in injecting drug use},
  booktitle =          {Eleventh Conference on Retroviruses and Opportunistic
Infections},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2004},
  OPTeditor =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {San Francisco, CA, 2004},
  OPTpublisher = {},
  note =          {Abstract No. 107.},
  OPTannote =          {}
}

@InProceedings{Harro2005,
  author =          {Harro, C and Edupuganti, S and Goepfert, P and et al.},
  title =          {Safety and Immunogenicity of Adenovirus Type 5 ($\mbox{Ad5}$) $\mbox{HIV-1}$ gag Vaccines},
  booktitle =          {Twelfth Conference on Retroviruses and Opportunistic
Infections},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2005},
  OPTeditor =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Boston, MA, 2005},
  OPTpublisher = {},
  note =          {Abstract No. 504.},
  OPTannote =          {}
}

@article{Coreyetal2011,
  title={{HIV-1} vaccines and adaptive trial designs},
  author={Corey, L and Nabel, GJ and Dieffenbach, C and Gilbert, Peter B and Haynes, BF and Johnston, M and Kublin, J and Lane, HC and Pantaleo, G and Picker, LJ and Fauci,AS},
  journal={Science Translational Medicine},
  volume={3},
  number={79},
  pages={79ps13},
  year={2011},
  publisher={NIH Public Access},
  note={PMCID: PMC3616511}
}


 

@Article{Gilbert2003,
  author =          {Gilbert, Peter B and DeGruttola, V and Hudgens, M and
Self, S
                  and Hammer, S and Corey, L},
  title =          {What constitutes efficacy for an $\mbox{HIV}$ vaccine that
                  ameliorates viremia: Issues involving surrogate endpoints
                  in $\mbox{Phase III}$ trials.},
  journal =          {Journal of Infectious Diseases},
  year =          {2003},
  Volume = 188,
  Pages = {179--93},
}

@Article{Pitisuttithumetal2006,
  author =          {Pitisuttithum, P and Gilbert, Peter B and Gurwith, M and Heyward, W and Martin, M and van Griensven, F and Hu, D and Tappero, JW and Choopanya, K and the Bangkok Vaccine Evaluation Group},
  title =          {Randomized, double-blind, placebo-controlled efficacy trial of a bivalent recombinant
glycoprotein 120 $\mbox{HIV-1}$ vaccine among injection drug users in Bangkok, Thailand.},
  journal =          {Journal of Infectious Diseases},
  year =          {2006},
  Volume = {194},
  Pages = {1661--1671}
}

@Article{ShepherdRedmanAnkerst2009,
author = {Shepherd, BE and Redman, MW and Ankerst, DP},
title = {Does finasteride affect the severity of prostate cancer? A causal sensitivity analysis},
journal = {Journal of the American Statistical Association},
year = {2008},
volume = {103},
pages = {1392--1404}
}
 

@article{TsiatisDavidian2001,
    Author = {Tsiatis, AA and Davidian, M},
    Title = {A Semiparametric Estimator for the Proportional Hazards Model
            With Longitudinal Covariates Measured With Error},
    Year = 2001,
    Journal = {Biometrika},
    Volume = 88,
    Number = 2,
    Pages = {447--458},
    Keywords = {[conditional score]; [measurement error]; [mixed effects
               model]; [regression calibration]; [semiparametric];
               [survival analysis]}
}

 

@article{Odell1992,
    Author = {Odell, PM and Anderson, KM and D'Agostino,
             RB},
    Title = {Maximum Likelihood Estimation for Interval-censored Data Using
            a {W}eibull-based Accelerated Failure Time Model},
    Year = 1992,
    Journal = {Biometrics},
    Volume = 48,
    Pages = {951--959}
}

 

@Article{Harro2004,
  author =          {Harro, CD and Judson, FN and Gorse, GJ and
Mayer,
KH and Kostman, JR and Brown,
SJ and Koblin, B and Marmor, M and Bartholow, BN and Popovic, V and for the $\mbox{VAX004}$ Study Group},
  title =          {Recruitment and baseline epidemiologic profile of
participants in the first phase 3 $\mbox{HIV}$ vaccine efficacy trials.},
  journal =          {Journal of Acquired Immunodeficiency Syndrome},
  year =          {2004},
  volume = {37},
  pages = {1385-1392}
}

 

@Article{Schacker1998,
  author =          {Schacker, TW and Hughes, JP and Shea, T and
Coombs,
RW and Corey, L},
  title =          {Biological and virologic characteristics of primary $\mbox{HIV}$
infection},
  journal =          {Annals of Internal Medicine},
  year =          {1998},
  volume =          {128},
  OPTnumber =          {},
  pages =          {613--20},
}

@Article{LittleAn2004,
  author =          {Little, RJA and An, H},
  title =          {Robust likelihood-based analysis of multivariate data with missing values.},
  journal =          {Statistica Sinica},
  year =          {2004},
  volume =          {14},
  OPTnumber =          {},
  pages =          {949--968}
}


 

@Article{Schacker2000,
  author =          {Schacker, T and Little, S and Connick, E and
et al.},
  title =          {Rapid accumulation of human immunodeficiency virus
($\mbox{HIV}$) in
                  lymphatic tissue reservoirs during acute and early $\mbox{HIV}$
infection: implications for timing of antiretroviral therapy.},
  journal =          {Journal of Infectious Diseases},
  year =          {2000},
  volume =          {181},
  OPTnumber =          {},
  pages =          {354--357},
}

 


@Article{CaiBetensky2003,
  author =       {Cai, T and Betensky, RA},
  title =        {Hazard regression for interval-censored data with
penalized splines},
  journal =      {Biometrics},
  year =         {2003},
  volume =       {59},
  pages =        {570--9},
}

@InProceedings{Branson2019,
  author =          {Branson, BM},
  title =          {{HIV testing: updates and challenges. International AIDS Society 2019: 10th IAS Conference on HIV Science}.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2019}, 
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Mexico City, Mexico, 2019},
  OPTpublisher = {},
  note =          {},
  OPTannote =          {}
}
 

@TechReport{CaiGilbert2004,
  author =          {Cai, T and Gilbert, Peter B},
  title =          {Asymptotic results and proofs for $\mbox{Cox}$ model
inferences on relative risks linked in two stages},
  institution =  {Harvard University},
  year =          {2004},
  OPTkey =          {},
  OPTtype =          {},
  OPTnumber =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

 



@Article{AndersonHanson2005,
author =          {Anderson, R and Hanson, M},
title =          {Potential public health impact of imperfect $\mbox{HIV}$ type 1
vaccines.},
journal =          {Journal Infectious Diseases},
year =          {2005},
volume =          {191},
pages =          {Suppl:S85-S96}
}

@Article{Baker2003,
  author =          {Baker, SG},
  title =          {The central role of receiver operating
characteristic (ROC) curves in evaluating tests for the early detection
of cancer.},
  journal =          {Journal of the National Cancer Institute},
  year =          {2003},
  volume =          {95},
  pages =          {511-515}
}

@Article{Beerenwinkel2002,
  author =          {Beerenwinkel, N and Schmidt, B and Walter, H and Kaiser, R and
Lengauer, T and Hoffmann, D and Korn, K and Selbig, J},
  title =          {Diversity and complexity of $\mbox{HIV}$-1 drug resistance: 
a bioinformatics approach to predicting phenotype from genotype.},
  journal =          {Proceedings of the National Academy of Science},
  year =          {2002},
  volume =          {99},
  pages =          {8271-8276}
}

 

@Article{Blattner2004,
author =          {Blattner, WA and Oursler, KA and Cleghorn, F and Charurat, M and Sill,
A and Bartholomew, C and Jack, N and O'Brien, T and Edwar,ds E and Tomaras, G and Weinhold, K
and Greenberg, M},
title =          {Rapid clearance of virus after acute $\mbox{HIV}-1$ infection:
Correlates of risk of $\mbox{AIDS}$.},
journal =          {Journal of Infectious Diseases},
year =          {2004},
volume =          {189},
pages =          {1793-1801}
}

@Article{Boaz2002,
  author =          {Boaz, MJ and Waters, A and Murad, S and Easterbrook, PJ
and Vyakarnam, A},
  title =          {Presence of $\mbox{HIV}$-1 $\mbox{Gag}$-specific $\mbox{IFN-gamma+IL-2+}$ and
$\mbox{CD28+IL-2+ CD4 T cell}$ responses is associated with nonprogression in
$\mbox{HIV}$-1 infection.},
  journal =          {Journal of Immunology},
  year =          {2002},
  volume =          {169},
  pages =          {6376-6385}
}

@article{Hongetal2016,
  title={Novel assays for measurement of total cell-associated {HIV-1 DNA and RNA}},
  author={Hong, Feiyu and Aga, Evgenia and Cillo, Anthony R and Yates, Aarika L and Besson, Guillaume and Fyne, Elizabeth and Koontz, Dianna L and Jennings, Cheryl and Zheng, Lu and Mellors, John W},
  journal={Journal of Clinical Microbiology},
  volume={54},
  number={4},
  pages={902--911},
  year={2016},
  publisher={Am Soc Microbiol},
  note={PMCID: PMC4809955}
}

@Book{Breiman1984,
  author =          {Breiman, L and Friedman, JH and Olshen, RA and Stone, CJ},
  ALTeditor =          {},
  title =          {Classification and Regression Trees.},
  publisher =          {Belmont: Wadsworth },
  year =          {1984},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  address =          {Belmont, CA},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Article{Breiman2001a,
  author =          {Breiman, L},
  title =          {Statistical modeling:  the two cultures.},
  journal =          {Statistical Science},
  year =          {2001},
  volume =          {16},
  pages =          {199-215}
}

@article{LongHudgensWu2015,
  title={Surrogates of protection in repeated low-dose challenge experiments},
  author={Long, Dustin M and Hudgens, Michael G and Wu, Chih-Da},
  journal={Statistics in Medicine},
  volume={34},
  number={10},
  pages={1747--1760},
  year={2015},
  publisher={Wiley Online Library},
  note={PMCID: PMC4390486}
}

@article{Hanetal2017,
  title={Mark-specific additive hazards regression with continuous marks},
  author={Han, Dongxiao and Sun, Liuquan and Sun, Yanqing and Qi, Li},
  journal={Lifetime Data Analysis},
  volume={23},
  number={3},
  pages={467--494},
  year={2017},
  publisher={Springer},
  note={PMCID: PMC5319915}
}

@Article{Breiman2001b,
  author =          {Breiman, L},
  title =          {Random forests.},
  journal =          {Machine Learning},
  year =          {2001},
  volume =          {45},
  pages =          {5-32}
}


@Article{BujaHastieTibshirani1989,
  author =          {Buja, A and Hastie, T and Tibshirani, R},
  title =          {Linear smoothers and additive models (with
discussions).},
  journal =          {Annals of Statistics},
  year =          {1989},
  volume =          {17},
  pages =          {453-555}
}


@Article{Burton2004,
  author =          {Burton, DR and Desrosiers, RC and Johnson, PR and Koff, WC},
  title =          {An $\mbox{AIDS}$ vaccine: no time to give up.},
  journal =          {Lancet},
  year =          {2004},
  volume =          {364},
  pages =          {1938}
}


@Article{Burton2004b,
  author =          {Burton, DR and Desrosiers, RC and Doms, RW and Koff, WC and Kwong,
PD and Moore, JP and Nabel, GJ and Sodroski, J and Wilson, IA and Wyatt, RT},
  title =          {$\mbox{HIV}$ vaccine design and the neutralizing antibody
problem.},
  journal =          {Nature Immunology},
  year =          {2004},
  volume =          {5},
  pages =          {233-236}
}

@Article{Bakeretal2009,
  author =          {Baker, BM and Block, BL and Rothchild, AC and Walker, BD},
  title =          {Elite control of $\mbox{HIV}$ infection: implications for vaccine design.},
  journal =          {Expert Opinion on Biological Therapy},
  year =          {2009},
  volume =          {9},
  pages =          {55---69},
  note={PMCID: PMC3731764}
}

@Article{BuyseMolenberghs1998,
  author =          {Buyse, M and Molenberghs, G},
  title =          {Criteria for the validation of surrogate endpoints
in randomized experiments.},
  journal =          {Biometrics},
  year =          {1998},
  volume =          {54},
  pages =          {1014-1029}
}

@Article{Buyse2000,
  author =          {Buyse, M and Molenberghs, G and Burzykowski, T and Renard, D
and Geys, H},
  title =          {The validation of surrogate endpoints in
meta-analyses of randomized experiments.},
  journal =          {Biostatistics},
  year =          {2000},
  volume =          {1},
  pages =          {49-67}
}


@Article{CarolWand1991,
  author =          {Carol, RJ and Wand, MP},
  title =          {Semiparametric estimation in logistic measurement
error models.},
  journal =          {Journal of the Royal Statistical Society, Series B},
  year =          {1991},
  volume =          {53},
  pages =          {573-587}
}


@Article{Chan2002,
  author =          {Chan, ISF and Shu, L and Matthews, H and Chan, C and Vessey, R and
Sadoff, J and Heyse, J},
  title =          {Use of statistical models for evaluating antibody
response as a correlate of protection against varicella.},
  journal =          {Statistics in Medicine},
  year =          {2002},
  volume =          {21},
  pages =          {3411-3430}
}

@Article{Vesseyetal2001,
  author =          {Vessey, SJR and Chan, CY and Kuter, BJ and Kaplan, KM and Waters, M and Kutzler, DP and Carfagno, PA and Sadoff, JC and Heyse, JF and Matthews, H and Li, S and Chan, ISF},
  title =          {Childhood vaccination against varicella: persistence of antibody, duration of protection, and vaccine efficacy.},
  journal =          {The Journal of Pediatrics},
  year =          {2001},
  volume =          {139},
  pages =          {297--304}
}


@Article{SadoffWittes2007,
  author =          {Sadoff, JC and Wittes, J}, 
  title =          {Correlates, surrogates, and vaccines.},
  journal =          {The Journal of Infectious Diseases},
  year =          {2007},
  volume =          {196},
  pages =          {1279--1281},
  note={PMCID: }
}

@article{Hernan2010,
  title={The hazards of hazard ratios},
  author={Hern{\'a}n, Miguel A},
  journal={Epidemiology},
  volume={21},
  number={1},
  pages={13-15},
  year={2010},
  publisher={NIH Public Access}
}

@article{hernanvanderWeele2011,
  title={Compound treatments and transportability of causal inference},
  author={Hern{\'a}n, Miguel A and VanderWeele, Tyler J},
  journal={Epidemiology},
  volume={22},
  number={3},
  pages={368-377},
  year={2011},
  publisher={NIH Public Access}
}

@Article{FDAGuidance2007,
  author =          {{FDA Guidance Document}}, 
  title =          {{FDA Guidance for Industry}: Clinical Trial Endpoints for the Approval of Cancer Drugs and Biologics.},
  year =          {2007}
}

@Article{ZhaoWangChan2008,
  author =          {Zhao, Y and Wang, WWB and Chan, ISF}, 
  title =          {Application of survival methodologies in vaccine trials.},
  journal =          {FDA/Industry Workshop on Applied Statistics},
  year =          {2008},
  volume =          {},
  pages =          {},
  note={PMCID: }
}

@Article{HuangGilbert2011,
  author =          {Huang, Y and Gilbert, Peter B},
  title =          {Comparing biomarkers as principal surrogate endpoints.},
  journal =          {Biometrics},
  year =          {2011},
  volume =          {67},
  pages =          {1442--1451},
note={PMCID: PMC3163011}
}
%  

@Article{JuGeng2010,
  author =          {Ju, C and Geng, Z},
  title =          {Criteria for surrogate end points based on causal distributions.},
  journal =          {Journal of the Royal Statistical Society Series B},
  year =          {2010},
  volume =          {72},
  pages =          {129--142}
}







@Article{Chen2001,
  author =          {Chen, K},
  title =          {Generalized case-cohort sampling.},
  journal =          {Journal of the Royal Statistical Society, Series B},
  year =          {2001},
  volume =          {63},
  pages =          {791-809}
}


@Article{ChenLo1999,
  author =          {Chen, K and Lo, S-H},
  title =          {Case-cohort and case-control analysis with $\mbox{Cox}$'s
model.},
  journal =          {Biometrika},
  year =          {1999},
  volume =          {86},
  pages =          {755-764}
}


@Article{Chen2002,
  author =          {Chen, HY},
  title =          { Double-semiparametric method for missing covariates
in $\mbox{Cox}$ regression models.},
  journal =          {Journal of the American Statistical Association},
  year =          {2002},
  volume =          {97},
  pages =          {565-575}
}


@Article{RV1442009,
 author = {Rerks-Ngarm, S and Pitisuttithum, P and Nitayaphan, S 
 and Kaewkungwal, J and Chiu, J and Paris, R and
 Premsri, N and Namwat, C and de Souza, M and Adams, E and Benenson, M and Gurunathan, S and Tartaglia, J and McNeil, 
 JG and Francis, DP and Stablein, D and Birx, DL and Chunsuttiwat, S and Khamboonruang, C and Thongcharoen, P and
 Robb, ML and Michael, NL and Kunasol, P and Kim, JH and the MOPH--TAVEG Investigators},
 title = {Vaccination with $\mbox{ALVAC}$ and $\mbox{AIDSVAX}$ to Prevent HIV-1 Infection in Thailand.},
   journal = {New England Journal of Medicine},
   year =          {2009},
   volume =          {361},
  pages =          {2209--2220}
}

@Article{RV1442009short,
 author = {Rerks-Ngarm, S and Pitisuttithum, P and Nitayaphan, S and et al.},
 title = {Vaccination with $\mbox{ALVAC}$ and $\mbox{AIDSVAX}$ to Prevent $\mbox{HIV-1}$ Infection in Thailand.},
   journal = {New England Journal of Medicine},
   year =          {2009},
   volume =          {361},
  pages =          {2209--2220}
}

@Article{RV1442009short2,
 author = {Rerks-Ngarm, S and Pitisuttithum, P and Nitayaphan, S and Kaewkungwal, J and Chiu, J and Paris, R and et al.},
 title = {Vaccination with $\mbox{ALVAC}$ and $\mbox{AIDSVAX}$ to Prevent $\mbox{HIV-1}$ Infection in Thailand.},
   journal = {New England Journal of Medicine},
   year =          {2009},
   volume =          {361},
  pages =          {2209--2220}
}

@Article{RerksNgarmetal2009short,
 author = {Rerks-Ngarm, S and Pitisuttithum, P and Nitayaphan, S and Kaewkungwal, J and Chiu, J and Paris, R and et al.},
 title = {Vaccination with $\mbox{ALVAC}$ and $\mbox{AIDSVAX}$ to Prevent $\mbox{HIV-1}$ Infection in Thailand.},
   journal = {New England Journal of Medicine},
   year =          {2009},
   volume =          {361},
  pages =          {2209--2220}
}

@Article{FalkBall2001,
 author = {Falk, L and Ball, LK},
 title = {Current status and future trends in vaccine regulation.}, 
   journal = {Vaccine},
   year =          {2001},
   volume =          {19},
  pages =          {1567--1572}
}




@Article{ChenLittle1999,
  author =          {Chen, HY and Little, RJ},
  title =          { Proportional hazards regression with missing
covariates.},
  journal =          {Journal of the American Statistical Association},
  year =          {1999},
  volume =          {94},
  pages =          {896-908}
}


@Book{ChristianiShawe-Taylor2000,
  author =          {Christiani, N and Shawe-Taylor, J},
  ALTeditor =          {},
  title =          {An Introduction to Support Vector Machines.},
  publisher =          {Cambridge University Press },
  year =          {2000},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  address =          {Cambridge},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{DanielsHughes1997,
  author =          {Daniels, MJ and Hughes, MD},
  title =          {Meta-analysis for the evaluation of potential
surrogate markers.},
  journal =          {Statistics in Medicine},
  year =          {1997},
  volume =          {16},
  pages =          {1965-1982}
}


@Article{DonohoJohnstone1995,
  author =          {Donoho, DL and Johnstone, IM},
  title =          { Adapting to unknown smoothness via wavelet shrinkage.},
  journal =          {Journal of the American Statistical Association},
  year =          {1995},
  volume =          {90},
  pages =          {1200-1224}
}


@Article{DudoitFridylandSpeed2002,
  author =          {Dudoit, S and Fridyland, JF and Speed, TP},
  title =          {Comparison of discrimination methods for tumor
classification based on microarray data.},
  journal =          {Journal of the American Statistical Association},
  year =          {2002},
  volume =          {97},
  pages =          {77-87}
}

@Article{FollmannFayProschan2009,
    title = {Chop-Lump Tests for Vaccine Trials},
    author = {Dean Follmann and Michael P. Fay and Michael Proschan},
    journal = {Biometrics},
    year = {2009},
    volume = {65},
    pages = {885--893}
}



@Article{Follmann2000,
author =          {Follmann, D},
title =          {On the effect of treatment among treatment compliers: 
An analysis of the multiple risk factor intervention trial.},
journal =          {Journal of the American Statistical Association},
year =          {2000},
volume =          {95},
pages =          {1101-1109}
}

@Article{ScheikeMartinussen2004,
author =          {Scheike, TH and Martinussen, T},
title =          {Maximum likelihood estimation for $\mbox{Cox}$'s regression model under case-cohort sampling.},
journal =          {Scandinavian Journal of Statistics},
year =          {2004},
volume =          {31},
pages =          {283--293}
}

@Article{FrangakisRubin2002,
author =          {Frangakis, CE and Rubin, DB},
title =          {Principal stratification in causal inference},
journal =          {Biometrics},
year =          {2002},
volume =          {58},
pages =          {21-29}
}

@Article{Rubin2000,
author =          {Rubin, DB},
title =          {Comment on ``$\mbox{Causal}$ inference without counterfactuals,''
by $\mbox{A.P. Dawid}$},
journal =          {Journal of the American Statistical Association},
year =          {2000},
volume =          {95},
pages =          {435--437}
}

@article{zolla2014vaccine,
  title={Vaccine-induced human antibodies specific for the third variable region of {HIV-1} gp120 impose immune pressure on infecting viruses},
  author={Zolla-Pazner, Susan and Edlefsen, Paul T and Rolland, Morgane and Kong, Xiang-Peng and deCamp, Allan and Gottardo, Raphael and Williams, Constance and Tovanabutra, Sodsai and Sharpe-Cohen, Sandra and Mullins, James I and deSouza, Mark S and Karasavvas, Nicos and Nitayaphan, Sorachai and Rerks-Ngarm, Supachai and Pitisuttihum, Punnee and Kaewkungwal, Jaranit and O'Connell, Robert J and Robb, Merlin L and Michael, Nelson L and Kim, Jerome H and Gilbert, Peter },
  journal={EBioMedicine},
  volume={1},
  number={1},
  pages={37--45},
  year={2014},
  publisher={Elsevier},
  note={PMCID: PMC4293639}
}


@InProceedings{FreundSchapire1996,
  author =          {Freund, Y and Schapire, R },
  title =          {Experiments with a new boosting algorithm},
  booktitle =          {Machine Learning:  Proceedings of the Thirteenth
 International Conference},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {148-156},
  year =          {1996},
  OPTeditor =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {},
  OPTpublisher = {},
  note =          {},
  OPTannote =          {}
}


@Book{FriedmanPopescu2004,
  author =          {Friedman, JH and Popescu, BE},
  ALTeditor =          {},
  title =          {Gradient directed regularization for linear
regression and classification.},
  publisher =          {Stanford University },
  year =          {2004},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {Technical Report},
  address =          {Department of Statistics, Stanford University},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@article{Plotkin2008,
        author = {Plotkin, Stanley A},
     journal = {Clinical Infectious Diseases},
        month = {August},
        number = {3},
        pages = {401--409},
                title = {Vaccines: Correlates of vaccine-induced immunity},
           volume = {47},
        year = {2008}
}


@article{Plotkin2010,
        author = {Plotkin, Stanley A},
        journal = {Clinical Vaccine Immunology},
        month = {May},
        number = {7},
        pages = {1055--1065},
        title = {Correlates of Protection Induced by Vaccination.},
        volume = {17},
        year = {2010},
        note={PMCID: PMC2897268}
}
%


@article{ImbensManski2004,
        author = {Imbens, GW and Manski, CF},
        journal = {Econometrica},
        pages = {1845--1857},
        title = {Confidence intervals for partially identified parameters},
        volume = {72},
        year = {2004}
}

@article{AngristImbensRubin1996,
        author = {Angrist, J and Imbens, G and Rubin, D},
        journal = {Journal of the American Statistical Association},
        pages = {444--472},
        title = {Identification of causal effects using instrumental variables (with comments)},
        volume = {91},
        year = {1996}
}

@article{RobinsGreenland1996, 
        author = {Robins, JM and Greenland, S},  
        journal = {Journal of the American Statistical Association},
        pages = {456--458},
        title = {Comment on, ``$\mbox{I}$dentification of causal effects using instrumental variables (with comments)".},
        volume = {91},
        year = {1996}
}




@article{BalkePearl1997,
        author = {Balke, A and Pearl, J},
        journal = {Journal of the American Statistical Association},
        pages = {1172--1176},
        title = {Bounds on treatment effects from studies with imperfect compliance.},
        volume = {92},
        year = {1997}
}







@Article{Gailetal2000,
author =          {Gail, MH and Pfeiffer, R and Van Houwelingen, HC and Carroll, RJ},
title =          {On meta-analytic assessment of surrogate outcomes.},
journal =          {Biostatistics},
year =          {2000},
volume =          {1},
pages =          {231-246}
}

@Article{Gao2004,
author =          {Gao, F and Korber, BT and Weaver, E and Liao, HX and Hahn, BH and 
Haynes, BF},
title =          {Centralized immunogens as a vaccine strategy to
overcome $\mbox{HIV}$-1 Diversity.},
journal =          {Experimental Retroviral Vaccines},
year =          {2004},
volume =          {Suppl 3},
pages =          {S161-S168}
}


@Article{GhoshChinnaiyan2005,
author =          {Ghosh, D and Chinnaiyan, AM},
title =          {Classification and selection of biomarkers in genomic
data using LASSO.},
journal =          {Journal of Biomedicine and Biotechnology},
year =          {in press},
pages =          {}
}


@Article{GilbertNovitskyEssex2005,
author =          {Gilbert, Peter B and Novitsky, V and Essex, M},
title =          {Covariability of selected amino acid positions for $\mbox{HIV}$
subtypes C and B.},
journal =          {AIDS Research and Human Retroviruses},
year =          {2005},
volume =          {in press},
pages =          {}
}


@Article{GilbertSun2005,
author =          {Gilbert, Peter B and Sun, Y},
title =          {Failure time analysis of $\mbox{HIV}$ vaccine effects on viral
load and antiretroviral therapy initiation.},
journal =          {Biostatistics},
year =          {2005},
volume =          {6},
pages =          {374-394}
}

@Article{GilbertSun2015,
author=  {Gilbert, Peter B and Sun, Y},
title= {Inferences on relative failure rates in stratified mark-specific proportional hazards models with missing marks, with application to {HIV} vaccine efficacy trials.},
journal= {Journal of the Royal Statistical Society: Series C (Applied Statistics)},
year = {2015},
volume =          {64},
pages =          {49-73},
note={PMCID:
    PMC4310507}
}

@Article{GilbertSun2013proceedings,
author =          {Gilbert, Peter B and Sun, Y},
title =          {Testing mark-specific vaccine efficacy with missing marks.},
year = {2013},
journal = {Proceedings of the 59th Institute Statistics International World Statistics Conference, Hong Kong, China},
  note={PMCID: }
}

@article{DaiLiGilbert2013,
  title={Case-only method for cause-specific hazards models with application to assessing differential vaccine efficacy by viral and host genetics},
  author={Dai, James Y and Li, Shuying S and Gilbert, Peter B},
  journal={Biostatistics},
  volume={15},
  number={1},
  pages={196--203},
  year={2013},
  publisher={Oxford University Press},
  note={PMCID: PMC3862206}
}

@article{dommaraju2014cd8,
  title={{CD8} and {CD4} epitope predictions in {RV144}: no strong evidence of a {T}-cell driven sieve effect in {HIV-1} breakthrough sequences from trial participants},
  author={Dommaraju, Kalpana and Kijak, Gustavo and Carlson, Jonathan M and Larsen, Brendan B and Tovanabutra, Sodsai and Geraghty, Dan E and Deng, Wenjie and Maust, Brandon S and Edlefsen, Paul T and Sanders-Buell, Eric and Ratto-Kim, Silvia and deSouza, Mark S and Rerks-Ngarm, Supachai and Nitayaphan, Sorachai and Pitisuttihum, Punnee and Kaewkungwal, Jaranit and O'Connell, Robert J and Robb, Merlin L and Michael, Nelson L and Mullins, James I and Kim, Jerome H and Rolland, Morgane},
  journal={PloS One},
  volume={9},
  number={10},
  pages={e111334},
  year={2014},
  publisher={Public Library of Science},
  note={PMCID: PMC4211711}
}


@Article{GolmHalloranLongini1998,
author =          {Golm, GT and Halloran, ME and Longini, IM},
title =          {Semiparametric models for mismeasured exposure
information in vaccine trials.},
journal =          {Statistics in Medicine},
year =          {1998},
volume =          {17},
pages =          {2335-2352}
}

@Article{HaneuseSaegusaLumley2011,
author = {Haneuse, S and Saegusa, T and Lumley, T},
title = {osDesign: an $\mbox{R}$ Package for the Analysis, evaluation, and
design of two-phase and case-control studies.},
journal = {Journal of Statistical Software},
year =          {2011},
volume =          {43}
}

@book{HalloranLonginiStruchiner2010,
  title={Design and Analysis of Vaccine Studies},
  author={Halloran, M Elizabeth and Longini, Ira M and Struchiner, Claudio J},
  year={2010},
  publisher={Springer}
}

@Article{GolmHalloranLongini1999,
author =          {Golm, GT and Halloran, ME and Longini, IM},
title =          {Semiparametric methods for multiple exposure
mismeasurement and a bivariate outcome in $\mbox{HIV}$ vaccine trials.},
journal =          {Biometrics},
year =          {1999},
volume =          {55},
pages =          {94-101}
}


@Article{Gonzalez2005,
author =          {Gonzalez, E and Kulkarni, H and Bolivar, H and Mangano, A and Sanchez,
R and Catano, G and Nibbs, RJ and Freedman, BI and Quinones, MP and Bamshad, MJ and
Murthy, KK and
Rovin, BH and Bradley, W and Clark, RA and Anderson, SA and O'Connell, RJ and Agan, BK and
Ahuja, SS and
Bologna, R and Sen, L and Dolan, MJ and Ahuja, SK},
title =          {The influence of $\mbox{CCL3L1}$ gene-containing segmental
duplications on $\mbox{HIV}$-1/$\mbox{AIDS}$ susceptibility.},
journal =          {Science},
year =          {2005},
volume =          {307},
pages =          {1434-1440}
}


@InProceedings{GuiLi2005,
  author =          {Gui, J and Li, H},
  title =          {Threshold gradient descent mthod for censored data
regression with applications in pharmacogenetics},
booktitle =          {Proceedings of Pacific Symposium of Biocomputating 2005},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {148-156},
  year =          {2005},
  OPTeditor =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {},
  OPTpublisher = {},
  note =          {},
  OPTannote =          {}
}


@Article{Hallstrom2001,
author =          {Hallstrom, AP and McAnulty, JH and Wilkoff, BL and Follmann, D and
Raitt, MH and Carlson, MD and Gillis, AM and Shih, HT and Powell, JL and Duff, H and
Halperin, BD},
title =          {Patients at lower risk of arrhythmia occurrence:  A
subgroup in whom implantable defibrillators may not offer benefit.},
journal =          {Journal of the American College of Cardiology},
year =          {2001},
volume =          {37},
pages =          {1093-1099}
}


@Book{HastieTibshirani1990,
  author =          {Hastie, TJ and Tibshirani, RJ},
  ALTeditor =          {},
  title =          {Generalized Additive Models.},
  publisher =          {Chapman and Hall },
  year =          {1990},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  address =          {London},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Book{Pearl2001,
  author =          {Pearl, J},
  title =          {Direct and {I}ndirect {E}ffects.},
  journal =         {Proceedings of the 17th annual conference on uncertainty in artifial intelligence (UAI-01)},
  year =          {2001},
  publisher =          {Morgan Kaufmann},
  address = {San Francisco},
  pages = {411-442}
}


@Book{HastieTibshiraniFriedman2001,
  author =          {Hastie, TJ and Tibshirani, RJ and Friedman, J},
  ALTeditor =          {},
  title =          {The Elements of Statistical Learning.},
  publisher =          {Springer-Verlag },
  year =          {2001},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  address =          {New York, NY},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{HastieTibshirani1993,
author =          {Hastie, TJ and Tibshirani, RJ},
title =          {Varying-coefficient models (with discussion).},
journal =          {Journal of the Royal Statistical Society B},
year =          {1993},
volume =          {55},
pages =          {757-796}
}

@Article{Saar-TsechanskyProvost2007,
author =          {Saar-Tsechansky, M and Provost, F},
title =          {Handling missing values when applying classification models.},
journal =          {Journal of Machine Learning Research},
year =          {2007},
volume =          {8},
pages =          {1623--1657}
}


@Article{HuLawless1996,
author =          {Hu, XJ and Lawless, JF},
title =          {Estimation from truncated lifetime data with
supplementary information on covariates and censoring time.},
journal =          {Biometrika},
year =          {1996},
volume =          {83},
pages =          {747-761}
}

@Article{GilbertHudgens2008,
author =          {Gilbert, Peter B and Hudgens, MG},
title =          {Evaluating candidate principal surrogate endpoints}, 
journal =          {Biometrics},
year =          {2008},
volume =         {64},
pages =          {1146-1154}
}
%note={PMCID: PMC2726718}

@Article{Nan2004,
author =          {Nan, B},
title =          {Efficient estimation for case-cohort studies},
journal =          {Canadian Journal of Statistics},
year =          {2004},
volume =         {32},
pages =          {403--419}
}

@Article{Hoofetal2009,
author =          {Hoof, I and Peters, B and Sidney, J and Pedersen, LE and Sette, A and Lune, O and Buus, S and Nielsen, M},
title =          {$\mbox{Net}$$\mbox{MHC}$pan, a method for $\mbox{MHC}$ class $\mbox{I}$ binding prediction beyond humans.},
journal =          {Immunogenetics},
year =          {2009},
volume =         {61},
pages =          {1--13},
  note={PMCID: PMC3319061}
}

@Article{Nielsenetal2007,
author =          {Nielsen, M and Lundegaard, C and Blicher, T and Lamberth, K and Harndahl, M and Justesen, S and 
Roder, G and Peters, B and Sette, A and Lune, O and Buus, S},
title =          {$\mbox{Net}$$\mbox{MHC}$pan, a method for quantitative predictions of peptide binding to any $\mbox{HLA-A}$ 
and $\mbox{-B}$ locus 
protein of known sequence.},
journal =          {PLoS ONE},
year =          {2007},
volume =         {2},
pages =          {e796},
  note={PMCID: PMC1949492}
}

@Article{Linetal2008,
author =          {Lin, HH and Ray, S and Tongchusak, S and Reinherz, EL and Brusic, V},
title =          {Evaluation of $\mbox{MHC}$ class $\mbox{I}$ peptide binding prediction servers: Applications for vaccine research.}, 
journal =          {BMC Immunology},
year =          {2008},
volume =         {9},
pages =          {8},
  note={PMCID: PMC2323361}
}


@Article{LiGilbertNan2008,
author =          {Li, Z and Gilbert, Peter B and Nan, B},
title =          {Weighted likelihood method for grouped survival data in case-cohort studies with application to $\mbox{HIV}$ vaccine trials.},
journal =          {Biometrics},
year =          {2008},
volume =         {64},
pages =          {1247--1255}
}


@Article{HudgensHalloran2006,
author =          {Hudgens, MG and Halloran, ME},
title =          {Causal vaccine effects on binary postinfection 
outcomes},
journal =          {Journal of the American Statistical Association},
year =          {2006},
volume =         {101},
pages =          {51-64}
}

@Article{BreslowWellner2007,
author =          {Breslow, N and Wellner, JA},
title =          {Weighted likelihood for semiparametric models and two-phase stratified samples, with application to $\mbox{Cox}$ regression.}, 
journal =          {Scandinavian Journal of Statistics},
year =          {2007},
volume =         {34},
pages =          {86-102},
  note={PMCID: }
}

@Article{JoffeGreene2009,
author =          {Joffe, MM and Greene, T},
title =          {Related causal frameworks for surrogate outcomes.},
journal =          {Biometrics},
year =          {2009},
volume =         {65},
pages =          {530--538} 
}
%note={PMCID: PMC2835417}



@Article{WolfsonGilbert2010,
author =          {Wolfson, J and Gilbert, Peter B},
title =          {Statistical identifiability and the surrogate endpoint problem, with application to vaccine trials.},
journal =          {Biometrics},
year =          {2010},
volume =         {66},
pages =          {1153--1161},
  note={PMCID: PMC3597127}
}


@Article{Hughes2002,
author =          {Hughes, MD},
title =          {Evaluating surrogate endpoints.},
journal =          {Controlled Clinical Trials},
year =          {2002},
volume =          {23},
pages =          {703-707}
}

@Article{GilbertQinSelf2008,
author =          {Gilbert, Peter B and Qin, L and Self, SG},
title =          {Evaluating a surrogate endpoint at three levels, with application to vaccine development.},
journal =          {Statistics in Medicine},
year =          {2008},
volume =          {27},
pages =          {4758--4778},
  note={PMCID: PMC2646675}
}

@Article{Dunning2008,
author =          {Dunning, AJ},
title =          {Comment on ``$\mbox{Evaluating}$ a surrogate endpoint at three levels, with application to vaccine development."},
journal =          {Statistics in Medicine},
year =          {2008},
volume =          {27},
pages =          {6268--6270},
  note={PMCID: }
}

@Article{GilbertQinSelf2009,
author =          {Gilbert, Peter B and Qin, L and Self, SG},
title =          {Response to $\mbox{Andrew Dunning's}$  Comment on ``$\mbox{Evaluating}$ a surrogate endpoint at three levels, with application to vaccine development"},
journal =          {Statistics in Medicine},
year =          {2009},
volume =          {28},
pages =          {716--719}
}


@Article{JonesTaylorThornton1992,
author =          {Jones, DT and Taylor, WR and Thornton, JM},
title =          {The rapid generation of mutation data matrices from
protein sequences.},
journal =          {Computations and Applied Biosciences},
year =          {1992},
volume =          {8},
pages =          {275-282}
}


@Article{KelesVanderLaanEisen2002,
author =          {Keles, S and Van der Laan, MJ and Eisen, MB},
title =          {Identification of regulatory elements using a feature
selection method.},
journal =          {Bioinformatics},
year =          {2002},
volume =          {18},
pages =          {1167-1175}
}


@Article{Kiepiela2004,
author =          {Kiepiela, P and Leslie, AJ and Honeyborne, I and Ramduth, D
and Thobakgale, C and Chetty, S and Rathnavalu, P and Moore, C and Pfafferott, KJ and Hilton, L
and Zimbwa, P and Moore, S and Allen, T and Brander, C and Addo, MM and Altfeld, M 
and Mallal, S and Bunce, M and Barber, LD and Szinger, J and Day, C and Klenerman, P and Mullins, JI
and Korber, B and Coovadia, HM and Walker, BD and Goulder, PJ},
title =          {Dominant influence of $\mbox{HLA-B}$ in mediating the potential
co-evolution of $\mbox{HIV}$ and $\mbox{HLA}$.},
journal =          {Nature},
year =          {2004},
volume =          {432},
pages =          {769-775}
}


@Article{KowalskiPaganoDeGruttola2002,
author =          {Kowalski, J and Pagano, M and De Gruttola, V},
title =          {A non-parametric approach to testing gene region
heterogeneity associated with phenotype.},
journal =          {Journal of the American Statistical Association},
year =          {2002},
volume =          {97},
pages =          {398-408}
}


@Article{KulichLin2000,
author =          {Kulich, M and Lin, DY},
title =          {Additive hazard regressions for case-cohort studies.},
journal =          {Biometrika},
year =          {2000},
volume =          {87},
pages =          {73-87}
}


@Article{KulichLin2004,
author =          {Kulich, M and Lin, DY},
title =          {Improving efficiency of relative-risk estimation in
case-cohort studies.},
journal =          {Journal of the American Statistical Association},
year =          {2004},
volume =          {99},
pages =          {832-844}
}


@Article{LangholzThomas1990,
author =          {Langholz, B and Thomas, D},
title =          {Nested case-control and case-cohort methods of
sampling from a cohort: A critical comparison.},
journal =          {American Journal of Epidemiology},
year =          {1990},
volume =          {131},
pages =          {169-176}
}


@Article{LangholzBorgan1995,
author =          {Langholz, B and Borgan, O},
title =          {Counter-matching:  A stratified nested case-control
sampling method.},
journal =          {Biometrika},
year =          {1995},
volume =          {82},
pages =          {69-79}
}


@Article{LiGui2004,
author =          {Li, H and Gui, J},
title =          {Partial $\mbox{Cox}$ regression analysis for high-dimensional
microarray gene expression data.},
journal =          {Bioinformatics},
year =          {2004},
volume =          {20},
pages =          {208-215}
}

@Article{Lichterfeld2004,
author =          {Lichterfeld, M and Kaufmann, DE and Yu, XG and Mui, SK and Addo, MM and
Johnston, MN and Cohen, D and Robbins, GK and Pae, E and Alter, G and Wurcel, A and Stone, D
and Rosenberg, ES and Walker, BD and Altfeld, M},
title =          {Loss of $\mbox{HIV}$-1 specific $\mbox{$\mbox{CD8}$}$+ $\mbox{T cell}$ proliferation after
acute $\mbox{HIV}$-1 infection and restoration by vaccine-induced $\mbox{HIV}$-1 specific
$\mbox{CD4}$+ $\mbox{T cell}$s.},
journal =          {Journal of Experimental Medicine},
year =          {2004},
volume =          {200},
pages =          {701-712}
}

@Article{Royall1992,
author =          {Royall, RM},
title =          {Robustness and optimal design under prediction models for finite populations.},
journal =          {Survey Methodology},
year =          {1992},
volume =          {18},
pages =          {179--185}
}




@Book{MerrillSinisiVanderLaan2004,
  author =          {Merrill, DB and Sinisi, SE and Van der Laan, MJ},
  ALTeditor =          {},
  title =          {Multiple testing and data adaptive regression:  An
application to $\mbox{HIV}$-1 sequence data.},
  publisher =          {},
  year =          {2004},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {U.C. Berkeley Division of Biostatistics Working
Paper Series},
  address =          {Department of Statistics, Stanford University},
  OPTedition =          {Working Paper 161},
  OPTmonth =          {},
  OPTnote =          {http://www.bepress.com/ucbbiostat/paper161},
  OPTannote =          {}
}


@Book{SarndalSwenssonWretman1992,
  author =          {S\"{a}rndal, C-E and Swensson, B and Wretman, J},
  ALTeditor =          {},
  title =          {Model Assisted Survey Sampling.},
  publisher =          {Springer-Verlag, New York},
  year =          {1992},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {}
}

@Book{Cochran1977,
  author =          {Cochran, WG},
  ALTeditor =          {},
  title =          {Sampling Techniques, 3rd Edition.},
  publisher =          {Wiley, New York},
  year =          {1977},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {}
}



@Article{Milik1998,
author =          {Milik, M and Sauer, D and Brunmark, AP and Yuan, L and Vitiello, A
and Jackson, R and Peterson, PA and Skolnick, J and Glass, CA},
title =          {Application of an artificial neural network to predict
specific class $\mbox{I}$ $\mbox{MHC}$ binding peptide sequences.},
journal =          {Nature Biotechnology},
year =          {1998},
volume =          {16},
pages =          {753-756}
}

@Article{Wright1983,
author =          {Wright, RL},
title =          {Finite population sampling with multivariate auxiliary information.},
journal =          {Journal of the American Statistical Association},
year =          {1983},
volume =          {78},
pages =          {879--884}
}



@Article{Molenberghs2002,
author =          {Molenberghs, G and Buyse, M and Geys, H and Renard, D and Burzykowski,
T and Alonso, A},
title =          {Statistical challenges in the evaluation of surrogate
endpoints in randomized trials.},
journal =          {Controlled Clinical Trials},
year =          {2002},
volume =          {23},
pages =          {607-625}
}

@Article{NguyenRocke2002,
author =          {Nguyen, D and Rocke, DM},
title =          {Tumor classification by partial least squares using
microarray gene expression data.},
journal =          {Bioinformatics},
year =          {2002},
volume =          {18},
pages =          {39-50}
}


@Article{Paik1997,
author =          {Paik, MC},
title =          {The generalized estimating equation approach when data
are not missing completely at random.},
journal =          {Journal of the American Statistical Association},
year =          {1997},
volume =          {92},
pages =          {1320-1329}
}


@Article{Pantophlet2003,
author =          {Pantophlet, R and Saphire, EO and Poignard, P and Parren, PWHI
and Wilson, IA and Burton, DR},
title =          {Fine mapping of the interaction of neutralizing and
nonneutralizing monoclonal antibodies with the $\mbox{CD4}$ binding site of Human
Immunodeficiency Virus Type 1 gp120.},
journal =          {Journal of Virology},
year =          {2003},
volume =          {77},
pages =          {642-658}
}

@Book{Pepe2003,
  author =          {Pepe, MS},
  ALTeditor =          {},
  title =          {The Statistical Evaluation of Medical Tests for
Classification and Prediction.},
  publisher =          {Oxford University Press},
  year =          {2003},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  address =          {United Kingdom},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{PepeCaiZhang2004,
  author =          {Pepe, MS and Cai, T and Zhang, Z},
  title =          {Combining predictors for classification using the
area under the ROC curve.},
  year =          {2004},
  journal =          {University of Washington Biostatistics Working
Paper Series}
}


@Article{PepeFleming1991,
author =          {Pepe, MS and Fleming, TR},
title =          {A non-parametric method for dealing with mismeasured
covariate data.},
journal =          {Journal of the American Statistical Association},
year =          {1991},
volume =          {86},
pages =          {108-113}
}



@Article{Quigg2002,
author =          {Quigg, M and Frost, SDW and McDonaugh, S and Burns, SM
and Clutterbuck, D and McMillan, A and Leen, CS and Brown, AJ},
title =          {Association of antiretroviral resistance genotypes
with response to therapy.},
journal =          {Antiviral Therapy},
year =          {2002},
volume =          {7},
pages =          {151-157}
}


@Article{Regoes2005,
author =          {Regoes, RR and Longini, IM and Feinberg, MB and Staprans, SI},
title =          {Preclinical assessment of $\mbox{HIV}$ vaccines and
microbicides by repeated low-dose virus challenges.},
journal =          {PLoS Medicine},
year =          {2005},
volume =          {2},
pages =          {e249}
}


@Article{RobinsRitov1997,
author =          {Robins, JM and Ritov, Y},
title =          {Toward a curse of dimensionally appropriate (CODA)
asymptotic theory for semiparametric models.},
journal =          {Statistics in Medicine},
year =          {1997},
volume =          {16},
pages =          {285-319}
}


@Article{Rouzioux2005,
author =          {Rouzioux, C and Hubert, J-B and Burgard, M and Deveau, C and Foujard,
C and Bary, M and Sereni, D and Virard, J-P and Delfraissy, J-F and Meyer, L and for the SEROCO
Cohort Study Group},
title =          {Early levels of $\mbox{HIV}$-1 $\mbox{DNA}$ in peripheral blood
mononuclear cells are predictive of disease progression independently of
$\mbox{HIV}$-1 $\mbox{RNA}$ levels and $\mbox{CD4}$+ $\mbox{T cell}$ counts.},
journal =          {Journal of Infectious Diseases},
year =          {2005},
volume =          {192},
pages =          {46-55}
}


@Article{Rubin2004,
author =          {Rubin, DB},
title =          {Direct and indirect causal effects via potential
outcomes.},
journal =          {Scandinavian Journal of Statistics},
year =          {2004},
volume =          {31},
pages =          {161-170}
}


@Article{Rubin2005,
author =          {Rubin, DB},
title =          {Causal inference using potential outcomes:  Design,
modeling, decisions.},
journal =          {Journal of the American Statistical Association},
year =          {2005},
volume =          {100},
pages =          {322-331}
}


@Article{RuczinskiKooperbergLeBlanc2003,
author =          {Ruczinski, I and Kooperberg, C and LeBlanc, M},
title =          {Logic Regression.},
journal =          {Journal of Computational and Graphical Statistics},
year =          {2003},
volume =          {12},
pages =          {475-511}
}



@Article{SegalCummingsHubbard2001,
author =          {Segal, MR and Cummings, MP and Hubbard, AE},
title =          {Relating amino acid sequence to phenotype:  Analysis
of peptide binding data.},
journal =          {Biometrics},
year =          {2001},
volume =          {57},
pages =          {632-643}
}

@article{Edlefsen2014leaky,
  title={Leaky Vaccines Protect Highly Exposed Recipients at a Lower Rate: Implications for Vaccine Efficacy Estimation and Sieve Analysis},
  author={Edlefsen, Paul T},
  journal={Computational and Mathematical Methods in Medicine},
  volume={2014},
  year={2014},
  publisher={Hindawi Publishing Corporation}
}



@Article{Shepherdetal2006,
author =          {Shepherd, B and Gilbert, Peter B and Jemiai, Y and Rotnitzky, A},
title =          {Sensitivity analyses comparing outcomes only existing
in a subset selected post-randomization, conditional on covariates, with
application to $\mbox{HIV}$ vaccine trials.},
journal =          {Biometrics},
year =          {2006},
volume =         {62},
pages =          {332--342}
}

@Article{BenkeserGilbertCarone2014,
author =          {Benkeser, D and Gilbert, Peter B and Carone, M},
title =          {Efficient and robust estimation of cumulative incidence in competing risks settings.},
journal =          {Technical report, Fred Hutchinson Cancer Research Center},
year =          {2014},
volume =         {},
pages =          {}
}



@Article{DavidianGallant1993,
author =          {Davidian, M and Gallant, AR},
title =          {The nonlinear mixed effects model with a smooth random effects density.},
journal =          {Biometrika},
year =          {1993},
volume =         {80},
pages =          {475--488}
}

@Article{ChibavanderWeele2011,
author =          {Chiba, Y and vanderWeele, TJ}, 
title =          {A simple method for principal strata effects when the outcome has been truncated due to death}, 
journal =          {American Journal of Epidemiology},
year =          {2011},
volume =         {173},
pages =          {745--751}
}
%  note={PMCID: PMC3070493}


@Article{DaiGilbertMasse2012,
author =          {Dai, JY and Gilbert, Peter B and Masse, BR}, 
title =          {Partially hidden {Markov} model for time-varying principal stratification in {HIV} prevention trials.},
journal =          {Journal of the American Statistical Association},
year =          {2012},
volume =         {107},
pages =          {52--65},
  note={PMCID: PMC3649016}
}

@Article{TchetgenTchetgen2014, 
author =          {Tchetgen Tchetgen, EJ}, 
title =          {Identification and estimation of survivor average causal effects}, 
journal =          {Statistics in Medicine}, 
year =          {2014},
volume =         {33},
pages =          {3601--3628}
}

volume={33},
  number={21},
  pages={3601--3628},
  year={2014},


@Article{HalloranStruchiner1995,
author =          {Halloran, ME and Struchiner, CJ},
title =          {Causal inferences in infectious diseases.},
journal =          {Epidemiology},
year =          {1995},
volume =         {6},
pages =          {142-151}
}



@Book{SegalBarbourGrant2004,
  author =          {Segal, MR and Barbour, JD and Grant, RM},
  ALTeditor =          {},
  title =          {Statistical Applications in Genetics in Molecular
Biology.},
  publisher =          {Berkely Electronic Press},
  year =          {2004},
  OPTkey =          {},
  OPTvolume =          {3},
  OPTnumber =          {Issue 1},
  OPTseries =          {Article 2},
  address =          {},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Book{Burzykowskietal2005,
  author =          {Burzykowski, T and Molenberghs, G and Buyse, M},
  ALTeditor =          {},
  title =          {The Evaluation of Surrogate Endpoints.},
  publisher =          {Springer},
  year =          {2005},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  address =          {},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{Siber1997,
author =          {Siber, GR},
title =          {Methods for estimating serological correlates of
protection.},
journal =          {Developments in Biological Standardization},
year =          {1997},
volume =          {89},
pages =          {283-296}
}


@Article{SinisiVanderLaan2004,
author =          {Sinisi, SE and Van der Laan, MJ},
title =          {Deletion/Substitution/Addition algorithm in learning
with applications in genomics.},
journal =          {Statistical Applications in Genetics and Molecular
Biology},
year =          {2004},
volume =          {3},
pages =          {Article 18}
}


@Article{SorensenAnderson2000,
author =          {Sorenson, P and Anderson, PK},
title =          {Competing risks analysis of the case-cohort design.},
journal =          {Biometrika},
year =          {2000},
volume =          {87},
pages =          {49-59}
}


@Article{Tibshirani1996,
author =          {Tibshirani, R},
title =          {Regression shrinkage and selection via the lasso.},
journal =          {Journal of the Royal Statistical Society},
year =          {1996},
volume =          {B 58},
pages =          {267-288}
}


@Article{Wilson2000,
author =          {Wilson, JK and Immi, N and Watkins, A and Gill, J and Hay, P and Gazzard,
B and Westby, M and Gotch, FM},
title =          {Loss of $\mbox{CD4}$+ $\mbox{T cell}$ proliferative ability but not loss
of human immunodeficiency virus type 1 specificity equates with
progression to disease.},
journal =          {Journal of Infectious Diseases},
year =          {2000},
volume =          {182},
pages =          {792-798}
}


 
@Book{VanderLaanRobins2003,
  author =          {Van der Laan, MJ and Robins, JM},
  ALTeditor =          {},
  title =          {Unified Methods for Censored Longitudinal Data and
Causality.},
  publisher =          {Springer},
  year =          {2003},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  address =          {},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{Vanhems2000,
author =          {Vanhems, P and Hirschel, B and Phillips, AN and et al.},
title =          {Incubation time of acute Human Immunodeficiency Virus
($\mbox{HIV}$) infection and duration of acute $\mbox{HIV}$ infection are independent
factors of progression to $\mbox{AIDS}$.},
journal =          {Journal of Infectious Diseases},
year =          {2000},
volume =          {182},
pages =          {334-337}
}


@Book{Korber2004,
  author =          {Korber, B},
  title =          {$\mbox{HIV}$ Immunology and Sequence Databases},
  pages =          {148-156},
  year =          {2004},
  publisher =  {Los Alamos National Laboratory},
}


@incollection{YanoverHertz2005,
	abstract = {Many important cellular response mechanisms are activated when a peptide binds to an appropriate receptor. In the immune system, the recognition of pathogen peptides begins when they bind to cell membrane Major Histocompatibility Complexes (MHCs). MHC proteins then carry these peptides to the cell surface in order to allow the activation of cytotoxic T-cells. The MHC binding cleft is highly polymorphic and therefore protein-peptide binding is highly specific. Developing computational methods for predicting protein-peptide binding is important for vaccine design and treatment of diseases like cancer. Previous learning approaches address the binding prediction problem using traditional margin based binary classifiers. In this paper we propose a novel approach for predicting binding affinity. Our approach is based on learning a peptide-peptide distance function. Moreover, we learn a single peptide-peptide distance function over an entire family of proteins (e.g MHC class I). This distance function can be used to compute the affinity of a novel peptide to any of the proteins in the given family. In order to learn these peptide-peptide distance functions, we formalize the problem as a semi-supervised learning problem with partial information in the form of equivalence constraints. Specifically we propose to use DistBoost [1, 2], which is a semi-supervised distance learning algorithm.We compare our method to various state-of-the-art binding prediction algorithms on MHC class I and MHC class II datasets. In almost all cases, our method outperforms all of its competitors. One of the major advantages of our novel approach is that it can also learn an affinity function over proteins for which only small amounts of labeled peptides exist. In these cases, DistBoost's performance gain, when compared to other computational methods, is even more pronounced.},
	author = {Yanover, Chen and Hertz, Tomer},
	citeulike-article-id = {5542116},
	citeulike-linkout-0 = {http://dx.doi.org/10.1007/11415770\_34},
	citeulike-linkout-1 = {http://www.springerlink.com/content/lanjv7v7m0gwqbtk},
	doi = {10.1007/11415770\_34},
	journal = {Research in Computational Molecular Biology},
	pages = {456--471},
	posted-at = {2009-08-22 01:20:42},
	priority = {2},
	title = {Predicting Protein-Peptide Binding Affinity by Learning Peptide-Peptide Distance Functions},
	url = {http://dx.doi.org/10.1007/11415770\_34},
	year = {2005}
}



@Article{HertzYanover2007,
author =          {Hertz, T and Yanover, C},
title =          {Identifying $\mbox{HLA}$ supertypes by learning distance functions.},
journal =          {Bioinformatics},
year =          {2007},
volume =          {23},
pages =          {e148--e155},
  note={PMCID: }
}

@Article{HertzYanover2006,
author =          {Hertz, T and Yanover, C},
title =          {PepDist: a new framework for protein-peptide binding prediction based on learning peptide distance functions.},
journal =          {BMC Bioinformatics},
year =          {2006},
volume =          {7 Suppl 1},
pages =          {S3}
}




@Article{Kwong2002,
author =          {Kwong, PD and Doyle, ML and Casper, DJ and Cicala, C and Leavitt, SA
and Mjeed, S and Steenbeke, TD and Venturi, M and Chaiken, I and Fung, M and Katinger, H and Parren,
PW and Robinson, J and Van Ryk, D and Wang, L and Burton, DR and Freire, E and Wyatt, R
and Sodroski, J and Hendrickson, WA and Arthos, J},
title =          {$\mbox{HIV}$-1 evades antibody-mediated neutralization through
conformational masking of receptor-binding sites.},
journal =          {Nature},
year =          {2002},
volume =          {420},
pages =          {678-682}
}


@Article{Wei2003,
author =          {Wei, XJ and Decker, JM and Wang, S and Hui, H and Kappes, JC and Wu, X
and Salazar-Gonzalez, JF and Salazar, MG and Kilby, JM and Saag, MS and Komarova, NL and Nowak,
MA and Hahn, B and Kwong, PD and Shaw, GM},
title =          {Antibody neutralization and escape by $\mbox{HIV}$-1.},
journal =          {Nature},
year =          {2003},
volume =          {422},
pages =          {307-312}
}

@Article{Wyatt1998,
author =          {Wyatt, R and Kwong, PD and Desjardins, E and Sweet, RW and Robinson,
J and Hendrickson, WA and Sodroski, JG},
title =          {The antigenic structure of the $\mbox{HIV}$ gp120 envelope
glycoprotein.},
journal =          {Nature},
year =          {1998},
volume =          {393},
pages =          {705-711}
}


@Article{Richman2003,
author =          {Richman, DD and Wren, T and Little, SJ and Petropoulos, CJ},
title =          {Rapid evolution of the neutralizing antibody response
to $\mbox{HIV}$ type 1 infection.},
journal =          {Proceedings of the National Academy of Sciences USA},
year =          {2003},
volume =          {100},
pages =          {4144-9}
}


@Article{Graham1994,
author =          {Graham, BS and Gorse, GJ and Schwartz, DH and Keefer, MC and McElrath,
MJ and Matthew, TJ and Wright, PF and Belshe, RB and Clements, ML and Dolin, R and et al.},
title =          {Determinants of antibody response after recombinant gp
160 boosting in vaccinia-na�ve volunteers primed with gp160-recombinant
vaccinia virus.  The National Institute of Allergy and Infectious
Diseases $\mbox{AIDS}$ Vaccine Trials Network},
journal =          {Journal of Infectious Diseases},
year =          {1994},
volume =          {170},
pages =          {782-786}
}


@Article{Calarese2003,
author =          {Calarese, DA and Scanlan, CN and Zwick, MB and Deechongkit, S
and Mimura, Y and Kunert, R and Zhu, P and Wormald, MR and Stanfield, RL and Roux, KH and Kelly, JW
and Rudd, PM and Dwek, RA and Katinger, H and Burton, DR and Wilson, IA},
title =          {Antibody domain exchange is an immunological solution
to carbohydrate cluster recognition.},
journal =          {Science},
year =          {2003},
volume =          {300},
pages =          {2065-71}
}

@Article{Darbha2004,
author =          {Darbha, R and Phogat, S and Labrijn, AF and Shu, Y and Gu, Y
and Andrykovitch, M and Zhang, MY and Pantophlet, R and Martin, L and Vita, C and Burton, DR
and Dimitrov, DS and Ji, X},
title =          {Crystal structure of the broadly cross-reactive $\mbox{HIV}$-1
neutralizing Fab X5 and fine mapping of its epitope.},
journal =          {Biochemistry},
year =          {2004},
volume =          {43},
pages =          {1410-7}
}


@Article{Kwong1998,
author =          {Kwong, PD and Wyatt, R and Robinson, J and Sweet, RW and Sodoroski, J
and Hendrickson, WA},
title =          {Structure of an $\mbox{HIV}$ gp120 envelope glycoprotein in
complex with the $\mbox{CD4}$ receptor and a neutralizing human antibody.},
journal =          {Nature},
year =          {1998},
volume =          {393},
pages =          {648-59}
}


@Article{Ofek2004,
author =          {Ofek, G and Tang, M and Sambor, A and Katinger, H and Mascola, JR
and Wyatt, R and Kwong, PD},
title =          {Structure and mechanistic analysis of the anti-human
immunodeficiency virus type 1 antibody 2F5 in complex with its gp41
epitope.},
journal =          {Journal of Virology},
year =          {2004},
volume =          {78},
pages =          {10724-37}
}


@Article{Saphire2001,
author =          {Saphire, EO and Warren, PW and Pantophlet, R and Zwick, MB and Morris,
GM and Rudd, PM and Dwek, RA and Stanfield, RL and Burton, DR and Wilson, IA},
title =          {Crystal structure of neutralizing human IGG against
$\mbox{HIV}$-1:  a template for vaccine design.},
journal =          {Science},
year =          {2001},
volume =          {293},
pages =          {1155-9}
}


@Article{Zwick2003,
author =          {Zwick, MB and Parren, PW and Saphire, EO and Church, S and Wang, M and
Scott, JK and Dawson, PE and Wilson, IA and Burton, DR},
title =          {Molecular features of the broadly neutralizing
immunoglobulin G1 b12 required for recognition of human immunodeficiency
virus type 1 gp120.},
journal =          {Journal of Virology},
year =          {2003},
volume =          {77},
pages =          {5863-76}
}

@Article{Scott2008,
author =          {Scott, J},
title =          {Stepped Wedge Cluster Randomized Trials.},
journal =          {PhD dissertation, University of Washington},
year =          {2008},
volume =          {},
pages =          {}
}

@Article{DeCamp2013thesis,
author = {DeCamp, AC},
title =          {Assessing Immune Correlates of Protection.},
journal =          {PhD dissertation, Department of Biostatistics, University of Washington},
year =          {2013},
volume =          {},
pages =          {}
}


@Article{Shoudissertation2013,
author =          {Shou, Q},
title =          {SEMIPARAMETRIC TIME-VARYING COEFFICIENT REGRESSION MODEL FOR LONGITUDINAL DATA WITH CENSORED TIME ORIGIN. {PhD dissertation (with Dr. Yanqing Sun), University of North Carolina at Charlotte}},
journal =          {},
year =          {2012},
volume =          {},
pages =          {}
}

@Article{deCamp2013,
author =          {deCamp, A},
title =          {{HIV} Vaccine Trials: {Assessment} and Discovery of Immune Correlates
of Protection.},
journal =          {PhD dissertation, University of Washington},
year =          {2013},
volume =          {},
pages =          {}
}




@article{schmader2012efficacy,
  title={Efficacy, safety, and tolerability of herpes zoster vaccine in persons aged 50--59 years},
  author={Schmader, Kenneth E and Levin, Myron J and Gnann, John W and McNeil, Shelly A and Vesikari, Timo and Betts, Robert F and Keay, Susan and Stek, Jon E and Bundick, Nickoya D and Su, Shu-Chih and others},
  journal={Clinical infectious diseases},
  volume={54},
  number={7},
  pages={922--928},
  year={2012},
  publisher={Oxford University Press}
}




@Article{Amara2001,
author =          {Amara, RR and Villinger, F and Altman, JD and Lydy, SL and O'Neil, SP
and Staprans, I and Montefiori, DC and Xu, Y and Herndon, JG and Wyatt, LS and Candido, MA and Kozyr,
NL and Earl, PL and Smith, JM and Ma, HL and Grimm, BD and Hulsey, ML and Miller, J and McClure, HM
and McNicholl, JM and Moss, B and Robinson, HL},
title =          {Control of a mucosal challenge and prevention of $\mbox{AIDS}$
by a multiprotein $\mbox{DNA/MVA}$ vaccine.},
journal =          {Science},
year =          {2001},
volume =          {292},
pages =          {69-74}
}


@Article{Barouch2001,
author =          {Barouch, DH and Santra, S and Kuroda, MJ and Schmitz, JE and Plishka,
R and Buckler-White, A and Gaitan, AE and Zin, R and Nam, JH and Wyatt, LS and Lifton, MA
and Nickerson, CE and Moss, B and Montefiori, DC and Hirsch, VM and Letvin, NL},
title =          {Reduction of simian-human immunodeficiency virus 89.6P
viremia in rhesus monkeys by recombinant modified vaccinia virus Ankara
vaccination.},
journal =          {Journal of Virology},
year =          {2001},
volume =          {75},
pages =          {5151-8}
}


@Article{Hertzetal2013,
author =          {Hertz, T and Ahmed, H and Friedrich, DP and Casimiro, DR and Self, SG and Corey, L and McElrath, MJ and Buchbinder, S and Horton, H and Frahm, N and Robertson, MN and Graham, BS and Gilbert, Peter B},
title =          {$\mbox{HIV-1}$ vaccine-induced $\mbox{T-cell}$ responses cluster in epitope hotspots that differ from those induced in natural infection with $\mbox{HIV-1}$.},
journal =          {PLoS Pathogens}, 
  volume={9},
  number={6},
  pages={e1003404},
  year={2013},
  publisher={Public Library of Science},
  note={PMCID: PMC3688560}
}

@Article{Barouch2000,
author =          {Barouch, DH and Santra, S and Schmitz, JE and Kuroda, MJ and Fu, TM
and Wagner, W and Bilska, M and Craiu, A and Zheng, XX and Krivulka, GR and Beaudry, K and Lifton,
MA and Nickerson, CE and Trigona, WL and Punt, K and Freed, DC and Guan, L and Dubey, S
and Casimiro, D and Simon, A and Davies, ME and Chastain, M and Strom, TB and Gelman, RS
and Montefiori, DC and Lewis, MG and Emini, EA and Shiver, JW and Letvin, NL},
title =          {Control of viremia and prevention of clinical $\mbox{AIDS}$ in
rhesus monekys by cytokine-augmented $\mbox{DNA}$ vaccination.},
journal =          {Science},
year =          {2000},
volume =          {290},
pages =          {486-92}
}


@Article{BenjaminiHochberg1995,
  author =       {Benjamini, Y and Hochberg, Y},
  title =        {Controlling the false discovery rate- a new and
powerful approach to multiple testing.},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =         {1995},
  volume =       {57},
  pages =        {289-300},
}


@Article{Buckner2004,
author =          {Buckner, C and Gines, LG and Saunders, CJ and Vojtech, L
and Srivastava, I and Gettie, A and Bohm, R and Blanchard, J and Barnett, SW and Safrit, JT
and Stamatatos, L},
title =          {Priming B cell-mediated anti-$\mbox{HIV}$ envelope responses by
vaccination allows for a long-term control of infection in macaques
exposed to a $\mbox{R5}$-tropic $\mbox{SHIV}$.},
journal =          {Virology},
year =          {2004},
volume =          {320},
pages =          {167-80}
}

@Article{Montefiori2003,
author =          {Montefiori, DC and Altfeld, M and Lee, PK and Bilska, M and Zhou, J
and Johnston, N and Gao, F and Walker, BD and Rosenberg, ES},
title =          {Viremia control despite escape from a rapid and potent
autologous neutralizing antibody response after therapy cessation in an
$\mbox{HIV}$-1-infected individual.},
journal =          {Journal of Immunology},
year =          {2003},
volume =          {170},
pages =          {3906-14}
}


@Article{Montefiori2001,
author =          {Montefiori, DC and Hill, TS and Vo, HT and Walker, BD and Rosenberg, ES},
title =          {Neutralizing antibodies associated with viremia
control in a subset of individuals after treatment of acute human
immunodeficiency virus type 1 infection.},
journal =          {Journal of Virology},
year =          {2001},
volume =          {75},
pages =          {10200-7}
}


@Article{Rasmussen2002,
author =          {Rasmussen, RA and Hofmann-Lehmann, R and Li, PL and Vlasak, J and
Schmitz, JE and Reimann, KA and Kuroda, MJ and Letvin, NL and Montefiori, DC and McClure, HM
and Ruprecht, RM},
title =          {Neutralizing antibodies as a potential secondary
protective mechanism during chronic $\mbox{SHIV}$ infection in $\mbox{CD8}$+
$\mbox{T-cell}$-depleted macaques.},
journal =          {AIDS},
year =          {2002},
volume =          {16},
pages =          {829-38}
}


@Article{Rose2001,
author =          {Rose, NF and Marx, PA and Luckay, A and Nixon, DF and Moretto, WJ
and Donahoe, SM and Montefiori, DC and Roberts, A and Buonocore, L and Rose, JK},
title =          {An effective $\mbox{AIDS}$ vaccine based on live attenuated
vesicular stomatitis virus recombinants.},
journal =          {Cell},
year =          {2001},
volume =          {106},
pages =          {539-49}
}


@Article{Schmitz2003,
author =          {Schmitz, JE and Kuroda, MJ and Santra, S and Simon, MA and Lifton, MA
and Lin, W and Khunkhun, R and Piatak, M and Lifson, JD and Grosschupff, G and Gelman, 
RS and Racz,
P and Tenner-Racz, K and Mansfield, KA and Letvin, NL and Montefiori, DC and Reimann, KA},
title =          {Effect of humoral immune responses on controlling
viremia during primary infection of rhesus monkeys with simian
immunodeficiency virus.},
journal =          {Journal of Virology},
year =          {2003},
volume =          {77},
pages =          {2165-73}
}


@Article{Trkola2004,
author =          {Trkola, A and Kuster, H and Leemann, C and Oxenius, A and Fagard, C
and Furrer, H and Battegay, M and Vernazza, P and Bernasconi, E and Weber, R and Hirschel, B
and Bonhoeffer, S and Gunthard, HF},
title =          {Humoral immunity to $\mbox{HIV}$-1: kinetics of antibody
responses in chronic infection reflects capacity of immune system to
improve viral set point.},
journal =          {Blood},
year =          {2004},
volume =          {104},
pages =          {1784-92}
}


@Article{Vodicka1997,
author =          {Vodicka, MA and Goh, WC and Wu, LI and Rogel, ME and Bartz, SR
and Schweickhart, VL and Raport, CJ and Emerman, M},
title =          {Indicator cell lines for detection of primary strains
of human and simian immunodeficiency viruses.},
journal =          {Virology},
year =          {1997},
volume =          {233},
pages =          {193-8}
}


@Article{Weber1987,
author =          {Weber, JN and Clapham, PR and Weiss, RA and Parker, D and Roberts, C
and Duncan, J and Weller, I and Carne, C and Tedder, RS and Pinching, AJ and et al.},
title =          {Human immunodeficiency virus infection in two cohorts
of homosexual men: neutralising sera and association of anti-gag
antibody with prognosis.},
journal =          {Lancet},
year =          {1987},
volume =          {1},
pages =          {119-22}
}


@Article{Binley2004,
author =          {Binley, JM and Wrin, T and Korber, B and Zwick, MB and Wang, M
and Chappey, C and Stiegler, G and Kunert, R and Zolla-Pazner, S and Katinger, H and Petropoulos,
CJ and Burton, DR},
title =          {Comprehensive cross-clade neutralization analysis of a
panel of anti-human immunodeficiency virus type 1 monoclonal antibodies.},
journal =          {Journal of Virology},
year =          {2004},
volume =          {78},
pages =          {13232-52}
}


@Article{Flynn2005,
author =          {Flynn, NM and Forthal, DN and Harro, CD and Judson, FN and Mayer, KH
and Para, MF and Gilbert, Peter B and the rgp120 $\mbox{HIV}$ Vaccine Study Group},
title =          {Placebo-controlled phase 3 trial of recombinant
glycoprotein 120 vaccine to prevent $\mbox{HIV}$-1 infection.},
journal =          {Journal of Infectious Diseases},
year =          {2005},
volume =          {191},
pages =          {654-65}
}


@Article{Flynnetal2005short,
author =          {Flynn, NM and Forthal, DN and Harro, CD and Judson, FN and Mayer, KH
and Para, MF and Gilbert, Peter B and the rgp120 $\mbox{HIV}$ Vaccine Study Group},
title =          {Placebo-controlled phase 3 trial of recombinant
glycoprotein 120 vaccine to prevent $\mbox{HIV}$-1 infection.},
journal =          {Journal of Infectious Diseases},
year =          {2005},
volume =          {191},
pages =          {654-65}
}

@Article{Forthaletal2007,
author =          {Forthal, D and Gilbert, P and Landucci, G and Phan, T},
title =          {Recombinant gp120 vaccine-induced antibodies inhibit clinical strains of HIV-1 in the presence of Fc receptor-bearing effector cells and correlate inversely with HIV infection rate.},
journal =          {Journal of Immunology},
year =          {2007},
volume =          {178},
pages =          {6596-6603}
}





@Article{Mascola2003,
author =          {Mascola, JR and Lewis, MG and VanCott, TC and Stiegler, G
and Katinger, H and Seaman, M and Beaudry, K and Barouch, DH and Korioth-Schmitz,
B and Krivulka,
G and Sambor, A and Welcher, B and Douek, DC and Montefiori, DC and Shiver, JW and Poignard, P and Burton, DR and Letvin, NL},
title =          {Cellular immunity elicited by human immunodeficiency
virus type 1/simian immunodeficiency virus $\mbox{DNA}$ vaccination does not
augment the sterile protection afforded by passive infusion of
neutralizing antibodies.},
journal =          {Journal of Virology},
year =          {2003},
volume =          {77},
pages =          {10348-56},
  note={PMCID: PMC228504}
}


@Article{Nishimura2002,
author =          {Nishimura, Y and Igarashi, T and Haigwood, N and Sadjadpour, R
and Plishka, RJ and Buckler-White, A and Shibata, R and Martin, MA},
title =          {Determination of a statistically valid neutralization
titer in plasma that confers protection against simian-human
immunodeficiency virus challenge following passive transfer of
high-titered neutralizing antibodies.},
journal =          {Journal of Virology},
year =          {2002},
volume =          {76},
pages =          {2123-30}
}


@Article{Shibata1999,
author =          {Shibata, R and Igarashi, T and Haigwood, N and Buckler-White, A
and Ogert, R and Ross, W and Willey, R and Cho, MW and Martin, MA},
title =          {Neutralizing antibody directed against the $\mbox{HIV}$-1
envelope glycoprotein can completely block $\mbox{HIV}$-1/$\mbox{SIV}$ chimeric virus
infections of macaque monkeys.},
journal =          {Nature Medicine},
year =          {1999},
volume =          {5},
pages =          {204-10}
}


@Article{Mora2003,
author =          {Mora, JR and Bono, MR and Manjunath, N and Weninger, W and Cavanagh,
LL and Rosemblatt, M and Von Andrian, UH},
title =          {Selective imprinting of gut-homing $\mbox{T cell}$s by Peyer?s
patch dendritic cells.},
journal =          {Nature},
year =          {2003},
volume =          {424},
pages =          {88-93}
}



@Book{Montefiori2004,
  author =          {Montefiori, DC},
  ALTeditor =          {},
  title =          {Current Protocols in Immunology.},
  publisher =          {John Wiley and Sons},
  year =          {2004},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},

  address =          { },

  OPTedition =          {J.E. Coligan, A.M. Kruisbeek, D.H. Margulies,
E.M. Shevach, W. Strober, and R. Coico (ed.)},

  OPTmonth =          {},

  OPTnote =          {Evaluating neutralizing antibodies against $\mbox{HIV}$,
$\mbox{SIV}$ and $\mbox{SHIV}$ in luciferase reporter gene assays, p. 12.11.1, 12.11.15.},

  OPTannote =          {}
}

@Article{StaggKammKnight2002,
author =          {Stagg, AJ and Kamm, MA and Knight, SC},
title =          {Intestinal dendritic cells increase $\mbox{T cell}$ expression
of alpha4beta7 integrin.},
journal =          {European Journal of Immunology},
year =          {2002},
volume =          {32},
pages =          {1445-54}
}


@Article{LefrancoisOlsonMasopust1999,
author =          {Lefrancois, L and Olson, S and Masopust, D},
title =          {A critical role for $\mbox{CD4}$0-CD40 ligand interactions in
amplification of the mucosal $\mbox{CD8}$ $\mbox{T cell}$ response.},
journal =          {Journal of Expermental Medicine},
year =          {1999},
volume =          {190},
pages =          {1275-84}
}


@Article{Brenchley2004,
author =          {Brenchley, JM and Schacker, TW and Ruff, LE and Price, DA and Taylor,
JH and Beilman, GJ and Nguyen, PL and Khoruts, A and Larson, M and Haase, AT and Douek, DC},
title =          {$\mbox{CD4+}$ $\mbox{T cell}$ depletion during all stages of $\mbox{HIV}$ disease
occurs predominantly in the gastrointestinal tract.},
journal =          {Journal of Experimental Medicine},
year =          {2004},
volume =          {200},
pages =          {749-59}
}


@Article{Mehandru2004,
author =          {Mehandru, S and $\mbox{Pol}$es, MA and Tenner-Racz, K and Horowitz, A
and Hurley, A and Hogan, C and Boden, D and Racz, P and Markowitz, M},
title =          {Primary $\mbox{HIV}$-1 infection is associated with
preferential depletion of $\mbox{CD4}$+ $\mbox{T lymphocytes}$ from effector sites in the
gastrointestinal tract.},
journal =          {Journal of Experimental Medicine},
year =          {2004},
volume =          {200},
pages =          {761-70}
}

@Article{Musey2003,
author =          {Musey, L and Ding, Y and Cao, J and Lee, J and Galloway, C and
Yuen, A
and Jerome, KR and McElrath, MJ},
title =          {Ontogeny and specificities of mucosal and blood human
immunodeficiency virus type 1-specific $\mbox{CD8}$(+) cytotoxic $\mbox{T lymphocytes}$.},
journal =          {Journal of Virology},
year =          {2003},
volume =          {77},
pages =          {291-300}
}

@Article{Musey1997,
  author =       {Musey, L and Hu, Y and Eckert, L and Christensen, M and Karchmer, T
and McElrath, MJ},
  title =        {$\mbox{HIV-1}$ induces cytotoxic $\mbox{T}$ lymphocytes in the cervix of
infected women.},
  journal =      {Journal of Experimental Medicine},
  year =         {1997},
  volume =       {185},
  pages =        {293-303},
}


@Article{AkiraTakedaKaisho2001,
  author =       {Akira, S and Takeda, K and Kaisho, T},
  title =        {Toll-like receptors: critical proteins linking innate
and acquired immunity.},
  journal =      {Nature Immunology},
  year =         {2001},
  volume =       {2},
  pages =        {675-80},
}


@Article{Krieg2003,
  author =       {Krieg, AM},
  title =        {CpG motifs: the active ingredient in bacterial extracts?},
  journal =      {Nature Medicine},
  year =         {2003},
  volume =       {9},
  pages =        {831-5},
}

@article{Pasinetal2019,
  title={Periods of high dengue transmission defined by rainfall do not impact efficacy of dengue vaccine in regions of endemic disease},
  author={Pasin, Chlo{\'e} and Halloran, M Elizabeth and Gilbert, Peter B and Langevin, Edith and Ochiai, R Leon and Pitisuttithum, Punnee and Capeding, Maria Rosario and Carrasquilla, Gabriel and Frago, Carina and Cort{\'e}s, Margarita and others},
  journal={PloS One},
  volume={13},
  number={12},
  pages={e0207878},
  year={2018},
  publisher={Public Library of Science},
  note={PMCID: PMC6292612}
}

@Article{Beutler2004,
  author =       {Beutler, B},
  title =        {Inferences, questions and possibilities in Toll-like
receptor signaling.},
  journal =      {Nature},
  year =         {2004},
  volume =       {430},
  pages =        {257-63},
}


@Article{PashineValianteUlmer2005,
  author =       {Pasine, A and Valiante, NM and Ulmer, JB},
  title =        {Targeting the innate immune response with improved
vaccine adjuvants.},
  journal =      {Nature Medicine},
  year =         {2005},
  volume =       {11},
  pages =        {S63-8},
}


@Article{Douek2002,
  author =       {Douek, DC and Brenchley, JM and Betts, MR and Ambrozak, DR and Hill,
BJ and Okamoto, Y and Casazza, JP and Kuruppu, J and Kunstman, K and Wolinsky, S and Grossman,
Z and Dybul, M and Oxenius, A and Price, DA and Connors, M and Koup, RA},
  title =        {$\mbox{HIV}$ preferentially infects $\mbox{HIV}$-specific $\mbox{CD4}$+ $\mbox{T cell}$s.},
  journal =      {Nature},
  year =         {2002},
  volume =       {417},
  pages =        {95-98},
}

@Article{Bettsetal2006,
author = {Betts, MR and Nason, MC and West, SM and De Rosa, SC and Migueles, SA and Abraham, J and Lederman, MM and Benito, JM and Goepfert, PA and 
Connors, M and Roederer, M and Koup, RA},
title = {HIV nonprogressors preferentially maintain highly functional HIV-specific $\mbox{CD8+ T}$ cells.},
journal = {Blood},
volume = {107},
pages = {4781-4789},
}




@Article{VeazeyLackner2003,
  author =       {Veazey, R and Lackner, A},
  title =        {The mucosal immune system and $\mbox{HIV}$-1 infection.},
  journal =      {AIDS Review},
  year =         {2003},
  volume =       {5},
  pages =        {245-52},
}


@Article{Migueles2002,
  author =       {Migueles, SA and Laborico, AC and Shupert, WL and Sabbaghian, MS
and Rabin, R and Hallahan, CW and Van Baarle, D and Kostense, S and Miedema, F and
McLaughlin, M
and Ehler, L and Metcalf, J and Liu, S and Connors, M},
  title =        {$\mbox{HIV}$-specific $\mbox{CD8}$+ $\mbox{T cell}$ proliferation is coupled to
perforin expression and is maintained in nonprogressors},
  journal =      {Nature Immunology},
  year =         {2002},
  volume =       {3},
  pages =        {1061-8},
}

@Article{Liuetal2009,
  author =       {Liu, J and O�Brien, KL and Lynch, DM and Simmons, NL and La Porte, A and 
Riggs, AM and Abbink, P and Coffey, RT and Grandpre, LE and Seaman, MS and Landucci, G and Forthal, DN
and Montefiori, DC and Carville, A and Mansfield, KG and Havenga, MJ and Pau, MG and Goudsmit, J and 
Barouch, DH},
  title =        {Immune control of an $\mbox{SIV}$ challenge by a $\mbox{T-cell}$-based vaccine in rhesus monkeys.},
  journal =      {Nature},
  year =         {2009},
  volume =       {457},
  pages =        {87--91},
  note={PMCID: PMC2614452}
}

@Article{Huangetal2009,
  author =       {Huang, Y and Gilbert, P and Montefiori, D and Self, S},
  title =        {Simultaneous evaluation of the magnitude and breadth of a left- and right-censored multivariate response, with application to HIV vaccine development.},
  journal =      {Statistics in Biopharmaceutical Research},
  year =         {2009},
  volume =       {1},
  pages =        {81--91},
  note={PMCID: PMC2805400}
}

@Article{PetersenSinisivanderLaan2006,
  author =       {Petersen, ML and Sinisi, SE and van der Laan, MJ},
  title =        {Estimation of direct causal effects.},
  journal =      {Epidemiology},
  year =         {2006},
  volume =       {17},
  pages =        {276--284}
}

@Article{vanderWeele2008,
  author =       {VanderWeele, TJ},
  title =        {Simple relations between principal stratification and direct and indirect effects.},
  journal =      {Statistics and Probability Letters},
  year =         {2008},
  volume =       {78},
  pages =        {2957--2962}
}


@Article{VanderWeele2009,
  author =       {VanderWeele, TJ},
  title =        {Marginal structural models for the estimation of direct and indirect effects.},
  journal =      {Epidemiology},
  year =         {2009},
  volume =       {20},
  pages =        {18--26}
}

@Article{ZiglerBelin2012,
  author =       {Zigler, CM and Belin, TR},
  title =        {A $\mbox{Bayesian}$ approach to improved estimation of causal effect predictiveness for a principal
surrogate endpoint}, 
  journal =      {Biometrics},
  year =         {2012},
  volume =       {68},
  pages =        {922--932}
}



@Article{vanderWeele2011,
  author =       {VanderWeele, TJ},
  title =        {Principal stratification-- Uses and limitations.},
  journal =      {The International Journal of Biostatistics},
  year =         {2011},
  volume =       {7},
  pages =        {Article 28},
  note={PMCID: PMC3154088}
}

@Article{Joffe2011,
  author =       {Joffe, MJ},
  title =        {Principal stratification and attribution prohibition: Good ideas taken too far},
  journal =      {The International Journal of Biostatistics},
  year =         {2011},
  volume =       {8},
  pages =        {Article 12}
}
%note={PMCID: PMC3204670}

@Article{vanderWeele2013,
  author =       {VanderWeele, TJ},
  title =        {Surrogate measures and consistent surrogates.}, 
  journal =      {Biometrics}, 
  year =         {2013},
  volume =       {69},
  pages =        {561--568},
  note={PMCID:
    PMC4221255}
}

@Article{Chenetal2007,
  author =       {Chen, H and Geng, Z and Jia, J},
  title =        {Criteria for surrogate end points.},
  journal =      {Journal of the Royal Statistical Society, Series B}, 
  year =         {2007},
  volume =       {69},
  pages =        {919--932}
}

@Article{Wuetal2011,
  author =       {Wu, A and He, P and Geng, Z},
  title =        {Sufficient conditions for concluding surrogacy based on observed data.},
  journal =      {Statistics in Medicine},
  year =         {2011},
  volume =       {30},
  pages =        {2422--2434}
}


@Article{Dean1996,
  author =       {Dean, M and Carrington, M and Winkler, C and Huttley, GA and
  Smith, MW
and Allikmets, R and Goedert, JJ and Buchbinder, SP and Vittinghoff, E and Gomperts, E
and Donfield, S and Vlahov, D and Kaslow, R and Saah, A and Rinaldo, C and Detels, R
and O'Brien, SJ},
  title =        {Genetic restriction of $\mbox{HIV}$-1 infection and progression
to $\mbox{AIDS}$ by a deletion allele of the $\mbox{CKR5}$ structural gene. Hemophilia
Growth Development Study, Multicenter AIDS Cohort Study Multicenter
Hemophilia Cohort Study, San Francisco City Cohort, ALIVE Study [see
comments] [published erratum appears in $\mbox{Science 1996 Nov}$
15;274(5290):1069]},
  journal =      {Science},
  year =         {1996},
  volume =       {273},
  pages =        {1856-62},
}

@article{StitelmanvanderLaan2010,
  title={Collaborative targeted maximum likelihood for time to event data.},
  author={Stitelman, Ori M and van der Laan, Mark J},
  year={2010},
  journal={The International Journal of Biostatistics},
  volume={6, Issue 1},
  pages={Article 21}  
}

@article{BalzervanderLaan2013,
  title={Estimating Effects on Rare Outcomes: Knowledge is Power},
  author={Balzer, Laura B and van der Laan, Mark J},
  year={2013},
  journal={U.C. Berkeley Division of Biostatistics Working Paper Series},
  volume={Working Paper 310}, 
  publisher={bepress}
}


@article{Sabchareonetal2012,
  title={Protective efficacy of the recombinant, live-attenuated, {CYD} tetravalent dengue vaccine in {Thai} schoolchildren: a randomised, controlled phase {2b} trial},
  author={Sabchareon, Arunee and Wallace, Derek and Sirivichayakul, Chukiat and Limkittikul, Kriengsak and Chanthavanich, Pornthep and Suvannadabba, Saravudh and Jiwariyavej, Vithaya and Dulyachai, Wut and Pengsaa, Krisana and Wartel, T Anh and others},
  journal={The Lancet},
  year={2012},
  volume={380},
  pages={1556--1567},
  publisher={Elsevier}
}

@article{Schmaderetal2012,
  title={Efficacy, safety, and tolerability of herpes zoster vaccine in persons aged 50--59 years},
  author={Schmader, Kenneth E and Levin, Myron J and Gnann, John W and McNeil, Shelly A and Vesikari, Timo and Betts, Robert F and Keay, Susan and Stek, Jon E and Bundick, Nickoya D and Su, Shu-Chih and others},
  journal={Clinical Infectious Diseases},
  volume={54},
  number={7},
  pages={922--928},
  year={2012},
  publisher={Oxford University Press}
}

@article{RosevanderLaan2011,
  title={A targeted maximum likelihood estimator for two-stage designs},
  author={Rose, Sherri and van der Laan, Mark J},
  journal={{The International Journal of Biostatistics}},
  volume={7},
  number={1},
  pages={1--21},
  year={2011}
}
%note={PMCID: PMC3083136}  



@article{Rubin2006,
  title={Causal inference through potential outcomes and principal stratification: application to studies with" censoring" due to death},
  author={Rubin, Donald B},
  journal={Statistical Science},
  pages={299--309},
  year={2006},
  publisher={JSTOR}
}

@article{MoorevanderLaan2009,
  title={Application of time-to-event methods in the assessment of safety in clinical trials},
  author={Moore, Kelly L and van der Laan, Mark J},
  year={2009},
  journal={U.C. Berkeley Division of Biostatistics Working Paper Series},
  volume={Working Paper 248}, 
  publisher={bepress}
}

@article{vanderLaanRubin2006,
  title={Targeted maximum likelihood learning},
  author={van der Laan, Mark J and Rubin, Daniel},
  year={2006},
  journal={U.C. Berkeley Division of Biostatistics Working Paper Series},
  volume={Working Paper 213}, 
  publisher={bepress}
}

@article{Duerretal2012,
  title={Extended follow-up confirms early vaccine-enhanced risk of {HIV} acquisition and demonstrates waning effect over time among participants in a randomized trial of recombinant adenovirus {HIV} vaccine ({Step study})},
  author={Duerr, Ann and Huang, Yunda and Buchbinder, Susan and Coombs, Robert W and Sanchez, Jorge and del Rio, Carlos and Casapia, Martin and Santiago, Steven and Gilbert, Peter and Corey, Lawrence and others},
  journal={Journal of Infectious Diseases},
  volume={206},
  number={2},
  pages={258--266},
  year={2012},
  publisher={Oxford University Press},
  note={PMCID: PMC3490694}
}


@Article{Buchbinderetal2008,
  author =       {Buchbinder, SP and Mehrotra, DV and Duerr, A and Fitzgerald,
DW and Mogg, R and Li, D and Gilbert, Peter B and Lama, JR and
Marmor, M and del Rio, C and McElrath, MJ and Casimiro, DR and Gottesdiener,
KM and Chodakewitz, JA and Corey, L and Robertson, MN}, 
  title =        {Efficacy assessment of a cell-mediated immunity $\mbox{HIV-1}$ vaccine (the $\mbox{Step Study}$): A double-blind, randomised, placebo-controlled, test-of-concept trial.},
  journal =      {Lancet},
  year =         {2008},
  volume =       {372},
  pages =        {1881--1893}
}

@Article{Buchbinderetal2008short,
  author =       {Buchbinder, SP and Mehrotra, DV and Duerr, A and Fitzgerald,
DW and Mogg, R and Li, D and Gilbert, Peter B and Lama, JR and
Marmor, M and del Rio, C and McElrath, MJ and Casimiro, DR and Gottesdiener,
KM and Chodakewitz, JA and Corey, L and Robertson, MN}, 
  title =        {Efficacy assessment of a cell-mediated immunity $\mbox{HIV-1}$ vaccine (the $\mbox{Step Study}$): A double-blind, randomised, placebo-controlled, test-of-concept trial.},
  journal =      {Lancet},
  year =         {2008},
  volume =       {372},
  pages =        {1881--1893}
}


@Article{McElrathetal2008,
  author =       {McElrath, MJ and De Rosa, SC and Moodie, Z and Dubey, S and Kierstead, L and Janes, H and
 Defawe, OD and Carter, DK and Hural, J and Akondy, R and Buchbinder, SP and Robertson, MN and Mehrotra, DV and
 Self, SG and Corey, L and Shiver, JW and Casimiro, DR and Step Study Protocol Team.},
  title =        {$\mbox{HIV-1}$ vaccine-induced immunity in the test-of-concept $\mbox{Step Study}$: {A} case-cohort analysis.},
  journal =      {Lancet},
  year =         {2008},
  volume =       {372},
  pages =        {1894--1905},
  note={PMCID: PMC2774110}
}

@article{Hertzetal2013,
  title={{HIV-1} vaccine-induced {T}-cell responses cluster in epitope hotspots that differ from those induced in natural infection with {HIV-1}},
  author={Hertz, Tomer and Ahmed, Hasan and Friedrich, David P and Casimiro, Danilo R and Self, Steven G and Corey, Lawrence and McElrath, M Juliana and Buchbinder, Susan and Horton, Helen and Frahm, Nicole and others},
  journal={PLoS Pathog},
  volume={9},
  number={6},
  pages={e1003404},
  year={2013}
}

@Article{Fischeretal2007,
  author =       {Fischer, W and Perkins, S and Theiler, J and Bhattacharya, T and Yusim, K and Funkhouser, R and Kuiken, C and Haynes, B and Letvin, NL and Walker, BD and Hahn, BH and Korber, BT},
  title =        {$\mbox{Pol}$yvalent vaccines for optimal coverage of potential $\mbox{T-cell}$ epitopes in global $\mbox{HIV-1}$ variants.},
  journal =      {Nature Medicine},
  year =         {2007},
  volume =       {13},
  pages =        {100--106},
  note={PMCID: }
}





@Article{SmithRodriguesFine1984,
  author =       {Smith, PG and Rodrigues, LC and Fine, PEM}, 
  title =        {Assessment of the protective efficacy of vaccines against common diseases using case-control and cohort studies.},
  journal =      {International Journal of Epidemiology},
  year =         {1984},
  volume =       {13},
  pages =        {87--93},
}


@Article{WacholderGailPee1991,
  author =       {Wacholder, S and Gail, M and Pee, D}, 
  title =        {Selecting an efficient design for assessing exposure-disease relationships in an assembled cohort.},
  journal =      {Biometrics},
  year =         {1991},
  volume =       {47},
  pages =        {63--76},
}

@Article{WHO1993,
  author =       {World Health Organization}, 
  title =        {The immunological basis for immunization series, Module 1.},
  journal =      {General Immunology},
  year =         {1993},
  volume =       {},
  pages =        {},
}

@Article{Storsaeteretal1998,
  author =       {Storsaeter, J and Hallander, HO and Gustafsson, L and Olin, P}, 
  title =        {Levels of anti-pertussis antibodies related to protection after household exposure to Bordetella pertussis.},
  journal =      {Vaccine},
  year =         {1998},
  volume =       {16},
  pages =        {1907--1916},
}




@Article{Gallopetal2009,
  author =       {Gallop, R and Small, D and Lin, J and Elliott, M and Joffe, M and Ten Have, T},
  title =        {Mediation analysis with principal stratification.},
  journal =      {Statistics in Medicine},
  year =         {2009},
  volume =       {28},
  pages =        {1108-1130},
  note={PMCID: PMC2669107}
}



@Article{Stremlau2004,
  author =       {Stremlau, M and Owens, CM and Perron, MJ and Kiessling, M
and Autissier, P and Sodroski, J},
  title =        {The cytoplasmic body component TRIM5alpha restricts
$\mbox{HIV-1}$ infection in Old World monkeys.},
  journal =      {Nature},
  year =         {2004},
  volume =       {427},
  pages =        {848-53},
}


@Article{CarringtonOBrien2003,
  author =       {Carrington, M and O'Brien, S},
  title =        {The Influence of $\mbox{HLA}$ Genotype on $\mbox{AIDS}$},
  journal =      {Annual Review of Medicine},
  year =         {2003},
  volume =       {54},
  pages =        {535-51},
}


@Article{Martin2002,
  author =       {Martin, MP and Gao, X and Lee, JH and Nelson, GW and Detels, R and Goedert,
JJ and Buchbinder, S and Hoots, K and Vlahov, D and Trowsdale, J and Wilson, M and O'Brien, SJand Carrington, M},
  title =        {Epistatic interaction between KIR3DS1 and $\mbox{HLA-B}$ delays
the progression to $\mbox{AIDS}$.},
  journal =      {Nature Genetics},
  year =         {2002},
  volume =       {31},
  pages =        {429-34},
}


@Article{Sprangers2003,
  author =       {Sprangers, MC and Lakhai, W and Koudstaal, W and Verhoeven, M and Koel,
BF and Vogels, R and Goudsmit, J and Havenga, MJ and Kostense, S},
  title =        {Quantifying adenovirus-neutralizing antibodies by
luciferase transgene detection: addressing preexisting immunity to
vaccine and gene therapy vectors.},
  journal =      {Journal of Clinical Microbiology},
  year =         {2003},
  volume =       {41},
  pages =        {5046-52},
}


@Article{Ewing1998,
  author =       {Ewing, B and Hillier, L and Wendl, MC and Green, P},
  title =        {Base-calling of automated sequencer traces using
phred. I. Accuracy assessment.},
  journal =      {Genome Research},
  year =         {1998},
  volume =       {8},
  pages =        {175-85},
}


@Article{Lore2003,
  author =       {Lore, K and Betts, MR and Brenchley, JM and Kuruppu, J and Khojasteh,
S and Perfetto, S and Roederer, M and Seder, RA and Koup, RA},
  title =        {Toll-like receptor ligands modulate dendritic cells to
augment cytomegalovirus- and $\mbox{HIV}$-1- specific $\mbox{T cell}$ responses.},
  journal =      {Journal of Immunology},
  year =         {2003},
  volume =       {171},
  pages =        {4320-8},
}

@Article{Hawn2003,
  author =       {Hawn, TR and Verbon, A and Lettinga, KD and Zhao, LP and Li, SS Laws,
RJ and Skerrett, SJ and Beutler, B and Schroeder, L and Nachman, A and Ozinsky, A and Smith, KDand Aderem A},
  title =        {A common dominant TLR5 stop codon polymorphism
abolishes flagellin signaling and is associated with susceptibility to
legionnaires? disease.},
  journal =      {Journal of Experimental Medicine},
  year =         {2003},
  volume =       {198},
  pages =        {1563-72},
}


@Article{Becker2002,
  author =       {Becker, TC and Wherry, EJ and Boone, D and Murali-Krishna, K and Antia,
R and Ma, A and Ahmed, R},
  title =        {Interleukin 15 is required for proliferative renewal
of virus-specific memory $\mbox{CD8}$ $\mbox{T cell}$s.},
  journal =      {Journal of Experimental Medicine},
  year =         {2002},
  volume =       {195},
  pages =        {1541-8},
}


@Article{Cao2003,
  author =       {Cao, J and McNevin, J and Holte, S and Fink, L and Corey, L and McElrath, MJ},
  title =        {Comprehensive analysis of $\mbox{Human Immunodeficiency Virus Type}$
1 ($\mbox{HIV-1}$)-specific Gamma Interferon-secreting $\mbox{CD8}$+ $\mbox{T cell}$s in
primary $\mbox{HIV}$-1 infection.},
  journal =      {Journal of Virology},
  year =         {2003},
  volume =       {77},
  pages =        {6867-6878},
}


@Article{Kaech2003,
  author =       {Kaech, SM and Tan, JT and Wherry, EJ and Konieczny, BT and Surh, CD
and Ahmed, R},
  title =        {Selective expression of the interleukin 7 receptor
identifies effector $\mbox{CD8}$ $\mbox{T cell}$s that give rise to long-lived memory cells.},
  journal =      {Nature Immunology},
  year =         {2003},
  volume =       {4},
  pages =        {1191-8},
}


@Article{Wherry2003,
  author =       {Wherry, EJ and Teichgraber, V and Becker, TC and Masopust, D and Kaech,
SM and Antia, R and von Andrian, UH and Ahmed, R},
  title =        {Lineage relationship and protective immunity of memory
$\mbox{CD8}$ $\mbox{T cell}$ subsets},
  journal =      {Nature Immunology},
  year =         {2003},
  volume =       {4},
  pages =        {225-34},
}


@Article{Wherry2004,
  author =       {Wherry, EJ and Barber, DL and Kaech, SM and Blattman, JN and Ahmed, R},
  title =        {Antigen-independent memory $\mbox{CD8}$ $\mbox{T cell}$s do not develop
during chronic viral infection.},
  journal =      {Proceedings of the Natonal Academy of Sciences USA},
  year =         {2004},
  volume =       {101},
  pages =        {16004-9},
}


@Article{Betts2003,
  author =       {Betts, MR and Brenchley, JM and Price, DA and De Rosa, SC and Douek,
DC and Roederer, M and Koup, RA},
  title =        {Sensitive and viable identification of
antigen-specific $\mbox{CD8}$+ $\mbox{T cell}$s by flow cytometric assay for degranulation},
  journal =      {Journal of Immunology Methods},
  year =         {2003},
  volume =       {281},
  pages =        {65-78},
}


@Article{SlifkaWhitton2001,
  author =       {Slifka, MK and Whitton, JL},
  title =        {Functional avidity maturation of $\mbox{CD8}$(+) $\mbox{T cell}$s
without selection of higher affinity TCR.},
  journal =      {Nature Immunology},
  year =         {2001},
  volume =       {2},
  pages =        {711-7},
}


@Article{WangAltman2003,
  author =       {Wang, XL and Altman, JD},
  title =        {Caveats in the design of $\mbox{MHC}$ class $\mbox{I}$
tetramer/antigen-specific $\mbox{T lymphocytes}$ dissociation assays.},
  journal =      {Journal of Immunology Methods},
  year =         {2003},
  volume =       {280},
  pages =        {25-35},
}


@Article{Douek2002b,
  author =       {Douek, DC and Betts, MR and Brenchley, JM and Hill, BJ and Ambrozak,
DR and Ngai, KL and Karandikar, NJ and Casazza, JP and Koup, RA},
  title =        {A novel approach to the analysis of specificity,
clonality, and frequency of $\mbox{HIV}$-specific $\mbox{T cell}$ responses reveals a
potential mechanism for control of viral escape.},
  journal =      {Journal of Immunology},
  year =         {2002},
  volume =       {168},
  pages =        {3099-104},
}


@Article{Meyer-Olson2004,
  author =       {Meyer-Olson, DK and Shoukry, NH and Brady, KW and Kim, H and Oson, DP
and Hartman, K and Shintani, AK and Walker, CM and Kalams, SA},
  title =        {Limited $\mbox{T cell}$ receptor diversity of HCV-specific T
cell responses is associated with $\mbox{CTL}$ escape.},
  journal =      {Journal of Experimental Medicine},
  year =         {2004},
  volume =       {200},
  pages =        {307-19},
}


@Article{Meyer-Olson2003,
  author =       {Meyer-Olson, DK and Brady, JT and Blackard, JT and Allen, TM and Islam,
S and Shoukry, NH and Hartman, K and Walker, CM and Kalams, SA},
  title =        {Analysis of the TCR beta variable gene repertoire in
chimpanzees: identification of functional homologs to human psuedogenes.},
  journal =      {Journal of Immunology},
  year =         {2003},
  volume =       {170},
  pages =        {4161-9},
}


@Article{Cohen2002,
  author =       {Cohen, GM and Islam, SA and Noble, MS and Lau, C and Brander, C
and Altfeld, MA and Rosenberg, ES and Schmitz, JE and Cameron, TO and Kalams, SA},
  title =        {Clonotype tracking of TCR repertoires during chronic
virus infections.},
  journal =      {Virology},
  year =         {2002},
  volume =       {304},
  pages =        {474-84},
}


@Article{Shannon1948,
  author =       {Shannon, CE},
  title =        {A mathematical theory of communication.},
  journal =      {Bell Systems Technical Journal},
  year =         {1948},
  volume =       {27},
  pages =        {379-423},
}


@Article{Chomczynski1993,
  author =       {Chomczynski, P},
  title =        {A reagent for the single-step simultaneous isolation
of $\mbox{RNA}$, $\mbox{DNA}$ and proteins from cell and tissue samples.},
  journal =      {Biotechniques},
  year =         {1993},
  volume =       {15},
  pages =        {532-4,536-7},
}


@Article{Hladik2003,
  author =       {Hladik, F and Desbien, A and Lang, J and Wang, L and Ding, Y and Holte, S
and Wilson, A and Xu, Y and Moerbe, M and Schmechel, S and McElrath, MJ},
  title =        {Most highly exposed seronegative men lack $\mbox{HIV}$-1
specific, IFN-gamma-secreting $\mbox{T cell}$s.},
  journal =      {Journal of Immunology},
  year =         {2003},
  volume =       {171},
  pages =        {2671-83},
}


@Article{GordonAbajianGreen1998,
  author =       {Gordon, D and Abajian, C and Green, P},
  title =        {Consed: a graphical tool for sequence finishing.},
  journal =      {Genome Research},
  year =         {1998},
  volume =       {8},
  pages =        {195-202},
}


@Article{Mascola2002,
  author =       {Mascola, JR and Louder, MK and Winter, R and Prabhakara, R and De Rosa,
C and Douek, DC and Hill, BJ and Gabuzda, D and Roederer, M},
  title =        {Human immunodeficiency virus type 1 neutralization
measured by flow cytometric quantitation of single-round infection of
primary human $\mbox{T cell}$s.},
  journal =      {Journal of Virology},
  year =         {2002},
  volume =       {76},
  pages =        {4810--21},
}


@Article{Betts2000,
  author =       {Betts, MR and Casazza, JP and Patterson, BA and Waldrop, S and Trigona,
W and Fu, TM and Kern, F and Picker, LJ and Koup, RA},
  title =        {Putative immunodominant human immunodeficiency
virus-specific $\mbox{CD8}$(+) $\mbox{T-cell}$ responses cannot be predicted by major
histocompatibility complex class $\mbox{I}$ haplotype.},
  journal =      {Journal of Virology},
  year =         {2000},
  volume =       {74},
  pages =        {9144-51},
}


@Article{Ferrari2001,
  author =       {Ferrari, G and Neal, W and Jones, A and Olender, N and Ottinger, J and Ha,
R and McElrath, MJ and Goepfert, P and Weinhold, KJ},
  title =        {$\mbox{CD8}$ $\mbox{CTL}$ responses in vaccines: emerging patterns of
$\mbox{HLA}$ restriction and epitope recognition.},
  journal =      {Immunology Letters},
  year =         {2001},
  volume =       {79},
  pages =        {37-45},
}


@Article{AalenJohansen1978,
  author =       {Aalen, OO and Johansen, S},
  title =        {An empirical transition matrix for non-homogeneous
Markov chains based on censored observations.},
  journal =      {Scandinavian Journal of Statistics},
  year =         {1978},
  volume =       {5},
  pages =        {141-150},
}

@Article{Follmann2014,
  author =       {Follmann, D},
  title =        {Incorporating Founder Virus Information in Vaccine Field Trials.}, 
  journal =      {Biometrics},
  year =         {2014},
  volume =       {in press},
  pages =        {}
}



@Article{AlyKocharMcKeague1994,
  author =       {Aly, EE and Kochar, SC and McKeague, IW},
  title =        {Some tests for comparing cumulative incidence
functions and cause-specific hazard rates.},
  journal =      {Journal of the American Statistical Association},
  year =         {1994},
  volume =       {89},
  pages =        {994-999},
}


@Article{BanerjeeWellner2001,
  author =       {Banerjee, M and Wellner, JA},
  title =        {Likelihood ratio tests for monotone functions.},
  journal =      {The Annals of Statistics},
  year =         {2001},
  volume =       {29},
  pages =        {1699-1731},
}


@Article{BetenskyFinkelstein1999,
  author =       {Betensky, RA and Finkelstein, DM},
  title =        {A non-parametric maximum likelihood estimator for
bivariate interval censored data.},
  journal =      {Statistics in Medicine},
  year =         {1999},
  volume =       {18},
  pages =        {3089-3100},
}


@Article{Bloom1996,
  author =       {Bloom, BR},
  title =        {A perspective on $\mbox{AIDS}$ vaccines.},
  journal =      {Science},
  year =         {1996},
  volume =       {272},
  pages =        {1888-1890},
}


@Article{Bures2002,
  author =       {Bures, R and Morris, L and Williamson, C and Ramjee, G and Deers, M
and Fiscus, SA and Abdool-Karim, S and Montefiori, DC},
  title =        {Regional clustering of shared neutralization
determinants on primary isolates of clade C human immunodeficiency virus
type 1 from South Africa.},
  journal =      {Journal of Virology},
  year =         {2002},
  volume =       {76},
  pages =        {2233-2244},
}


@Article{Cao1997,
  author =       {Cao, H and Kanki, P and Sankale, P and Dieng-Sarr, JL and Mazzara, GP
and Kalams, SA and Korber, B and Mboup, S and Walker, BD},
  title =        {Cytotoxic T-lymphocyte cross-reactivity among
different human immunodeficiency virus type 1 clades: implications for
vaccine development.},
  journal =      {Journal of Virology},
  year =         {1997},
  volume =       {71},
  pages =        {8615-8623},
}


@Article{Connor1998,
  author =       {Connor, RI and Korber, BTM and Graham, BS and Hahn, BH and Ho, DD
and Walker, BD and Neumann, AU and Vermund, SH and Mestecky, J and Jackson, S and Fenamore, E
and Cao, Y and Gao, F and Kalams, S and Kunstman, KJ and McDonald, D and McWilliams, N
and Trkola, A
and Moore, JP and Wolinsky, SM},
  title =        {Immunological and virological analyses of persons
infected by human immunodeficiency virus type 1 while participating in
trials of recombinant gp120 subunit vaccines.},
  journal =      {Journal of Virology},
  year =         {1998},
  volume =       {72},
  pages =        {1552-1576},
}

@Article{MooreHo1995,
  author =       {Moore, JP and Ho, DD},
  title =        {$\mbox{HIV-1}$ neutralization: the consequences of viral adaptation to growth on transformed
$\mbox{T cell}$s.},
  journal =      {AIDS},
  year =         {1995},
  volume =       {9 (Suppl A)},
  pages =        {S117-S136},
}



@Article{Dawson2001,
  author =       {Dawson, DV and Ozgur, M and Sari, K and Ghanayem, M and Kostyu, DD},
  title =        {Ramifications of $\mbox{HLA}$ class $\mbox{I}$ polymorphism and
population genetics for vaccine development.},
  journal =      {Genetic Epidemiology},
  year =         {2001},
  volume =       {20},
  pages =        {87-106},
}


@Book{DayhoffSchwartzOrcutt1978,
  author =          {Dayhoff, MO and Schwartz, RM and Orcutt, BC},
  ALTeditor =          {},
  title =          {A model of evolutionary change in proteins. In:
Atlas of Protein Sequence and Structure.},
  publisher =          {Washington D.C. National Biomedical Research
Foundation},
  year =          {1978},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {Washington, D.C.},
  OPTedition =          {M.O. Dayoff, ed.},
  OPTmonth =          {},
  OPTnote =          {pp. 345-362},
  OPTannote =          {}
}


@Article{DeGruttola2002,
  author =       {DeGruttola, VG and Clax, P and DeMets, DL and Downing, GJ
and Ellenberg, SS and Friedman, L and Gail, MH and Prentice, R and Wittes, J and Zeger, SL},
  title =        {Considerations in the evaluation of surrogate
endpoints in clinical trials.},
  journal =      {Controlled Clinical Trials},
  year =         {2002},
  volume =       {22},
  pages =        {485-502},
}


@Book{DHHSGuidelines2004,
  author =          {DHHS Guidelines, Panel on Clinical Practices for
Treatment of $\mbox{HIV}$ Infection, Department of Health and Human Services},
  ALTeditor =          {},
  title =          {Guidelines for the Use of Antiretroviral Agents in
HIV-Infected Adults and Adolescents.},
  publisher =          {Washington D.C. National Biomedical Research
Foundation},
  year =          {October 29, 2004},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          { },
  OPTedition =          { },
  OPTmonth =          {},
  OPTnote =          {Available at:
http://www.aidsinfo.nih.govguidelinesdefaultdb2.asp?id=50.},
  OPTannote =          {}
}


@Article{Dixon1993,
  author =       {Dixon, DO and Rida, WN and Fast, PE and Hoth, R},
  title =        {$\mbox{HIV}$ vaccine trials: some design issues including
sample size calculation.},
  journal =      {Journal of the Acquired Immune Deficiency Syndrome},
  year =         {1993},
  volume =       {6},
  pages =        {485-496},
}

@Article{Rida1997,
  author =       {Rida, W and Fast, P and Hoff, R and Fleming T},
  title =        {Intermediate-size trials for the evaluation of an $\mbox{HIV}$ vaccine candidate: a workshop
summary.},
  journal =      {Journal of the Acquired Immune Deficiency Syndrome and Human Retrovirology},
  year =         {1997},
  volume =       {16},
  pages =        {195-203},
}

@book{WestfallYoung1993,
  title={Resampling-based multiple testing: Examples and methods for p-value adjustment},
  author={Westfall, Peter H and Young, S Stanley and others},
  volume={279},
  year={1993},
  publisher={John Wiley \& Sons}
}

@article{GeDudoitSpeed2003,
  title={Resampling-based multiple testing for microarray data analysis},
  author={Ge, Youngchao and Dudoit, Sandrine and Speed, Terence P},
  journal={Test},
  volume={12},
  number={1},
  pages={1--77},
  year={2003},
  publisher={Springer}
}

@Article{Cohen2007,
  author =       {Cohen, J},
  title =        {Promising $\mbox{AIDS}$  vaccine's failure leaves field reeling.},
  journal =      {Science},
  year =         {2007},
  volume =       {318},
  pages =        {28-29},
  note={PMCID: }
}

@Article{AndersonGarnett1996,
  author =       {Anderson, RM and Garnett, GP},
  title =        {Low-efficacy $\mbox{HIV}$ vaccines: potential for community-based intervention programs.},
  journal =      {Lancet},
  year =         {1996},
  volume =       {348},
  pages =        {1010-1013},
}






@Article{Doolan1997,
  author =       {Doolan, DL and Hoffman, SL and Southwood, S and Wentworth, PA
and Sidney, J and Chesnut, RW and Keogh, E and Appella, E and Nutman, TB and Lal, AA and
Gordon, DM
and Oloo, A and Sette, A},
  title =        {Degenerate cytotoxic $\mbox{T cell}$ epitopes from P.
falciparum restricted by multiple $\mbox{HLA-A}$ and $\mbox{HLA-B}$ supertype alleles.},
  journal =      {Immunity},
  year =         {1997},
  volume =       {7},
  pages =        {97-112},
}


@Article{Dorrell1999,
  author =       {Dorrell, L and Dong, T and Ogg, SG and Lister, S and McAdam, S and Rostron,
T and Conlon, C and McMichael, AJ and Rowland-Jones, SL},
  title =        {Distinct recognition of non-clade B human
immunodeficiency virus type 1 epitopes by cytotoxic T lymphocytes
generated from donors infected in Africa.},
  journal =      {Journal of Virology},
  year =         {1999},
  volume =       {73},
  pages =        {1708-1714},
}

@article{Coreyetal2015immune,
  title={Immune correlates of vaccine protection against {HIV-1} acquisition},
  author={Corey, Lawrence and Gilbert, Peter B and Tomaras, Georgia D and Haynes, Barton F and Pantaleo, Giuseppe and Fauci, Anthony S},
  journal={Science Translational Medicine},
  volume={7},
  number={310},
  pages={310rv7--310rv7},
  year={2015},
  publisher={American Association for the Advancement of Science},
  note={PMCID: PMC4751141}
}

@Article{EsparzaBhamarapravti2000,
  author =       {Esparza, J and Bhamarapravti, N},
  title =        {Accelerating the development and future availability
of $\mbox{HIV}$-1 vaccines: why, when, where and how?},
  journal =      {Lancet},
  year =         {2000},
  volume =       {355},
  pages =        {2061-2066},
}


@Article{Fauci1999,
  author =       {Fauci, AS},
  title =        {The $\mbox{AIDS}$ epidemic- Considerations for the 21st century.},
  journal =      {New England Journal of Medicine},
  year =         {1999},
  volume =       {341},
  pages =        {1046-1050},
}

@Article{Faucietal2008,
  author =       {Fauci, AS and Johnston, MI and Dieffenbach, CW and Burton, DR and Hammer, SM and Hoxie, JA and Martin, M and Overbaugh, J and Watkins, DI and Mahmoud, A and Greene, WC},
  title =        {$\mbox{HIV}$ vaccine research: the way forward.},
  journal =      {Science},
  year =         {2008},
  volume =       {321},
  pages =        {530--532},
  note={PMCID: NIHMS142560}
}

@Article{FineGray1999,
  author =       {Fine, JP and Gray, RJ},
  title =        {A proportional hazards model for the subdistribution
of a competing risk.},
  journal =      {Journal of the American Statistical Association},
  year =         {1999},
  volume =       {94},
  pages =        {496-509},
}


@Article{Fine1999,
  author =       {Fine, JP},
  title =        {Analysing competing risks data with transformation
models.},
  journal =      {Journal of the Royal Statistical Society, Series B},
  year =         {1999},
  volume =       {61},
  pages =        {817-830},
}


@Article{Fleming1994,
  author =       {Fleming, TR},
  title =        {Surrogate markers in $\mbox{AIDS}$ and cancer trials.},
  journal =      {Statistics in Medicine},
  year =         {1994},
  volume =       {13},
  pages =        {1423-1435},
}


@Article{FlemingDeMets1996,
  author =       {Fleming, TR and DeMets, DL},
  title =        {Surrogate endpoints in clinical trials: Are we being
misled?},
  journal =      {Annals of Internal Medicine},
  year =         {1996},
  volume =       {125},
  pages =        {605-613},
}


@Article{GentlemanVandal2001,
  author =       {Gentleman, R and Vandal, AC},
  title =        {Computational algorithms for censored-data problems
using intersection graphs.},
  journal =      {Journal of Computational and Graphical Statistics},
  year =         {2001},
  volume =       {10},
  pages =        {403-421},
}


@Article{GilbertSelfAshby1998,
  author =       {Gilbert, Peter B and Self, S and Ashby, M},
  title =        {Statistical methods for assessing differential vaccine
protection against human immunodeficiency virus types.},
  journal =      {Biometrics},
  year =         {1998},
  volume =       {54},
  pages =        {799-814},
}


@Article{GilbertLeleVardi1999,
  author =       {Gilbert, Peter B and Lele, S and Vardi, Y},
  title =        {Maximum likelihood estimation in semiparametric
selection bias models with application to $\mbox{AIDS}$ vaccine trials.},
  journal =      {Biometrika},
  year =         {1999},
  volume =       {86},
  pages =        {27-43},
}

@Article{QinZhang1997,
  author =       {Qin, J and Zhang, B},
  title =        {A goodness-of-fit test for logistic regression models based on case-control data.},
  journal =      {Biometrika},
  year =         {1997},
  volume =       {84},
  pages =        {609--618},
}


@Article{Gilbert2000a,
  author =       {Gilbert, Peter B},
  title =        {Comparison of competing risks failure time methods and
time-independent methods for assessing strain variations in vaccine
protection.},
  journal =      {Statistics in Medicine},
  year =         {2000},
  volume =       {19},
  pages =        {3065-3086},
}


@Article{Gilbert2000b,
  author =       {Gilbert, Peter B},
  title =        {Interpretability and robustness of sieve analysis
models for assessing $\mbox{HIV}$ strain variations in vaccine efficacy.},
  journal =      {Statistics in Medicine},
  year =         {2000},
  volume =       {20},
  pages =        {263-279},
}


@Article{Gilbert2000c,
  author =       {Gilbert, Peter B},
  title =        {Large sample theory of maximum likelihood estimates in
semiparametric biased sampling models.},
  journal =      {Annals of Statistics},
  year =         {2000},
  volume =       {28},
  pages =        {151-194},
}


@Article{Gilbert2000d,
  author =       {Gilbert, Peter B},
  title =        {Some statistical issues in the design and analysis of
$\mbox{HIV}$ vaccine and treatment trials.},
  journal =      {Statistical Methods in Medical Research},
  year =         {2000},
  volume =       {9},
  pages =        {207-229},
}


@Article{Gilbert2000,
  author =       {Gilbert, Peter B and Hanna, G and DeGruttola, V and Martinez-Picado, J
and Kuritzkes, D and Johnson, V and Richman, D and D'Aquila, R},
  title =        {Comparative analysis of $\mbox{HIV}$ type 1 genotypic
resistance across antiretroviral trial treatment regimens.},
  journal =      {AIDS Research and Human Retroviruses},
  year =         {2000},
  volume =       {16},
  pages =        {1325-1336},
}


@Article{Gilbert2001a,
  author =       {Gilbert, Peter B and Self, S and Rao, M and Naficy, A and Clemens, J},
  title =        {Sieve analysis: Methods for assessing how vaccine
efficacy depends on genotypic and phenotypic pathogen variation from
vaccine trial data.},
  journal =      {Journal of Clinical Epidemiology},
  year =         {2001},
  volume =       {54},
  pages =        {68-85},
}


@Article{Gilbert2001b,
  author =       {Gilbert, Peter B and Novitsky, V and Montano, M and Essex, M},
  title =        {An efficient test for comparing $\mbox{HIV}$ sequence diversity
between populations.},
  journal =      {The Journal of Computational Biology},
  year =         {2001},
  volume =       {8},
  pages =        {123-139},
}


@Article{Gilbert2001c,
  author =       {Gilbert, Peter B and DeGruttola, V and Hammer, S and Kuritzkes, D},
  title =        {Virological and regimen termination surrogate
endpoints in $\mbox{AIDS}$ clinical trials.},
  journal =      {The Journal of the American Medical Association},
  year =         {2001},
  volume =       {285},
  pages =        {775-782},
}


@Article{Gilbert2002b,
  author =       {Gilbert, Peter B and Wei, LJ and Kosorok, MR and Clemens, JD},
  title =        {Simultaneous inference on the contrast of two hazard
functions with censored observations.},
  journal =      {Biometrics},
  year =         {2002},
  volume =       {58},
  pages =        {773-780},
}


@Article{Gilbert2003a,
  author =       {Gilbert, Peter B and McKeague, I and Eisen, G and Mullins, C
and Gueye-Ndiaye, A and Mboup, S and Kanki, P},
  title =        {Comparison of $\mbox{HIV}$-1 and $\mbox{HIV}$-2 infectivity from a
prospective cohort study in Senegal.},
  journal =      {Statistics in Medicine},
  year =         {2003},
  volume =       {22},
  pages =        {573-593}
}


@Article{GliddenWei1999,
  author =       {Glidden, DV and Wei, LJ},
  title =        {Rank estimation of treatment differences based on
repeated measurements subject to dependent censoring.},
  journal =      {Journal of the American Statistical Association},
  year =         {1999},
  volume =       {94},
  pages =        {888-895},
}


@Book{GrahamKarzon1998,
  author =          {Graham, BS and Karzon, DT},
  ALTeditor =          {Merigan TC, Jr, Bartlett JG, Bolognesi D., eds.},
  title =          {$\mbox{AIDS}$ vaccine development. In:  Textbook of $\mbox{AIDS}$
Medicine.},
  publisher =          {Williams and Wilkins},
  year =          {1998},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {Baltimore},
  OPTedition =          {2nd},
  OPTmonth =          {},
  OPTnote =          {pp. 689-724},
  OPTannote =          {}
}

@Book{BenkeserCaroneGilbert2018,
  author =          {Benkeser, D and Carone, M and Gilbert, PB},
  ALTeditor =          {van der Laan MJ, Rose S, eds.},
  title =          {{Targeted estimation of cumulative vaccine 
sieve effects. In: Targeted Learning in Data Science: Causal Inference for 
Complex Longitudinal Studies}},
  publisher =          {Springer},
  year =          {2018},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@article{Hammeretal2013,
   author = {Hammer, S.M. and Sobieszczyk, M.E. and Janes, H. and Karuna, S.T. and Mulligan, M. J. and Grove, D. and Koblin, B.A. and Buchbinder, S.P. and Keefer, M. C. and Tomaras, G.D. and Frahm, N. and Hural, J. and Anude, C. and Graham, B.S. and Enama, M.E. and Adams, E. and DeJesus, E. and Novak, R.M. and Frank, I. and Bentley, C. and Ramirez, S. and Fu, R. and Koup, R. A. and Mascola, J. and Nabel, G.J. and Montefiori, D. C. and Kublin, J. and McElrath, M. J. and Corey, L. C. and Gilbert, P.B. and the HVTN 505 Study Team},
   title = {Efficacy trial of a $\mbox{DNA/rAd5 HIV-1}$ preventive vaccine},  
   journal = {New England Journal of Medicine},
   year = {2013},
   volume={369},
   pages={283--292},
   note={PMCID:
    PMC4030634}
}

@article{Hammeretal2013short,
   author = {Hammer, S.M. and Sobieszczyk, M.E. and Janes, H. and et al.},
   title = {Efficacy trial of a $\mbox{DNA/rAd5 HIV-1}$ preventive vaccine},
   journal = {New Engl J Med},
   year = {2013},
   volume={369},
   pages={283--292}
}

@article{Hammeretal2013short2,
   author = {Hammer, S.M. and Sobieszczyk, M.E. and Janes, H. and Karuna, S.T. and Mulligan, M. J. and Grove, D. and Koblin, B.A. and et al.},
   title = {Efficacy trial of a $\mbox{DNA/rAd5 HIV-1}$ preventive vaccine},  
   journal = {New England Journal of Medicine},
   year = {2013},
   volume={369},
   pages={283--292}
}


@Book{Miaoetal2013,
  author =          {Miao, C and Li, X and Gilbert, Peter B and Chan, ISF},
  ALTeditor =          {Ting Lee, M-L and Gail, M and Satten, G and Cai, T and Pfeiffer, R and Gandy, A}, 
  title =          {A multiple imputation approach for surrogate marker evaluation in the principal stratification causal inference framework. {In: Risk Assessment and Evaluation of Predictions}},
  publisher =          {Springer, New York},
  year =          {2013},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}



@Article{Graham1999,
  author =       {Graham, BS and McElrath, MJ and Connor, RI and Schwartz, DH and Gorse,
GJ and Keefer, MC and Mulligan, MJ and Matthew, TJ and Wolinsky, SM and Montefiori, DC
and Vermund, SH and Lambert, JS and Belshe, RB and Dolin, R and Wright, PF and Korber, BT and
Wolff,
MC and Fast, PE and the $\mbox{AIDS}$ Vaccine Evaluation Group and the Correlates
of $\mbox{HIV}$ Immune Protection Group},
  title =        {Analysis of intercurrent human immunodeficiency virus
type 1 infections in $\mbox{Phase I and II}$ trials of candidate $\mbox{AIDS}$ vaccines.},
  journal =      {Journal of Infectious Diseases},
  year =         {1999},
  volume =       {177},
  pages =        {310-319},
}


@Article{Graham2002,
  author =       {Graham, BS},
  title =        {Clinical trials of $\mbox{HIV}$ vaccines.},
  journal =      {Annual Review of Medicine},
  year =         {2002},
  volume =       {53},
  pages =        {207-221},
}


@Article{Gray1988,
  author =       {Gray, RJ},
  title =        {A class of K-sample tests for comparing the cumulative
incidence of a competing risk.},
  journal =      {Annals of Statistics},
  year =         {1988},
  volume =       {16},
  pages =        {1141-1154},
}


@Book{GroeneboomWellner1992,
  author =          {Groeneboom, P and Wellner, JA},
  ALTeditor =          { },
  title =          {Information bounds and nonparametric maximum
likelihood estimation.},
  publisher =          {Birkhaueser, Basel},
  year =          {1992},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{HIVSurrogateMarkerCollaborativeGroup2000,
  author =       {$\mbox{HIV}$ Surrogate Marker Collaborative Group},
  title =        {Human immunodeficiency virus type 1 $\mbox{RNA}$ level and $\mbox{CD4}$
count as prognostic markers and surrogate endpoints: A meta-analysis.},
  journal =      {AIDS Research and Human Retroviruses},
  year =         {2000},
  volume =       {16},
  pages =        {1123-1133},
}


@Article{Holland1986,
  author =       {Holland, P},
  title =        {Statistics and causal inference.},
  journal =      {Journal of the American Statistical Association},
  year =         {1986},
  volume =       {81},
  pages =        {945-961},
}


@Article{HuTsai1999,
  author =       {Hu, XS and Tsai, WY},
  title =        {Linear rank tests for competing risks model.},
  journal =      {Statistica Sinica},
  year =         {1999},
  volume =       {9},
  pages =        {971-983},
}


@Article{Hudgens2001,
  author =       {Hudgens, MG and Longini, IM and Choopanya, K and Vanichsensi, S
and Kitayaporn, D and Mastro, TD and Mock, PA and Halloran, ME},
  title =        {Estimating the $\mbox{HIV}$-1 transmission probability in
injecting drug users in Thailand.},
  journal =      {Applied Statistics},
  year =         {2001},
  volume =       {50},
  pages =        {1-14},
}


@Article{Hudgens2002,
  author =       {Hudgens, MG and Longini, IM and Choopanya, K and Vanischseni, S
and Kitayaportn, D and Mastro, TD and Mock, PA and Halloran, ME and Hu, DJ and Satten, GA},
  title =        {Subtype-specific transmission probabilities for Human
Immunodeficiency Virus Type 1 among injecting drug users in Bangkok,
Thailand.},
  journal =      {American Journal of Epidemiology},
  year =         {2002},
  volume =       {155},
  pages =        {159-168},
}


@Article{HudgensHoeringSelf2003,
  author =       {Hudgens, MG and Hoering, A and Self, SG},
  title =        {On the analysis of viral load endpoints in $\mbox{HIV}$ vaccine
 trials},
  journal =      {Statistics in Medicine},
  year =         {2003},
  volume =       {22},
  pages =        {2281-2298},
}


@Book{KankiSankaleMboup2002,
  author =          {Kanki, PJ and Sankale, J-L and Mboup, S},
  ALTeditor =          {M. Essex, S. Mboup, P. Kanki, R. Marlink, Tlou
S., eds.},
  title =          {Biology of Human Immunodeficiency Virus Type 2
(HIV-2). In: $\mbox{AIDS}$ in Africa.},
  publisher =          {Kluwer Academic, New York},
  year =          {2002},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          { },
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          { },
  OPTannote =          {}
}

@Book{Kuiken2002,
  author =          {Kuiken, C and Foley, B and Hahn, B and Marx, P and McCutchan, F
and Mellors, J and Wolinsky, S and Korber (ed.), B},
  title =          {$\mbox{HIV}$ Sequence Compendium 2001.},
  year =          {2002},
  publisher = {Theoretical Biology and Biophysics Group, Los Alamos
National Laboratory},
}


@Article{LagakosKimRobins1990,
  author =       {Lagakos, S and Kim, L and Robins, JM},
  title =        {Adjusting for early treatment initiation in
comparative clinical trials.},
  journal =      {Statistics in Medicine},
  year =         {1990},
  volume =       {9},
  pages =        {1417-1424}
}


@Article{Lalvani1997,
  author =       {Lalvani, A and Brookes, R and Hableton, S and Britton, WJ and Hill, AV
and McMichael, AJ},
  title =        {Rapid effector function in $\mbox{CD8}$+ memory $\mbox{T cell}$s.},
  journal =      {Journal of Experimental Medicine},
  year =         {1997},
  volume =       {186},
  pages =        {859-865}
}


@Article{Lam1998,
  author =       {Lam, KF},
  title =        {A class of tests for the equality of k cause-specific
hazard rates in a competing risks model.},
  journal =      {Biometrika},
  year =         {1998},
  volume =       {85},
  pages =        {179-188},
}

@Article{LarsonDinse1985,
  author =       {Larson, MG and Dinse, GE},
  title =        {A mixture model for the regression analysis of
competing risks data.},
  journal =      {Applied Statistics},
  year =         {1985},
  volume =       {34},
  pages =        {201-211},
}


@Article{Larsson1999,
  author =       {Larsson, M and Jin, X and Ramratnam, B and Ogg, GS and Engelmayer, J
and Demoitie, MA and McMichael, AJ and Cox, WI and Steinman, RM and Nixon, D and Bhardwaj, N},
  title =        {A recombinant vaccinia virus based $\mbox{ELISpot}$ assay
detects high frequencies of $\mbox{Pol}$-specific $\mbox{CD8}$ $\mbox{T cell}$s in $\mbox{HIV}$-1 positive
individuals.},
  journal =      {AIDS},
  year =         {1999},
  volume =       {13},
  pages =        {767-777},
}


@Article{LiSun2000,
  author =       {Li, G and Sun, Y},
  title =        {A simulation-based goodness-of-fit test for survival
data.},
  journal =      {Statistics and Probability Letters},
  year =         {2000},
  volume =       {47},
  pages =        {403-410},
}


@Article{LiangZeger1986,
  author =       {Liang, KY and Zeger, SL},
  title =        {Longitudinal data analysis using the generalized
linear model.},
  journal =      {Biometrika},
  year =         {1986},
  volume =       {73},
  pages =        {13-22},
}


@Article{LinRobinsWei1996,
  author =       {Lin, DY and Robins, JM and Wei, LJ},
  title =        {Comparing two failure time distributions in the
presence of dependent censoring.},
  journal =      {Biometrika},
  year =         {1996},
  volume =       {83},
  pages =        {381-393},
}


@Article{LinWeiYing1993,
  author =       {Lin, DY and Wei, LJ and Ying, Z},
  title =        {Checking the $\mbox{Cox}$ model with cumulative sums of
martingale-based residuals.},
  journal =      {Biometrika},
  year =         {1993},
  volume =       {80},
  pages =        {557-572},
}


@Article{Little1995,
  author =       {Little, RJA},
  title =        {Modeling the drop-out mechanism in repeated measures
studies.},
  journal =      {Journal of the American Statistical Association},
  year =         {1995},
  volume =       {88},
  pages =        {125-134},
}


@Article{LonginiDattaHalloran1996,
  author =       {Longini, IM and Datta, S and Halloran, ME},
  title =        {Measuring vaccine efficacy for both susceptibility to
infection and reduction in infectiousness for prophylactic $\mbox{HIV}$-1 vaccines.},
  journal =      {Journal of Acquired Immune Deficiency Syndromes and
Human Retrovirology},
  year =         {1996},
  volume =       {13},
  pages =        {440-447},
}


@Book{LonginiHudgensHalloran2002,
  author =          {Longini, IM and Hudgens, MG and Halloran, ME},
  ALTeditor =          {E. Kaplan and R. Brookmeyer eds.},
  title =          {Estimation of vaccine efficacy for both
susceptibility to infection and reduction in infectiousness for
prophylactic $\mbox{HIV}$ vaccines with partner augmentation. In: The
Quantitative Evaluation of $\mbox{HIV}$ Prevention Programs..},
  publisher =          {Yale University Press},
  year =          {2002},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New Haven},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          { },
  OPTannote =          {}
}

 

@Article{LunnMcNeil1995,
  author =       {Lunn, M and McNeil, D},
  title =        {Applying $\mbox{Cox}$ regression to competing risks.},
  journal =      {Biometrics},
  year =         {1995},
  volume =       {51},
  pages =        {524-532},
}


@Article{LuoTurnbull1999,
  author =       {Luo, X and Turnbull, B},
  title =        {Comparing two treatments with multiple competing risks
endpoints.},
  journal =      {Statistica Sinica},
  year =         {1999},
  volume =       {9},
  pages =        {985-997},
}


@Article{Mani2002,
  author =       {Mani, I and Gilbert, Peter B and Sankale, J-L and Eisen, G and Mboup, S
and Kanki, PJ},
  title =        {Intrapatient diversity and its correlation with viral
setpoint in $\mbox{Human Immunodeficiency Virus Type 1}$ $\mbox{CRF02 A/G-IbNG}$ infection.},
  journal =      {Journal of Virology},
  year =         {2002},
  volume =       {76},
  pages =        {10745-10755},
}


@Article{McKeagueGilbertKanki2001,
  author =       {McKeague, I and Gilbert, Peter B and Kanki, P},
  title =        {Comparison of competing risks with adjustment for
covariate effects.},
  journal =      {Biometrics},
  year =         {2001},
  volume =       {57},
  pages =        {818-828},
}


@Article{McKeagueSun1996,
  author =       {McKeague, I and Sun, Y},
  title =        {Towards an omnibus distribution-free goodness-of-fit
test for the $\mbox{Cox}$ model.},
  journal =      {Statistica Sinica},
  year =         {1996},
  volume =       {6},
  pages =        {579-588},
}


@Article{Nabel2001,
  author =       {Nabel, GJ},
  title =        {Challenges and opportunities for development of an
$\mbox{AIDS}$  vaccine.},
  journal =      {Nature},
  year =         {2001},
  volume =       {410},
  pages =        {1002-1007},
}

@Article{Novitsky2001,
  author =       {Novitsky, V and Rybak, N and McLane, MF and Gilbert, Peter B and Chigwedere,
P and Klein, I and Gaolekwe, S and Chang, SY and Peter, T and Thior, I and Ndung'u, T and
Vannberg,
F and Foley, BT and Marlink, R and Lee, TH and Essex, M},
  title =        {Identification of human immunodeficiency virus type 1
subtype C $\mbox{Gag}$-, $\mbox{Tat}$-, $\mbox{Rev}$-, and $\mbox{Nef}$- specific $\mbox{Elispot}$-based $\mbox{CTL}$
responses for $\mbox{AIDS}$ vaccine design.},
  journal =      {Journal of Virology},
  year =         {2001},
  volume =       {75},
  pages =        {9210-9228},
}


@Article{Novitsky2002b,
  author =       {Novitsky, V and Cao, H and Rybak, N and Gilbert, Peter B and McLane, MF
and Gaolekwe, S and Peter, T and Thior, I and Ndung'u, T and Marlink, R and Lee, TH and
Essex, M},
  title =        {Magnitude and frequency of Cytotoxic $\mbox{T-lymphocyte}$
responses: Identification of immunodominant regions of Human
Immunodeficiency Virus Type 1 Subtype C.},
  journal =      {Journal of Virology},
  year =         {2002},
  volume =       {76},
  pages =        {10155-10168},
}


@Article{Rida1996,
  author =       {Rida, WN},
  title =        {Assessing the effect of $\mbox{HIV}$ vaccination on
infectiousness.},
  journal =      {Statistics in Medicine},
  year =         {1996},
  volume =       {15},
  pages =        {2393-2404},
}


@Article{RotnitzkyRobinsScharfstein1998,
  author =       {Rotnitzky, A and Robins, JM and Scharfstein, DO},
  title =        {Semiparametric regression for repeated outcomes with
nonignorable nonresponses.},
  journal =      {Journal of the American Statistical Association},
  year =         {1998},
  volume =       {93},
  pages =        {1321-1339},
}

@Article{ScharfsteinTsiatisGilbert1998,
  author =       {Scharfstein, DO and Tsiatis, AA and Gilbert, Peter B},
  title =        {Semiparametric efficient estimation in the generalized odds-rate class of regression models for right-censored time-to-event data.},
  journal =      {Lifetime Data Analysis},
  year =         {1998},
  volume =       {4},
  pages =        {355--391}
}


@Article{ZhangGilbert2010,
  author =       {Zhang, M and Gilbert, Peter B},
  title =        {Increasing the efficiency of prevention trials by incorporating baseline covariates.},
  journal =      {Statistical Communications in Infectious Diseases},
  year =         {2010},
  volume =       {2},
  pages =        {Iss. 1, Article 1},
  note={PMCID: PMC2997740}
}



@Article{Rowland-Jones1998,
  author =       {Rowland-Jones, SL and Dong, T and Fowke, KR and et al.},
  title =        {Cytotoxic $\mbox{T cell}$ responses to multiple conserved $\mbox{HIV}$
epitopes in $\mbox{HIV}$-resistant prostitutes in Nairobi.},
  journal =      {Journal of Clinical Investigation},
  year =         {1998},
  volume =       {102},
  pages =        {1758-1765},
}


@Article{Rubin1974,
  author =       {Rubin, DB},
  title =        {Estimating causal effects of treatments in randomized
and nonrandomized studies.},
  journal =      {Journal of Educational Psychology},
  year =         {1974},
  volume =       {66},
  pages =        {688-701},
}


@Article{Rubin1978,
  author =       {Rubin, DB},
  title =        {Bayesian inference for causal effects.},
  journal =      {Annals of Statistics},
  year =         {1978},
  volume =       {6},
  pages =        {34-58},
}


@Article{Sarr2000,
  author =       {Sarr, AD and Sankale, JL and Gueye-Ndiaye, A and Essex, M and Mboup, S
and Kanki, PJ},
  title =        {Genetic analysis of $\mbox{HIV}$ type 2 in monotypic and dual
$\mbox{HIV}$ infections.},
  journal =      {AIDS Research and Human Retroviruses},
  year =         {2000},
  volume =       {10:16},
  pages =        {295-298},
}


@Article{ScharfsteinRotnitzkyRobins1999,
  author =       {Scharfstein, DO and Rotnitzky, A and Robins, JM},
  title =        {Adjusting for nonignorable drop-out using
semiparametric nonresponse models.},
  journal =      {Journal of the American Statistical Association},
  year =         {1999},
  volume =       {94},
  pages =        {1096-1146},
}


@Article{SchickYu2000,
  author =       {Schick, A and Yu, Q},
  title =        {Consistency of the GMLE with mixed case
interval-censored data.},
  journal =      {Scandinavian Journal of Statistics},
  year =         {2000},
  volume =       {27},
  pages =        {45-55},
}


@Article{Shiver2002,
  author =       {Shiver, JW and Fu, TM and Chen, L and et al.},
  title =        {Replication-incompetent adenoviral vaccine vector
elicits effective anti-immunodeficiency virus immunity.},
  journal =      {Nature},
  year =         {2002},
  volume =       {415},
  pages =        {331-335},
}

%  Casimiro DR, Davies ME,
%Evans RK, Zhang ZQ, Simon AJ, Trigona WL, Dubey SA, Huang L, Harris VA,
%Long RS, Liang X, Handt L, Schleif WA, Zhu L, Freed DC, Persaud NV, Guan
%L, Punt KS, Tang A, Chen M, Wilson KA, Collins KB, Heidecker GJ,
%Fernandez VR, Perry HC, Joyce JG, Grimm KM, Cook JC, Keller PM, Kresock
%DS, Mach H, Troutman RD, Isopi LA, Williams DM, Xu Z, Bohannon KE,
%Volkin DB, Montefiori DC, Miura A, Krivulka GR, Lifton MA, Kuroda MJ,
%Schmitz JE, Letvin NL, Caulfield MJ, Bett AJ, Youil R, Kaslow DC, Emini EA



@Article{Sun2001,
  author =       {Sun, Y},
  title =        {Generalized nonparametric test procedures for
comparing multiple cause-specific hazard rates.},
  journal =      {Journal of Nonparametric Statistics},
  year =         {2001},
  volume =       {13},
  pages =        {171-207},
}

 

@Book{ SunTiwari1995,
  author =          {Sun, Y and Tiwari, RC},
  ALTeditor =          {H.L. Koul and J.V. Deshpand�, eds.},
  title =          { Comparing cause-specific hazard rates of a
competing risks model with censored data. IMS Lecture Notes-Monograph
Series },
  publisher =          {},
  year =          {1995},
  OPTkey =          {},
  OPTvolume =          {27},
 OPTnumber =          {},
 OPTseries =          {},
  address =          { },
  OPTedition =          { Analysis of Censored Data },
  OPTmonth =          {},
  OPTnote =          {255-270},
  OPTannote =          {}
}

 

@Article{SunTiwariZalkikar2001,
  author =       {Sun, Y and Tiwari, RC and Zalkikar, JN},
  title =        {Goodness-of-fit tests for multiplicative intensity
models with application to competing risks data.},
  journal =      {Scandinavian Journal of Statistics},
  year =         {2001},
  volume =       {28},
  pages =        {241-256},
}


@Article{Travers1995,
  author =       {Travers, K and Mboup, S and Marlink, R and Gueye-Nidaye, A and Siby, T
and Thior, I and Traore, I and Dieng-Sarr, A and Sankale, JL and Mullins, C and et al.},
  title =        {Natural protection against $\mbox{HIV}$-1 infection provided by
HIV-2.},
  journal =      {Science},
  year =         {1995},
  volume =       {268},
  pages =        {1612-1615},
}

@Article{Shapiroetal2006,
  author =       {Shapiro, RL and Thior, I and Gilbert, P and Lockman, S and Wester, C and Smeaton, LM and Stevens, L and
 Heymann, JS and Ndung�u, T and Gaseitswe, S and Novitsky, V and Makhema, J and Lagakos, S and Essex, M and the Mashi Study Team},
  title =        {Maternal single-dose nevirapine versus placebo as part of an antiretroviral strategy to prevent mother-to-child $\mbox{HIV}$ transmission in $\mbox{Botswana}$.},
  journal =      {AIDS},
  year =         {2006},
  volume =       {20},
  pages =        {1281--1288}
}

@Article{Thioretal2006,
  author =       {Thior, I and Lockman, S and Smeaton, L and Shapiro, RL and Wester, C and Heymann, JS and
 Gilbert, P and Stevens, L and Peter, T and Kim, S and van Widenfelt, E and Moffat, C and Ndase, P and Arimi, P and
 $\mbox{Pol}$oko, K and Mazonde, P and Makhema, J and McIntosh, K and Novitsky, V and Lee, T-H and Marlink, R and Lagakos, S and
 Essex, M and The Mashi Study Team},
  title =        {Breastfeeding plus 6 months of infant Zidovudine prophylaxis vs formula feeding plus infant Zidovudine for 1 month to reduce $\mbox{HIV}$ transmission in $\mbox{Botswana}$. A randomized trial: The Mashi Study.},
  journal =      {Journal of the American Medical Assocation},
  year =         {2006},
  volume =       {296},
  pages =        {794--805}
}

@Article{Rosenbaum1987,
  author =       {Rosenbaum, PR},
  title =        {Sensitivity analysis for certain permutation inferences in matched observational studies.},
  journal =      {Biometrika},
  year =         {1987},
  volume =       {74},
  pages =        {13--26}
}

@Article{Travers1998,
  author =       {Travers, K and Eisen, G and Marlink, R and Kanki, P and Mboup, S},
  title =        {Protection from $\mbox{HIV}$-1 infection by $\mbox{HIV}$-2.},
  journal =      {AIDS},
  year =         {1998},
  volume =       {12},
  pages =        {224-225},
}

@article{vanderLaanetal2007,
  title={Super learner},
  author={van der Laan, Mark J and Polley, Eric C and Hubbard, Alan E},
  journal={Statistical Applications in Genetics and Molecular Biology},
  year={2007},
  volume={6},
  pages={number 1}
}

@article{Wolpert1992,
  title={Stacked generalization},
  author={Wolpert, DH},
  journal={Neural Networks},
  year={1992},
  volume={5}, 
  number={2},
  pages={241--259}
}






@article{LedellPetersenvanderLaan2012,
  title={Computationally efficient confidence intervals for cross-validated
area under the ROC curve estimates.},
  author={LeDell, E and Petersen, ML and van der Laan, Mark J},
  journal={U.C. Berkely Division of
Biostatistics Working Paper Series},
  pages={Paper 304},
  year={2012}
}

@article{DudoitVanderLaan2005,
  title={Asymptotics of cross-validated risk estimation in estimator selection and performance assessment.},
  author={van der Laan, Mark J and Dudoit, S},
  year={2013},
  journal={Statistical Methodology},
  volume={2},
  pages={131--154}
}

@article{HubbardPajouhvanderLaan2016,
  title={Statistical inference for data adaptive target parameters},
  author={Hubbard, Alan E and Khered-Pajouh, S and van der Laan, Mark J},
  year={2016},
  journal={The International Journal of Biostatistics},
  volume={12},
  number={1},
  pages={3--19}
}



@book{vanderLaanRose2011,
  title={Targeted Learning: Causal Inference for Observational and Experimental Data},
  author={van der Laan, Mark J and Rose, Sherri},
  year={2011},
  publisher={Springer},
  address =          {New York}
}

@book{vanderLaanRose2018,
  title={Targeted Learning in Data Science: Causal Inference for Complex Longitudinal Studies},
  author={van der Laan, Mark J and Rose, Sherri},
  year={2018},
  publisher={Springer},
  address =          {New York}
}

@Book{VerbekeMolenberghs2000,
  author =          {Verbeke, G and Molenberghs, G},
  ALTeditor =          {},
  title =          { Linear mixed models for longitudinal data.},
  publisher =          {Springer},
  year =          {2000},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          { },
  OPTmonth =          {},
  OPTnote =          {255-270},
  OPTannote =          {}
}

@Book{Rosenbaum2010,
  author =          {Rosenbaum, PR},
  ALTeditor =          {},
  title =          {Design of Observational Studies.},
  publisher =          {Springer},
  year =          {2010},
  address =          {New York},
}




 

%Jim
@Article{WeiJohnson1985,
  author =       {Wei, LJ and Johnson, WE},
  title =        {Combining dependent tests with incomplete repeated
measurements.},
  journal =      {Biometrika},
  year =         {1985},
  volume =       {72},
  pages =        {359--364},
}

%Jim
@Article{PuttChinchilli2000,
  author =       {Putt, ME and Chinchilli, VM},
  title =        {A robust analysis of crossover designs using multisample generalized L-statistics.},
  journal =      {Journal of the American Statistical Association},
  year =         {2000},
  volume =       {95},
  pages =        {1256--1262},
}

%Jim
@Article{ChinchilliEsinhart1996,
  author =       {Chinchilli, VM and Esinhart, JD},
  title =        {Design and analysis of intra-subject variability in crossover experiments.},
  journal =      {Statistics in Medicine},
  year =         {1996},
  volume =       {15},
  pages =        {1619--1634},
}

@article{Juraskaetal2018,
  title={Viral genetic diversity and protective efficacy of a tetravalent dengue vaccine in two phase 3 trials},
  author={Juraska, Michal and Magaret, Craig A and Shao, Jason and Carpp, Lindsay N and Fiore-Gartland, Andrew J and Benkeser, David and Girerd-Chambaz, Yves and Langevin, Edith and Frago, Carina and Guy, Bruno and Jackson, Nicholas and Thi Hue, Kien Duong and Simmons, Cameron P and Edlefsen, Paul T and Gilbert, Peter B},
  journal={Proceedings of the National Academy of Sciences},
  volume={115},
  number={36},
  pages={E8378--E8387},
  year={2018},
  publisher={National Acad Sciences},
  note={PMCID:
    PMC6130398} 
}

%Jim
@Article{Keeleetal2008,
  author =       {Keele, BF and Giorgi, EE and Salazar-Gonzalez, JF and et al.},
  title =        {Identification and characterization of transmitted and early founder virus envelopes
in primary $\mbox{HIV-1}$ infection.},
  journal =      {Proceedings of the National Academy of Sciences},
  year =         {2008},
  volume =       {105},
  pages =        {7552--7557},
  note={PMCID: PMC2387184}
}



@Article{WHO-UNAIDS2001b,
  author =       {WHO-UNAIDS Report from a WHO-UNAIDS consultation,
Geneva, 2-3 October 2000},
  title =        {Future access to $\mbox{HIV}$ vaccines.},
  journal =      {AIDS},
  year =         {2001},
  volume =       {15},
  pages =        {W27-W24},
}

 

 

@Article{WestfallWolfinger1997,
  author =       {Westfall, PH and Wolfinger, RD},
  title =        {Multiple tests with discrete distributions.},
  journal =      {The American Statistician},
  year =         {1997},
  volume =       {51},
  pages =        {3-8},
}

 

 

@Article{WongYu1999,
  author =       {Wong, GYC and Yu, Q},
  title =        {Generalized MLE of a joint distribution function with
multivariate interval censored data.},
  journal =      {Journal of Multivariate Analysis},
  year =         {1999},
  volume =       {69},
  pages =        {155-166},
}

 

 

@Article{Yang1997,
  author =       {Yang, Z},
  title =        {PAML: a program package for phylogenetic analysis by
maximum likelihood.},
  journal =      {Computational Applied Biosciences},
  year =         {1997},
  volume =       {13},
  pages =        {555-556},
}


@Article{Yang2000,
  author =       {Yang, Z and Nielsen, R and Goldman, N and Pedersen, AM},
  title =        {Codon-substitution models for heterogenous selection
pressure at amino acid sites.},
  journal =      {Genetics},
  year =         {2000},
  volume =       {155},
  pages =        {431-449},
}


@Article{YuLiWong1998,
  author =       {Yu, Q and Li, L and Wong, GYC},
  title =        {Asymptotic variance of the GMLE of a survival function
with interval-censored data.},
  journal =      {Sankhy$\bar{a}$, Series A},
  year =         {1998},
  volume =       {60},
  pages =        {184-187},
}


@Article{Yusim2002,
  author =       {Yusim, K and Kesmir, C and Gaschen, B and Addo, MM and Altfeld, M
and Brunak, S and Chigaev, A and Detours, V and Korber, BT},
  title =        {Clustering patterns of cytotoxic T-lymphocyte epitopes
in human immunodeficiency virus type 1 (HIV-1) proteins reveal imprints
of immune evasion on $\mbox{HIV}$-1 global variation.},
  journal =      {Journal of Virology},
  year =         {2002},
  volume =       {76},
  pages =        {8757-8768}
}


@article{Subbarao2006,
author={Subbarao, S and Otten, R and Ramos, A and Jackson, E and 
Monsour, M and Bashirian, S and  Kim, C and
and Johnson, J and Soriano, V and Hudgens, MG and Butera, S and
Janssen, R and Paxton, L and Greenberg, A and Folks, T},
title={
Chemoprophylaxis with Tenofovir Disoproxil Fumarate provided
partial protection against Simian Human Immunodeficiency Virus infection in 
macaques given multiple virus challenges.}, 
journal={Journal of Infectious Diseases},
year={2006},
volume={194},
pages={904--911}
}



@Article{Klausner2003,
  author =          {Klausner, RD and Fauci, AS and Corey, L and Nabel, GJ and Gayle, H and Berkley, S and Haynes, BF and
 Baltimore, D and 
Collins, C and Douglas, RG and Esparza, J and Francis, DP and Ganguly, NK and Gerberding, JL and Johnston, MI and 
Kazatchkine, MD and McMichael, AJ and Makgoba, MP and Pantaleo, G and Piot, P and Shao, Y and Tramont, E and Varmus, V
and Wasserheit, JN},
  title =          {The need for a global $\mbox{HIV}$ vaccine enterprise.},
  journal =          {Science},
  year =          {2003},
  volume =          {300},
  pages =          {2036-2039}
}


@Book{Korber2003,
  author =          {Korber, B and Brander, C and Haynes, BF and Koup, R and Moore, GP eds.},
  title =          {$\mbox{HIV}$ Immunology and Database 2003},
  year =          {2003},
  publisher =  {Theoretical Biology and Biophysics Group, Los Alamos National Laboratory, Los Alamos, NM}
}


@Article{Prentice1986,
  author =          {Prentice, RL},
  title =          {A case-cohort design for epidemiologic cohort studies and disease prevention trials.},
  journal =          {Biometrika},
  year =          {1986},
  volume =          {73},
  pages =          {1-11}
}

@Article{Schoenfeld1981,
  author =          {Schoenfeld, D},
  title =          {The asymptotic properties of nonparametric tests for comparing survival distributions.},
  journal =          {Biometrika},
  year =          {1981},
  volume =          {68},
  pages =          {316--331}
}

@Article{Schoenfeld1982,
  author =          {Schoenfeld, D},
  title =          {Partial residuals for the proportional hazards regression model.},
  journal =          {Biometrika},
  year =          {1982},
  volume =          {69},
  pages =          {239--241}
}



@Article{SelfPrentice1988,
 author =          {Self, SG and Prentice, RL},
 title =          {Asymptotic distribution
 theory and efficiency results for case-cohort studies.},
 journal =          {Annals of Statistics},
 year =          {1988},
 volume =          {16},
 pages =          {64-81}
 }


@Article{Barlow1994,
 author =          {Barlow, WE},
 title =          {Robust variance estimation for the
 case-cohort design.},
 journal =          {Biometrics},
 year =          {1994},
 volume =          {50},
 pages =          {1064-1072}
 }

@Article{Barlowetal1999,
 author =          {Barlow, WE and Ichikawa, L and Rosber, D and Izumi, S},
 title =          {Analysis of case-cohort designs.},
 journal =          {Journal of Clinical Epidemiology},
 year =          {1999},
 volume =          {52},
 pages =          {1165-1172}
 }

@Article{CaiZheng2007,
 author =          {Cai, J and Zheng, D},
 title =          {Power calculation for case-cohort studies with nonrare events.},
 journal =          {Biometrics},
 year =          {2007},
 volume =          {63},
 pages =          {1288-1295}
 }

@Article{CaiZheng2004,
 author =          {Cai, J and Zheng, D},
 title =          {Sample size/Power calculation for case-cohort studies.},
 journal =          {Biometrics},
 year =          {2004},
 volume =          {60},
 pages =          {1015-1024}
 }

@Article{ChanBohidar1998,
 author =          {Chan, ISF and Bohidar, NR},
 title =          {Exact power and sample size for vaccine efficacy studies.},
 journal =          {Communications in Statistics, Theory and Methods},
 year =          {1998},
 volume =          {27},
 pages =          {1305-1322}
 }

@Article{SorensenAndersen2000,
 author =          {Sorensen, P and Andersen, PK},
 title =          {Competing risks
 analysis of the case-cohort design.},
 journal =          {Biometrika},
 year =          {2000},
 volume =          {87},
 pages =          {49-59}
 }

@Article{Borgan2000,
 author =          {Borgan, O and Langholz, B and Samuelsen, SO and Goldstein, L and
 Pogoda, J},
 title =          {Exposure stratified case-cohort designs.},
 journal =          {Lifetime Data Analysis},
 year =          {2000},
 volume =          {6},
 pages =          {39-58}
 }

@Article{BenichouGail1990,
 author =          {Benichou, J and Gail, MH},
 title =          {Estimates of absolute cause-specific
 risk in cohort studies.},
 journal =          {Biometrics},
 year =          {1990},
 volume =          {46},
 pages =          {813-826}
 }


@Article{Gilbertetal2005a,
 author =          {Gilbert, Peter B and Peterson, ML and Follmann, D and Hudgens, MG and
 Francis, DP and Gurwith, M and Heyward, WL and Jobes, DV and Popovic, V and Self, SG and
 Sinangil, F and Burke, D and Berman, PW.},
 title =          {Correlation between immunologic responses to a recombinant glycoprotein 120 
 vaccine and incidence of $\mbox{HIV}$-1 infection in a $\mbox{Phase 3}$ $\mbox{HIV}$-1 preventive vaccine trial.},
 journal =          {Journal of Infectious Diseases},
 year =          {2005},
 volume =          {191},
 pages =          {666-677}
 }

@Article{Gilbert2005ashort,
 author =          {Gilbert, Peter B and Peterson, ML and Follmann, D and et al.},
 title =          {Correlation between immunologic responses to a recombinant glycoprotein 120
 vaccine and incidence of $\mbox{HIV}$-1 infection in a $\mbox{Phase 3}$ $\mbox{HIV}$-1 preventive vaccine trial.},
 journal =          {Journal of Infectious Diseases},
 year =          {2005},
 volume =          {191},
 pages =          {666-677}
 }

@Article{DCCT2011,
 author =          {DCCT/EDIC RESEARCH GROUP},
 title =          {Intensive diabetes therapy and glomerular filtration rate in
type 1 diabetes.},
 journal =          {The New England Journal of Medicine},
 year =          {2011},
 volume =          {365},
 pages =          {2366--2376}
 }




@Article{Gilbertetal2005b,
 author =          {Gilbert, Peter B and Ackers, ML and Berman, PW and 
 Francis, DP and Popovic, V and Hu, DJ and Heyward, WL and 
 Sinangil, F and Shepherd, B and Gurwith, M.},
 title =          {$\mbox{HIV-1}$ virologic and immunologic progression and antiretroviral therapy initiation among 
HIV-1-infected participants
 in an efficacy trial of recombinant glycoprotein 120 vaccine.},
 journal =          {Journal of Infectious Diseases},
 year =          {2005},
 volume =          {192},
 pages =          {974-983}
 }

@Book{GilbertSun2004,
  author =          {Gilbert, Peter B and Sun, Y},
  ALTeditor =          {W.-Y. Tan and H. Wu},
  title =          {Simultaneous inferences of $\mbox{HIV}$ vaccine effects on viral load, $\mbox{CD4}$ cell count,
  and antiretroviral therapy initiation in $\mbox{Phase 3}$ trials.},
  booktitle = {Deterministic and Stochastic Models of $\mbox{HIV}$ with Intervention},
  publisher =          {},
  year =          {2004},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  OPTedition =          {}
}

@Book{ChanWangHeyse2004,
  author =          {Chan, ISF and Wang, WW and Heyse, JF},
  ALTeditor =          {},
  title =          {Exact power and sample size for vaccine efficacy studies.},
  booktitle = {Encyclopedia of Biopharmaceutical Statistics, 2nd Edition},
  publisher =          {Informa Healthcare},
  year =          {2004},
  pages = {1005-1022},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  OPTedition =          {}
}



@Article{Follmann2006,
 author =          {Follmann, D},
 title =          {Augmented designs to assess immune response in vaccine trials},
 journal =          {Biometrics},
 year =          {2006},
 volume = {62},
 pages = {1161-1169}
 }
 %note={PMCID:
 %   PMC2536776}
@Article{Chenetal1990,
 author =          {Chen, RT and Markowitz, LE and Albrecht, P and Stewart, JA and Mofenson, LM and Preblud, SR and Orenstein, WA},
 title =          {Measles antibody: reevaluation of protective titers.},
 journal =          {The Journal of Infectious Diseases},
 year =          {1990},
 volume = {162},
 pages = {1036-1042}
 }

@Article{GilbertGabrieletal2014,
 author =          {Gilbert, Peter B and Gabriel, E and Miao, X and Li, X and Su, S-C and Chan, ISF},
 title =          {Fold Rise in Antibody Titers by Measured by Glycoprotein-Based Enzyme-Linked Immunosorbent Assay Is an Excellent Correlate of Protection for a Herpes Zoster Vaccine, Demonstrated via the Vaccine Efficacy Curve},
 journal =          {The Journal of Infectious Diseases},
 year =          {2014},
 volume = {10},
 pages = {1573--1581},
 note={PMCID: PMC4215071}
 }

@Article{GilbertGabrielHuangChan2015,
 author =          {Gilbert, Peter B and Gabriel, E and Huang, Y and Chan, ISF}, 
 title =          {Surrogate endpoint evaluation: Principal
 stratification criteria and the {Prentice} definition},
 journal =          {Journal of Causal Inference},
 year =          {2015},
 volume = {3(2)},
 pages = {157--175},
 note={PMCID:
    PMC4692254}
 }



                                                                                                                     
@Article{Gilbert2003b,
 author =          {Gilbert, Peter B},
 title =          {Goodness-of-fit tests for semiparametric biased sampling models with application
 to $\mbox{AIDS}$ vaccine trials.},
 journal =          {Journal of Statistical Planning and Inference},
 year =          {2003},
 volume = {118},
 pages={51-81}
 }

@Book{KelesVanderLaanVulpe2004,
  author =          {Keles, S and Van der Laan, MJ and Vulpe, C},
  ALTeditor =          {},
  title =          {Regulatory motif finding by logic regression.},
  publisher =          {},
  year =          {2004},
  OPTkey =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {U.C. Berkeley Division of Biostatistics Working
Paper Series},
  OPTedition =          {Working Paper 145},
  OPTmonth =          {},
  OPTnote =          {http://www.bepress.com/ucbbiostat/paper145},
  OPTannote =          {}
}

@Article{ReschHoffmanSwanstrom2001,
  author =          {Resch, W and Hoffman, N and Swanstrom, R},
  title =          {Improved success of phenotype prediction of $\mbox{HIV}$-1 from
envelope variable loop 3 sequence using neutral networks.}, 
  journal =          {Virology},
  year =          {2001},
  volume =          {288},
  pages =          {51-62}
}

@Book{Shafer2000,
  author =          {Shafer, R},
  title =          {Stanford $\mbox{HIV}$ RT and Protease Sequence Database 1998-2000.},
  year =          {2000},
  publisher =  {Stanford University, Stanford, CA},
  OPTnote =          {http://hivdb.stanford.edu}
}

@Article{Gilbert2005,
  author =          {Gilbert, Peter B},
  title =          {A modified false discovery rate multiple comparisons procedure for discrete data,
applied to
$\mbox{HIV}$ genetics.},
  journal =          {Applied Statistics},
  year =          {2005},
  volume =          {54},
  pages =          {143-158}
}

@Article{Barouch2002,
  author =          {Barouch, DH and Kunstman, J and Kuroda, MJ and Schmitz, JE and Santra, S and Peyerl, FW and Krivulka, GR and Beaudry, K and Lifton, MA and Gorgone, DA and Montefiori, DC and Lewis, MG and Wolinsky, SM and Letvin, NL},
  title =          {Eventual $\mbox{AIDS}$ vaccine failure in a rhesus monkey by viral escape from cytotoxic T lymphocytes.},
  journal =          {Nature},
  year =          {2002},
  volume =          {415},
  pages =          {335-339}
}

@Article{Gray2001,
  author =          {Gray, RH and Wawer, MJ and Brookmeyer, R and Sewankambo, NK and Serwadda, D and Wabwire-Mangen, F and Lutalo, T and Li, X and vanCott, T and Quinn, TC and Rakai Project Team},
  title =          {Probability of $\mbox{HIV}$-1 transmission per coital act in monogamous, heterosexual, $\mbox{HIV}$-1-discordant couples in Rakai, Uganda.},
  journal =          {Lancet},
  year =          {2001},
  volume =          {357},
  pages =          {1149-1153}
}

@Article{Lyles2000,
  author =          {Lyles, RH and Munoz, A and Yamashita, TE and Bazmi, H and Detels, R and Rinaldo, CR and Margolick, JB and Phair, JP and Mellors, JW},
  title =          {Natural history of human immunodeficiency virus type 1 viremia after seroconversion and proximal to $\mbox{AIDS}$ in a large cohort of homosexual men. Multicenter $\mbox{AIDS}$ Cohort Study.},
  journal =          {Journal of Infectious Diseases},
  year =          {2000},
  volume =          {181},
  pages =          {872-880}
}

@Article{GilbertBoschHudgens2003,
  author =          {Gilbert, Peter B and Bosch, R and Hudgens, M},
  title =          {Sensitivity analysis for the
 assessment of vaccine effects on viral load
 in $\mbox{HIV}$ vaccine trials},
  journal =          {Biometrics},
  year =          {2003},
  volume =          {59},
  pages =          {531-541}
}

@Article{MehrotraLiGilbert2006,
  author =          {Mehrotra, DV and Li, X and Gilbert, Peter B},
  title =          {A comparison of eight methods for the dual-endpoint evaluation of efficacy in a proof-of-concept $\mbox{HIV}$ vaccine trial.},
  journal =          {Biometrics},
  year =          {2006},
  volume =        {62},
  pages =          {893-900}
}


@Article{Mehrotra2005,
  author =          {Mehrotra, D and Gilbert, Peter B and Li, X and Heyse, J and Self, S and Buchbinder, S and Robertson, M},
  title =          {A prototype efficacy
 trial design for establishing proof-of-concept of cell mediated immunity-based vaccines.},
  journal =          {},
  year =          {Submitted},
  pages =          {}
}

@Article{Neyman1923,
  author =          {Neyman, J},
  title =          {On the application of probability theory to agricultural experiments: Essay on principles.},
  journal =          {Statistical Science},
  year =          {1923},
  volume =          {5},
  pages =          {465-480}
}

@Article{Hughes1999,
  author =          {Hughes, JP},
  title =          {Mixed effects models with censored data with application to $\mbox{HIV}$ $\mbox{RNA}$ levels.},
  journal =          {Biometrics},
  year =          {1999},
  volume =          {55},
  pages =          {625-629}
}

@Article{Jemiaietal2007,
  author =          {Jemiai, Y and Rotnitzky, A and Shepherd, B and Gilbert, Peter B},
  title =          {Semiparametric estimation of treatment effects given base-line covariates on an outcome measured after a post-randomization event occurs},
  journal =          {Journal of the Royal Statistical
Society, Series B},
  year =          {2007},
  volume = {69},
  pages =          {879--902} 
}
%note={PMCID: PMC2837843}

@Article{HaynesPantaleoFauci1996,
  author =          {Haynes, BF and Pantaleo, G and Fauci, AS},
  title =          {Toward an understanding of the correlates of protective immunity to $\mbox{HIV}$ infection.},
  journal =          {Science},
  year =          {1996},
  volume =          {271},
  pages =          {324-328}
}

@Article{Prentice1989,
  author =          {Prentice, RL},
  title =          {Surrogate endpoints in clinical trials: definition and operational criteria},
  journal =          {Statistics in Medicine},
  year =          {1989},
  volume =          {8},
  pages =          {431-440}
}

@Article{LinFlemingDeGruttola1997,
  author =          {Lin, DY and Fleming, TR and De Gruttola, V},
  title =          {Estimating the proportion of treatment effect explained by a surrogate marker.},
  journal =          {Statistics in Medicine},
  year =          {1997},
  volume =          {16},
  pages =          {1515-1527}
}

@Article{FeinbergMoore2002,
  author =          {Feinberg, MB and Moore, JP},
  title =          {$\mbox{AIDS}$  vaccine models: challenging challenge viruses.},
  journal =          {Nature Medicine},
  year =          {2002},
  volume =          {8},
  pages =          {207-210}
}

@Article{Otten2005,
  author =          {Otten, RA and Adams, DR and Kim, CN and Jackson, E and Pullium, JK and Lee, K and Grohskopf, LA and Monsour, M and Butera, S and Folks, TM},
  title =          {Multiple vaginal exposures to low doses of R5 simian-human immunodeficiency virus: strategy to study $\mbox{HIV}$ preclinical interventions in nonhuman primates.},
  journal =          {Journal of Infectious Diseases},
  year =          {2005},
  volume =          {191},
  pages =          {164-173}
}

@Article{HudgensGilbertSelf2004,
  author =          {Hudgens, MG and Gilbert, Peter B and Self, SG},
  title =          {Endpoints in
 vaccine trials.},
  journal =          {Statistical Methods in Medical
 Research},
  year =          {2004},
  volume =          {13},
  pages =          {89-114}
}

@InProceedings{Choopanya2002,
  author =          {Choopanya, K and Tappero, J and Pitisuttithum, P and et al.},
  title =          {Ongoing follow-up of infecting drug users (IDUs) in the $\mbox{AIDSVAX}$ $\mbox{B/E}$ vaccine efficacy trial in Bangkok, Thailand.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {Fourteenth International $\mbox{AIDS}$ Conference},
  OPTeditor =          {},
  OPTvolume =          {},
  OPTnumber =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Barcelona, 2002},
  OPTpublisher = {},
  note =          {Abstract WeOrD1300.},
  OPTannote =          {}
}


@InProceedings{Francis2004,
  author =          {Francis, DP and Choopanya, K and Heyward, W and Gurwith, M and Gilbert, Peter B and Berman, PW},
  title =          {Comparison of two phase 3 trials support further study of $\mbox{AIDSVAX}$ $\mbox{B/B}$},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {AIDS Vaccine 2004 International Conference},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Lausanne, Switzerland, 2004},
  OPTpublisher = {},
  note =          {Abstract P260.},
  OPTannote =          {}
}

@InProceedings{deCamp2006JSM,
  author =          {deCamp, A and Gilbert, Peter B},
  title =          {Antigen scanning methods for identifying peptide signatures.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {Joint Statistical Meetings 2006},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Seattle, Washington, 2009},
  OPTpublisher = {},
  OPTannote =          {}
}

@InProceedings{GilbertCHAVI2007,
  author =          {Gilbert, Peter B and deCamp, A and Wang, Z and Magaret, C and Korber, BT and Haynes, B},
  title =          {Molecular signatures of acutely infecting viruses.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {Second International Conference on $\mbox{HIV}$ Transmission 2007},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Washington, DC 2007},
  OPTpublisher = {},
  OPTannote =          {}
}



@InProceedings{GilbertKeystone2009,
  author =          {Gilbert, Peter B},
  title =          {Leveraging baseline characteristics to improve $\mbox{HIV}$ prevention trials.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {Keystone Symposium on $\mbox{HIV}$ Prevention 2009},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Keystone, Colorado, 2009},
  OPTpublisher = {},
  OPTannote =          {}
}


@InProceedings{Janesetal2008,
  author =          {Janes, H and Mehrotra, D and Duerr, A and Gilbert, P and Buchbinder, S and Robertson, M and
Fitzgerald, D},
  title =          {Vaccine effects on $\mbox{HIV-1}$ progression in the Step study.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {AIDS Vaccine 2008 International Conference},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Cape Town, South Africa, 2008},
  OPTpublisher = {},
  OPTannote =          {}
}



@Article{JanesFrahmetal2013,
  author =          {Janes, HE and Friedrich, D and Krambrink, A and Smith, R and Kallas, E and Horton, H and
Casimiro, DR and Carrington, M and Geraghty, D and Gilbert, Peter B and McElrath, MJ and Frahm, N},
  title =          {Increased breadth of $\mbox{Gag-specific T-cell responses to MRKAd5/HIV
Gag/Pol/Nef}$ vaccination and protective {HLA} class {I} alleles are independently associated with reduced
viremia after {HIV} infection.},
  journal =          {Journal of Infectious Diseases, In Press},
  year =          {2013},
  OPTkey =          {},
  volume =          {},
  OPTnumber =          {},
  pages =          {}
}


@InProceedings{Gilbert2009HVTN,
  author =          {Gilbert, P and Rolland, M and deCamp, A and Margaret, C and Heath, L and 
Geraghty, D and McElrath, J and Mullins, J}, 
  title =          {Sieve analysis of Step $\mbox{HIV}$ sequences.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {Annual HVTN Meeting 2009},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Washington DC, May 2009},
  OPTpublisher = {},
  OPTannote =          {}
}

@Article{Rollandetal2009,
  author =          {Rolland, M and Tovanabutra, S and Gilbert, Peter B and Sanders-Buell, E and Heath, L and deCamp, AC and Magaret, C and Bose, M and Bradfield, A and O'Sullivan, A and Crossler, J and Jones, T and
Nau, M and Maust, BS and Deng, W and Zhao, H and Wong, K and Stoddard, JN and Raugi, DN and
Sorenson, S and Hural, J and Dubey, S and Frahm, N and Michael, NL and Shiver, J and
Corey, L and Li, F and Self, SG and Kim, J and Buchbinder, S and Casimiro, DR and Robertson, MN and McElrath, MJ and McCutchan, FE and Mullins, JI},
  title =          {Evidence for vaccine-induced changes in breakthrough $\mbox{HIV-1}$ strains from the $\mbox{Step}$ trial.},
  journal =          {Retrovirology},
  year =          {2009},
  volume =          {6, Suppl 3},
  pages =          {OA06-06 LB},
note={PMCID: PMC2767565}
}


@InProceedings{Hudgensetal2008AIDSVaccine,
  author =          {Hudgens, M and Gilbert, P and Wu, C-D and Barouch, D and Mascola, J and Self, S},
  title =          {Power to detect vaccine effects in repeated low-dose challenge experiments.},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {AIDS Vaccine 2008 International Conference},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Cape Town, South Africa, 2008},
  OPTpublisher = {},
  OPTannote =          {}
}


@Article{GilbertMcKeagueSun2004,
  author =          {Gilbert, Peter B and McKeague, I and Sun, Y},
  title =          {Tests for comparing mark-specific
hazards and cumulative
incidence functions.},
  journal =          {Lifetime Data Analysis},
  year =          {2004},
  volume =          {10},
  pages =          {5-28}
}

@article{hudgens2009,
author={M. G. Hudgens and P. B. Gilbert},
title={{Assessing vaccine effects
in repeated low-dose challenge experiments}},
journal={Biometrics},
volume={65},
pages={1223--1232},
year={2009},
note={PMCID: PMC2794923}
}


@Article{SunGilbertMcKeague2009,
  author =          {Sun, Y and Gilbert, Peter B and McKeague, I},
  title =          {Proportional hazards models with continuous marks.},
  journal =          {Annals of Statistics},
  year =          {2009},
  volume =          {37},
  pages =          {394--426},
note={PMCID: PMC2762218}
}

@article{vanderLaanPolley2007,
  title={Super learner},
  author={van der Laan, Mark J and Polley, Eric C and Hubbard, Alan E},
  journal={Statistical applications in genetics and molecular biology},
  volume={6},
  number={1},
  year={2007}
}

@article{EdlefsenRollandetal2015,
  title={Comprehensive Sieve Analysis of Breakthrough {HIV-1} Sequences in the {RV144} Vaccine Efficacy Trial.},
  author={Edlefsen, Paul T and Rolland, Morgane and Hertz, Tomer and Tovanabutra, Sodsai and Gartland, Andrew J and deCamp, Allan C and Magaret, Craig A and Ahmed, Hasan and Gottardo, Raphael and Juraska, Michal and McCoy, Connor and Larsen, Brendan B and Sanders-Buell, Eric and Carrico, Chris and Menis, Sergey and Bose, Meera and RV144 Sequencing Team, and Arroyo, Miguel A and O'Connell, Robert J and Nitayaphan, Sorachai and Pitisuttithum, Punnee and Kaewkungwal, Jaranit and Rerks-Ngarm, Supachai and Robb, Merlin L and Kirys, Tatsiana and Georgiev, Ivelin S and Kwong, Peter D and Scheffler, Konrad and Kosakovsky Pond, Sergei L and Carlson, Jonathan M and Michael, Nelson L and Schief, William R and Mullins, James I and Kim, Jerome H and Gilbert, Peter B},
  journal={PLoS Computational Biology},
  volume={11},
  number={2},
  pages={e1003973--e1003973},
  year={2015},
  publisher={Public Library of Science}
}

@Article{SunGilbert2012,
  author =          {Sun, Y and Gilbert, Peter B},
  title =          {Estimation of stratified mark-specific proportional hazards models with missing marks.},
  journal =          {Scandinavian Journal of Statistics},
  year =          {2012},
  volume =          {39},
  pages =          {34--52},
note={PMCID: PMC3601495}
}


@Article{GilbertMcKeagueSun2008,
  author =          {Gilbert, Peter B and McKeague, I and Sun, Y},
  title =          {The two-sample problem for failure rates depending on a continuous
mark: an application to vaccine efficacy.},
  journal =          {Biostatistics},
  year =          {2008},
  volume =          {9},
  pages =          {263--276}
}


@Article{HudgensSatten2002,
  author =          {Hudgens, MG and Satten, GA},
  title =          {Midrank unification of rank tests for exact, tied and interval
censored data.},
  journal =          {Journal of Nonparametric Statistics},
  year =          {2002},
  volume =          {14},
  pages =          {569-581}
}

@Article{HudgensMaathuisGilbert2007,
  author =          {Hudgens, MG and Maathuis, M and Gilbert, Peter B},
  title =          {Nonparametric estimation of the joint distribution of a survival time subject to interval censoring and a continuous mark variable.}, 
  journal =          {Biometrics},
  year =          {2007},
  volume = {63},
  pages =          {1152--1163}
}

@Article{HyunSunSundaram2009,
  author =          {Hyun, S and Sun, Y and Sundaram, R},
  title =          {Assessing cumulative incidence functions under the
semiparametric additive risk model.},
  journal =          {Statistics in Medicine},
  year =          {2009},
  volume = {22},
  pages =          {2748--2768},
  note={PMCID: PMC2773213}
}

  author =          {Hudgens, MG and Maathuis, M and Gilbert, Peter B},
  title =          {Nonparametric estimation of the joint distribution of a survival time subject to interval censoring and a continuous mark variable.}, 
  journal =          {Biometrics},
  year =          {2007},
  volume = {63},
  pages =          {1152--1163}



@Article{GilbertRossiniShankarappa2005,
  author =          {Gilbert, Peter B and Rossini, AJ and Shankarappa, R},
  title =          {Two-sample tests for comparing intra-individual genetic sequence diversity between populations.},
  journal =          {Biometrics},
  year =          {in press},
  pages =          {}
}


@Article{Nickleetal2007,
  author =          {Nickle, DC and Heath, L and Jensen, MA and Gilbert, Peter B and Mullins, JI and Pond, S},
  title =          {$\mbox{HIV}$-specific probabilistic models of protein evolution.},
  journal =          {PLoS One},
  year =          {2007},
  volume =          {2:e503},
  pages =          {},
  note={PMCID: PMC1876811}
}

@Article{CaiGilbertSelf2006,
  author =          {Cai, T and Gilbert, Peter B and Self, S},
  title =          {Joint inferences on vaccine efficacy against infection and disease, with application to the first $\mbox{HIV}$ vaccine efficacy trial.},
  journal =          {Journal of Biopharmaceutical Statistics},
  year =          {2006},
  volume =          {16},
  pages =          {517--538}
}

@Article{SunWu2003,
  author =          {Sun, Y and Wu, H},
  title =          {$\mbox{AUC}$-based tests for nonparametric functions with
longitudinal data.},
  journal =          {Statistica Sinica},
  year =          {2003},
  volume =          {13},
  pages =          {593-612}
}

@Article{SunWu2005,
  author =          {Sun, Y and Wu, H},
  title =          {Semiparametric time-varying coefficients
regression model for longitudinal data.},
  journal =          {Scandinavian Journal of
Statistics},
  year =          {2005},
  volume =          {32},
  pages =          {21-48}
}

@article{long2012comparing,
  title={Comparing competing risk outcomes within principal strata, with application to studies of mother-to-child transmission of HIV},
  author={Long, Dustin M and Hudgens, Michael G},
  journal={Statistics in Medicine},
  volume={31},
  number={27},
  pages={3406--3418},
  year={2012},
  publisher={Wiley Online Library},
  note={PMCID: PMC3494821}
}

@Article{BanerjeeMcKeague2004,
  author =          {Banerjee, M and McKeague, IW},
  title =          {Confidence sets for split points in decision trees.},
  journal =          {Annals of Statistics},
  year =          {under revision},
  volume =          {},
  pages =          {}
}


@Article{BuneaMcKeague2005,
  author =          {Bunea, F and McKeague, IW},
  title =          {Covariate selection for semiparametric hazard function regression
models.},
  journal =          {Journal of Multivariate Analysis},
  year =          {2005},
  volume =          {92},
  pages =          {186-204}
}

@Article{McKeagueZhao2004a,
  author =          {McKeague, IW and Zhao, Y},
  title =          {Width-scaled confidence bands for survival functions.},
  journal =          {Statistics and Probability Letters},
  year =          {in press},
  volume =          {},
  pages =          {}
}

@Article{McKeagueZhao2004b,
  author =          {McKeague, IW and Zhao, Y},
  title =          {Comparing distribution functions via empirical likelihood.},
  journal =          {Scandinavian Journal of Statistics},
  year =          {Submitted},
  volume =          {},
  pages =          {}
}

@Article{KalbfleischLawless1988,
  author =          {Kalbfleisch, JD and Lawless, JF},
  title =          {Likelihood
analysis of multi-state models for disease incidence and
mortality.}, 
  journal =          {Statistics in Medicine},
  year =          {1988},
  volume =          {7},
  pages =          {149-160}
}


@Article{ChickBarth-JonesKoopman2001,
  author =          {Chick, SE and Barth-Jones, D and Koopman, JS},
  title =          {Bias reduction for risk ratio and vaccine effect estimators.},
  journal =          {Statistics in Medicine},
  year =          {2001},
  volume =          {20},
  pages =          {1609-1624}
}


@Article{CaiSun2003,
  author =          {Cai, Z and Sun, Y},
  title =          { Local linear estimation for time-dependent coefficients in $\mbox{Cox}$'s
regression
models.},
  journal =          {Scandinavian Journal of Statistics},
  year =          {2003},
  volume =          {30},
  pages =          {93-111}
}

@Article{MaHuang2005,
  author =          {Ma, S and Huang, J},
  title =          {Regularized ROC estimation: With applications to disease classification
using microarray data.},
  journal =          {},
  year =          {Submitted},
  volume =          {},
  pages =          {}
}

@Article{HeagertyLumleyPepe2000,
  author =          {Heagerty, PJ and Lumley, T and Pepe, M},
  title =          {Time-dependent ROC curves for censored survival data and a di
agnostic marker.},
  journal =          {Biometrics},
  year =          {2000},
  volume =          {56},
  pages =          {337-344}
}

@Article{ShepherdGilbertLumley2007,
  author =          {Shepherd, BE and Gilbert, Peter B and Lumley, T},
  title =          {Sensitivity analyses comparing time-to-event outcomes only existing in a subset selected post-randomization, conditional on covariates, with application to $\mbox{HIV}$ vaccine trials.},
  journal =          {Journal of the American Statistical Association},
  year =          {2007},
  volume =          {102},
  pages =          {573--582},
  note={PMCID: PMC2613336}
}

@Article{ShepherdGilbertDupont2011,
  author =          {Shepherd, BE and Gilbert, Peter B and Dupont, CT},
  title =          {Sensitivity analyses for comparing time-to-event outcomes only existing in a subset selected postrandomization and relaxing monotonicity},
  journal =          {Biometrics},
  year =          {2011},
  volume =          {67},
  pages =          {1100--1110}
}
%  note={PMCID: PMC3116075}

@Article{ChenTsiatis2001,
  author =          {Chen, PY and Tsiatis AA},
  title =          {Causal inference on the difference of the restricted
mean lifetime between two groups.},
  journal =          {Biometrics},
  year =          {2001},
  volume =          {57},
  pages =          {1030-1038}
}

@Article{Stute1995,
  author =          {Stute, W},
  title =          {The central limit theorem under random censorship.},
  journal =          {Annals of Statistics},
  year =          {1995},
  volume =          {23},
  pages =          {422-439}
}


@Article{RobinsRotnitzkyZhao1994,
  author =          {Robins, JM and Rotnitzky, A and Zhao, LP},
  title =          {Estimation of regression-coefficients when some regressors are not always observed},
  journal =          {Journal of the American Statistical Association},
  year =          {1994},
  volume =          {89},
  pages =          {846-866}
}

@Article{RobinsRotnitzkyZhao1995,
  author =          {Robins, JM and Rotnitzky, A and Zhao, LP},
  title =          {Analysis of semiparametric
regression models for repeated outcomes in the presence of missing data.},
  journal =          {Journal of the American Statistical Association},
  year =          {1995},
  volume =          {90},
  pages =          {106-121}
}

%Jim
@Article{ZhangTsiatisDavidian2008,
  author =          {Zhang, M and Tsiatis, AA and Davidian, M},
  title =          {Improving efficiency of inferences in randomized clinical trials using auxiliary covariates},
  journal =          {Biometrics},
  year =          {2008},
  volume =          {64},
  pages =          {707--715}}

@Article{TsiatisDavidianZhangLu2008,
  author =          {Tsiatis, AA and Davidian, M and Zhang, M and Lu, X},
  title =          {Covariate adjustment for two-sample treatment comparisons in randomized clinical trials.},
  journal =          {Statistics in Medicine},
  year =          {2008},
  volume =          {27},
  pages =          {4658--4677}
}

@Article{Pococketal2002,
  author =          {Pocock, SJ and Assmann, SE and Enos, LE and Kasten, LE},
  title =          {Subgroup analysis, covariate adjustment and baseline comparisons in clinical trial
reporting: current practice and problems},
  journal =          {Statistics in Medicine},
  year =          {2002},
  volume =          {21},
  pages =          {2917--2930}
}

@Article{CaoTsiatisDavidian2008,
  author =          {Cao, W and Tsiatis, AA and Davidian, M},
  title =          {Improving efficiency and robustness of the doubly robust estimator for a population mean with incomplete data.},
  journal =          {Biometrika},
  year =          {2008},
  volume =          {94},
  pages =          {1--18},
  note={PMCID: PMC2798744}
}




@Book{LittleRubin2002,
  author =          {Little, RJA and Rubin, DB},
  ALTeditor =          {},
  title =          {Statistical Analysis with Missing Data, Second Edition},
  publisher =          {Wiley},
  year =          {2002},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Book{Rubin1987,
  author =          {Rubin, DB},
  ALTeditor =          {},
  title =          {Multiple Imputation for Nonresponse in Surveys},
  publisher =          {Wiley, New York},
  year =          {1987},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Book{BreslowDay1980,
  author =          {Breslow, NE and Day, NE},
  ALTeditor =          {},
  title =          {Statistical Methods in Cancer Research, Volume 1},
  publisher =          {International Agency for Research on Cancer},
  year =          {1980},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {Lyon, France},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Book{KalbfleischPrentice2002,
  author =          {Kalbfleisch, JD and Prentice, RL},
  ALTeditor =          {},
  title =          {The Statistical Analysis of Failure Time
Data, Second Edition.},
  publisher =          {John Wiley and Sons},
  year =          {2002},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Article{Hengetal2019,
  author =          {Heng, F and Sun, Y and Hyun, S and Gilbert, PB},
  title =          {Analysis of the time-varying Cox model for cause-specific hazard functions with missing causes},
  journal =          {},
  year =          {Submitted},
  volume =          {},
  pages =          {}
}

@Article{ChengGuessHeyse1994,
  author =          {Chang, MN and Guess, HA and Heyse, JF},
  title =          {Reduction in the burden of illness: a new efficacy measure for prevention trials.},
  journal =          {Statistics in Medicine},
  year =          {1994},
  volume =          {13},
  pages =          {1807-1814}
}

@Article{ChengWeiYing1995,
  author =          {Cheng, SC and Wei, LJ and Ying, Z},
  title =          {Analysis of transformation models with censored data.},
  journal =          {Biometrika},
  year =          {1995},
  volume =          {83},
  pages =          {835--846}
}

@Article{FineYingWei1998,
  author =          {Fine, JP and Ying, Z and Wei, LJ},
  title =          {On the linear transformation model with censored data.},
  journal =          {Biometrika},
  year =          {1998},
  volume =          {85},
  pages =          {980--986}
}

@Article{ChengWeiYing1997,
  author =          {Cheng, SC and Wei, LJ and Ying, Z},
  title =          {Predicting survival probabilities with semiparametric transformation models.},
  journal =          {Journal of the American Statistical Association},
  year =          {1997},
  volume =          {92},
  pages =          {227--235}
}

@Article{EfronFeldman1991,
  author =          {Efron, B and Feldman, D},
  title =          {Compliance as an explanatory variable
in clinical trials.},
  journal =          {Journal of the American Statistical Association},
  year =          {1991},
  volume =          {86},
  pages =          {9-26}
}

@Article{ChatterjeeChenBreslow2003,
  author =          {Chatterjee, N and Chen, Y-H and Breslow, NE},
  title =          {A pseudoscore estimator for regression problems
with two-phase sampling.},
  journal =          {Journal of the American Statistical Association},
  year =          {2003},
  volume =          {98},
  pages =          {158-167}
}

@Book{Carroll1995,
  author =          {Carroll, RJ},
  ALTeditor =          {},
  title =          {Measurement Error in Nonlinear Models},
  publisher =          {Chapman \& Hall},
  year =          {1995},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {London},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}

@Article{CarrollWand1991,
  author =          {Carroll, RJ and Wand, MP},
  title =          {Semiparametric estimation in logistic measurement
error models. },
  journal =          {Journal of the Royal Statistical Society, Series B},
  year =          {1991},
  volume =          {53},
  pages =          {573-585}
}

@Article{BreslowMcNenyWellner2003,
  author =          {Breslow, NE and McNeney, B and Wellner, JA},
  title =          {Large sample theory for semiparametric
regression models with two-phase, outcome-dependent sampling.},
  journal =          {Annals of Statistics},
  year =          {2003},
  volume =          {31},
  pages =          {1110-1139}
}

@Article{HuangWang2001,
  author =          {Huang, Y and Wang, CY},
  title =          {Consistent functional methods for logistic regression
with errors in covariates.},
  journal =          {Journal of the American Statistical Association},
  year =          {2001},
  volume =          {96},
  pages =          {1469-1482}
}

@Article{HuangGilbertJanes2012,
  author =          {Huang, Y and Gilbert, Peter B and Janes, H},
  title =          {Assessing treatment-selection markers using a potential outcomes framework.},
  journal =          {Biometrics},
  year =          {2012},
  volume =          {68},
  pages =          {687--696} 
}
%note={PMCID: PMC3417090}

@Article{RhodesHalloranLongini1996,
  author =          {Rhodes, PH and Halloran, ME and Longini, IM},
  title =          {Counting
process models for infectious disease data: distinguishing exposure to infection from susceptibility.},
  journal =          {Journal of the Royal Statistical Society, Series B},
  year =          {1996},
  volume =          {58},
  pages =          {751-762}
}

@Article{Ellenberger2006,
  author =          {Ellenberger, D and Otten, RA and Li, B and Rodriguez, V and Sariol, CA and
Martinez, M and Monsour, M and Wyatt, L and Hudgens, MG and Kraiselburd, E and
Moss, B and Robinson, H and Folks, T and Butera, S},
  title =          {Repeated
mucosal $\mbox{SHIV}$ challenges of macaques after $\mbox{HIV}$-1 $\mbox{DNA/MVA}$ vaccination provides evidence of
protection for systemic infection consistent with a leaky vaccine effect.},
  journal =          {Virology},
  year =          {2006},
  volume =          {352},
  pages =          {216--225}
}

@Article{FoulkesDeGruttola2003,
  author =          {Foulkes, AS and DeGruttola, V},
  title =          {Characterizing the progression of viral mutations over time.},
  journal =         {Journal of the American Statistical Association},
  year =          {2003},
  volume =          {98},
  pages =          {859-867}
}


@Article{LonginiHalloran1996,
  author =          {Longini, IM and Halloran, ME},
  title =          {A frailty mixture model for estimating
vaccine efficacy.},
  journal =         {Applied Statistics},
  year =          {1996},
  volume =          {45},
  pages =          {165-173}
}

@Article{MaKosorokFine2005,
  author =          {Ma, S and Kosorok, MR and Fine, JP},
  title =          {Additive risk models for survival data with high dimensional covariates.},
  journal =         {Biometrics},
  year =          {in press},
  volume =          {},
  pages =          {}
}

@Article{LedoitWolf2004,
  author =          {Ledoit, O and Wolf, M},
  title =          {A well-conditioned estimator for large-dimensional covariance matrices.},
  journal =         {Journal of Multivariate Analysis},
  year =          {2004},
  volume =          {88},
  pages =          {365-411}
}


@Article{Alonso2006,
  author =          {Alonso, A and Molenberghs, G and Geys, H and Buyse, M and Vangeneugden, T},
  title =          {A unifying approach for surrogate marker validation based on $\mbox{P}$rentice's criteria.},
  journal =         {Statistics in Medicine},
  year =          {2006},
  volume =          {25},
  pages =          {205-221}
}

@Article{LiMeredithHoseyni2001,
  author =          {Li, Z and Meredith, MP and Hoseyni, MS},
  title =          {A method to assess the proportion of treatment effect explained by a surrogate endpoint.},
  journal =         {Statistics in Medicine},
  year =          {2001},
  volume =          {20},
  pages =          {3175-3188}
}

@Article{Rubin1986,
  author =          {Rubin, DB},
  title =          {Statistics and causal inference: which ifs have causal
answers.},
  journal =         {Journal of the American Statistical Association},
  year =          {1986},
  volume =          {81},
  pages =          {961-962}
}

@Article{Qinetal2007,
  author =          {Qin, L and Gilbert, Peter B and Corey, L and McElrath, J and Self, SG},
  title =          {A framework for assessing immunological correlates of protection in vaccine trials.},
  journal =         {The Journal of Infectious Diseases},
  year =          {2007},
  volume =          {196},
  pages =          {1304--1312}
}

@Article{Qin1998,
  author =          {Qin, J},
  title =          {Inferences for case-control and semiparametric two-sample density ratio models.},
  journal =         {Biometrika},
  year =          {1998},
  volume =          {85},
  pages =          {619--630}
}

@Article{Zhang2000,
  author =          {Zhang, B},
  title =          {A goodness-of-fit test for multiplicative-intercept risk models based on case-control data.},
  journal =         {Statistica Sinica},
  year =          {2000},
  volume =          {10},
  pages =          {839--865}
}




@Article{HuangPepeFeng2007,
  author =          {Huang, Y and Pepe, MS and Feng, Z},
  title =          {Evaluating the predictiveness of a continuous marker.},
  journal =         {Biometrics},
  year =          {2007},
  volume =          {63},
  pages = {1181--1188},
  note={PMCID: PMC3059154}
}

@Article{PepeEtal2008,
  author =          {Pepe, MS and Feng, Z and Janes, H and Bossuyt, PM and Potter, JD}, 
  title =          {Pivotal evaluation of the accuracy of a biomarker used for classification
or prediction: Standards for study design.},
  journal =         {Journal of the National Cancer Institute},
  year =          {2008},
  volume =          {100},
  pages = {1432--1438},
  note={PMCID: PMC2567415}


}


@Article{HoffmanSenWeinberg2001,
  author =          {Hoffman, EB and Sen, PK and Weinberg, CR},
  title =          {Within-cluster resampling.},
  journal =         {Biometrika}, 
  year =          {2011},
  volume =          {88},
  pages = {1121--1134}
}


@Article{GilbertJin2010,
  author =          {Gilbert, Peter B and Jin, Y},
  title =          {Semiparametric estimation of the average causal effect of treatment on an outcome measured after a post-randomization event, with missing outcome data.},
  journal =         {Biostatistics},
  year =          {2010},
  volume =          {11},
  pages = {34--47},
  note={PMCID: PMC2800161}
}


@Article{HuangPepe2009,
  author =          {Huang, Y and Pepe, MS},
  title =          {Biomarker evaluation and comparison using the controls as a reference population.},
  journal =         {Biostatistics},
  year =          {2009},
  volume =          {10},
  pages = {228--244},
  note={PMCID: PMC2648906}
}

@Article{BuraAndGastwirth2001,
  author =          {Bura, R and Gastwirth, JL},
  title =          {The binary regression quantile plot: Assessing the importance of predictors in binary regression visually.},
  journal =         {Biometrical Journal},
  year =          {2001},
  volume =          {43},
  pages = {5--21}
}




@Article{Pasquettoetal2005,
  author =          {Pasquetto, V and Bui, HH and Giannino, R and Banh, C and Mirza, F and Sidney, J and Oseroff, C and Tscharke, DC and Irvine, K and
Bennink, JR et al.},
  title =          {$\mbox{HLA-A* HLA-A*1101, and HLA-B*0702}$ transgenic mice recognize numerous poxvirus determinants from a wide variety of viral
gene products.},
  journal =         {Journal of Immunology},
  year =          {2005},
  volume =          {175},
  pages = {5504--5515}
}

@Article{Francoetal2000,
  author =          {Franco, A and Tilly, DA and Gramaglia, I and Croft, M and Cipolla, L and Meidal, M and Grey, HM},
  title =          {Epitope affinity for $\mbox{MHC}$ class $\mbox{I}$ determines helper requirement for $\mbox{CTL}$ priming.},
  journal =         {Nature Immunology},
  year =          {2000},
  volume =          {1},
  pages = {145--150}
}

@Article{GrambschTherneau1994,
  author =          {Grambsch, P and Therneau, T},
  title =          {Proportional hazards tests and
     diagnostics based on weighted residuals.},
  journal =         {Biometrika},
  year =          {1994},
  volume =          {81},
  pages = {515--526}
}

@Article{Louzounetal2006,
  author =          {Louzoun, Y and Vider, T and Weigert, M},
  title =          {$\mbox{T-cell}$ epitope repertoire as predicted from human and viral genomes.},
  journal =         {Molecular Immunology},
  year =          {2006},
  volume =          {43},
  pages = {559--569}
}

@Article{Robinsonetal2006,
  author =          {Robinson, J and Waller, MJ and Fail, SC and Marsh, SG},
  title =          {The $\mbox{IMGT}$\/$\mbox{HLA}$ and $\mbox{IPD}$ databases.},
  journal =         {Human Mutation},
  year =          {2006},
  volume =          {27},
  pages = {1192--1199}
}


@Article{ColeFrangakis2009,
   Author="Cole, S. R.  and Frangakis, C. E. ",
   Title="{{T}he consistency statement in causal inference: a definition or an assumption?}",
   Journal="Epidemiology",
   Year="2009",
   Volume="20",
   Pages="3--5",
   Month="Jan"
}


@Article{Pearl2011,
  author =          {Pearl, J},
  title =          {Principal stratification-- a goal or a tool?},
  journal =         {The International Journal of Biostatistics},
  year =          {2011},
  volume =          {7},
  pages = {Article 20} 
}
%note={PMCID: PMC3083139}

@Article{GilbertHudgensWolfson2011,
  author =          {Gilbert, Peter B and Hudgens, MG and Wolfson, J},
  title =          {Commentary on ``$\mbox{Principal}$ stratification-- a goal or a tool?" by $\mbox{Judea Pearl}$},
  journal =         {The International Journal of Biostatistics},
  year =          {2011},
  volume =          {7},
  pages = {Article 1}
}
%note={PMCID: PMC3204668}

@Article{Levinetal2013,
  author =          {Levin, MJ and Schmader, KE and Gnann, JW and McNeil, SA and Vesikari, T and Betts, RF and
Keay, S and Stek, JE and Bundick, ND and Su, S-C and Zhao, Y and Li, X and Chan, IS and Annunziato, PW and Parrino, J},
  title =          {Varicella-Zoster Virus-Specific Antibody Responses in 50--59-Year-Old Recipients of Zoster Vaccine}, 
  journal =         {Journal of Infectious Diseases},
  year =          {2013},
  volume =          {},
  pages = {},
  note={PMCID: (in process)}
}


@Article{Robbetal2012,
  author =          {Robb, ML and Rerks-Ngarm,S and Nitayaphani, S and Pitisuttithum, P and Kaewkungwal, J and Kunasol, P and
 Khamboonruang, C and Thongcharoen, P and Morgan, P and Benenson, M and Paris, RM and Chiu, J and Adams, E and Francis, D and
 Gurunathan, S and Tartaglia, J and Gilbert, Peter B and Stablein, D and Michael, NL and Kim, JH},
  title =          {Risk behaviour and time as covariates for efficacy of the {HIV} vaccine regimen {ALVAC-HIV (vCP1521) and AIDSVAX B/E}: a post-hoc analysis of the {T}hai phase 3 efficacy trial {RV144}.},
  journal =         {Lancet Infectious Diseases},
  year =          {2012},
  volume =          {12},
  pages = {531--537},
note={PMCID: PMC3530398}}
%

@Article{Robbetal2012short,
  author =          {Robb, ML and Rerks-Ngarm,S and Nitayaphani, S and et al.},
  title =          {Risk behaviour and time as covariates for efficacy of the {HIV} vaccine regimen {ALVAC-HIV (vCP1521) and AIDSVAX B/E}: a post-hoc analysis of the Thai phase 3 efficacy trial {RV144}.},
  journal =         {Lancet Infectious Diseases},
  year =          {2012},
  volume =          {12},
  pages = {531--537}
}
%note={PMCID: PMC3530398}




@Article{HuangGilbertWolfson2013,
  author =          {Huang, Y and Gilbert, Peter B and Wolfson, J},
  title =          {Design and estimation for evaluating principal surrogate markers in vaccine trials},
  journal =         {Biometrics},
  year =          {2013},
  volume =          {69},
  pages = {301--309}
}
%note={PMCID: PMC3713795}

@Article{GabrielGilbert2014,
  author =          {Gabriel, E and Gilbert, Peter B},
  title =          {Evaluating principal surrogate endpoints with time-to-event data accounting for time-varying treatment efficacy.},
  journal =         {Biostatistics},
  year =          {2014},
  volume =          {15},
  pages = {251--265},
  note={PMCID:
    PMC3944974}
}


@Article{PlotkinGilbert2012,
  author =          {Plotkin, SA and Gilbert, Peter B},
  title =          {Nomenclature for immune correlates of protection after vaccination},
  journal =         {Clinical Infectious Diseases},
  year =          {2012},
  volume =          {54},
  pages = {1615--1617},
  note={PMCID: PMC3348952}
}
%note=

@Article{Robins1986,
  author =          {Robins, JM},
  title =          {A new approach to causal inference in mortality studies
with sustained exposure periods - Application to control of the healthy worker
survivor effect.},
  journal =         {Mathematical Modeling},
  year =          {1986},
  volume =          {7},
  pages = {1393--1512}
}





@Article{HuangZhang2008,
  author =          {Huang, X and Zhang, N},
  title =          {Regression survival analysis with an assumed copula for dependent censoring:
A sensitivity analysis.},
  journal =         {Biometrics},
  year =          {2008},
  volume =          {64},
  pages = {1090--1099}
}

@Article{Houghgaard1986,
  author =          {Houghgaard, P},
  title =          {A class of multivariate failure time distributions.},
  journal =         {Biometrika},
  year =          {1986},
  volume =          {73},
  pages = {671--678}
}

@Article{Frank1979,
  author =          {Frank, MJ},
  title =          {On the simultaneous association of $F(x,y)$ and $x+y-F(x,y)$.},
  journal =         {Aequationes Mathematics},
  year =          {1979},
  volume =          {21},
  pages = {37--38}
}

@Article{Clayton1978,
  author =          {Clayton, DG},
  title =          {A model for association in bivariate life tables and its application in epidemiological
studies of familial tendency in chronic disease incidence.},
  journal =         {Biometrika},
  year =          {1978},
  volume =          {65},
  pages = {141--151}
}

@Article{Petersetal2006,
  author =          {Peters, B and Bui, H-H and Frankild, S and Nielsen, M and Lundegaard, C and Kostem, E and
Basch, D and Lamberth, K and Harndahl, M and Fleri, W and Wilson, SS and Sidney, J and
Lund, O and Buus, S and Sette, A},
  title =          {A community resource benchmarking predictions of peptide binding to $\mbox{MHC}$-I molecules.},
  journal =         {PLoS Computational Biology},
  year =          {2006},
  volume =          {2},
  pages = {e65}
}

@Article{Korberetal2006,
  author =          {Korber, B and LaBute, M and Yusim, K},
  title =          {Immunoinformatics comes of age.},
  journal =         {PLoS Computational Biology},
  year =          {2006},
  volume =          {2},
  pages = {e71}
}

@Article{PetrovskyBrusic2002,
  author =          {Petrovsky, B and Brusic, V},
  title =          {Computational immunology: The coming of age.},
  journal =         {Immunology and Cell Biology},
  year =          {2002},
  volume =          {80},
  pages = {248--254}
}


@article{Zhu2006,
author = {Zhu, M and Ghodsi, A},
title = {Atomatic dimensionality selection from the scree plot via the use of profile likelihood},
journal = {Computational Statistics and Data Analysis},
volume = {51},
pages = {918--930},
year = {2006},
}

@article{Ramsay1982,
author = {Ramsay, JO},
title = {Some statistical approaches to multidimensional scaling data},
journal = {Journal of the Royal Statistical Society. Series A (General)},
volume = {145},
pages = {285--312},
year = {1982},
}

@article{Groenen2006,
author = {Groenen, PJF and Winsberg, S and Rodriguez, O and Diday, E},
title = {I-Scal: multidimensional scaling of interval dissimilarities},
journal = {Computational Statistics and Data Analysis},
volume = {51},
pages = {360--378},
year = {2006},
}

@article{Groenen1997,
author = {Groenen, PJF and Heiser, WJ and Meulman, JJ},
title = {Global optimization in least squares multidimensional scaling by distance smoothing},
journal = {},
volume = {},
pages = {},
year = {1997},
}

@article{Herden2005,
author = {Herden, G and Pallack, A},
title = {Adequateness and interpretability of objective functions in ordinal data analysis},
journal = {Journal of Multiviariate Analysis},
volume = {94},
pages = {19--69},
year = {2005},
}

@article{Groenen1996,
author = {Groenen, PJF and Heiser, WJ},
title = {The tunneling method for global optimization in multidimensional scaling},
journal = {Psychometrika},
volume = {61},
pages = {529--550},
year = {1996},
}

@article{DeSarbo2008,
author = {DeSarbo, WS and Park, J and Scott, CJ},
title = {A model-based approach for visualizing the dimensional structure of ordered successive categories preference data},
journal = {Psychometrika},
volume = {73},
pages = {1--20},
year = {2008},
}

@article{Ramsay1977,
author = {Ramsay, JO},
title = {Maximum likelihood estimation in multidimensional scaling},
journal = {Psychometrika},
volume = {42},
pages = {241--266},
year = {1977},
}



@article{Graef1979,
author = {Graef, J and Spence, I},
title = {Using distance information in the design of large multidimensional scaling experiments},
journal = {Psychological Bulletin},
volume = {86},
pages = {60--66},
year = {1979},
}


@article{Guttman1968,
author = {Guttman, L},
title = {A general nometric technique for finding the smallest coordinate space for a configuration of points},
journal = {Psychometrika},
volume = {33},
pages = {469--504},
year = {1968},
}


@article{Spence1974,
author = {Spence, I and Domensy, DW},
title = {Single subject incomplete designs for nonmetric multidimensional scaling},
journal = {Psychometrika},
volume = {39},
pages = {469--490},
year = {1974},
}



@article{Winsberg2002,
author = {Winsberg, S and De Soete, G},
title = {A bootstrap procedure for mixture models: {A}pplied to multidimensional scaling laten class models},
journal = {Applied stochastic models in business and industry},
volume = {18},
pages = {391--406},
year = {2002},
}

@article{DeSarbo1997,
author = {DeSarbo, WS and Young, MR and Rangaswamy, A},
title = {A parametric multidimensional unfolding procedure for incomplete nonmetric preference/choice set data in markerting research},
journal = {Journal of Marketing Research},
volume = {34},
pages = {499--516},
year = {1997},
}

@article{Bijmolt1999,
author = {Bijmolt, THA and Wedel, M},
title = {A comparison of multidimensional scaling methods for perceptual mapping},
journal = {Journal of Marketing Research},
volume = {36},
pages = {277--285},
year = {1999},
}



@article{Groenen1995,
author = {Groenen, PJF and Mathar, R},
title = {The majorization approach to multidimensional scaling for {M}inkowski distances},
journal = {Journal of Classification},
volume = {12},
pages = {3--19},
year = {1995},
}

@article{Groenen1999,
author = {Groenen, PJF and Heiser, WJ and Meulman, JJ},
title = {Global optimization in least-squares multidimensional scaling by distance smoothing},
journal = {Journal of Classification},
volume = {16},
pages = {225--254},
year = {1999},
}

@article{Smith2004,
author = {Smith, DJ and Lapedes, AS and de Jong, JC and Bestebroer, TM and Rimmelzwaan, GF and Osterhaus, ADME and Fouchier, RAM},
title = {Mapping the antigenic and genetic evolution of influenza virus},
journal = {Science},
volume = {305},
pages = {371--376},
year = {2004},
}

@article{Oh2003,
author = {Oh, MS and Raftery, A},
title = {Model-based clustering with dissimilarities: {A} {B}ayesian approach},
journal = {UW Working paper no. 38, Center for Statistics and the Social Sciences},
volume = {},
pages = {},
year = {2003},
}

@article{Oh2001,
author = {Oh, MS and Raftery, A},
title = {Bayesian multidimensional scaling and choice of dimension},
journal = {Journal of the American Statistical Association},
volume = {96},
pages = {1031--1044},
year = {2001},
}

@article{Lee2008,
author = {Lee, AB and Nadler, B and Wasserman, L},
title = {Treelets-an adaptive multi-scale basis for sparse unordered data},
journal = {The Annals of Applied Statistics},
volume = {2},
pages = {435--471},
year = {2008},
}

@article{LinZha2008,
author = {Lin, T and Zha, H},
title = {Riemannian manifold learning},
journal = {IEEE Transactions on pattern analysis and machine intelligence},
volume = {30},
pages = {796--809},
year = {2008}
}

@article{Yang2008,
author = {Yang, L},
title = {Alighment of overlapping locally scaled patches for multidimensional scaling and dimension reduction},
journal = {IEEE Transactions on pattern analysis and machine intelligence},
volume = {30},
pages = {438--450},
year = {2008}
}

@article{Yangetal2008,
author = {Yang, Y and Gilbert, Peter B and Longini, IM Jr. and Halloran, ME},
title = {Estimating vaccine efficacy per infectious contact: A $\mbox{Bayesian}$ framework with adjustment for measurement error.},
year = {2008},
journal = {Annals of Applied Statistics},
volume =  {2},
pages = {1409--1431},
  note={PMCID: PMC2630256}
}


@article{Donoho2003,
author = {Donoho, DL and Grimes, C},
title = {Hessian eigenmaps: locally linear embedding techniques for high-dimensional data},
journal = {PNAS},
volume = {100},
pages = {5591--5596},
year = {2003},
}

@article{Droge1987,
author = {Dr\"{o}ge, C and Darmon, RY},
title = {Associative positioning strategies through comparative advertising: {A}ttribute versus overall similarity approaches},
journal = {Journal of Markerting Research},
volume = {24},
pages = {377--388},
year = {1987},
}

@article{Rust1995,
author = {Rust, RT and Simester, D and Brodie, RJ and Nilikant, BV},
title = {Model selection criteria: {A}n investigation of relative accuracy, posterior probabilities and combinations of criteria},
journal = {Management Science},
volume = {41},
pages = {322--333},
year = {1995},
}


@article{Busing2005,
author = {Busing, FMTA and Groenen, PJK and Heiser, WJ},
title = {Avoiding degeneracy in multidimensional unfolding by penalizing on the coefficient of variation},
journal = {Psychometrika},
volume = {70},
pages = {71--98},
year = {2005},
}


@article{Kruskal1964a,
author = {Kruskal, JB},
title = {Multidimensional scaling by optimizing goodness of fit to a nonmetric hypothesis},
journal = {Psychometrika},
volume = {29},
pages = {1--27},
year = {1964},
}


@article{Kruskal1964b,
author = {Kruskal, JB},
title = {Nonmetric multidimensional scaling: a numerical method},
journal = {Psychometrika},
volume = {29},
pages = {115--129},
year = {1964},
}


@article{Takane1977,
author = {Takane, Y and Young, FW and DE Leeuw, J},
title = {Nonmetric individual differences multidimensional scaling: {A}n alternating least squares methods with optimal scaling features},
journal = {Psychometrika},
volume = {42},
pages = {7--67},
year = {1977},
}



@article{Lapedes2001,
author = {Lapedes, A and Faber, R},
title = {The Geometry of Shape Space: {A}pplication to Influenza},
journal = {Journal of Theoretical Biology},
volume = {212},
pages = {57--69},
year = {2001},
}

@article{Commandeur1999,
author = {Commandeur, JJF and Groenen, PJF and Meulman, JJ},
title = {A distance-based variety of nonlinear multivariate data analysis, including weights for objects and variables},
journal = {Psychometrika},
volume = {64},
pages = {169--186},
year = {1999}
}

@article{DeSarbo1999,
author = {DeSarbo, WS and Kim, Y and Fong, D},
title = {A $\mbox{Bayesian}$ multidimensional scaling procedure for the spatial analysis of revealed choice data},
journal = {Journal of Econometrics},
volume = {89},
pages = {79--108},
year = {1999}
}

@article{Portnoy1988,
author = {Portnoy, S},
title = {Asymptotic bahavior of likelihood methods for exponential families when the number of parameters tens to infinity},
journal = {The Annals of Statistics},
volume = {16},
pages = {356--366},
year = {1988}
}

@article{Gilbert2001,
author = {Gilbert, Peter B and Self, GS and Rao, M and Naficy, A and Clemens, J},
title = {Sieve analysis: Methods for assessing how vaccine efficacy depends on genotypic and
phenotypic pathogen variation from vaccine trial data },
journal = {Journal of Clinical Epidemiology},
volume = {54},
pages = {68--85},
year = {2001}
}

@article{GilbertWuJobes2008,
author = {Gilbert, Peter B and Wu, C and Jobes, DV},
title = {Genome scanning tests for comparing amino acid sequences between groups},
journal = {Biometrics},
volume = {64},
pages = {198--207},
year = {2008}
}


@article{Qin2006,
author = {Qin, L and Guo, W},
title = {State Space Representation for Smoothing Spline ANOVA Models},
journal = {Journal of Computational and Graphical Statistics},
volume = {15},
pages = {830--847},
year = {2006}
}

@article{Qin2007,
author = {Qin, L and Guo, W and Litt, B},
title = {A time-frequency functional model for locally stationary time series data},
journal = {Journal of Computational and Graphical Statistics},
volume = {in press},
pages = { },
year = {2007}
}

@article{Qin2008,
author = {Qin, L and Wang, Y},
title = {Nonparametric spectral analysis with applications to seizure characterization using {IEEG} time series},
journal = {Annals of Applied Statistics},
volume = {in press},
pages = { },
year = {2008} 
}

@article{Perelson1979,
author = {Perelson, AS and Oster, GF},
title = {Theoretical studies of clonal selection: {M}inimal antibody repertoire size and reliability of self-non-self discrimination},
journal = {Journal of theoretical biology},
volume = {81},
pages = {645--670},
year = {1979}
}

@article{Akaike1974,
author = {Akaike, H},
title = {A new look at the statistical model identification},
journal = {IEEE Transactions on Automatic Control},
volume = {AC-19},
pages = {716--723},
year = {1974}
}

@article{Wang2000,
author = {Wang, Y and Guo, W and Brown, MB},
title = {Spline Smoothing For Bivariate Data With Applications To Association Between Hormones},
journal = {Statistica Sinica},
volume = {10},
pages = {377--397},
year = {2000}
}



@article{Heckman1986,
author = {Heckman, NE},
title = {Spline Smoothing in a partly linear model},
journal = {Journal of the Royal Statistical Society, Series B},
volume = {48},
pages = {244--248},
year = {1986}
}


@article{Opsomer1999,
author = {Opsomer, JD and Ruppert, D},
title = {A root-n consistent backfitting estimator for semiparametric additive modeling},
journal = {Journal of computation and graphical statistics},
volume = {8},
pages = {715--732},
year = {1999}
}

@article{Werthenbach1998,
author = {Werthenbach, C and Herrmann, E},
title = {A fast and stable updating algorithm for bivariate nonparametric curve estimation},
journal = {Journal of computation and graphical statistics},
volume = {7},
pages = {61--76},
year = {1998}
}

@article{Zhang1997,
author = {Zhang, H},
title = {Multivariate adaptive splines for analysis of longitudinal data},
journal = {Journal of computation and graphical statistics},
volume = {6},
pages = {74--91},
year = {1997},
}

@article{ChenV1999,
author = {Chen, VCP and Ruppert, D and Shoemaker, CA},
title = {Multivariate adaptive splines for analysis of longitudinal data},
journal = {Operations Research},
volume = {47},
pages = {38--53},
year = {1999},
}

@article{Leathwick2006,
author = {Leathwich, JR and Elith, J and Hastie, T},
title = {Comparative performance of generalized additive models and multivariate adaptive regression splines for statistical modelling of species distributions},
journal = {Ecological Modelling},
volume = {199},
pages = {188--196},
year = {2006},
}

@article{Linzhang2006,
author = {Lin, Y and Zhang, HH},
title = {Component selection and smoothing in multivariate nonparametric regression},
journal = {The Annals of Statistics},
volume = {34},
pages = {2272--2297},
year = {2006},
}

@article{Eglestonetal2009,
  title={On estimation of the survivor average causal effect in observational studies when important confounders are missing due to death},
  author={Egleston, Brian L and Scharfstein, Daniel O and MacKenzie, Ellen},
  journal={Biometrics},
  volume={65},
  number={2},
  pages={497--504},
  year={2009},
  publisher={Wiley Online Library}
}

@article{Imai2008,
author = {Imai, K},
title = {Sharp bounds on the causal effects in randomized experiments with `truncation by death'},
journal = {Statistics and Probability Letters},
volume = {78},
pages = {144--149},
year = {2008},
}

@article{ZhangRubin2003,
author = {Zhang, JL and Rubin, DB}, 
title = {Estimation of causal effects via principal stratification when some outcomes are truncated by ``death"},
journal = {Journal of Educational and Behavioral Statistics},
volume = {28},
pages = {353--368},
year = {2003},
}


@article{Chiba2012,
author = {Chiba, Y}, 
title = {The large sample bounds on the principal strata effect with application to a prostate cancer prevention trial},
journal = {The International Journal of Biostatistics},
volume = {8, Issue 1},
pages = {Article 12},
year = {2012}
}



@article{Breiman2001,
author = {Breiman, L},
title = {Random forests},
journal = {Machine Learning},
volume = {45},
pages = {5--32},
year = {2001},
}


@article{Efron1997,
author = {Efron, B and Tibshirani, RJ},
title = {Improvements on cross-validation: {T}he 632+ bootstrap method},
journal = {Journal of the Americal Statistical Association},
volume = {92},
pages = {548--560},
year = {1997},
}

@article{Li2003,
author = {Li, KC and Aragon, Y and Shedden, K and Agnan, CT},
title = {Dimension reduction for multivariate response data},
journal = {Journal of the American Statistical Association},
volume = {98},
pages = {99--109},
year = {2003},
}

@article{Li1991,
author = {Li, KC},
title = {Slice inverse regression for dimension reduction},
journal = {Journal of the American Statistical Association},
volume = {86},
pages = {316--342},
year = {1991},
}

@article{Mackay1983,
author = {MacKay, DB},
title = {Alternative probabilistic scaling models for spatial data},
journal = {Geographical Analysis},
volume = {15},
pages = {173--186},
year = {1983},
}

@article{Bozdogan1987,
author = {Bozdogan, H},
title = {Model selection and {A}kaike's {I}nformation {Criterion} ({AIC}): The general theory and its analytical extensions},
journal = {Psychometrika},
volume = {52},
pages = {345--370},
year = {1987},
}

@article{Hope1968,
author = {Hope, AC},
title = {A simplified {M}onte {C}arlo significance test procedure},
journal = {Journal of the Royal Statistical Society, Series B},
volume = {30},
pages = {582--598},
year = {1968},
}



@article{Eilers2003,
author = {Eilers, PHC and Marx, BD},
title = {Multivariate calibration with temperature interaction using two-dimensional penalized signal regression},
journal = {Chemometrics and intelligent laboratory systems},
volume = {66},
pages = {159--174},
year = {2003},
}

@article{Coull2004,
author = {Coull, BA and Staudenmayer, J},
title = {Self-modeling regression for multivariate curve data},
journal = {Statistica Sinica},
volume = {14},
pages = {695--711},
year = {2004},
}

@article{Cleveland1988,
author = {Cleveland, WS and Devlin, SJ},
title = {Locally weighted regression: an application to regression analysis by local fitting},
journal = {Journal of the American Statistical Association},
volume = {83},
pages = {596--610},
year = {1988},
}

@article{Friedman1991,
author = {Friedman, JH},
title = {Multivariate adaptive regression splines},
journal = {The Annals of Statistics},
volume = {19},
pages = {1--67},
year = {1991},
}

@article{Friedman2004,
author = {Friedman, JH and Popescu, BE},
title = {Gradient directed regularization for linear regression and classification},
journal = {Technical report},
volume = {CA Department of Statistics, Stanford University},
pages = {},
year = {2004},
}


@article{Breiman1995,
author = {Breiman, L},
title = {Better subset selection using the nonnegative garrote},
journal = {Technometrics},
volume = {37},
pages = {373--384},
year = {1995},
}

@article{Vera2007,
author = {Vera, JF and Heiser, WJ and Murillo, A},
title = {Global optimization in any {M}inkowski metric: {A} permutation-translation
simulated annealing algorithim for multidimensional scaling},
journal = {Journal of Classification},
volume = {24},
pages = {277--301},
year = {2007},
}

@article{Efron2004,
author = {Efron, B and Hastie, T and Johnstone, I and Tibshirani, R},
title = {Least angle regression (with discussion)},
journal = {The Annals of Statistics},
volume = {32},
pages = {407--499},
year = {2004},
}


@article{James1961,
author = {James, W and Stein, C},
title = {Estimation with quadratic loss},
journal = {Proc. Fourth Berkeley Symp. Math. Statist. Prob.},
volume = {1},
pages = {361--379},
year = {1961},
}

@book{Duppert2003,
author ={Duppert, D and Wand, MP and Carroll, RJ},
title = {Semiparametric regression},
publisher = {Cambridge University Press},
year = {2003},
}


@book{Wahba90,
author ={Wahba, G},
title = {Spline Models for Observational Data},
publisher = {CBMS-NSF Regional Conference Series in Applied Mathematics},
address = {SIAM},
year = {1990},
}

@book{Gu02,
author = {Gu, C},
title = {Smoothing Spline ANOVA Models},
publisher = {New York: Springer-Verlag},
year = {2002},
}


@book{Hastie1990,
author = {Hastie, TJ and Tibshirani, RJ},
title = {Generalized additive models},
publisher = {Chapman and Hall},
year = {1990},
}

@book{Hastie2001,
author = {Hastie, TJ and Tibshirani, RJ and Friedman, JH},
title = {The Elements of Statistical Learning},
publisher = {New York: Springer},
year = {2001},
}

@book{Spence1982,
   author={Spence, I},
   title={Incomplete experimental design for multidimensional scaling.  In R.G. Golledge and J.N. Rayer (Eds.), Proximity and Preference:
   Problems in the Multidimensional Analysis of Large Data Sets, pp. 29-46},
   publisher={Minneapolis, MN: University of Minnesota Press},
   year={1982},
}

@book{Good2005,
author = {Good, PI},
title = {Permutation, parametric and bootstrap tests of hypotheses},
publisher = {New York: Springer},
year = {2005},
}


@book{Borg1997,
author = {Borg, I and Groenen, P},
title = {Modern multidimensional scaling},
publisher = {New York: Springer},
year = {1997},
}

@article{TianCaiGoetWei2007,
author = {Tian, L and Cai, T and Goetghebeur, E and Wei, LJ},
title = {Model evaluation based on the distribution of estimated absolute
prediction error.},
journal = {Biometrika},
volume = {94},
pages = {297--311},
year = {2007}
}

@article{Follmannetal2003, 
author = {Follmann, D and Proschan, M and Leifer, E.},
title = {Multiple Outputation: Inference for Complex Clustered Data
by Averaging Analyses from Independent Data.},
journal = {Biometrics},
volume = {59},
pages = {420--429}, 
year = {2003} 
}


@article{LuTsiatis2008,
author = {Lu, X and Tsiatis, AA},
title = {Improving the efficiency of the log-rank test using auxiliary covariates.},
journal = {Biometrika},
volume = {95},
pages = {679--694},
year = {2008}
}




@article{Wick04,
author = {Wick, D and Self, SG},
title = {On simulating strongly-interacting stochastic population models},
journal = {Mathematical Biosciences},
volume = {187},
pages = {1--20},
year = {2004},
}

@article{QinGilbertFollmannLi2008,
author = {Qin, L and Gilbert, Peter B and Follmann, D and Li, D},
title = {Assessing surrogate endpoints in vaccine trials with case-cohort sampling and the $\mbox{Cox}$ model},
journal = {Annals of Applied Statistics},
volume = {2},
pages = {386--407},
year = {2008},
note={PMCID: PMC2601643}
}
%note={PMCID: PMC2601643}


@article{Hooveretal1998,
author = {Hoover, DR and Rice, JA and Wu, CO and Yang, LP},
title = {Nonparametric smoothing estimates of time-varying coefficient
models with longitudinal data.},
journal = {Biometrika},
volume = {85},
pages = {809-822},
year = {1998}
}

@article{LiangWuCarroll2003,
author = {Liang, H and Wu, H and Carroll, RJ},
title = {The relationship between virologic and immunologic responses in $\mbox{AIDS}$ 
clinical research using mixed-effects varying-coefficient semiparametric
models with measurement error.}, 
journal = {Biostatistics},
volume = {4},
pages = {297--312},
year = {2003}
}

@article{LinYing2001,
author = {Lin, DY and Ying, Z},
title = {Semiparametric and nonparametric regression
analysis of longitudinal data (with discussion).},
journal = {Journal of the American Statistical Association},
volume = {96},
pages = {103--113},
year = {2001}
}

@article{MartinussenScheike1999,
author = {Martinussen, T and Scheike, TH},
title = {A semiparametric additive
regression model for longitudinal data.},
journal = {Biometrika},
volume = {86},
pages = {691--702},
year = {1999}
}

@article{MartinussenScheike2000,
author = {Martinussen, T and Scheike, TH},
title = {A nonparametric dynamic
additive regression model for longitudinal data.},
journal = {Annals of Statistics},
volume = {28},
pages = {1000--1025},
year = {2000}
}

@article{Scheikeetal2010,
author = {Scheike, T and Sun, Y and Zhang, M-J and Jensen, TK},
title = {A semiparametric
random effects model for multivariate competing risks data.},
journal = {Biometrika},
volume = {97},
pages = {133--145},
year = {2010},
  note={PMCID: PMC3633199}
}



@book{LeeScheikeSun2011,
author ={Lee, J and Scheike, T and Sun, Y},
title = {Regression analysis in failure time
mixture models with change points according to thresholds of a covariate. {In}: {Recent Advances in Biostatistics -- False Discovery Rates, Survival Analysis,
and Related Topics, Series in Biostatistics}.},
booktitle= {Recent Advances in Biostatistics -- False Discovery Rates, Survival Analysis,
and Related Topics, Series in Biostatistics, Vol. 4},
publisher = {World Scientific, New Jersey},
volume = {4},
year = {2011}
}


@InProceedings{Buchbinder2009AIDSVaccine,
  author =          {Buchbinder, S},
  title =          {Clinical results from the Step study.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {AIDS Vaccine 2009},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Paris, France, October 2009},
  OPTpublisher = {},
  OPTannote =          {}
}






@article{ScheikeSun2007,
author = {Scheike, T and Sun, Y},
title = {Likelihood estimation for tied survival data under $\mbox{Cox}$ regression
model via EM-algorithm.},
journal = {Lifetime Data Analysis},
volume = {13},
pages = {399--420},
year = {2007}
}

@article{ScheikeSun2012,
author = {Scheike, T and Sun, Y},
title = {On cross-odds ratio for multivariate competing risks data.},
journal = {Biostatistics}, 
volume = {13},
pages = {680--694},
year = {2012},
  note={PMCID: PMC3440240}
}


@article{SunSundaramZhao2009,
author = {Sun, Y and Sundaram, R and Zhao, Y},
title = {Empirical likelihood inference for the $\mbox{Cox}$ model with time-dependent coefficients via local partial likelihood.},
journal = {Scandinavian Journal of Statistics},
volume = {36},
pages = {444--462},
year = {2009},
  note={PMCID: PMC2762234}
}









@article{MartinussenScheike2001,
author = {Martinussen, T and Scheike, TH},
title = {Sampling adjusted analysis
of dynamic additive regression models for longitudinal data.},
journal = {Scandanavian Journal of Statistics},
volume = {28},
pages = {303--323},
year = {2001}
}

@article{MoyeedDiggle1994,
author = {Moyeed, RA and Diggle, PJ},
title = {Rates of convergence in semiparametric
modelling of longitudinal data.},
journal = {Australian Journal of Statistics},
volume = {36},
pages = {75--93},
year = {1994}
}

@article{WuChiangHoover1998,
author = {Wu, CO and Chiang, CT and Hoover, DR},
title = {Asymptotic confidence
regions for kernel smoothing of a time-varying coefficient model
with longitudinal data.},
journal = {Journal of the American Statistical Association},
volume = {88},
pages = {1388-1402},
year = {1998}
}

@article{WuZhang2002a,
author = {Wu, H and Zhang, JT},
title = {The study of long-term $\mbox{HIV}$ dynamics using semiparametric nonlinear
mixed-effects models.},
journal = {Statistics in Medicine},
volume = {21},
pages = {3655--3675},
year = {2002}
}

@article{WuZhang2002b,
author = {Wu, H and Zhang, JT},
title = {Local polynomial mixed-effects models for longitudinal data.},
journal = {Journal of the American Statistical Association},
volume = {97},
pages = {883--897},
year = {2002}
}

@article{LongHudgens2012,
  title={Comparing competing risk outcomes within principal strata, with application to studies of mother-to-child transmission of {HIV}},
  author={Long, Dustin M and Hudgens, Michael G},
  journal={Statistics in Medicine},
  volume={31},
  number={27},
  pages={3406--3418},
  year={2012},
  publisher={Wiley Online Library},
  note={PMCID: PMC3494821}
}


@article{Letvinetal2009,
author = {Letvin, N and Mascola, J and Rao, S and Buzby, A and Roederer, M and Hudgens, M and Gilbert, P and Seder, R and Douek, D and Koup, R and Graham, B and Nabel, G},
title = {Gene-based vaccination protects against mucosal infection by a heterologous highly pathogenic SIV isolate in rhesus monkeys.},
journal = {Retrovirology},
volume = {6 Suppl 3},
pages = {P19-57 LB},
year = {2009}
}

@article{Hansenetal2009,
author = {Hansen, SG and Vieville, C and Whizin, N and Coyne-Johnson, L and Siess, DC and Drummond, DD and Legasse, AW and Axthelm, MK and Oswald, K and Trubey, CM and Piatak Jr., M and Lifson, JD and Nelson, JA and Jarvis, MA and Picker, LJ},
title = {Effector-memory {T} cell responses are associated with protection of rhesus monkeys from mucosal {SIV} challenge.},
journal = {Nature Medicine}, 
volume = {15},
pages = {293--299},
year = {2009},
  note={PMCID: PMC2720091}
}

@article{LiTaylorElliott2010,
author = {Li, Y and Taylor, JMG and Elliott, MR},
title = {A $\mbox{Bayesian}$ approach to surrogacy assessment using principal stratification in clinical trials},
journal = {Biometrics},
volume = {66},
pages = {523--531},
year = {2010}
}


@article{ScheikeZhang1998,
author = {Scheike, TH and Zhang, MJ},
title = {Cumulative regression function
tests for longitudinal data.},
journal = {Annals of Statistics},
volume = {26},
pages = {1328--1355},
year = {1998}
}




@article{WuLiang2004,
author = {Wu, H and Liang, H},
title = {Random varying-coefficient models with smoothing covariates,
applications to an $\mbox{AIDS}$  clinical study.},
journal = {Scandanavian Journal of Statistics},
volume = {31},
pages = {3--19},
year = {2004}
}

@article{ZegerDiggle1994,
author = {Zeger, SL and Diggle, PJ},
title = {Semiparametric models for
longitudinal data with application to $\mbox{CD4}$ cell numbers in $\mbox{HIV}$
seroconverters.}, 
journal = {Biometrics},
volume = {55},
pages = {452--459},
year = {1994}
}

@Article{McDermottetal2004,
    Author="McDermott, A. B.  and Mitchen, J.  and Piaskowski, S.  and De Souza, I.  and Yant, L. J.  and Stephany, J.  and Furlott, J.  and Watkins, D. I. ",
    Title="{{R}epeated low-dose mucosal simian immunodeficiency virus {S}{I}{V}mac239 challenge results in the same viral and immunological kinetics as high-dose challenge: a model for the evaluation of vaccine efficacy in nonhuman primates}",
    Journal="J. Virol.",
    Year="2004",
    Volume="78",
    Pages="3140--3144",
    Month="Mar"
}

@Article{Wilsonetal2006,
    Author="Wilson, N. A.  and Reed, J.  and Napoe, G. S.  and Piaskowski, S.  and Szymanski, A.  and Furlott, J.  and Gonzalez, E. J.  and Yant, L. J.  and Maness, N. J.  and May, G. E.  and Soma, T. 
and Reynolds, M. R.  and Rakasz, E.  and Rudersdorf, R.  and McDermott, A. B.  and O'Connor, D. H.  and Friedrich, T. C.  and Allison, D. B.  and Patki, A.  and Picker, L. J.  and Burton, D. R.  and Lin, J.  and Huang, L.  and Patel, D.  and Heindecker, G.  and Fan, J.  and Citron, M.  and Horton, M.  and Wang, F.  and Liang, X.  and Shiver, J. W.  and Casimiro, D. R.  and Watkins, D. I. ",
    Title="{{V}accine-induced cellular immune responses reduce plasma viral concentrations after repeated low-dose challenge with pathogenic simian immunodeficiency virus {S}{I}{V}mac239}",
    Journal="J. Virol.",
    Year="2006",
    Volume="80",
    Pages="5875--5885",
    Month="Jun"
}


@article{Villarietal2004,
author = {Villari, P and Manzoli, L and Boccia, A},
title = {Methodological quality of studies and patients age as major sources of variation
in vaccine efficacy estimates of influenza vaccination in healthy adults: a meta-analysis.},
journal = {Vaccine},
volume = {22},
pages = {3475--3486},
year = {2004}
}

@Article{RotnitzkyRobins1995,
author =          {Rotnitzky, A and Robins, JM},
title =          {Semiparametric regression estimation in the presence of dependent censoring.},
journal =          {Biometrika},
year =          {1995},
volume =          {82},
pages =          {805--820}
}

@article{Gnanakaranetal2011,
  title={Recurrent signature patterns in {HIV-1 B} clade envelope glycoproteins associated with either early or chronic infections},
  author={Gnanakaran, S and Bhattacharya, T and Daniels, M and Keele, BF and Hraber, PT and Lapedes, AS and Shen, T and Gaschen, B and Krishnamoorthy, M and Li, H and Decker, JM and Salazar-Gonzalez, JF and Wang, SY and Jiang, CL and Gao, F and Swanstrom, R and Anderson, JA and Ping, LH and Cohen, MS and Markowitz, M and Goepfert, PA and
 Saag, MS and Eron, JJ and Hicks, CB and Blattner, WA and Tomaras, GD and Asmal, M and Letvin, NL and
 Gilbert, Peter B and DeCamp, AC and Magaret, CA and Schief, WR and Ban, YEA and Zhang, M and Soderberg, KA and Sodroski,
JG and Haynes, BF and Shaw, GM and Hahn, BH and Korber, BR},
  journal={PLoS Pathogens},
  volume={7},
  number={9},
  pages={e1002209},
  year={2011},
  publisher={Public Library of Science},
  note={PMCID: PMC3182927}
}

@article{dahmengeneralized2004,
	title = {Generalized Estimating Equations in Controlled Clinical Trials: Hypotheses Testing},
	volume = {46},
	copyright = {Copyright 2004 {WILEY-VCH} Verlag {GmbH} \& Co. {KGaA}, Weinheim},
	issn = {1521-4036},
	shorttitle = {Generalized Estimating Equations in Controlled Clinical Trials},
	url = {http://onlinelibrary.wiley.com/doi/10.1002/bimj.200310018/abstract},
	doi = {10.1002/bimj.200310018},
	language = {en},
	number = {2},
	urldate = {2013-02-14},
	journal = {Biometrical Journal},
	author = {Dahmen, G. and Ziegler, A.},
	year = {2004},
	keywords = {Controlled clinical trials, Generalized estimating equations, Missing data, Sample size calculations, Weighted estimating equations},
	pages = {214--232}
}

@article{faysmallsample2001,
	title = {Small-Sample Adjustments for Wald-Type Tests Using Sandwich Estimators},
	volume = {57},
	copyright = {Copyright 2001 International Biometric Society},
	issn = {0006-{341X}},
	url = {http://www.jstor.org/stable/3068253},
	doi = {10.2307/3068253},
	abstract = {The sandwich estimator of variance may be used to create robust Wald-type tests from estimating equations that are sums of K independent or approximately independent terms. For example, for repeated measures data on K individuals, each term relates to a different individual. These tests applied to a parameter may have greater than nominal size if K is small, or more generally if the parameter to be tested is essentially estimated from a small number of terms in the estimating equation. We offer some practical modifications to these robust Wald-type tests, which asymptotically approach the usual robust Wald-type tests. We show that one of these modifications provides exact coverage for a simple case and examine by simulation the modifications applied to the generalized estimating equations of Liang and Zeger (1986), conditional logistic regression, and the Cox proportional hazard model.},
	number = {4},
	urldate = {2013-02-13},
	journal = {Biometrics},
	author = {Fay, Michael P. and Graubard, Barry I.},
	month = dec,
	year = {2001},
	pages = {1198--1206},
	file = {JSTOR Full Text PDF:/home/adecamp/.mozilla/firefox/pcya5epu.default/zotero/storage/7I5GPHIE/Fay and Graubard - 2001 - Small-Sample Adjustments for Wald-Type Tests Using.pdf:application/pdf}
}

@article{kauermannnote2001,
	title = {A Note on the Efficiency of Sandwich Covariance Matrix Estimation},
	volume = {96},
	copyright = {Copyright 2001 American Statistical Association},
	issn = {0162-1459},
	url = {http://www.jstor.org/stable/3085907},
	doi = {10.2307/3085907},
	abstract = {The sandwich estimator, also known as robust covariance matrix estimator, heteroscedasticity-consistent covariance matrix estimate, or empirical covariance matrix estimator, has achieved increasing use in the econometric literature as well as with the growing popularity of generalized estimating equations. Its virtue is that it provides consistent estimates of the covariance matrix for parameter estimates even when the fitted parametric model fails to hold or is not even specified. Surprisingly though, there has been little discussion of properties of the sandwich method other than consistency. We investigate the sandwich estimator in quasi-likelihood models asymptotically, and in the linear case analytically. We show that under certain circumstances when the quasi-likelihood model is correct, the sandwich estimate is often far more variable than the usual parametric variance estimate. The increased variance is a fixed feature of the method and the price that one pays to obtain consistency even when the parametric model fails or when there is heteroscedasticity. We show that the additional variability directly affects the coverage probability of confidence intervals constructed from sandwich variance estimates. In fact, the use of sandwich variance estimates combined with t-distribution quantiles gives confidence intervals with coverage probability falling below the nominal value. We propose an adjustment to compensate for this fact.},
	number = {456},
	urldate = {2013-02-14},
	journal = {Journal of the American Statistical Association},
	author = {Kauermann, G{\"o}ran and Carroll, Raymond J.},
	month = dec,
	year = {2001},
	pages = {1387--1396},
	file = {JSTOR Full Text PDF:/home/adecamp/.mozilla/firefox/pcya5epu.default/zotero/storage/HAHN2WSZ/Kauermann and Carroll - 2001 - A Note on the Efficiency of Sandwich Covariance Ma.pdf:application/pdf}
}

@article{lu_comparison_2007,
	title = {A comparison of two bias-corrected covariance estimators for generalized estimating equations},
	volume = {63},
	issn = {0006-{341X}},
	doi = {10.1111/j.1541-0420.2007.00764.x},
	abstract = {Mancl and {DeRouen} (2001, Biometrics57, 126-134) and Kauermann and Carroll (2001, {JASA96}, 1387-1398) proposed alternative bias-corrected covariance estimators for generalized estimating equations parameter estimates of regression models for marginal means. The finite sample properties of these estimators are compared to those of the uncorrected sandwich estimator that underestimates variances in small samples. Although the formula of Mancl and {DeRouen} generally overestimates variances, it often leads to coverage of 95\% confidence intervals near the nominal level even in some situations with as few as 10 clusters. An explanation for these seemingly contradictory results is that the tendency to undercoverage resulting from the substantial variability of sandwich estimators counteracts the impact of overcorrecting the bias. However, these positive results do not generally hold; for small cluster sizes (e.g., {\textless}10) their estimator often results in overcoverage, and the bias-corrected covariance estimator of Kauermann and Carroll may be preferred. The methods are illustrated using data from a nested cross-sectional cluster intervention trial on reducing underage drinking.},
	number = {3},
	journal = {Biometrics},
	author = {Lu, Bing and Preisser, John S and Qaqish, Bahjat F and Suchindran, Chirayath and Bangdiwala, Shrikant I and Wolfson, Mark},
	month = sep,
	year = {2007},
	keywords = {Algorithms, Bias (Epidemiology), Biometry, Clinical Trials as Topic, Cluster Analysis, Data Interpretation, Statistical, Regression Analysis, Reproducibility of Results, Sensitivity and Specificity},
	pages = {935--941}
}

@article{manclcovariance2001,
	title = {A covariance estimator for {GEE} with improved small-sample properties},
	volume = {57},
	issn = {0006-{341X}},
	abstract = {In this paper, we propose an alternative covariance estimator to the robust covariance estimator of generalized estimating equations ({GEE).} Hypothesis tests using the robust covariance estimator can have inflated size when the number of independent clusters is small. Resampling methods, such as the jackknife and bootstrap, have been suggested for covariance estimation when the number of clusters is small. A drawback of the resampling methods when the response is binary is that the methods can break down when the number of subjects is small due to zero or near-zero cell counts caused by resampling. We propose a bias-corrected covariance estimator that avoids this problem. In a small simulation study, we compare the bias-corrected covariance estimator to the robust and jackknife covariance estimators for binary responses for situations involving 10-40 subjects with equal and unequal cluster sizes of 16-64 observations. The bias-corrected covariance estimator gave tests with sizes close to the nominal level even when the number of subjects was 10 and cluster sizes were unequal, whereas the robust and jackknife covariance estimators gave tests with sizes that could be 2-3 times the nominal level. The methods are illustrated using data from a randomized clinical trial on treatment for bone loss in subjects with periodontal disease.},
	number = {1},
	journal = {Biometrics},
	author = {Mancl, L A and {DeRouen}, T A},
	month = mar,
	year = {2001},
	keywords = {Alveolar Bone Loss, Analysis of Variance, Bias (Epidemiology), Biometry, Computer Simulation, Humans, Logistic Models, Models, Statistical, Periodontal Diseases, Randomized Controlled Trials as Topic},
	pages = {126--134}
}

@article{morelsmall2003,
	title = {Small Sample Correction for the Variance of {GEE} Estimators},
	volume = {45},
	copyright = {Copyright 2003 {WILEY-VCH} Verlag {GmbH} \& Co. {KGaA}, Weinheim},
	issn = {1521-4036},
	url = {http://onlinelibrary.wiley.com/doi/10.1002/bimj.200390021/abstract},
	doi = {10.1002/bimj.200390021},
	abstract = {When clustered multinomial responses are fit using the generalized logistic link, Morel (1989) introduced a small sample correction in the Taylor series based estimator of the covariance matrix of the parameter estimates. The correction reduces the bias of the Type I error rates in small samples and guarantees positive definiteness of the estimated variance-covariance matrix. It is well known that small sample bias in the use of the Delta method persists in any application of the Generalized Estimating Equations ({GEE)} methodology. In this article, we extend the correction originally suggested for the generalized logistic link, to other link functions and distributions, when parameters are estimated by {GEE.} In a Monte Carlo study with correlated data generated under different sampling schemes, the small sample correction has been shown to be effective in reducing the Type I error rates when the number of clusters is relatively small.},
	language = {en},
	number = {4},
	urldate = {2013-02-14},
	journal = {Biometrical Journal},
	author = {Morel, J.g. and Bokossa, M.c. and Neerchal, N.k.},
	year = {2003},
	keywords = {Correlated Bernoulli outcomes, Correlated normal outcomes, Identity link, Logarithm link, Logit link, Multinomial finite mixtures, Negative-binomial distribution, Overdispersion, Proportional-odds function},
	pages = {395--409}
}

@article{pan_robust_2001,
	title = {On the Robust Variance Estimator in Generalised Estimating Equations},
	volume = {88},
	copyright = {Copyright 2001 Biometrika Trust},
	issn = {0006-3444},
	url = {http://www.jstor.org/stable/2673458},
	doi = {10.2307/2673458},
	abstract = {The variance matrix of the estimated regression coefficient in the Liang-Zeger generalised estimating equation approach can be consistently estimated by the so-called sandwich or robust estimator. In this note, we propose a modification to the Liang-Zeger prescription for implementing the robust variance estimator. Analytical and numerical evidence shows the superior performance of our proposal.},
	number = {3},
	urldate = {2013-02-13},
	journal = {Biometrika},
	author = {Pan, Wei},
	month = sep,
	year = {2001},
	pages = {901--906},
	file = {JSTOR Full Text PDF:/home/adecamp/.mozilla/firefox/pcya5epu.default/zotero/storage/D3H9PHKI/Pan - 2001 - On the Robust Variance Estimator in Generalised Es.pdf:application/pdf}
}

@article{Pailaetal2008,
  title={Genome bias influences amino acid choices: analysis of amino acid substitution and re-compilation of substitution matrices exclusive to an AT-biased genome},
  author={Paila, Umadevi and Kondam, Rohini and Ranjan, Akash},
  journal={Nucleic acids research},
  volume={36},
  number={21},
  pages={6664--6675},
  year={2008},
  publisher={Oxford Univ Press}
}







@article{warton_regularized_2011,
	title = {Regularized sandwich estimators for analysis of high-dimensional data using generalized estimating equations},
	 volume={67},
	doi = {10.1111/j.1541-0420.2010.01438.x},
	number = {1},
	journal = {Biometrics},
	author = {Warton, David I},
	month = mar,
	year = {2011},
	keywords = {Algorithms, Animals, Biometry, Computer Simulation, Data Interpretation, Statistical, Ecosystem, Models, Statistical, Nematoda, Population Growth},
	pages = {116--123}
}

@article{Qietal2017,
  title={Generalized semiparametric varying-coefficient model for longitudinal data with applications to adaptive treatment randomizations},
  author={Qi, Li and Sun, Yanqing and Gilbert, Peter B},
  journal={Biometrics},
  volume={73},
  number={2},
  pages={441--451},
  year={2017},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC5459686}
}

@article{SunZhangetal2019,
  title={Estimation of a semiparametric varying-coefficient mixed regressive spatial autoregressive model},
  author={Sun, Yanqing and Zhang, Yuanqing and Huang, Jianhua Z},
  journal={Econometrics and statistics},
  volume={9},
  pages={140--155},
  year={2019},
  publisher={Elsevier}
}

@article{Lietal2018,
  title={Semiparametric varying-coefficient regression analysis of recurrent
events with applications to treatment switching},
  author={Li, Y and Qi, Li and Sun, Yanqing},
  journal={Statistics in Medicine},
  volume={37},
  number={},
  pages={3959--3974},
  year={2018},
  publisher={Wiley Online Library},
  note={doi: 10.1002/sim.7856. PubMed PMID: 29992591. NIHMSID: NIHMS1033642}
}


@book{zieglergeneralized2011,
	address = {New York},
	title = {Generalized {E}stimating {E}quations},
	isbn = {9781461404996  1461404991},
	url = {http://public.eblib.com/EBLPublic/PublicView.do?ptiID=763916},
	language = {English},
	urldate = {2013-02-13},
	publisher = {Springer},
	author = {Ziegler, Andreas},
	year = {2011}
}

@Article{Hubbardetal2010,
author =          {Hubbard, AE and Ahern, J and Fleischer, NL and van der Laan, MJ and Lippman, SA and Jewell, N and Bruckner, T and Satarianob, WA},
title =          {To {GEE} or not to {GEE}: Comparing population average and mixed models for estimating the associations between neighborhood risk factors and health.},
journal =          {Epidemiology},
year =          {2010},
volume =          {21},
pages =          {467--474}
}

@Article{Huangetal2015,
author = {Huang, Y and Follmann, D and Nason, M and Zhang, L and Huang, Y and Mehrotra, D and Moodie, Z and et al.}, 
title = {Effect of {rAd5}-vector {HIV-1} preventive vaccines on {HIV-1} acquisition: a participant-level meta-analysis of randomized trials},
journal = {PLoS One},
year = {2015},
volume = {10},
pages = {e0136626}
}
% PMCID: PMC4558095.

@InProceedings{GilbertAIDSVaccine2013,
  author =          {Gilbert, Peter B and Huang, Y and Follmann, D and Zhang, L and Huang, Y and Nason, M and Moodie, Z and Janes, H and Metch, B and Graham, B and Masola, J and Kublin, J and Hammer, S and Buchbinder, S and Gray, G and Corey, L},
  title =          {Meta-analysis of {Ad5}-vector {HIV} Vaccine Trials to Assess the Vaccine Effect on {HIV} Acquisition. {AIDS Vaccine 2013 International Conference}.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2013}, 
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Barcelona, Spain, 2013},
  OPTpublisher = {},
  note =          {Abstract PL04.06.},
  OPTannote =          {}
}

@InProceedings{Grayetal2013,
  author =          {Gray, GE and Moodie, Z and Metch, B and Gilbert, Peter B and Bekker, LG and Churchyard, G and Nchabeleng, M and Mlisana, K and Allen, M and McElrath, JM and Robertson, MD and Kublin, J and Corey, L},
  title =          {An Update on the {Phambili/HVTN 503 Study}, a {Phase IIB HIV} Vaccine Efficacy Study 
Investigating {MRK Ad5 HIV-1} Subtype {B} gag/pol/nef Vaccine. {AIDS Vaccine 2013 International Conference}.},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2013},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Barcelona, Spain, 2013},
  OPTpublisher = {},
  note =          {Abstract PL04.05.},
  OPTannote =          {}
}

@InProceedings{LassauniereTiemessen2014,
author =          {Lassauniere, R and Tiemessen, CT},
title = {Fc-gamma receptor variability in the {S}outh {A}frican population-- {W}ill this impact on {HVTN}097 and vaccine efficacy? {HIV Research for Prevention 2014 (HIV R4P)}},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2014},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Cape Town, South Africa, 2014},
  OPTpublisher = {},
  note =          {Abstract P37.05.},
  OPTannote =          {}
}

@InProceedings{LassauniereTiemessen2014short,
author =          {Lassauniere, R and Tiemessen, CT},
title = {Fc-gamma receptor variability in the {S}outh {A}frican population-- {W}ill this impact on {HVTN}097 and vaccine efficacy? {HIV R4P Conference}},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2014},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Cape Town, South Africa, 2014},
  OPTpublisher = {},
  note =          {Abstract P37.05.},
  OPTannote =          {}
}

 


@InProceedings{Cameronetal2013,
  author =          {Cameron, Mark and Sabnis, Amit and Lefebvre, Francois and Gottardo, Raphael and Frahm, Nicole and De Rosa, Stephen and  Wilkinson, Peter and Stafova, Petra and Kaewkungwal, Jaranit and Pitisuttithum, Punnee and Nitayanphan, Sorachai and Rerks-Ngarm, Supachai and Michael, Nelson and Kim, Jerome and McElrath, M. Juliana and Sekaly, Rafick},
  title =          {Transcriptional profiling of {RV144} participants reveals a gene expression signature that correlates with immunogenicity. {AIDS Vaccine 2013 International Conference}.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2013},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Barcelona, Spain, 2013},
  OPTpublisher = {},
  note =          {Abstract PL04.05.},
  OPTannote =          {}
}

@Article{WHO-UNAIDS2001a,
  author =       {WHO-UNAIDS},
  title =        {Approaches to the development of broadly protective
$\mbox{HIV}$ vaccines: Challenges posed by genetic, biological and antigenic
variability of $\mbox{HIV}$-1: {WHO-UNAIDS} Report from a meeting of the {WHO-UNAIDS
Vaccine Advisory Committee Geneva} 21-23 {February} 2000.},
  journal =      {AIDS},
  year =         {2001},
  volume =       {15},
  pages =        {W1-W25},
}

@Article{PearlBareinboim2011,
  author =          {Pearl, J and Bareinboim, E},
  title =          {Transportability of causal and statistical relations: {A} formal approach.},
  journal =         {Proceedings of the
Twenty-Fifth National Conference on Artificial Intelligence, Menlo Park, CA},
  year =          {2011},
  volume =          {},
  pages = {247--254}
}


@Article{BareinboimPearl2012,
  author =          {Bareinboim, E and Pearl, J},
  title =          {Transportability of causal effects: {Completeness} results.},
  journal =         {Proceedings of the
Twenty-Sixth National Conference on Artificial Intelligence, Menlo Park, CA},
  year =          {2012},
  volume =          {},
  pages = {698--704}
}

@Article{ColeStuart2010,
  author =          {Cole, SR and Stuart, EA},
  title =          {Generalizing evidence from randomized clinical
trials to target populations: {T}he {ACTG} 320 trial.},
  journal =         {American Journal of Epidemiology},
  year =          {2010},
  volume =          {172},
  pages = {107--115},
  note={PMCID: PMC2915476}
}


@InProceedings{Lietal2013,
  author =          {Li, Shuying S and Gilbert, Peter B and Tomaras, Georgia D and Kijak, Gustavo and Ferrari, Guido and Thomas, Rasmi and Zolla-Pazner, Susan and Evans, David T and Yao, Li and Gottardo, Raphael and Dai, James Y and Janes, Holly E and Morris, Daryl and Fong, Youyi and Edlefsen, PT and Li, Fusheng and Magaret, Craig A and Frahm, Nicole and Alpert, Michael D and Rerks-Ngarm, Supachai and Pitisuttithum, Punnee and Kaewkungwal, Jaranit and Nitayaphan, Sorachai and Robb, Merlin L and O'Connell, Robert J and Michael, Nelson L and Kim, Jerome H and McElrath, M Juliana and Geraghty, Daniel E},
  title =          {Association of {Fc}-$\gamma${RIIC} Polymorphism with Vaccine Efficacy and Correlate of {HIV-1} Infection Risk in {RV144}. {AIDS Vaccine 2013 International Conference}.},
  booktitle =          {},
  OPTcrossref =  {},
  OPTkey =          {},
  OPTpages =          {},
  year =          {2013},
  OPTeditor =          {},
  OPTseries =          {},
  OPTaddress =          {},
  OPTmonth =          {},
  organization = {Barcelona, Spain, 2013},
  OPTpublisher = {},
  note =          {Abstract PL04.05.},
  OPTannote =          {}
}

@article{GabrielSachsGilbert2015,
  title={Comparing and combining biomarkers as principal surrogates for time-to-event clinical endpoints},
  author={Gabriel, Erin E and Sachs, Michael C and Gilbert, Peter B},
  journal={Statistics in Medicine},
  volume={34},
  number={3},
  pages={381--395},
  year={2015},
  publisher={Wiley Online Library}
}
%note={PMCID: PMC4801510}


@article{Trottetal2011,
  title={Evidence for an increased risk of transmission of simian immunodeficiency virus and malaria in a rhesus macaque coinfection model.},
  author={Trott, Kristin A and Chau, Jennifer Y and Hudgens, Michael G and Fine, Jason and Mfalila, Chelu K and Tarara, Ross P and Collins, William E and Sullivan, JoAnn and Luckhart, Shirley and Abel, Kristina},
  journal={Journal of Virology},
  volume={85},
  number={22},
  pages={11655--11663},
  year={2011},
  publisher={Am Soc Microbiol}
}

@article{Trottetal2013,
  title={Immune activation and regulation in {SIV-P.} fragile co-infected rhesus macaques.},
  author={Trott, Kristin A and Richardson, Amy and Hudgens, Michael A and Abel, Kristina},
  journal={Journal of Virology, in press},
  year={2013}
}

@article{Kiepielaetal2007,
title={$\mbox{CD8+ T}$-Cell Responses to Different $\mbox{HIV}$ Proteins Have Discordant Associations with Viral Load.},
author={Kiepiela, P and Ngumbela, K and Thobakgale, C and et al.},
journal={Nature Medicine},
volume={13},
pages={46--53},
year={2007}
}

@article{ZollaPazneretal2014,
author={Zolla-Pazner, S and DeCamp, A and Gilbert, Peter B and Williams, C and Yates, NL and Williams, WT and Howington, R and Fong, Y and Morris, DE and Soderberg, KA and Irene, C and Reichman, C and Pinter, A and Parks, R and Pitisuttithum, P and Kaewkungwal, J and Rerks-Ngarm, S and Nitayaphan, S and Andrews, C and O'Connell, RJ and Yang, ZY and Nabel, GJ and Kim, JH and Michael, NL and Montefiori, DC and Liao, HX and Haynes, BF and Tomaras, GD},
title={Vaccine-induced $\mbox{IgG}$ antibodies to $\mbox{V1V2}$ regions of multiple $\mbox{HIV-1}$ subtypes correlate with decreased risk of $\mbox{HIV-1}$ infection.},
journal={PLoS One},
year={2014},
volume={9},
pages={e87572}
}

@article{ZollaPazneretal2014short,
author={Zolla-Pazner, S and DeCamp, A and Gilbert, Peter B et al.},
title={Vaccine-induced $\mbox{IgG}$ antibodies to $\mbox{V1V2}$ regions of multiple $\mbox{HIV-1}$ subtypes correlate with decreased risk of $\mbox{HIV-1}$ infection.},
journal={PLoS One},
year={2014},
volume={9},
pages={e87572}
}

@article{cai2004sample,
  title={Sample size/power calculation for case--cohort studies},
  author={Cai, Jianwen and Zeng, Donglin},
  journal={Biometrics},
  volume={60},
  number={4},
  pages={1015--1024},
  year={2004},
  publisher={Wiley Online Library}
}


@article{dupont1990power,
  title={Power and sample size calculations: a review and computer program},
  author={Dupont, William D and Plummer Jr, Walton D},
  journal={{Controlled Clinical Trials}},
  volume={11},
  number={2},
  pages={116--128},
  year={1990},
  publisher={Elsevier}
}

@article{garcia1999power,
  title={Power and sample size calculations in case-control studies of gene-environment interactions: comments on different approaches.},
  author={Garc{\'\i}a-Closas, Montserrat and Lubin, Jay H},
  journal={{American Journal of Epidemiology}},
  volume={149},
  number={8},
  pages={689--692},
  year={1999}
}



@article{ZollaPazneretal2014short,
author={Zolla-Pazner, S and DeCamp, A and Gilbert, Peter B and et al.}, 
title={Vaccine-induced $\mbox{IgG}$ antibodies to $\mbox{V1V2}$ regions of multiple $\mbox{HIV-1}$ subtypes correlate with decreased risk of $\mbox{HIV-1}$ infection.},
journal={PLoS One},
year={2014},
volume={9},
pages={e87572}
}


@article{LiGilbertetal2014,
author={Li, Shuying S and Gilbert, Peter B and Tomaras, Georgia D and Kijak, Gustavo and Ferrari, Guido and Thomas, Rasmi and Zolla-Pazner, Susan and Evans, David T and Yao, Li and Gottardo, Raphael and Dai, James Y and Janes, Holly E and Morris, Daryl and Fong, Youyi and Edlefsen, PT and Li, Fusheng and Magaret, Craig A and Frahm, Nicole and Alpert, Michael D and Rerks-Ngarm, Supachai and Pitisuttithum, Punnee and Kaewkungwal, Jaranit and Nitayaphan, Sorachai and Robb, Merlin L and O'Connell, Robert J and Michael, Nelson L and Kim, Jerome H and McElrath, M Juliana and Geraghty, Daniel E}, 
title={{FCGR2C} polymorphisms associate with {HIV-1} vaccine protection in {RV144} trial},
journal={Journal of Clinical Investigation},
year={2014},
volume={124},
pages={3879--3890},
note={$^*$Contributed equally. PMCID: PMC4151214}
}

@article{GenomesProject2012,
author={Genomes Project Consortium, 1000 and Abecasis, GR and Auton, A and Brooks, LD and DePristo, MA and Durbin, RM and
Handsaker, RE and Kang, HM and Marth, GT and McVean, GA},
title={An integrated map of
genetic variation from 1,092 human genomes.},
journal={Nature},
year={2012},
volume={491},
pages={59--65}
}

@article{Staessenetal2005,
author={Staessen, JA and Yan, L and Lutgarde, T and Wang, J-G}, 
title={Blood Pressure Reduction and Cardiovascular Prevention: An Update Including the 2003--2004 Secondary Prevention Trials.},
journal={Hypertension Research},
year={2005},
volume={28},
pages={385--407}
}

@article{fleming2011some,
  title={Some essential considerations in the design and conduct of non-inferiority trials},
  author={Fleming, Thomas R and Odem-Davis, Katherine and Rothmann, Mark D and Shen, Yuan Li},
  journal={Clinical Trials},
  volume={8},
  number={4},
  pages={432--439},
  year={2011},
  publisher={SAGE Publications}
}

@article{Grayetal2014,
  title={Recombinant adenovirus type 5 {HIV} gag/pol/nef vaccine in {South Africa}: unblinded, long-term follow-up of the phase 2b {HVTN 503/Phambili} study},
  author={Gray, Glenda E and Moodie, Zoe and Metch, Barbara and Gilbert, Peter B and Bekker, Linda-Gail and Churchyard, Gavin and Nchabeleng, Maphoshane and Mlisana, Koleka and Laher, Fatima and Roux, Surita and Corey, L},
  journal={The Lancet Infectious Diseases},
  volume={14},
  number={5},
  pages={388--396},
  year={2014},
  publisher={Elsevier}
}

@article{Grayetal2014short,
  title={Recombinant adenovirus type 5 {HIV} gag/pol/nef vaccine in {South Africa}: unblinded, long-term follow-up of the phase 2b {HVTN 503/Phambili} study},
  author={Gray, Glenda E and Moodie, Zoe and Metch, Barbara and Gilbert, Peter B and Bekker, Linda-Gail and Churchyard, Gavin and et al.},
  journal={The Lancet Infectious Diseases},
  volume={14},
  number={5},
  pages={388--396},
  year={2014},
  publisher={Elsevier}
}


@article{UNAIDS2013,
  author =       {UNAIDS},
  title =        {Global Report: {R}eport on the global AIDS epidemic 2013.},
  journal =      {UNAIDS Global Report},
  year =         {2013},
  volume =       {UNAIDS/JC2502/1/E}
}

@article{UNAIDS2019,
  author =       {UNAIDS},
  title =        {{Global HIV and AIDS Statistics} - 2019 fact sheet},
  journal =      {UNAIDS Global Report},
  year =         {},
  volume = {},
  note = {http://www.unaids.org/en/resources/fact-sheet. Accessed 7 Aug, 2019}
}

@article{GrahamAmbrosino2015,
  title={History of passive antibody administration for prevention and treatment of infectious diseases.},
  author={Graham, BS and Ambrosino, DM},
  journal={Current Opinion in HIV and AIDS},
  volume={10},
  pages={129--134},
  year={2015}
}

@article{Wuetal2010,
  title={Rational design of envelope identifies broadly neutralizing human monoclonal antibodies to {HIV-1}.},
  author={Wu, X and Yang, ZY and Li, Y and Hogerkorp, CM and Schief, WR and
 Seaman, MS and Zhou, T and Schmidt, SD and Wu, L and Xu, L and Longo, NS and McKee, K and O'Dell, S and Louder, MK and Wycuff, DL and Feng, Y and Nason, M and
 Doria-Rose, N and Connors, M and Kwong, PD and Roederer, M and Wyatt, RT and Nabel, GJ and Mascola, JR.},
  journal={Science},
  volume={329},
  pages={856--861},
  year={2010}
}

@article{Georgievetal2013,
  title={Elicitation of {HIV-1}-neutralizing antibodies against the {CD4}-binding site.},
  author={Georgiev, IS and Gordon, JM and Zhou, T and Kwong, PD},
  journal={Current Opinion in HIV and AIDS},
  volume={8},
  pages={382--392},
  year={2013}
}

@article{Montefiori2014,
  title={Importance of neutralization sieve analyses when seeking correlates of {HIV-1} vaccine efficacy.},
  author={Montefiori, DC},
  journal={Human Vaccine Immunotherapy},
  volume={10(8)},
  pages={2507--2511},
  year={2014}
}

@book{Wu2009,
  title={{Mixed Effects Models for Complex Data}},
  author={Wu, Lang},
  year={2009},
  publisher={CRC Press}
}



@article{krause1981restless,
  title={The restless tide: the persistent challenge of the microbial world},
  author={Krause, Richard M},
  journal={Washington, DC},
  year={1981}
}

@book{janeway1997immunobiology,
  title={Immunobiology: the immune system in health and disease},
  author={Janeway, Charles A and Travers, Paul and Walport, Mark and Shlomchik, Mark J},
  volume={1},
  year={1997},
  publisher={Current Biology}
}

@book{sompayrac2015immune,
  title={How the immune system works},
  author={Sompayrac, Lauren M},
  year={2015},
  publisher={John Wiley \& Sons}
}


@book{de2002microbe,
  title={Microbe hunters},
  author={De Kruif, Paul},
  year={2002},
  publisher={Houghton Mifflin Harcourt}
}


@article{lewis1990arrowsmith,
  title={Arrowsmith},
  author={Lewis, Sinclair},
  year={1990}
}

@article{nason2010design,
  title={Design and analysis of crossover trials for absorbing binary endpoints},
  author={Nason, Martha and Follmann, Dean},
  journal={Biometrics},
  volume={66},
  number={3},
  pages={958--965},
  year={2010},
  publisher={Wiley Online Library}
}


@article{sarzotti2014optimization,
  title={Optimization and validation of the TZM-bl assay for standardized assessments of neutralizing antibodies against HIV-1},
  author={Sarzotti-Kelsoe, Marcella and Bailer, Robert T and Turk, Ellen and Lin, Chen-li and Bilska, Miroslawa and Greene, Kelli M and Gao, Hongmei and Todd, Christopher A and Ozaki, Daniel A and Seaman, Michael S and others},
  journal={Journal of immunological methods},
  volume={409},
  pages={131--146},
  year={2014},
  publisher={Elsevier}}



@article{gilbert2010magnitude,
  title={Magnitude and breadth of a nonprotective neutralizing antibody response in an efficacy trial of a candidate HIV-1 gp120 vaccine},
  author={Gilbert, Peter and Wang, Maggie and Wrin, Terri and Petropoulos, Chris and Gurwith, Marc and Sinangil, Faruk and D'Souza, Patricia and Rodriguez-Chavez, Isaac R and DeCamp, Allan and Giganti, Mike and others},
  journal={Journal of Infectious Diseases},
  volume={202},
  number={4},
  pages={595--605},
  year={2010},
  publisher={Oxford University Press}
}

@article{nason2006patterns,
  title={Patterns of immune response to a vaccine or virus as measured by intracellular cytokine staining in flow cytometry: hypothesis generation and comparison of groups},
  author={Nason, M},
  journal={Journal of biopharmaceutical statistics},
  volume={16},
  number={4},
  pages={483--498},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{finak2013mixture,
  title={Mixture models for single-cell assays with applications to vaccine studies},
  author={Finak, Greg and McDavid, Andrew and Chattopadhyay, Pratip and Dominguez, Maria and De Rosa, Steve and Roederer, Mario and Gottardo, Raphael},
  journal={Biostatistics},
  pages={1-15},
  year={2013},
  publisher={Biometrika Trust}
}

@article{swihart2017smfa,
  title={Statistical methods for standard membrane-feeding assays to measure transmission blocking or reducing activity in malaria},
  author={Swihart, Bruce and Fay, Michael and Kazutoyo Miura},
  journal={Working Draft},
  pages={1-20},
  year={2017},
  publisher={Working Draft}
}

@article{hu2015two,
  title={Two-part test of vaccine effect},
  author={Hu, Zonghui and Proschan, Michael},
  journal={Statistics in medicine},
  volume={34},
  number={11},
  pages={1904--1911},
  year={2015},
  publisher={Wiley Online Library}
}


@article{meier1990polio,
  title={Polio trial: an early efficient clinical trial},
  author={Meier, Paul},
  journal={Statistics in medicine},
  volume={9},
  number={1-2},
  pages={13--16},
  year={1990},
  publisher={Wiley Online Library}
}


@article{meier1972biggest,
  title={The biggest public health experiment ever: the 1954 field trial of the Salk poliomyelitis vaccine},
  author={Meier, Paul and others},
  journal={Statistics: a guide to the unknown. San Francisco: Holden-Day},
  pages={2--13},
  year={1972}
}


@article{wang2006statistical,
  title={Statistical considerations for noninferiority/equivalence trials in vaccine development},
  author={Wang, WWB and Mehrotra, DV and Chan, ISF and Heyse, JF},
  journal={Journal of biopharmaceutical statistics},
  volume={16},
  number={4},
  pages={429--441},
  year={2006},
  publisher={Taylor \& Francis}
}

@misc{wang2003encyclopedia,
  title={Vaccine clincial trials.  Encyclopedia of Biopharmaceutical Statistics},
  author={Chan, I and Wang, W and Heyse, J.},
  pages={1005-1019},
  year={2003},
  publisher={Taylor \& Francis}
}


@article{lachenbruch1998sensitivity,
  title={Sensitivity, specificity, and vaccine efficacy},
  author={Lachenbruch, Peter A},
  journal={Controlled clinical trials},
  volume={19},
  number={6},
  pages={569--574},
  year={1998},
  publisher={Elsevier}
}

@article{halloran2001using,
  title={Using validation sets for outcomes and exposure to infection in vaccine field studies},
  author={Halloran, M Elizabeth and Longini, Ira M},
  journal={American Journal of Epidemiology},
  volume={154},
  number={5},
  pages={391--398},
  year={2001},
  publisher={Oxford Univ Press}
}


@article{gart1985approximate,
  title={Approximate tests and interval estimation of the common relative risk in the combination of 2$\times$ 2 tables},
  author={Gart, John J},
  journal={Biometrika},
  volume={72},
  number={3},
  pages={673--677},
  year={1985},
  publisher={Biometrika Trust}
}


@article{farrington1990test,
  title={Test statistics and sample size formulae for comparative binomial trials with null hypothesis of non-zero risk difference or non-unity relative risk},
  author={Farrington, Conor P and Manning, Godfrey},
  journal={Statistics in medicine},
  volume={9},
  number={12},
  pages={1447--1454},
  year={1990},
  publisher={Wiley Online Library}
}

@article{blackwelder1993sample,
  title={Sample size and power for prospective analysis of relative risk},
  author={Blackwelder, William C},
  journal={Statistics in medicine},
  volume={12},
  number={7},
  pages={691--698},
  year={1993},
  publisher={Wiley Online Library}
}

@article{chan1998exact,
  title={Exact power and sample size for vaccine efficacy studies},
  author={Chan, Ivan SF and Bohidar, Norman R},
  journal={Communications in Statistics-Theory and Methods},
  volume={27},
  number={6},
  pages={1305--1322},
  year={1998},
  publisher={Taylor \& Francis}
}


@article{fay2012anthrax,
  title={Anthrax vaccine--induced antibodies provide cross-species prediction of survival to aerosol challenge},
  author={Fay, Michael P and Follmann, Dean A and Lynn, Freyja and Schiffer, Jarad M and Stark, Gregory V and Kohberger, Robert and Quinn, Conrad P and Nuzum, Edwin O},
  journal={Science translational medicine},
  volume={4},
  number={151},
  pages={151ra126--151ra126},
  year={2012},
  publisher={American Association for the Advancement of Science}
}


@article{farrington1993estimation,
  title={Estimation of vaccine effectiveness using the screening method},
  author={Farrington, CP},
  journal={International journal of epidemiology},
  volume={22},
  number={4},
  pages={742--746},
  year={1993},
  publisher={IEA}
}


@article{jackson2013test,
  title={The test-negative design for estimating influenza vaccine effectiveness},
  author={Jackson, Michael L and Nelson, Jennifer C},
  journal={Vaccine},
  volume={31},
  number={17},
  pages={2165--2168},
  year={2013},
  publisher={Elsevier}
}


@article{ohmit2014influenza,
  title={Influenza vaccine effectiveness in the 2011--2012 season: protection against each circulating virus and the effect of prior vaccination on estimates},
  author={Ohmit, Suzanne E and Thompson, Mark G and Petrie, Joshua G and Thaker, Swathi N and Jackson, Michael L and Belongia, Edward A and Zimmerman, Richard K and Gaglani, Manjusha and Lamerato, Lois and Spencer, Sarah M and others},
  journal={Clinical infectious diseases},
  volume={58},
  number={3},
  pages={319--327},
  year={2014},
  publisher={Oxford University Press}
}

@article{ross1916application,
  title={An application of the theory of probabilities to the study of a priori pathometry. Part I},
  author={Ross, Ronald},
  journal={Proceedings of the Royal Society of London. Series A, Containing papers of a mathematical and physical character},
  volume={92},
  number={638},
  pages={204--230},
  year={1916},
  publisher={JSTOR}
}



@article{loeb2010effect,
  title={Effect of influenza vaccination of children on infection rates in Hutterite communities: a randomized trial},
  author={Loeb, Mark and Russell, Margaret L and Moss, Lorraine and Fonseca, Kevin and Fox, Julie and Earn, David JD and Aoki, Fred and Horsman, Gregory and Van Caeseele, Paul and Chokani, Khami and others},
  journal={Jama},
  volume={303},
  number={10},
  pages={943--950},
  year={2010},
  publisher={American Medical Association}
}

@article{son2011vibriocidal,
  title={Vibriocidal assays to determine the antibody titer of patient sera samples},
  author={Son, Mike S and Taylor, Ronald K},
  journal={Current protocols in microbiology},
  pages={6A--3},
  year={2011},
  publisher={Wiley Online Library}
}

@article{hussey2007design,
  title={Design and analysis of stepped wedge cluster randomized trials},
  author={Hussey, Michael A and Hughes, James P},
  journal={Contemporary clinical trials},
  volume={28},
  number={2},
  pages={182--191},
  year={2007},
  publisher={Elsevier}
}

@article{fay2012package,
  title={Package �saws�},
  author={Fay, Michael P and Fay, Maintainer Michael P and Suggests, MASS},
  year={2012}
}

@article{fay2001small,
  title={Small-Sample Adjustments for Wald-Type Tests Using Sandwich Estimators},
  author={Fay, Michael P and Graubard, Barry I},
  journal={Biometrics},
  volume={57},
  number={4},
  pages={1198--1206},
  year={2001},
  publisher={Wiley Online Library}
}


@article{gambia1987gambia,
  title={The Gambia hepatitis intervention study},
  author={Gambia Hepatitis Study Group and others},
  journal={Cancer Research},
  volume={47},
  number={21},
  pages={5782--5787},
  year={1987},
  publisher={AACR}
}

@article{kennedy2016implementation,
  title={Implementation of an Ebola virus disease vaccine clinical trial during the Ebola epidemic in Liberia: Design, procedures, and challenges},
  author={Kennedy, Stephen B and Neaton, James D and Lane, H Clifford and Kieh, Mark WS and Massaquoi, Moses BF and Touchette, Nancy A and Nason, Martha C and Follmann, Dean A and Boley, Fatorma K and Johnson, Melvin P and others},
  journal={Clinical Trials},
  pages={1740774515621037},
  year={2016},
  publisher={SAGE Publications}
}

@article{henao2015efficacy,
  title={Efficacy and effectiveness of an rVSV-vectored vaccine expressing Ebola surface glycoprotein: interim results from the Guinea ring vaccination cluster-randomised trial},
  author={Henao-Restrepo, Ana Maria and Longini, Ira M and Egger, Matthias and Dean, Natalie E and Edmunds, W John and Camacho, Anton and Carroll, Miles W and Doumbia, Moussa and Draguez, Bertrand and Duraffour, Sophie and others},
  journal={The Lancet},
  volume={386},
  number={9996},
  pages={857--866},
  year={2015},
  publisher={Elsevier}
}

@article{henao2015ring,
  title={The ring vaccination trial: a novel cluster randomised controlled trial design to evaluate vaccine efficacy and effectiveness during outbreaks, with special reference to Ebola},
  author={Henao-Restrepo, Ana Maria},
  journal={BMJ-BRITISH MEDICAL JOURNAL},
  volume={351},
  year={2015},
  publisher={BMJ PUBLISHING GROUP BRITISH MED ASSOC HOUSE, TAVISTOCK SQUARE, LONDON WC1H 9JR, ENGLAND}
}

@article{smith1984assessment,
  title={Assessment of the protective efficacy of vaccines against common diseases using case-control and cohort studies},
  author={Smith, PG and Rodrigues, LC and Fine, PEM},
  journal={International journal of epidemiology},
  volume={13},
  number={1},
  pages={87--93},
  year={1984},
  publisher={IEA}
}

@article{struchiner1990behaviour,
  title={The behaviour of common measures of association used to assess a vaccination programme under complex disease transmission patterns�a computer simulation study of malaria vaccines},
  author={Struchiner, Claudio J and HALLORAN, MARY ELIZABETH and Robins, James M and Spielman, Andrew},
  journal={International journal of epidemiology},
  volume={19},
  number={1},
  pages={187--196},
  year={1990},
  publisher={IEA}
}



@article{halloran1991direct,
  title={Direct and indirect effects in vaccine efficacy and effectiveness},
  author={Halloran, M Elizabeth and Haber, Michael and Longini, Ira M and Struchiner, Claudio J},
  journal={American Journal of Epidemiology},
  volume={133},
  number={4},
  pages={323--331},
  year={1991},
  publisher={Oxford Univ Press}
}

@article{halloran1991study,
  title={Study designs for dependent happenings.},
  author={Halloran, M Elizabeth and Struchiner, Claudio J},
  journal={Epidemiology},
  volume={2},
  number={5},
  pages={331--338},
  year={1991},
  publisher={LWW}
}

@article{follmann2015incorporating,
  title={Incorporating founder virus information in vaccine field trials},
  author={Follmann, Dean and Huang, Chiung-Yu},
  journal={Biometrics},
  volume={71},
  number={2},
  pages={386--396},
  year={2015},
  publisher={Wiley Online Library}
}

@article{Neafseyetal2015,
  title={Genetic diversity and protective efficacy of the {RTS,S/AS01} malaria vaccine},
  author={Neafsey, Daniel E and Juraska, Michal and Bedford, Trevor and Benkeser, David and Valim, Clarissa and Griggs, Allison and Lievens, Marc and Abdulla, Salim and Adjei, Samuel and Agbenyega, Tsiri and Agnandji, Selidji T and Aide, Pedro and Anderson, Scott and Ansong, Daniel and Aponte, John J and Asante, Kwaku Poku and Bejon, Philip and Birkett, Ashley J and Bruls, Myriam and Connolly, Kristen M and D'Alessandro, Umberto and Doba{\~n}o, Carlota and Gesase, Samwel and Greenwood, Brian and Grimsby, Jonna and Tinto, Halidou and Hamel, Mary J and Hoffman, Irving and Kamthunzi, Portia and Kariuki, Simon and Kremsner, Peter G and Leach, Amanda and Lell, Bertrand and Lennon, Niall J and Lusingu, John and Marsh, Kevin and Martinson, Francis and Molel, Jackson T and Moss, Eli L and Njuguna, Patricia and Ockenhouse, Christian F and Ogutu, Bernhards Ragama and Otieno, Walter and Otieno, Lucas and Otieno, Kephas and Owusu-Agyei, Seth and Park, Daniel J and Pell\'e , Karell and Robbins, Dana and Russ, Carsten and Ryan, Elizabeth M and Sacarlal, Jahit and Sogoloff, Brian and Sorgho, Hermann and Tanner, Marcel and Theander, Thor and Valea, Innocent and Volkman, Sarah K and Yu, Qing and Lapierre, Didier and Birren, Bruce W and Gilbert, Peter B and Wirth, Dyann F},
  journal={New England Journal of Medicine},
  volume={373},
  number={21},
  pages={2025--2037},
  year={2015},
  publisher={Mass Medical Soc},
  note={PMCID:
    PMC4762279}
}

@article{BenkeserCaroneGilbert2018,
  title={Improved estimation of the cumulative incidence of rare outcomes.},
  author={Benkeser, D and Carone, M and Gilbert, Peter B},
  journal={Statistics in Medicine},
  volume={37},
  number={2},
  pages={280--293},
  year={2018},
 note={PMCID:
    PMC5735003}
}

@article{Tsiatis2004,
  title={Joint modeling of longitudinal and time-to-event data: an overview},
  author={Tsiatis, A and Davidian, M},
  journal={Statistica Sinica},
  volume={14},
  number={},
  pages={809--834},
  year={2004}
}

@article{Wu2012,
  title={Analysis of longitudinal and survival data: joint modeling, inference methods, and issues},
  author={Wu, L and Liu, W and Yi, G and Huang, Y},
  journal={Journal of Probability
and Statistics},
  volume={doi:10.1155/2012/640153},
  number={},
  pages={},
  year={2012}
}

@article{McCrink2013,
  title={Advances in joint modelling: a review of recent developments with application to the survival of end stage renal disease patients},
  author={McCrink, LM and Marshall, AH and Cairns, KJ},
  journal={International Statistical Review },
  volume={81},
  number={2},
  pages={249--269},
  year={2013}
}

@article{friesen2010new,
  title={New class of monoclonal antibodies against severe influenza: prophylactic and therapeutic efficacy in ferrets},
  author={Friesen, Robert HE and Koudstaal, Wouter and Koldijk, Martin H and Weverling, Gerrit Jan and Brakenhoff, Just PJ and Lenting, Peter J and Stittelaar, Koert J and Osterhaus, Albert DME and Kompier, Ronald and Goudsmit, Jaap},
  journal={PLos One},
  volume={5},
  number={2},
  pages={e9106},
  year={2010},
  publisher={Public Library of Science},
  note={PMCID:
    PMC2817000
}
}

@article{simmons2007prophylactic,
  title={Prophylactic and therapeutic efficacy of human monoclonal antibodies against {H5N1} influenza},
  author={Simmons, Cameron P and Bernasconi, Nadia L and Suguitan Jr, Amorsolo L and Mills, Kimberly and Ward, Jerrold M and Chau, Nguyen Van Vinh and Hien, Tran Tinh and Sallusto, Federica and Farrar, Jeremy and De Jong, Menno D and Lanzavecchia, Antonio and Subbarao, Kanta},
  journal={PLoS Medicine},
  volume={4},
  number={5},
  pages={e178},
  year={2007},
  publisher={Public Library of Science},
  note={PMCID:
    PMC1880850
}
}

@article{Lin2000,
  title={On fitting {Cox's} proportional hazards models to survey data.},
  author={Lin, DY},
  journal={Biometrika},
  volume={87},
  number={1},
  pages={37--47},
  year={2000}
}

@article{zeitlin2000preventing,
  title={Preventing infectious disease with passive immunization},
  author={Zeitlin, Larry and Cone, Richard A and Moench, Thomas R and Whaley, Kevin J},
  journal={Microbes and Infection},
  volume={2},
  number={6},
  pages={701--708},
  year={2000},
  publisher={Elsevier}
}

@article{groothuis2002prevention,
  title={Prevention of respiratory syncytial virus infections in high-risk 
infants by monoclonal antibody (palivizumab)},
  author={Groothuis, Jessie R and Nishida, Hiroshi},
  journal={Pediatrics International},
  volume={44},
  number={3},
  pages={235--241},
  year={2002},
  publisher={Wiley Online Library}
}

@article{meissner1999immunoprophylaxis,
  title={Immunoprophylaxis with palivizumab, a humanized respiratory syncytial virus monoclonal antibody, for prevention of respiratory syncytial virus infection in high risk infants: a consensus opinion},
  author={Meissner, H Cody and Welliver, Robert C and Chartrand, Stephan A and Law, Barbara J and Weisman, Leonard E and Dorkin, Henry L and Rodriguez, William J},
  journal={The Pediatric Infectious Disease Journal},
  volume={18},
  number={3},
  pages={223--231},
  year={1999},
  publisher={LWW}
}


@article{BenkeserJuraskaGilbert2019,
  title={Assessing Trends in Vaccine Efficacy by Pathogen Genetic Distance.},
  author={Benkeser, D and Juraska, M and Gilbert, Peter B},
  journal={French Royal Statistical Society},
  volume={},
  number={},
  pages={},
  year={2018}
}

@article{Donovanetal2019,
  title={Nonparametric inference for immune response thresholds of risk in vaccine studies.},
  author={Donovan, K and Hudgens, M and Gilbert, Peter B.},
  journal={Annals of Applied Statistics},
volume={13},
  number={2},
  pages={1147--1165},
  year={2019},
  publisher={Institute of Mathematical Statistics},
  note={PMCID:
    PMC6613658
    Delayed release (embargo): [Available on 2020-06-01]}}


@article{GilbertHuangetal2019,
  title={Bridging efficacy of a tetravalent dengue vaccine from 
children/adolescents to adults in high endemic countries based 
on neutralizing antibody response.},
  author={Gilbert, Peter B and Huang, Y and Juraska, MJ and Moodie, Z and Fong, Y 
and Luedtke, AR and Zhuang, Y and Shao, J and Carpp, LN and Jackson, N and 
Chambonneau, L and Bouckenooghe, A and Zambrano, B and Frago, C and 
Pallardy, S and Noriega, F},
  journal={American Journal of Tropical Medicine and Hygiene},
  year={2019},
volume = {101},
   number = {1},
   pages = {164-179},
   doi = {https://doi.org/10.4269/ajtmh.18-0534},
   note= {PMCID:
    PMC6609170
   [Delayed release (embargo): Available on 2020-07-01]}
}

@article{BenkeserGilbertCarone2019b,
  title={Estimating and Testing Vaccine Sieve Effects Using Machine Learning},
  author={Benkeser, David and Gilbert, Peter B and Carone, Marco},
  journal={Journal of the American Statistical Association},
  pages={1--12},
  year={2019},
  publisher={Taylor \& Francis}
}

@article{follmann2003multiple,
  title={Multiple outputation: inference for complex clustered data by averaging analyses from independent data},
  author={Follmann, Dean and Proschan, Michael and Leifer, Eric},
  journal={Biometrics},
  volume={59},
  number={2},
  pages={420--429},
  year={2003},
  publisher={Wiley Online Library}
}

@article{hoffman2001within,
  title={Within-cluster resampling},
  author={Hoffman, Elaine B and Sen, Pranab K and Weinberg, Clarice R},
  journal={Biometrika},
  volume={88},
  number={4},
  pages={1121--1134},
  year={2001},
  publisher={Biometrika Trust}
}


@article{gilbert1998statistical,
  title={Statistical methods for assessing differential vaccine protection against human immunodeficiency virus types},
  author={Gilbert, Peter B and Self, Steven G and Ashby, Mark A},
  journal={Biometrics},
  pages={799--814},
  year={1998},
  publisher={JSTOR}
}

@article{BurtonHangartner2016,
  title={Broadly neutralizing antibodies to {HIV} and their role in vaccine design},
  author={Burton, Dennis R and Hangartner, Lars},
  journal={Annual Review of Immunology},
  volume={34},
  pages={635--659},
  year={2016},
  publisher={Annual Reviews}
}

@article{Gilbertetal2017short,
author={Gilbert, Peter B and Juraska, M and deCamp, A and Karuna, S and Edupuganti, S and Mgodi, N and Donnell, D and et al.},
title={Basis and statistical design of the passive {HIV-1} antibody mediated prevention ({AMP}) test-of-concept efficacy trials},
journal={Statistical Communications in Infectious Diseases},
year={2017},
volume={9;1}
}

@article{Gilbertetal2017,
author={Gilbert, Peter B and Juraska, M and deCamp, A and Karuna, S and Edupuganti, S and Mgodi, N and Donnell, D and Bentley, C and Sista, N and Andrew, P and Isaacs, A and 
Huang, Y and Zhang, L and Capparelli, E and Kochar, N and Wang, J and Eshleman, S and Mayer, K and Magaret, C and Hural, J and Kublin, J and Gray, G and Montefiori, D and Gomez, M and Burns, D and McElrath, MJ and Ledgerwood, J and Graham, B and Mascola, J and Cohen, M and Corey, L},
title={Basis and statistical design of the passive {HIV-1} {Antibody Mediated Prevention} ({AMP}) test-of-concept efficacy trials},
journal={Statistical Communications in Infectious Diseases},
year={2017},
volume={9;1},
note={PMCID:
    PMC5714515}
}

@article{PriceGilbertvanderLaan2018,
  title={Estimation of the optimal surrogate based on a randomized trial},
  author={Price, Brenda L and Gilbert, Peter B and van der Laan, Mark J},
  journal={Biometrics},
  volume={74},
  number={4},
  pages={1271--1281},
  year={2018},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC6393111}
}

@article{Huangetal2017,
author={Huang, Y and Zhang, L and Ledgerwood, J and Gruneberg, N and Bailer, R and Isaacs, A and Seaton, K and Mayer, KH and Capparelli, E and Corey, L and Gilbert, Peter B.},
title={Population pharmacokinetics analysis of {VRC01}, a broadly neutralizing {HIV-1} monoclonal antibody, in healthy adults.},
journal={mAbs},
year={2017},
volume={9(5)},
pages={792--800},
note={PMCID: PMC5524155}
}

@article{Rossenkhanetal2018,
title={Coupling Gold Standard Datasets and Statistical Methods to Improve {HIV-1} Infection Time and Founder Multiplicity Estimates toward towards Improved Vaccine Efficacy Assessment.},
author={Rossenkhan, R and Rolland, M and Labuschagne, P and Magaret, CA and Carpp, LN and Huang, Y and Rudnicki, EE and Zhang, L and Ndabambi, N and Logan, M and Holzman, T and Abrahams, MR and Anthony, C and Tovanabutra, S and Warth, C and Botha, G and Matten, D and Nitayaphan, S and Rono, K and Sekiziyivu, A and Michael, N and Chopera, D and Eller, LA and Matsen IV, FA and Travers, S and Poon, A and Robb, ML and Williamson, C and Gilbert, Peter B and Edlefsen, PT},
journal={submitted},
year={2018}
}

@article{Rossenkhanetal2019,
title={Combining Viral Genetics and Statistical Modeling to Improve {HIV-1} 
Time-of-infection Estimation towards Enhanced Vaccine Efficacy Assessment},
author={Rossenkhan, R and Rolland, M and Labuschagne, JPL and Ferreira, RC and
 Magaret, CA and Carpp, LN and Matsen IV, FA and Huang, Y and Rudnicki, EE 
and Zhang, Y and Ndabambi, N and Logan, M and Holzman, T and Abrahams, M-R and
Anthony, C and Tovanabutra, S and Warth, C and Botha, G and Matten, D and
Nitayaphan, S and Kibuuka, H and Sawe, FK and Chopera, D and Eller, LA and
Travers, S and Robb, ML and Williamson, C and Gilbert, Peter B and Edlefsen, PT},
journal={Viruses},
year={2019},
volume={11},
pages={607},
note={PubMed PMID: 31277299. PMCID: PMC Journal –- In Process.}
}

@article{Janesetal2015,
  title={{HIV-1} infections with multiple founders are associated with higher viral loads than infections with single founders},
  author={Janes, Holly and Herbeck, Joshua T and Tovanabutra, Sodsai and Thomas, Rasmi and Frahm, Nicole and Duerr, Ann and Hural, John and Corey, Lawrence and Self, Steve G and Buchbinder, Susan P and
  McElrath, Juliana M and O'Connell, Robert J  and Paris, Robert M and Rerks-Ngarm, Supachai and Nitayaphan, Sorachai  and  Pitisuttihum, Punnee and  Kaewkungwal, Jaranit and Robb, Merlin L and Michael,  Nelson L and Mullins, James I and Kim, Jerome H and Gilbert, Peter B and Rolland, Morgane},
  journal={Nature Medicine},
  volume={21},
  number={10},
  pages={1139},
  year={2015},
  publisher={Nature Publishing Group},
  note={PMCID: PMC4598284}
}

@article{Janesetal2017,
  title={Higher {T-cell} responses induced by {DNA/rAd5 HIV-1} preventive vaccine are associated with lower {HIV-1} infection risk in an efficacy trial},
  author={Janes, Holly E and Cohen, Kristen W and Frahm, Nicole and De Rosa, Stephen C and Sanchez, Brittany and Hural, John and Magaret, Craig A and Karuna, Shelly and Bentley, Carter and Gottardo, Raphael and Finak, Greg and Grove, Douglas and Shen, Mingchao and Graham, Berney S and Koup, Richard A and Mulligan, Mark J and Koblin, Beryl and Buchbinder, Susan P and Keefer, Michael C and Adams, Elizabeth and Anude, Chuka and Corey, Lawrence and Sobieszczyk, Magdalena and Hammer, Scott M and Gilbert, Peter B and McElrath, M Juliana},
  journal={The Journal of Infectious Diseases},
  volume={215},
  number={9},
  pages={1376--1385},
  year={2017},
  note={PMCID:
    PMC5853653}
}

@article{Janesetal2017short,
  title={Higher {T-cell} responses induced by {DNA/rAd5 HIV-1} preventive vaccine are associated with lower {HIV-1} infection risk in an efficacy trial},
  author={Janes, Holly E and Cohen, Kristen W and Frahm, Nicole and De Rosa, Stephen C and Sanchez, Brittany and Hural, John and Magaret, Craig A and et al.},
  journal={The Journal of Infectious Diseases},
  volume={215},
  number={9},
  pages={1376--1385},
  year={2017}
}

@article{Pasinetal2018,
  title={Periods of high dengue transmission defined by rainfall do not impact efficacy of dengue vaccine in regions of endemic disease.},
  author={Pasin, C and Halloran, ME and Gilbert, Peter B and Langevin, E and Ochiai, R and Pitisuttithum, P and Capeding, R and Carrasquilla, G and Frago, C and Cortes, M and Chambonneau, L and Moodie, Z},
  journal={PLoS One},
  volume={13},
  number={12},
  pages={e0207878},
  year={2018},
  note={PMCID: PMC6292612}
}


@article{Fongetal2018short,
  title={Modification of the Association Between {T}-Cell Immune Responses and Human Immunodeficiency Virus Type 1 Infection Risk by Vaccine-Induced Antibody Responses in the {HVTN 505} Trial},
  author={Fong,Y and Shen, X and Ashley, VC and Deal, A and Seaton, KE and Yu, C and Grant, Shannon SP and 
Ferrari, G and deCamp, A and Bailer, RT and Koup, RA and Montefiori, D and
 Haynes, BF
and Sarzotti-Kelsoe, M and Graham, BS and Carpp, LN and Hammer, SM and
 Sobieszczyk, M and Karuna, S 
and Swann, E and DeJesus, E and Mulligan, M and Frank, I and Buchbinder, S and
 Novak, RM and McElrath, MJ 
and Kalams, S and Keefer, M and Frahm, NA and Janes, HE and Gilbert, Peter B and 
Tomaras, GD},
  journal={Journal of Infectious Diseases},
  volume={217},
  number={8},
  pages={1280--1288},
  year={2018},
  note={PMCID:
    PMC6018910}
}

@article{Fongetal2018,
  title={Modification of the Association Between {T}-Cell Immune Responses and Human Immunodeficiency Virus Type 1 Infection Risk by Vaccine-Induced Antibody Responses in the {HVTN 505} Trial},
  author={Fong, Y and Shen, X and Ashley, VC and Deal, A and Seaton, KE and 
Yu, C and Grant, Shannon SP and 
Ferrari, G and deCamp, A and Bailer, RT and Koup, RA and Montefiori, D and
 Haynes, BF
and Sarzotti-Kelsoe, M and Graham, BS and Carpp, LN and Hammer, SM and
 Sobieszczyk, M and Karuna, S 
and Swann, E and DeJesus, E and Mulligan, M and Frank, I and Buchbinder, S and
 Novak, RM and McElrath, MJ 
and Kalams, S and Keefer, M and Frahm, NA and Janes, HE and Gilbert, Peter B and 
Tomaras, GD},
  journal={Journal of Infectious Diseases},
  volume={217},
  number={8},
  pages={1280--1288},
  year={2018},
  note={PMCID:
    PMC6018910}
}

@article{DeSouzaetal2016,
  title={Initiation of antiretroviral therapy during acute {HIV-1} infection leads to a high rate of nonreactive {HIV} serology},
  author={de Souza, Mark S and Pinyakorn, Suteeraporn and  Akapirat, Siriwat and Pattanachaiwit, Supanit and Fletcher, James LK and Chomchey, N and Kroon, ED and Ubolyam, S and Michael, NL and Robb, ML and Phanuphak, P and Kim, JH and Phanuphak, N and Ananworanich, J and {RV254/SEARCH010 Study Group}},
  journal={Reviews of Infectious Diseases},
  volume={63},
  number={4},
  pages={555--561},
  year={2016},
  publisher={Infectious Diseases Society of America}
}

@article{Keatingetal2016,
  title={Editorial Commentary: Timing Is Everything: Shortcomings of Current {HIV} Diagnostics in the Early Treatment Era},
  author={Keating, SM and Pilcher, CD and Busch, MP},
  journal={Clinical Infectious Diseases},
  volume={63},
  number={4},
  pages={562--564},
  year={2016},
  url={https://doi.org/10.1093/cid/ciw369},
  publisher={Infectious Diseases Society of America},
  note={https://doi.org/10.1093/cid/ciw369}
}

@Article{Mayeretal2017,
author =   {Kenneth H. Mayer and Kelly E. Seaton and Yunda Huang and Nicole Grunenberg and Abby Isaacs and Mary Allen and Julie E. Ledgerwood and Ian Frank and Magdalena E. Sobieszczyk and Lindsey R. Baden and Benigno Rodriguez and Hong Van Tieu and Georgia D. Tomaras and Aaron Deal and Derrick Goodman and Robert T. Bailer and Guido Ferrari and Ryan Jensen and John Hural and Barney S. Graham and John R. Mascola and Lawrence Corey and {David C. Montefiori  on behalf of the HVTN 104 Protocol Team and the NIAID HIV Vaccine Trials Network}},
title =    {Safety, pharmacokinetics, and immunological activities of multiple intravenous or subcutaneous doses of an anti-{HIV} monoclonal antibody, {VRC01}, administered to {HIV}-uninfected adults in a randomized trial},
journal =    {{PLoS} Medicine},
year =     {2017},
volume =   {14},
number={11},pages =    {e1002435},
note={PMCID:
    PMC5685476
}
}


@article{Mayeretal2017short,
  title={Safety, pharmacokinetics, and immunological activities of multiple intravenous or subcutaneous doses of an anti-HIV monoclonal antibody, VRC01, administered to HIV-uninfected adults: Results of a phase 1 randomized trial},
  author={Mayer, Kenneth H and Seaton, Kelly E and Huang, Yunda and Grunenberg, Nicole and Isaacs, Abby and Allen, Mary and Ledgerwood, Julie E and et al.},
  journal={PLoS Medicine},
  volume={14},
  number={11},
  pages={e1002435},
  year={2017},
  publisher={Public Library of Science}
}


 





@Article{Zhangetal2017,
author =   {Yuanyuan Zhang and Peter B. Gilbert and Edmund Capparelli and Yunda Huang},
title =    {Pharmacokinetics Simulations for Studying Correlates of Prevention Efficacy of Passive {HIV-1} Antibody Prophylaxis in the {Antibody Mediated Prevention (AMP)} Study},
journal =    {},
year =     {},
volume={arXiv:1801.08626 [q-bio.QM] [Preprint] 25 Jan 2018. Cited 3 Sep 2019. Available from https://arxiv.org/abs/1801.08626}
}

@Article{HuangZhangetal2018,
author =   {Yunda Huang and Yuanyuan Zhang and Zong Zhang and Peter B. Gilbert},
title =    {Generating survival times using {Cox} proportional hazards models with cyclic time-varying covariates, with application to a monoclonal antibody clinical trial},
journal =      {},
year =     {},
volume={arXiv:1801.08248 [stat.ME] [Preprint] 25 Jan 2018. Cited 3 Sep 2019. Available from https://arxiv.org/abs/1801.08248}
}

@article{Fauci2015,
  title={Ending the {HIV/AIDS} Pandemic-- Follow the Science},
  author={Fauci, AS and Marston, HD},
  journal={New England Journal of Medicine},
  volume={373},
  pages={2197--2199},
  year={2015},
  publisher={Mass Medical Soc}
}

@Article{DeatonReynoldsMyers1983,
   author =   {Deaton, M.L. and Reynolds, M.R. and Myers, R.H.},
   title =    {Estimation and Hypothesis Testing in Regression in the Presence of Nonhomogeneous Error Variance},
   journal =      {Communications in Statistics: Simulation and Computation},
   year =     {1983},
   volume =   {12},
   pages =    {45-66}
}

@Book{Williams1975,
  author =          {Williams, JS},
  ALTeditor =          {Srivastava, JN},
  title =          {Lower bounds on convergence rates of weighted least squares to best linear unbiased estimators. In: {A Survey of Statistical Design and Linear Models}},
  publisher =          {Academic Press},
  year =          {1975},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {pp. 555--570},
  OPTannote =          {}
}

 
@Article{Phambili_Gray2011,
   author =   {Gray GE, Allen M, Moodie Z, Churchyard G, Bekker LG, Nchabeleng M, Mlisana K, Metch B, de Bruyn G, Latka MH, Roux S, Mathebula M, Naicker N, Ducar C, Carter DK, Puren A, Eaton N, McElrath MJ, Robertson M, Corey L, Kublin JG, HVTN 503/Phambili study team},
   title =    {Safety and efficacy of the HVTN 503/Phambili study of a clade-B-based HIV-1 vaccine in South Africa: a double-blind, randomised, placebo-controlled test-of-concept phase 2b study},
   journal =      {Lancet Infect Dis.},
   year =     {2011},
   volume =   {11},
   pages =    {507-15},
}

@Article{Step_Buchbinder2008,
   author =   {Buchbinder SP, Mehrotra DV, Duerr A, Fitzgerald DW, Mogg R, Li D, Gilbert PB, Lama JR, Marmor M, Del Rio C, McElrath MJ, Casimiro DR, Gottesdiener KM, Chodakewitz JA, Corey L, Robertson MN, Step Study Protocol Team},
   title =    {Efficacy assessment of a cell-mediated immunity HIV-1 vaccine (the Step Study): a double-blind, randomised, placebo-controlled, test-of-concept trial},
   journal =      {Lancet},
   year =     {2008},
   volume =   {372},
   pages =    {1881-93},
}

@Article{GabrielDanielsHalloran2016,
   author =   {Gabriel EE, Daniels MJ, Halloran ME},
   title =    {Comparing biomarkers as trial level general surrogates},
   journal =      {Biometrics},
   year =     {2016},
   volume =   {72},
   pages =    {1046-1054}
}

@Article{GabrielSachsHalloran2017,
   author =   {Gabriel EE, Sachs MC, Halloran ME},
   title =    {Evaluation and comparison of predictive individual-level general surrogates},
   journal =      {Biostatistics},
   year =     {2017},
   volume =   {0},
   pages =    {1-18}
}

@Article{LuedtkeWu2018,
   author =   {Luedtke, AR and Wu, J},
   title =      {Efficient Principally Stratified Treatment Effect
Estimation in Crossover Studies with Absorptive Binary Endpoints},
   journal={arxiv},
year =     {2018},
   volume =   {1712.05835},
   pages =    {}
}

@Article{LuedtkeGilbert2017,
   author =   {Luedtke, AR and Gilbert, Peter B},
   title =      {Partial bridging of vaccine efficacy to new populations},
   journal={},
year =     {},
   volume =   {arXiv:1701.06739 [stat.ME] [Preprint] 24 Jan 2017. Cited 3 Sep 2019. Available from https://arxiv.org/abs/1701.06739}
}

@article{RJ-2016-046,
  author = {Michael C. Sachs and Erin E. Gabriel},
  title = {{An Introduction to Principal Surrogate Evaluation with the
          pseval Package}},
 year = {2016},
  journal = {{The R Journal}},
  url = {https://journal.r-project.org/archive/2016/RJ-2016-046/index.html},
  pages = {277--292},
  volume = {8},
  number = {2}
}


@article{HallRacineLi2004,
  author = {Hall, P and Racine, J and Li, Q},
    title = {Cross-validation and the estimation of conditional probability densities},
 year = {2004},
  journal = {Journal of the American Statistical Association},
  pages = {1015--1026},
  volume = {99}
}

@Article{Zhuangetal2019,
author = {Zhuang, YY and Huang, Y and Gilbert, PB},
title = {Evaluation of treatment effect modification by biomarkers measured pre- and post-randomization in the presence of non-monotone missingness},
journal={},
year={Submitted},
volume={},
}



@Article{Moodieetal2018,
author = {Moodie, Z and Juraska, M and Huang, Y and Zhuang, Y and Fong, Y and Carpp, LN and Self, SG and Chambonneau, L and Small, R and Jackson, N and Noriega, F and Gilbert, Peter B},
title = {Neutralizing antibody correlates analysis of tetravalent dengue vaccine efficacy trials in {Asia} and {Latin America}.},
journal={Journal of Infectious Diseases},
year={2018}
,volume={217(5)},pages={742--753},
note={PMCID:
    PMC5854020}
}

@Article{JuraskaGilbert2016,
author = {Juraska, M and Gilbert, Peter B},
title = {Mark-specific hazard ratio model with missing multivariate marks.},
journal={Lifetime Data Analysis},
year={2016},
volume={22},
number={4},
pages={606--625},
note={PMCID:
    PMC4848257}
}

@Article{JuraskaGilbert2016b,
author = {Juraska, M and Gilbert, Peter B},
title = {Nonparametric smoothing method for assessing effect modification by a post-randomization biomarker with application to vaccine efficacy trials.},
year={2016},
journal={Fred Hutch Technical Report},
volume={},
number={},
pages={}
}


@Article{YangSunQiGilbert2017,
author = {Yang, G and Sun, Y and Qi, L and Gilbert, Peter B},
title = {Estimation of Stratified Mark-Specific Proportional Hazards Models Under Two-Phase Sampling with Application to {HIV} Vaccine Efficacy Trials.},
journal={Statistical Biosciences},
year={2017},
volume={9},
pages={259--283},
note={PMCID:
    PMC5540271}
}

@article{LiGilbertetal2019,
  title={Fc gamma receptor polymorphisms modulated the vaccine effect on HIV-1 risk in the HVTN 505 HIV vaccine trial},
  author={Li, Shuying S and Gilbert, Peter B and Carpp, Lindsay N and Pyo, Chul-Woo and Janes, Holly and Fong, Youyi and Shen, Xiaoying and Neidich, Scott D and Goodman, Derrick and deCamp, Allan and others},
  journal={Journal of virology},
  volume={93},
  number={21},
  pages={e02041--18},
  year={2019},
  publisher={Am Soc Microbiol}
}


@Article{SunQiYangGilbert2018,
author = {Sun, Y and Qi, L and Yang, G and Gilbert, Peter B},
title = {Hypothesis tests for stratified mark-specific proportional hazards models with missing covariates, with application to {HIV} vaccine efficacy trials.},
year={2018},
journal={Biometrical Journal},
volume={60(3)},
pages={516--536},
note={PMCID:
    PMC6447062}
}


@article{Hertzetal2016,
title = "A study of vaccine-induced immune pressure on breakthrough infections in the {P}hambili phase 2b {HIV-1} vaccine efficacy trial",
journal = "Vaccine",
volume = "34",
number = "47",
pages = "5792 - 5801",
year = "2016",
issn = "0264-410X",
doi = "https://doi.org/10.1016/j.vaccine.2016.09.054",
url = "http://www.sciencedirect.com/science/article/pii/S0264410X16308805",
author = "T. Hertz and M.G. Logan and M. Rolland and C.A. Magaret and C. Rademeyer and A. Fiore-Gartland and P.T. Edlefsen and A. DeCamp and H. Ahmed and N. Ngandu and B.B. Larsen and N. Frahm and J. Marais and R. Thebus and D. Geraghty and J. Hural and L. Corey and J. Kublin and G. Gray and M.J. McElrath and J.I. Mullins and P.B. Gilbert and C. Williamson",
keywords = "HIV-1 vaccine, Phambili, Step, Sieve analysis, HVTN-503",
note="PMCID:
    PMC5309337"
}

@article{deCampetal2017,
author={deCamp, AC and Rolland, M and Edlefsen, PT and Sanders-Buell, E 
and Hall, B and Magaret, CA and Fiore-Gartland, AJ and Juraska, MJ and Carpp, LN and 
Karuna, ST and Bose, M and LePore, S and Miller, S and O'Sullivan,
A and Poltavee, K and Bai, H and Dommaraju, K and Zhao, H and Wong, K and
 Chen, L and Ahmed, H and
Gottardo, R and Koup, RA and Bailer, R and Mascola, JR and Graham, BS and 
Roederer, M and O'Connell, RJ and Michael, NL and Robb, ML and Adams, E and
 D'Souza, P and Kublin, J and Corey, L and Geraghty, DE and Frahm, N and 
Tomaras, GD and McElrath, MJ and Frenkel, L and 
Strychak, S and Tovanabutra, S and Sobieszczyk, M and Hammer, 
SM and Kim, JH and Mullins, JI and Gilbert, Peter B},
title={Sieve analysis of breakthrough {HIV-1} sequences in {HVTN} 505 identifies 
vaccine pressure targeting the {CD4} binding site of {E}nv-gp120},
journal={PLoS One},
year={2017},
volume={12},
number={11},
pages={e0185959},
note={PMCID:
    PMC5693417}
}
   
 @article{white2013relationship,
  title={{The relationship between RTS, S vaccine-induced antibodies, CD4+ T cell responses and protection against Plasmodium falciparum infection}},
  author={White, Michael T and Bejon, Philip and Olotu, Ally and Griffin, Jamie T and Riley, Eleanor M and Kester, Kent E and Ockenhouse, Christian F and Ghani, Azra C},
  journal={PloS One},
  volume={8},
  number={4},
  pages={e61395},
  year={2013},
  publisher={Public Library of Science},
  note={PMCID: PMC3628884}
}


@article{SunLiGilbert2016,
author={Sun, Y and Li, M and Gilbert, Peter B},
title={Goodness-of-fit test of the stratified mark-specific proportional hazards model with continuous mark.},
journal={Computational Statistics and Data Analysis},
year={2016},
volume={93},
pages={348--358},
note={PMCID: PMC4598956}
}

@article{Magaretetal2019,
author={Magaret, CA and Benkeser, D and Williamson, BD and Borate, BR and
 Carpp, LN and Georgiev, IS and Setliff, I and Dingens, AS and Simon, N and
 Carone, M and Simpkins, C and 
Montefiori, DC and Alter, G and Yu, W-H and Juraska, MJ and Edlefsen, PT and
 Karuna, S and 
Mgodi, NM and Edugupanti, S and Gilbert, Peter B},
title={Prediction of {VRC01} neutralization 
sensitivity by {HIV-1} gp160 sequence features.},
  journal={PLoS Computational Biology},
  volume={15},
  number={4},
  pages={e1006952},
  year={2019},
  note={PMCID:
    PMC6459550}
}
 
@article{Buyseetal2016,
  title={Statistical evaluation of surrogate endpoints with examples from cancer clinical trials},
  author={Buyse, Marc and Molenberghs, Geert and Paoletti, Xavier and Oba, Koji and Alonso, Ariel and der Elst, Wim and Burzykowski, Tomasz},
  journal={Biometrical Journal},
  volume={58},
  number={1},
  pages={104--132},
  year={2016},
  publisher={Wiley Online Library}
}

 

@article{Katzelnicketal2017,
  title={Antibody-dependent enhancement of severe dengue disease in humans},
  author={Katzelnick, Leah C and Gresh, Lionel and Halloran, M Elizabeth and Mercado, Juan Carlos and Kuan, Guillermina and Gordon, Aubree and Balmaseda, Angel and Harris, Eva},
  journal={Science},
  volume={358},
  number={6365},
  pages={929--932},
  year={2017},
  publisher={American Association for the Advancement of Science}
}

@article{Peguetal2017,
  title={Use of broadly neutralizing antibodies for HIV-1 prevention},
  author={Pegu, Amarendra and Hessell, Ann J and Mascola, John R and Haigwood, Nancy L},
  journal={Immunological reviews},
  volume={275},
  number={1},
  pages={296--312},
  year={2017},
  publisher={Wiley Online Library}
}

@article{GilbertFongetal2019,
  title={{HAI and NAI} titer correlates of inactivated and live attenuated influenza vaccine efficacy},
  author={Gilbert, Peter B and Fong, Youyi and Juraska, Michal and Carpp, Lindsay N and Monto, Arnold S and Martin, Emily T and Petrie, Joshua G},
  journal={BMC Infectious Diseases},
  volume={19},
  number={1},
  pages={453},
  year={2019},
  publisher={BioMed Central},
  note={PMCID: PMC6530189}
}

@article{Peguetal2019,
  title={A Meta-analysis of Passive Immunization Studies Shows that Serum-Neutralizing Antibody Titer Associates with Protection against {SHIV} Challenge},
  author={Pegu, Amarendra and Borate, Bhavesh and Huang, Yunda and Pauthner, Matthias G and Hessell, Ann J and Julg, Boris and Doria-Rose, Nicole A and Schmidt, Stephen D and Carpp, Lindsay N and Cully, Michelle D and others},
  journal={Cell Host \& Microbe},
  volume={26},
  number={3},
  pages={336--346},
  year={2019},
  publisher={Elsevier}
}


@article{Carppetal2019,
  title={Microneutralization Assay Titer Correlates Analysis in Two {Phase 3} Trials of the {CYD-TDV} Tetravalent Dengue Vaccine in {Asia and Latin America}},
  author={Carpp, LN and Fong, Y and Bonaparte, M and Moodie, M and Juraska, M and Huang, Y and Price, BL and Zhuang, Y and Shao, J and Zheng, L and Chambonneau, L and Small, R and Sridhar, S and DiazGranados, C and Gilbert, PB.},
  journal={},
  volume={},
  number={},
  pages={},
  year={Submitted}
}
	    
@article{Liuetal2016,
  title={Covariate-adjusted Spearman's rank correlation with probability-scale residuals},
  author={Liu, Qi and Li, Chun and Wanga, Valentine and Shepherd, Bryan E},
  journal={Biometrics},
  year={2017},
  volume={10.1111/biom.12812},
  publisher={Wiley Online Library}
}

@article{Keoghetal2016,
  title={Estimating time-varying exposure-outcome associations using case-control data: logistic and case-cohort analyses},
  author={Keogh, RH and Mangtani, P and Rodrigues, K and Djomo, PN},
  journal={BMC Medical Research Methodology},
  year={2016},
  volume={16(2)},
  publisher={Wiley Online Library}
}

@book{Sunetal2007,
  title={The statistical analysis of interval-censored failure time data},
  author={Sun, Jianguo},
  year={2007},
  publisher={Springer Science \& Business Media}
}

@book{Grenander1981,
author={Grenander, U},
title={Abstract Inference},
year={1981},
publisher={Wiley, New York. Wiley Series in Probability and Mathematical Statistics},
}

@article{LeskowRozanski1989,
  title={Histogram maximum likelihood estimator in the multiplicative intensity model},
  author={Le{\'s}kow, Jacek and R{\'o}{\.z}a{\'n}ski, Roman},
  journal={Stochastic Processes and their Applications},
  volume={31},
  number={1},
  pages={151--159},
  year={1989},
  publisher={Elsevier}
}

@article{Karr1987,
  title={Maximum likelihood estimation in the multiplicative intensity model via sieves},
  author={Karr, Alan F},
  journal={The Annals of Statistics},
  volume={15},
  number={2},
  pages={473--490},
  year={1987},
  publisher={Institute of Mathematical Statistics}
}

@article{LinYing1993,
  title={Cox regression with incomplete covariate measurements.},
  author={Lin, DY and Ying, Z},
  journal={Journal of the American Statistical Association},
  year={1993},
  volume={88},
  pages={1341--1349}
}

@article{ZengMaoLin2016,
  title={Maximum likelihood estimation for semiparametric transformation models with interval-censored data},
  author={Zeng, Donglin and Mao, Lu and Lin, DY},
  journal={Biometrika},
  volume={103},
  number={2},
  pages={253--271},
  year={2016},
  publisher={Oxford University Press},
  note={PMCID:
    PMC4890294}
}

@article{MaoLinZeng2017,
  title={Semiparametric regression analysis of interval-censored competing risks data},
  author={Mao, L and Lin, DY and Zeng, D},
  journal={Biometrics},
  volume={73},
  number={3},
  pages={857--865},
  year={2017},
  note={PMCID:
    PMC5561531}
}

@article{Gaoetal2019,
  title={Semiparametric Regression Analysis of Multiple Right- and Interval-Censored Events},
  author={Gao, F and Zeng, D and Couper, D and Lin, DY},
  journal={Journal of the American Statistical Association},
  volume={doi: 10.1080/01621459.2018.1482756},
  number={},
  pages={},
  year={2019}
}

@article{Zhouetal2018,
  title={Outcome-dependent sampling with interval-censored failure time data},
  author={Zhou, Q and Cai, J and Zhou, H},
  journal={Biometrics},
  volume={74},
  number={1},
  pages={58--67},
  year={2018},
  note={PMCID: PMC5797528}
}

@article{Zhouetal2017,
  title={Case-cohort studies with interval-censored failure time data},
  author={Zhou, Q and Zhou, H and Cai, J},
  journal={Biometrika},
  volume={104},
  number={1},
  pages={17--29},
  year={2017},
  note={PMCID: PMC5608290}
}


@article{GrubervanderLaan2012,
  title={An {R} package for targeted maximum likelihood estimation},
  author={Gruber, S and van der Laan, MJ}, 
  journal={Journal of Statistical Software},
  volume={51},
  number={13},
  year={2012}
}


@article{Reid1981,
  title={Estimating the median survival time},
  author={Reid, Nancy},
  journal={Biometrika},
  volume={68},
  number={3},
  pages={601--608},
  year={1981},
  publisher={Oxford University Press}
}

@article{Kochetal2018,
  title={Covariate selection with group lasso and doubly robust estimation of causal effects},
  author={Koch, Brandon and Vock, David M and Wolfson, Julian},
  journal={Biometrics},
  volume={74},
  number={1},
  pages={8--17},
  year={2018},
  publisher={Wiley Online Library}
}

@article{SaulHudgens2017,
title={The calculus of {M}-estimation in {R} with geex},
journal={},
volume={arXiv:1709.01413 [stat.AP] [Preprint] 5 Sep 2017. Last revised 5 Jan 2019. Cited 3 Sep 2019. Available from https://arxiv.org/abs/1709.01413},
author={Saul, BC and Hudgens, MG},
year={2017}
}

@book{vanderWeele2015,
  title={Explanation in Causal Inference: Methods for Mediation and Interaction},
  author={VanderWeele, Tyler},
  year={2015},
  address={New York},
  publisher={Oxford University Press}
}

@article{Branson2007,
title={State of the art for diagnosis of HIV infection},
journal={Clinical Infectious Diseases},
volume={45},
pages={S221-S225},
author={Branson, BM},
year={2007}
}

@book{Coombs2008,
  title={Clinical laboratory diagnosis of {HIV-1} and use of viral {RNA} to monitor infection. {In: Sexually Transmitted Diseases}},
  author={Coombs, RW},
  editor={Holmes, KK},
  year={2008},
  address={New York},
  publisher={McGraw-Hill}
} 

@article{HuangKarunaetal2018,
  title={Modeling cumulative overall prevention efficacy for the {VRC01} phase 2b efficacy trials},
  author={Huang, Yunda and Karuna, Shelly and Carpp, Lindsay N and Reeves, Daniel and Pegu, Amarendra and Seaton, Kelly and Mayer, Kenneth and Schiffer, Joshua and Mascola, John and Gilbert, Peter B},
  journal={Human Vaccines \& Immunotherapeutics},
  volume={14},
  number={9},
  pages={2116--2127},
  year={2018},
  publisher={Taylor \& Francis},
  note={PMCID: PMC6183277}
}

@article{LedgerwoodGraham_CEI2015,
author={Ledgerwood, JE and Coates, EE and Yamshchikov, G and Saunders, JG and Holman, L and Enama, ME and DeZure, A and Lynch, RM and Gordon, I and et al.},
title={Safety, pharmacokinetics and neutralization of the broadly neutralizing {HIV} human monoclonal antibody {VRC01} in healthy adults.},
journal={Clin Exp Immunol},
year={2015},
volume={182(3)},
pages={289--301}
}


@article{Pegu_STM2014,
author={Pegu, A and Yang, ZY and Boyington, JC and Wu, L and Ko, SY and Schmidt, SD and McKee, K and Kong, WP and Shi, W and Chen, X and et al.},
title={Neutralizing antibodies to {HIV} envelope protect more effectively in vivo than those to the {CD4} receptor.},
journal={Sci Transl Med},
year={2014},
volume={6:243ra88}
}

 Implications of 
 
1994; 139(4): 415-421.

@article{McKeown1994,
author={McKeown-Eyssen, GE and Tibshirani, R.},
title={Implications of measurement error in exposure for the sample sizes of 
case-control studies.},
journal={American Journal of Epidemiology},
year={1994},
volume={139},
number={4},
pages={415--421}
}

@article{Lemos2016,
author={Lemos, M and Naidoo, A and Fong, Y and Fleming, L and Mkhize, N and Astronomo, R and Mukudu, H and Lebina, L and Martinson, N and Ochsenbauer, C and et al.},
title={Broadly Neutralizing Antibodies Can Prevent HIV Infection in Foreskin Ex-vivo Explant Infection Models.},
journal={AIDS Res Hum Retroviruses},
year={2016},
volume={32(S1):39}
}

@article{Waghetal2016,
  title={Optimal combinations of broadly neutralizing antibodies for prevention and treatment of {HIV-1} clade {C} infection},
  author={Wagh, Kshitij and Bhattacharya, Tanmoy and Williamson, Carolyn and Robles, Alex and Bayne, Madeleine and Garrity, Jetta and Rist, Michael and Rademeyer, Cecilia and Yoon, Hyejin and Lapedes, Alan and Gao, Hongmei and Greene, Kelli and Louder, Mark K and Kong, Rui and Abdool Karim, Salim and Burton, Dennis R and Barouch, Dan H and Nussenzweig, Michel C and Mascola, John R and Morris, Lynn and Montefiori, David C and Korber, Bette and Seaman, Michael S},
  journal={PLoS Pathogens},
  volume={12},
  number={3},
  pages={e1005520},
  year={2016},
  publisher={Public Library of Science},
  note={PMCID:
    PMC4814126}
}


@article{Carlsonetal2016,
  title={Impact of pre-adapted HIV transmission},
  author={Carlson, Jonathan M and Du, Victor Y and Pfeifer, Nico and others},
  journal={Nature Medicine},
  volume={22},
  number={6},
  pages={606},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{BoppanaGoepfert2018,
  title={Understanding the CD8 T-cell response in natural HIV control},
  author={Boppana, Sushma and Goepfert, Paul},
  journal={F1000Research},
  volume={7},
  year={2018},
  publisher={Faculty of 1000 Ltd}
}

@article{Heetal2016,
  title={Follicular CXCR5-expressing CD8+ T cells curtail chronic viral infection},
  author={He, Ran and Hou, Shiyue and Liu, Cheng and Zhang, Anli and Bai, Qiang and Han, Miao and Yang, Yu and Wei, Gang and Shen, Ting and Yang, Xinxin and others},
  journal={Nature},
  volume={537},
  number={7620},
  pages={412},
  year={2016},
  publisher={Nature Publishing Group}
}

@article{Halpernetal2015,
  title={Randomized trial of four financial-incentive programs for smoking cessation},
  author={Halpern, Scott D and French, Benjamin and Small, Dylan S and Saulsgiver, Kathryn and Harhay, Michael O and Audrain-McGovern, Janet and Loewenstein, George and Brennan, Troyen A and Asch, David A and Volpp, Kevin G},
  journal={New England Journal of Medicine},
  volume={372},
  number={22},
  pages={2108--2117},
  year={2015},
  publisher={Mass Medical Soc}
}


@article{Halpernetal2015short,
  title={Randomized trial of four financial-incentive programs for smoking cessation},
  author={Halpern, Scott D and French, Benjamin and Small, Dylan S and others},
  journal={New England Journal of Medicine},
  volume={372},
  number={22},
  pages={2108--2117},
  year={2015},
  publisher={Mass Medical Soc}
}

@article{Manssonetal2007,
  title={On the estimation and use of propensity scores in case-control and case-cohort studies},
  author={M{\aa}nsson, Roger and Joffe, Marshall M and Sun, Wenguang and Hennessy, Sean},
  journal={American Journal of Epidemiology},
  volume={166},
  number={3},
  pages={332--339},
  year={2007},
  publisher={Oxford University Press}
}

@article{Linetal2000,
  title={On fitting Cox's proportional hazards models to survey data},
  author={Lin, DY},
  journal={Biometrika},
  volume={87},
  number={1},
  pages={37--47},
  year={2000},
  publisher={Oxford University Press}
}

@article{CDCguidelines2014,
  title={Laboratory testing for the diagnosis of HIV infection: updated recommendations},
  author={Branson, Bernard M and Owen, S Michele and Wesolowski, Laura G and Bennett, Berry and Werner, Barbara G and Wroblewski, Kelly E and Pentella, Michael A},
  year={2014}
}

@article{JuraskaHuangGilbert2018,
  title={Inference on treatment effect modification by biomarker response in a three-phase sampling design},
  author={Juraska, Michal and Huang, Ying and Gilbert, Peter B},
  journal={Biostatistics},
  year={2018},
  note={PMID:
    30590450; PMCID: PMC Journal –- In Process}
}


@article{ZhengvanderLaan2017,
  title={Longitudinal mediation analysis with time-varying mediators and exposures, with application to survival outcomes},
  author={Zheng, Wenjing and van der Laan, Mark},
  journal={Journal of Causal Inference},
  volume={5},
  number={2},
  year={2017},
  publisher={De Gruyter},
  note={PMCID:
    PMC5459686}
}

@article{FuGilbert2017,
  title={Joint modeling of longitudinal and survival data with the {C}ox model 
and two-phase sampling},
  author={Fu, Rong and Gilbert, Peter B},
  journal={Lifetime Data Analysis},
  volume={23},
  number={1},
  pages={136--159},
  year={2017},
  publisher={Springer},
  note={PMCID:
    PMC5035179
}
}

@article{YuWuGilbert2017,
  title={A joint model for mixed and truncated longitudinal data and survival data, with application to {HIV} vaccine studies},
  author={Yu, Tingting and Wu, Lang and Gilbert, Peter B},
  journal={Biostatistics},
  volume={19},
  number={3},
  pages={374--390},
  year={2017},
  publisher={Oxford University Press},
  note={PMCID: PMC6193623
}
}

@article{YuWuGilbert2018,
  title={New approaches for censored longitudinal data in joint modelling of longitudinal and survival data, with application to {HIV} vaccine studies},
  author={Yu, Tingting and Wu, Lang and Gilbert, Peter},
  journal={Lifetime Data Analysis},
volume={25},
  number={2},
  pages={229--258},
  year={2019},
  publisher={Springer},
  note={PMCID:
    PMC6286694
    [Delayed release (embargo): Available on 2020-04-01]}
}

@article{Heller2011,
  title={Proportional hazards regression with interval censored data using an inverse probability weight},
  author={Heller, Glenn},
  journal={Lifetime data analysis},
  volume={17},
  number={3},
  pages={373--385},
  year={2011},
  publisher={Springer}
}


@article{Leeetal2018,
  title={Analysis of generalized semiparametric regression models for cumulative incidence functions with missing covariates},
  author={Lee, U and Sun, Y and Scheike, TH and Gilbert, Peter B},
  journal={Computational Statistics and Data Analysis},
  volume={122},
  pages={59--79},
  year={2018},
  note={PMCID:
    PMC5993453}
}

@article{Earlyetal2018,
  title={Detection of low-density {P}lasmodium falciparum infections using amplicon deep sequencing},
  author={Early, AM and Daniels, RF and Farrell, TM and Grimsby, J and Volkman, SK and Wirth, DF and MacInnis, BL and Neafsey, DE},
  journal={Malaria Journal},
  year={2019},
  volume={18},
  number={1},
  pages={219},
  note={PMCID: PMC6604269}
}



@article{mccoy2017identification,
  title={Identification and specificity of broadly neutralizing antibodies against {HIV}},
  author={McCoy, Laura E and Burton, Dennis R},
  journal={Immunological Reviews},
  volume={275},
  number={1},
  pages={11--20},
  year={2017},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC5299474}
}

@article{sok2018recent,
  title={Recent progress in broadly neutralizing antibodies to {HIV}},
  author={Sok, Devin and Burton, Dennis R},
  journal={Nature Immunology},
  volume={19},
  number={11},
  pages={1179},
  year={2018},
  publisher={Nature Publishing Group},
  note={PMCID:
    PMC6440471
}
}

@article{hessell2018passive,
  title={Passive and active antibody studies in primates to inform {HIV} vaccines},
  author={Hessell, Ann J and Malherbe, Delphine C and Haigwood, Nancy L},
  journal={Expert Review of Vaccines},
  volume={17},
  number={2},
  pages={127--144},
  year={2018},
  publisher={Taylor \& Francis},
  note={PMCID:
    PMC6587971}
}

@article{pegu2017use,
  title={Use of broadly neutralizing antibodies for {HIV-1} prevention},
  author={Pegu, Amarendra and Hessell, Ann J and Mascola, John R and Haigwood, Nancy L},
  journal={Immunological Reviews},
  volume={275},
  number={1},
  pages={296--312},
  year={2017},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC5314445}
}

@article{morris2017prospects,
  title={Prospects for passive immunity to prevent {HIV} infection},
  author={Morris, Lynn and Mkhize, Nonhlanhla N},
  journal={PLoS Medicine},
  volume={14},
  number={11},
  pages={e1002436},
  year={2017},
  publisher={Public Library of Science},
  note={PMCID:
    PMC5685477}
}

@article{Barouchetal2018,
  title={Evaluation of a mosaic {HIV-1} vaccine in a multicentre, randomised, double-blind, placebo-controlled, phase 1/2a clinical trial {(APPROACH)} and in rhesus monkeys ({NHP} 13-19)},
  author={Barouch, D H and Tomaka, F L and Wegmann, F and Stieh, D J and Alter, G and Robb, M L and Michael, N L and Peter, L and Nkolola, J P and Borducchi, E N and Chandrashekar, A and Jetton, D and Stephenson, K E and Li, W and Korber, B and Tomaras, G D and Montefiori, D C and Gray, G and Frahm, N and McElrath, M J and Baden, L and Johnson, J and Hutter, J and Swann, E and Karita, E and Kibuuka, H and Mpendo, J and Garrett, N and Mngadi, K and Chinyenze, K and Priddy, F and Lazarus, E and Laher, F and Nitayapan, S and Pitisuttithum, P and Bart, S and Campbell, T and Feldman, R and Lucksinger, G and Borremans, C and Callewaert, K and Roten, R and Sadoff, J and Scheppler, L and Weijtens, M and Feddes-de Boer, K and van Manen, D and Vreugdenhil, J and Zahn, R and Lavreys, L and Nijs, S and Tolboom, J and Hendriks, J and Euler, Z and Pau, M G and Schuitemaker, H},
  journal={The Lancet},
  volume={392},
  number={10143},
  pages={232--243},
  year={2018},
  publisher={Elsevier},
  note={PMCID:
    PMC6192527
}
}

@article{shen2008dose,
  title={Dose-response curve slope sets class-specific limits on inhibitory potential of anti-HIV drugs},
  author={Shen, Lin and Peterson, Susan and Sedaghat, Ahmad R and McMahon, Moira A and Callender, Marc and Zhang, Haili and Zhou, Yan and Pitt, Eleanor and Anderson, Karen S and Acosta, Edward P and others},
  journal={Nature medicine},
  volume={14},
  number={7},
  pages={762},
  year={2008},
  publisher={Nature Publishing Group}
}

@article{williams2017initiation,
  title={Initiation of {HIV} neutralizing {B} cell lineages with sequential envelope immunizations.},
  author={Williams, W B and Zhang, J and Jiang, C and Nicely, N I and Fera, D and Luo, K and Moody, M A and Liao, H X and Alam, S M and Kepler, T B and Ramesh, A and Wiehe, K and Holland, J A and Bradley, T and Vandergrift, N and Saunders, K O and Parks, R and Foulger, A and Xia, S M and Bonsignori, M and Montefiori, D C and Louder, M and Eaton, A and Santra, S and Scearce, R and Sutherland, L and Newman, A and Bouton-Verville, H and Bowman, C and Bomze, H and Gao, F and Marshall, D J and Whitesides, J F and Nie, X and Kelsoe, G and Reed, S G and Fox, C B and Clary, K and Koutsoukos, M and Franco, D and Mascola, J R and Harrison, S C and Haynes, B F and Verkoczy, L},
journal={Nature Communications},
volume={8},
pages={1732},
  year={2017},
  note={PMCID:
    PMC5701043}
}

@article{Saundersetal2017,
  title={Vaccine induction of heterologous tier 2 {HIV-1} neutralizing antibodies in animal models},
  author={Saunders, KO and Verkoczy, LK and Jiang, C and Zhang, J and Parks, R and Chen, H and Housman, M and Bouton-Verville, H and Shen, X and Trama, AM and Scearce, R},
  journal={Cell Reports},
  volume={21},
  number={13},
  pages={3681--3690},
  year={2017},
  note={PMCID:
    PMC5777169}
}

 

 
@incollection{BenkeserCaroneGilbert2018b,
  author       = {Benkeser, D and Carone, M and Gilbert, Peter B}, 
  title        = {Targeted estimation of cumulative vaccine sieve effects},
  booktitle    = {Targeted Learning in Data Science: Causal Inference for Complex Longitudinal Studies},
  publisher    = {Chapman \& Hall Ltd },
  year         = {2018},
  editor       = {van der Laan, MJ and Rose, S},
  volume       = {},
  series       = {},
  chapter      = {},
  pages        = {165--174},
  address      = {Springer; New York},
  edition      = {},
  month        = {},
  note         = {}
}


@article{GilbertBletteetal2019,
  title={Post-randomization Biomarker Effect Modification in an {HIV} Vaccine 
Clinical Trial.},
  author={Gilbert, Peter B and Blette, B and Shepherd, BE and Hudgens, MG},
  journal={},
  volume={},
  number={},
  pages={},
  year={Submitted}
}

@article{rts2011first,
  title={First results of phase 3 trial of {RTS,S/AS01} malaria 
vaccine in {African} children},
  author={{The RTS,S Clinical Trials Partnership: ST Agnandji} and Lell, B and Soulanoudjingar, SS and Fernandes, JF and Abossolo, BP and Conzelmann, C and Methogo, BG and Doucka, Y and Flamen, A and Mordmuller, B and Issifou, S and Kremsner, PG and Sacarlal, J and Aide, P and Lanaspa, M and Aponte, JJ and Nhamuave, A and Quelhas, D and Bassat, Q and Mandjate, S and Macete, E and Alonso, P and Abdulla, S and Salim, N and Juma, O and Shomari, M and Shubis, K and Machera, F and Hamad, AS and Minja, R and Mtoro, A and Sykes, A and Ahmed, S and Urassa, AM and Ali, AM and Mwangoka, G and Tanner, M and Tinto, H and D'Alessandro, U and Sorgho, H and Valea, I and Tahita, MC and Kabore, W and Ouedraogo, S and Sandrine, Y and Guiguemde, RT and Ouedraogo, JB and Hamel, MJ and Kariuki, S and Odero, C and Oneko, M and Otieno, K and Awino, N and Omoto, J and Williamson, J and Muturi-Kioi, V and Laserson, KF and Slutsker, L and Otieno, W and Otieno, L and Nekoye, O and Gondi, S and Otieno, A and Ogutu, B and Wasuna, R and Owira, V and Jones, D and Onyango, AA and Njuguna, P and Chilengi, R and Akoo, P and Kerubo, C and Gitaka, J and Maingi, C and Lang, T and Olotu, A and Tsofa, B and Bejon, P and Peshu, N and Marsh, K and Owusu-Agyei, S and Asante, KP and Osei-Kwakye, K and Boahen, O and Ayamba, S and Kayan, K and Owusu-Ofori, R and Dosoo, D and Asante, I and Adjei, G and Adjei, G and Chandramohan, D and Greenwood, B and Lusingu, J and Gesase, S and Malabeja, A and Abdul, O and Kilavo, H and Mahende, C and Liheluka, E and Lemnge, M and Theander, T and Drakeley, C and Ansong, D and Agbenyega, T and Adjei, S and Boateng, HO and Rettig, T and Bawa, J and Sylverken, J and Sambian, D and Agyekum, A and Owusu, L and Martinson, F and Hoffman, I and Mvalo, T and Kamthunzi, P and Nkomo, R and Msika, A and Jumbe, A and Chome, N and Nyakuipa, D and Chintedza, J and Ballou, WR and Bruls, M and Cohen, J and Guerra, Y and Jongert, E and Lapierre, D and Leach, A and Lievens, M and Ofori-Anyinam, O and Vekemans, J and Carter, T and Leboulleux, D and Loucq, C and Radford, A and Savarese, B and Schellenberg, D and Sillman, M and Vansadia, P},
  journal={New England Journal of Medicine},
  volume={365},
  number={20},
  pages={1863--1875},
  year={2011},
  publisher={Mass Medical Soc},
  note={DOI:
    10.1056/NEJMoa1102287}
}


@article{rts2012phase,
  title={A phase 3 trial of {RTS,S/AS01} malaria vaccine in {A}frican infants},
  author={{The RTS,S Clinical Trials Partnership: ST Agnandji} and Agnandji, ST and Lell, B and Fernandes, JF and Abossolo, BP and Methogo, BG and Kabwende, AL and Adegnika, AA and Mordm{\"u}ller, B and Issifou, S and Kremsner, PG and Sacarlal, J and Aide, P and Lanaspa, M and Aponte, JJ and Machevo, S and Acacio, S and Bulo, H and Sigauque, B and Macete, E and Alonso, P and Abdulla, S and Salim, N and Minja, R and Mpina, M and Ahmed, S and Ali, AM and Mtoro, AT and Hamad, AS and Mutani, P and Tanner, M and Tinto, H and D'Alessandro, U and Sorgho, H and Valea, I and Bihoun, B and Guiraud, I and Kabor\'e, B and Sombi\'e, O and Guiguemd\'e, RT and Ou\'edraogo, JB and Hamel, MJ and Kariuki, S and Oneko, M and Odero, C and Otieno, K and Awino, N and McMorrow, M and Muturi-Kioi, V and Laserson, KF and Slutsker, L and Otieno, W and Otieno, L and Otsyula, N and Gondi, S and Otieno, A and Owira, V and Oguk, E and Odongo, G and Woods, JB and Ogutu, B and Njuguna, P and Chilengi, R and Akoo, P and Kerubo, C and Maingi, C and Lang, T and Olotu, A and Bejon, P and Marsh, K and Mwambingu, G and Owusu-Agyei, S and Asante, KP and Osei-Kwakye, K and Boahen, O and Dosoo, D and Asante, I and Adjei, G and Kwara, E and Chandramohan, D and Greenwood, B and Lusingu, J and Gesase, S and Malabeja, A and Abdul, O and Mahende, C and Liheluka, E and Malle, L and Lemnge, M and Theander, TG and Drakeley, C and Ansong, D and Agbenyega, T and Adjei, S and Boateng, HO and Rettig, T and Bawa, J and Sylverken, J and Sambian, D and Sarfo, A and Agyekum, A and Martinson, F and Hoffman, I and Mvalo, T and Kamthunzi, P and Nkomo, R and Tembo, T and Tegha, G and Tsidya, M and Kilembe, J and Chawinga, C and Ballou, WR and Cohen, J and Guerra, Y and Jongert, E and Lapierre, D and Leach, A and Lievens, M and Ofori-Anyinam, O and Olivier, A and Vekemans, J and Carter, T and Kaslow, D and Leboulleux, D and Loucq, C and Radford, A and Savarese, B and Schellenberg, D and Sillman, M and Vansadia, P},
  journal={New England Journal of Medicine},
  volume={367},
  number={24},
  pages={2284--2295},
  year={2012},
  publisher={Mass Medical Soc},
  note={DOI:
    10.1056/NEJMoa1208394}
}

@article{rts2014efficacy,
  title={Efficacy and safety of the {RTS, S/AS01} malaria vaccine during 18 months after vaccination: a phase 3 randomized, controlled trial in children and young infants at 11 {A}frican sites},
  author={{The RTS,S Clinical Trials Partnership: Selidji Todagbe Agnandji} and Lell, Bertrand and Fernandes, Jos\'e Francisco and Abossolo, B\'eatrice Peggy and Kabwende, Anita Lumeka and Adegnika, Ayola Akim and Mordm{\"u}ller, Benjamin and Issifou, Saadou and Kremsner, Peter Gottfried and Loembe, Marguerite Massinga and Sacarlal, Jahit and Aide, Pedro and Madrid, Lola and Lanaspa, Miguel and Mandjate, Sofia and Aponte, John J and Bulo, Helder and Nhama, Abel and Macete, Eus\'ebio and Alonso, Pedro and Abdulla, Salim and Salim, Nahya and Mtoro, Ali Takadir and Mutani, Paul and Tanner, Marcel and Mavere, Caroline and Mwangoka, Grace and Lweno, Omar and Juma, Omar Ali and Shekalaghe, Seif and Tinto, Halidou and D'Alessandro, Umberto and Sorgho, Hermann and Valea, Innocent and Ou\'edraogo, Jean Bosco and Lompo, Palpouguini and Diallo, Salou and Traore, Ousmane and Bassole, Armand and Dao, Edgard and Hamel, Mary J and Kariuki, Simon and Oneko, Martina and Odero, Chris and Otieno, Kephas and Awino, Norbert and Muturi-Kioi, Vincent and Omoto, Jackton and Laserson, Kayla F and Slutsker, Laurence and Otieno, Walter and Otieno, Lucas and Otsyula, Nekoye and Gondi, Stacey and Otieno, Allan and Ogutu, Bernhards and Ochola, Jew and Onyango, Irene and Oyieko, Janet and Njuguna, Patricia and Chilengi, Roma and Akoo, Pauline and Kerubo, Christine and Maingi, Charity and Olotu, Ally and Bejon, Philip and Marsh, Kevin and Mwabingu, Gabriel and Gitaka, Jesse and Owusu-Agyei, Seth and Asante, Kwaku Poku and Boahen, Owusu and Dosoo, David and Adjei, George and Adeniji, Elisha and Yawson, Abena Kunadu and Kayan, Kingsley and Chandramohan, Daniel and Greenwood, Brian and Lusingu, John and Gesase, Samwel and Malabeja, Anangisye and Abdul, Omari and Mahende, Coline and Liheluka, Edwin and Lemnge, Martha and Theander, Thor G and Drakeley, Chris and Mbwana, Joyce and Ansong, Daniel and Agbenyega, Tsiri and Adjei, Samuel and Boateng, Harry Owusu and Rettig, Theresa and Bawa, John and Sylverken, Justice and Sambian, David and Sarfo, Anima and Agyekum, Alex and Martinson, Francis and Hoffman, Irving and Mvalo, Tisungane and Kamthunzi, Portia and Nkomo, Rutendo and Tembo, Tapiwa and Tsidya, Gerald Tegha Mercy and Kilembe, Jane and Chawinga, Chimwemwe and Ballou, W Ripley and Cohen, Joe and Guerra, Yolanda and Jongert, Erik and Lapierre, Didier and Leach, Amanda and Lievens, Marc and Ofori-Anyinam, Opokua and Olivier, Aur\'elie and Vekemans, Johan and Kaslow, David and Leboulleux, Didier and Savarese, Barbara and Schellenberg, David.},
  journal={PLoS Medicine},
  volume={11},
  number={7},
  pages={e1001685},
  year={2014},
  publisher={Public Library of Science San Francisco, USA},
  note={PMCID:
    PMC4114488}
}



@article{theander2015efficacy,
  title={Efficacy and safety of {RTS, S/AS01} malaria vaccine with or without a booster dose in infants and children in {A}frica: final results of a phase 3, individually randomised, controlled trial},
  author={{The RTS,S Clinical Trials Partnership: H Tinto, U D'Alessandro, H Sorgho, I Valea, M C Tahita, W Kabore, F Kiemde, P Lompo, S Ouédraogo, K Derra, F Ouédraogo, J B Ouédraogo W R Ballou, J Cohen, Y Guerra, D Heerwegh, E Jongert, D Lapierre, A Leach, M Lievens, O Ofori-Anyinam, A Olivier, J Vekemans, S T Agnandji, B Lell, J F Fernandes, B P Abossolo, A L Kabwende, A A Adegnika, B Mordmüller, S Issifou, P G Kremsner, M M Loembe, E Bache, A Alabi, S Owusu-Agyei, K P Asante, O Boahen, D Dosoo, I Asante, Z Yidana, J Anim, E Adeniji, A K Yawson, K Kayan, D Chandramohan, B Greenwood D Ansong, T Agbenyega, S Adjei, H O Boateng, T Rettig, J Sylverken, D Sambian, A Badu-Prepah, A Kotey, P Buabeng, V Paintsil, A Enimil, M J Hamel, S Kariuki, M Oneko, C Odero, K Otieno, N Awino, V Muturi-Kioi, J Omoto, T Sang, S Odhiambo, K F Laserson, L Slutsker, W Otieno, L Otieno, N Otsyula, S Gondi, J Ochola, G Okoth, D C Mabunde, A Wangwe, A Otieno, J Oyieko, J Cowden, B Ogutu, P Njuguna, K Marsh, P Akoo, C Kerubo, C Maingi, P Bejon, A Olotu, R Chilengi, B Tsofa, T Lang, J Gitaka, K Awuondo, F Martinson, I Hoffman, T Mvalo, P Kamthunzi, R Nkomo, T Tembo, G Tegha, C Chawinga, T Banda, S Khan, S Mwambakulu, E Mzembe J Sacarlal, P Aide, L Madrid, S Mandjate, J J Aponte, H Bulo, S Massora, E Varela, E Macete, P Alonso, J Lusingu, S Gesase, A Malabeja, O Abdul, C Mahende, E Liheluka, M Lemnge, T G Theander, C Drakeley, J Mbwana, R Olomi, B Mmbando, S Abdulla, N Salim, A Mtoro, S Ahmed, A Hamad, S Kafuruki, R Minja, M Tanner, M Maganga, A Mdemu, C Gwandu, A Mohammed D Kaslow, D Leboulleux, B Savarese, and D Schellenberg}},
  journal={Lancet},
  volume={386},
  number={9988},
  pages={31--45},
  year={2015},
  note={PMCID:
    PMC5626001}
}

@article{bhatt2013global,
  title={The global distribution and burden of dengue},
  author={Bhatt, Samir and Gething, Peter W and Brady, Oliver J and Messina, Jane P and Farlow, Andrew W and Moyes, Catherine L and Drake, John M and Brownstein, John S and Hoen, Anne G and Sankoh, Osman and Myers, Monica F and George, Dylan B and Jaenisch, Thomas and Wint, GR William and Simmons, Cameron P and Scott, Thomas W and Farrar, Jeremy J and Hay, Simon I},
  journal={Nature},
  volume={496},
  number={7446},
  pages={504},
  year={2013},
  publisher={Nature Publishing Group},
  note={PMCID:
    PMC3651993}
}

@article{WHO2016fact,
  title={Dengue and severe dengue.  {Key facts. 15 Apr 2019.}
 {https://www.who.int/news-room/fact-sheets/detail/dengue-and-severe-dengue. Accessed 9 Aug 2018}},
  author={{World Health Organization}},
  journal={},
  year={}
}

@article{lafond2016global,
  title={Global role and burden of influenza in pediatric respiratory hospitalizations, 1982--2012: a systematic analysis},
  author={Lafond, Kathryn E and Nair, Harish and Rasooly, Mohammad Hafiz and Valente, F{\'a}tima and Booy, Robert and Rahman, Mahmudur and Kitsutani, Paul and Yu, Hongjie and Guzman, Guiselle and Coulibaly, Daouda and Armero, Julio and Jima, Daddi and Howie, Stephen RC and Ampofo, William and Mena, Ricardo and Chadha, Mandeep and Sampurno, Ondri Dwi and Emukule, Gideon O and Nurmatov, Zuridin and Corwin, Andrew and Heraud, Jean Michel and Noyola, Daniel E and Cojocaru, Radu and Nymadawa, Pagbajabyn and Barakat, Amal and Adedeji, Adebayo and von Horoch, Marta and Olveda, Remigio and Nyatanyi, Thierry and Venter, Marietjie and Mmbaga, Vida and Chittaganpitch, Malinee and Nguyen, Tran Hien and Theo, Andros and Whaley, Melissa and Azziz-Baumgartner, Eduardo and Bresee, Joseph and Campbell, Harry and Widdowson, Marc-Alain and the Global Respiratory Hospitalizations -— Influenza Proportion Positive (GRIPP) Working Group,},
  journal={PLoS Medicine},
  volume={13},
  number={3},
  pages={e1001977},
  year={2016},
  publisher={Public Library of Science},
  note={PMCID:
    PMC4807087}
}

@article{Bekkeretal2019,
  title={{Subtype C ALVAC-HIV and bivalent subtype C gp120/MF59 HIV-1 vaccine in 
low-risk, HIV-uninfected, South African adults: a phase 1/2 trial.}},
  author={Bekker, LG and Moodie, Z and Grunenberg, N and Laher, F and
 Tomaras, GD and Cohen, KW and 
Allen, M and Malahleha, M and Mngadi, K and Daniels, B and Innes, C and
 Bentley, C and Frahm, N and Morris, DE and 
Morris, L and Mkhize, NN and Montefiori, DC and Sarzotti-Kelsoe, M and
 Grant, S and Yu, C and 
Mehra, VL and Pensiero, MN and Phogat, S and DiazGranados, CA and
 Barnett, SW and Kanesa-Thasan, N and 
Koutsoukos, M and Michael, NL and Robb, ML and Kublin, JG and
 Gilbert, Peter B and Corey, L and Gray, GE and 
McElrath, MJ},
  journal={The Lancet HIV},
  volume={5},
  number={7},
  pages={e366-e378},
  year={2019},
  note={PMCID:
    PMC6028742}
}


@article{jefferys2017, 
 title={{HIV} research in the era of {P}r{EP}: The implications of {TDF/FTC} for biomedical prevention trials},
 journal={}, 
 year={2017},
 author={{Treatment Action Group: Prepared with R. Jefferys, T. Horn, and J. Johnson}},
 note={http://www.treatmentactiongroup.org/users/hiv-prep-prevention-trials}
}

@article{gilbert2017basis,
  title={Basis and statistical design of the passive HIV-1 antibody mediated prevention (AMP) test-of-concept efficacy trials},
  author={Gilbert, Peter B and Juraska, Michal and deCamp, Allan C and Karuna, Shelly and Edupuganti, Srilatha and Mgodi, Nyaradzo and Donnell, Deborah J and Bentley, Carter and Sista, Nirupama and Andrew, Philip and others},
  journal={Statistical communications in infectious diseases},
  volume={9},
  number={1},
year={2017},
  publisher={De Gruyter}
}
 
@article{bailey2013,
  title={Social justice and {HIV} vaccine research in the age of pre-exposure prophylaxis and treatment as prevention},
  author={C Bailey, Theodore and Sugarman, Jeremy},
  journal={Current HIV Research},
  volume={11},
  number={6},
  pages={473--480},
  year={2013},
  publisher={Bentham Science Publishers},
  note={PMCID:
    PMC4084567}
}
@article{hendrix2016,
  title={Dose frequency ranging pharmacokinetic study of tenofovir-emtricitabine after directly observed dosing in healthy volunteers to establish adherence benchmarks ({HPTN} 066)},
  author={Hendrix, Craig W and Andrade, Adriana and Bumpus, Namandj{\'e} N and Kashuba, Angela D and Marzinke, Mark A and Moore, Ayana and Anderson, Peter L and Bushman, Lane R and Fuchs, Edward J and Wiggins, Ilene and Radebaugh, D and Prince, HA and Bakshi, RP and Wang, R and Richardson, P and Shieh, E and McKinstry, L and Li, X and Donnell, D and Elharrar, V and Mayer, KH and Patterson, KB},
  journal={AIDS Research and Human Retroviruses},
  volume={32},
  number={1},
  pages={32--43},
  year={2016},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA},
  note={PMCID:
    PMC4692123}
}
 
@article{janes2013pursuit,
  title={In pursuit of an HIV vaccine: designing efficacy trials in the context of partially effective nonvaccine prevention modalities},
  author={Janes, Holly and Gilbert, Peter and Buchbinder, Susan and Kublin, James and Sobieszczyk, Magdalena E and Hammer, Scott M},
  journal={AIDS research and human retroviruses},
  volume={29},
  number={11},
  pages={1513--1523},
  year={2013},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA},
  note={PMCID:
    PMC3809388}
}
 
@article{jefferys2017, 
 title={{HIV} research in the era of {P}r{EP}: The implications of {TDF/FTC} for biomedical prevention trials},
 author={{Treatment Action Group. Prepared with prepared with Richard Jefferys, Tim Horn, and Jeremiah Johnson}},
 journal={}, 
 year={2017},
 note={http://www.treatmentactiongroup.org/users/hiv-prep-prevention-trials}
}

@article{gilbert2017basis,
  title={Basis and statistical design of the passive HIV-1 antibody mediated prevention (AMP) test-of-concept efficacy trials},
  author={Gilbert, Peter B and Juraska, Michal and deCamp, Allan C and Karuna, Shelly and Edupuganti, Srilatha and Mgodi, Nyaradzo and Donnell, Deborah J and Bentley, Carter and Sista, Nirupama and Andrew, Philip and others},
  journal={Statistical communications in infectious diseases},
  volume={9},
  number={1},
year={2017},
  publisher={De Gruyter}
}

@article{HalloranLonginiGilbert2020,
  title={Designing a study of correlates of risk for ebola vaccination},
  author={Halloran, ME and Longini, IM Jr. and Gilbert, PB},  
  journal={American Journal of Epidemiology},
  volume={},
  number={},
year={in press}
}
 
@article{Gilbert2019,
  title={Ongoing vaccine and monoclonal antibody {HIV} prevention efficacy trials and considerations for sequel efficacy trial design},
  author={Gilbert, Peter B},
  journal={Statistical Communications in Infectious Diseases},
  volume={In Press},
  number={},
year={2019},
  publisher={De Gruyter}
}

@article{Gilbert2019arXiv,
  title={Ongoing Vaccine and Monoclonal Antibody {HIV} Prevention Efficacy Trials and Considerations for Sequel Efficacy Trial Designs},
  author={Gilbert, Peter B},
  journal={arXiv:1906.08409},
  volume={[stat.AP] [Preprint] 20 Jun 2019. Cited 3 Sep 2019. Available from https://arxiv.org/abs/1906.08409},
  year={2019}
}

@article{Bellachetal2020,
  title={General regression model for the subdistribution of a competing risk under 
left-truncation and right-censoring},
  author={Bellach, A and Kosorok, MR and Gilbert, Peter B},
  journal={Biometrika},
  volume={},
  number={},
year={In Press}
}

@article{GilbertJuraskaetal2017,
  title={Basis and statistical design of the passive HIV-1 antibody mediated prevention (AMP) test-of-concept efficacy trials},
  author={Gilbert, Peter B and Juraska, Michal and deCamp, Allan C and Karuna, Shelly and Edupuganti, Srilatha and Mgodi, Nyaradzo and Donnell, Deborah J and Bentley, Carter and Sista, Nirupama and Andrew, Philip and Isaacs, A and Huang, Y and Zhang, L and Capparelli, E and Kochar, N and Wang, J and Mayer, KH and Magaret, CA and Hural, J and Kublin, JG and Montefiori, DC and Gomez, MM and Burns, DN and McElrath, MJ and Ledgerwood, J and Graham, BS and Mascola, JR and Cohen, M and Corey, L},
  journal={Statistical communications in infectious diseases},
  volume={9},
  number={1},
year={2017},
  publisher={De Gruyter}
}


 
@article{bailey2013,
  title={Social justice and HIV vaccine research in the age of pre-exposure prophylaxis and treatment as prevention},
  author={C Bailey, Theodore and Sugarman, Jeremy},
  journal={Current HIV research},
  volume={11},
  number={6},
  pages={473--480},
  year={2013},
  publisher={Bentham Science Publishers},
  note={PMCID:
    PMC4084567}
}
@article{hendrix2016,
  title={Dose frequency ranging pharmacokinetic study of tenofovir-emtricitabine after directly observed dosing in healthy volunteers to establish adherence benchmarks (HPTN 066)},
  author={Hendrix, Craig W and Andrade, Adriana and Bumpus, Namandj{\'e} N and Kashuba, Angela D and Marzinke, Mark A and Moore, Ayana and Anderson, Peter L and Bushman, Lane R and Fuchs, Edward J and Wiggins, Ilene and others},
  journal={AIDS research and human retroviruses},
  volume={32},
  number={1},
  pages={32--43},
  year={2016},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA}
}
 
@article{janes2013pursuit,
  title={In pursuit of an HIV vaccine: designing efficacy trials in the context of partially effective nonvaccine prevention modalities},
  author={Janes, Holly and Gilbert, Peter and Buchbinder, Susan and Kublin, James and Sobieszczyk, Magdalena E and Hammer, Scott M},
  journal={AIDS research and human retroviruses},
  volume={29},
  number={11},
  pages={1513--1523},
  year={2013},
  publisher={Mary Ann Liebert, Inc. 140 Huguenot Street, 3rd Floor New Rochelle, NY 10801 USA},
  note={PMCID:
    PMC3809388}
}
 
@article{LuncefordDavidian2004,
  title={Stratification and weighting via the propensity score in estimation of causal treatment effects: a comparative study},
  author={Lunceford, Jared K and Davidian, Marie},
  journal={Statistics in medicine},
  volume={23},
  number={19},
  pages={2937--2960},
  year={2004},
  publisher={Wiley Online Library}
}


@article{Maoetal2008,
  title={On the propensity score weighting analysis with survival outcome: Estimands, estimation, and inference},
  author={Mao, Huzhang and Li, Liang and Yang, Wei and Shen, Yu},
  journal={Statistics in medicine},
  volume={37},
  number={26},
  pages={3745--3763},
  year={2018},
  publisher={Wiley Online Library}
}
 
@article{Baetenetal2012,
  title={Antiretroviral prophylaxis for {HIV} prevention in heterosexual men and women},
  author={Baeten, Jared M and Donnell, Deborah and Ndase, Patrick and Mugo, Nelly R and Campbell, James D and Wangisi, Jonathan and Tappero, Jordan W and Bukusi, Elizabeth A and Cohen, Craig R and Katabira, Elly and Ronald, Allan and Tumwesigye, Elioda and Were, Edwin and Fife, Kenneth H and Kiarie, James and Farquhar, Carey and JHohn-Stewart, Grace and Kakia, Aloysious and Odoyo, Josephine and Mucunguzi, Akasiima and Nakku-Joloba, Edith and Twesigye, Rogers and Ngure, Kenneth and Apaka, Cosmas and Tamooh, Harrison and Gabona, Fridah and Mujugira, Andrew and Panteleeff, Dana and Thomas, Katherine K and Kidoguchi, Lara and Krows, Meighan and Revall, Jennifer and Morrison, Susan and Haugen, Harald and Emmanuel-Ogier, Mira and Ondrejcek, Lisa and Coombs, Robert W and Frenkel, Lisa and Hendrix, Craig and Bumpus, Namandje and Bangsberg, David and Haberer, Jessica E and Stevens, Wendy S and Lingappa, Jairam R and {Connie Celum, for the Partners PrEP Study Team}},
  journal={New England Journal of Medicine},
  volume={367},
  number={5},
  pages={399--410},
  year={2012},
  publisher={Mass Medical Soc},
  note={PMCID:
    PMC3770474
}
}

@article{McCormacketal2016,
  title={Pre-exposure prophylaxis to prevent the acquisition of {HIV-1} infection {(PROUD)}: effectiveness results from the pilot phase of a pragmatic open-label randomised trial},
  author={McCormack, Sheena and Dunn, David T and Desai, Monica and Dolling, David I and Gafos, Mitzy and Gilson, Richard and Sullivan, Ann K and Clarke, Amanda and Reeves, Iain and Schembri, Gabriel and Mackie, Nicola and Bowman, Christine and Lacey, Charles J and Apea, Vanessa and Brady, Michael and Fox, Julie and Taylor, Stephen and Antonucci, Simone and Khoo, Saye H and Rooney, James and Nardone, Anthony and Fisher, Martin and McOwan, Alan and Phillips, Andrew N and Johnson, Anne M and Gazzard, Brian and Gill, Owen N},
  journal={The Lancet},
  volume={387},
  number={10013},
  pages={53--60},
  year={2016},
  publisher={Elsevier},
  note={PMCID:
    PMC4700047}
}

@article{Fonneretal2016,
  title={Effectiveness and safety of oral {HIV} preexposure prophylaxis for all populations},
  author={Fonner, Virginia A and Dalglish, Sarah L and Kennedy, Caitlin E and Baggaley, Rachel and O'Reilly, Kevin R and Koechlin, Florence M and Rodolph, Michelle and Hodges-Mameletzis, Ioannis and Grant, Robert M},
  journal={AIDS (London, England)},
  volume={30},
  number={12},
  pages={1973},
  year={2016},
  publisher={Wolters Kluwer Health},
  note={PMCID:
    PMC4949005}
}

@article{Waghetal2018,
  title={Potential of conventional \& bispecific broadly neutralizing antibodies for prevention of {HIV-1} subtype {A, C \& D} infections},
  author={Wagh, Kshitij and Seaman, Michael S and Zingg, Marshall and Fitzsimons, Tomas and Barouch, Dan H and Burton, Dennis R and Connors, Mark and Ho, David D and Mascola, John R and Nussenzweig, Michel C and Ravetch, Jeffrey and Gautam, Rajeev and Martin, Malcolm A and Montefiori, David C and Korber, Bette},
  journal={PLoS Pathogens},
  volume={14},
  number={3},
  pages={e1006860},
  year={2018},
  publisher={Public Library of Science},
  note={PMCID:
    PMC5854441}
}


@article{Labuschagne2019,
  title={{hiv-founder-id. Estimate founders of HIV-1 infection using nucleotide sequences from very acute infection [cited Mar 29, 2019]}},
  author={Labuschagne, JPL},
  journal={},
  volume={},
  year={2019},
  note={https://github.com/philliplab/hiv-founder-id}
}

@article{LabuschagneEdlefsen2019,
  title={{hypermutR. R package. Version 0.0.1.0. [cited Mar 29, 2019]}},
  author={Labuschagne, JPL and Edlefsen, PE},
  journal={},
  volume={},
  year={2019},
  note={https://github.com/philliplab/hypermutR}
}

@article{baker2018predictors,
  title={Predictors of over-reporting {HIV} pre-exposure prophylaxis ({P}r{EP}) adherence among young men who have sex with men ({YMSM}) in self-reported versus biomarker data},
  author={Baker, Zo{\"e} and Javanbakht, Marjan and Mierzwa, Stan and Pavel, Craig and Lally, Michelle and Zimet, Gregory and Gorbach, Pamina},
  journal={AIDS and Behavior},
  volume={22},
  number={4},
  pages={1174--1183},
  year={2018},
  publisher={Springer},
  note={PMCID:
    PMC6038811
}
}

@article{abaasa2018utility,
  title={Utility of different adherence measures for {P}r{EP}: patterns and incremental value},
  author={Abaasa, Andrew and Hendrix, Craig and Gandhi, Monica and Anderson, Peter and Kamali, Anatoli and Kibengo, Freddie and Sanders, Eduard J and Mutua, Gaudensia and Bumpus, Namandj{\'e} N and Priddy, Frances and Haberer, Jessica E},
  journal={AIDS and Behavior},
  volume={22},
  number={4},
  pages={1165--1173},
  year={2018},
  publisher={Springer},
  note={PMCID:
    PMC5878836}
}

@Book{Yietal2017,
  author =          {Yi, GY},
  title =          {Statistical Analysis with Measurement Error or Misclassification.},
  publisher =          {Springer: New York},
  year =          {2017},
}

@article{musinguzi2016comparison,
  title={Comparison of subjective and objective adherence measures for preexposure prophylaxis against {HIV} infection among serodiscordant couples in {E}ast {A}frica},
  author={Musinguzi, Nicholas and Muganzi, Collins D and Boum, II and Ronald, Allan and Marzinke, Mark A and Hendrix, Craig W and Celum, Connie and Baeten, Jared M and Bangsberg, David R and {Jessica E Haberer, for the Partners PrEP Ancillary Adherence Study Team}},
  journal={AIDS},
  volume={30},
  number={7},
  pages={1121--1129},
  year={2016},
  publisher={Wolters Kluwer}
}

@article{salazar2017antibody,
  title={Antibody therapies for the prevention and treatment of viral infections},
  author={Salazar, Georgina and Zhang, Ningyan and Fu, Tong-Ming and An, Zhiqiang},
  journal={npj Vaccines},
  volume={2},
  number={1},
  pages={19},
  year={2017},
  publisher={Nature Publishing Group},
  note={PMCID:
    PMC5627241}
}

@article{fleming2012biomarkers,
  title={Biomarkers and surrogate endpoints in clinical trials},
  author={Fleming, Thomas R and Powers, John H},
  journal={Statistics in Medicine},
  volume={31},
  number={25},
  pages={2973--2984},
  year={2012},
  publisher={Wiley Online Library},
  note={PMCID:
    PMC3551627}
}

@article{gilbert2017basis,
  title={Basis and statistical design of the passive {HIV-1} antibody mediated prevention ({AMP}) test-of-concept efficacy trials},
  author={Gilbert, Peter B and Juraska, Michal and deCamp, Allan C and Karuna, Shelly and Edupuganti, Srilatha and Mgodi, Nyaradzo and Donnell, Deborah J and Bentley, Carter and Sista, Nirupama and Andrew, Philip and others},
  journal={Statistical Communications in Infectious Diseases},
  volume={9},
  number={1},
  year={2017},
  publisher={De Gruyter}
}

@article{doolan2009acquired,
  title={Acquired immunity to malaria},
  author={Doolan, Denise L and Doba{\~n}o, Carlota and Baird, J Kevin},
  journal={Clinical Microbiology Reviews},
  volume={22},
  number={1},
  pages={13--36},
  year={2009},
  publisher={Am Soc Microbiol},
  note={PMCID:
    PMC2620631}
}

@article{SunQietal2019,
  title={Analysis of generalized semiparametric mixed varying-coefficient effects models for longitudinal data},
  author={Sun, Y and Qi, L and Heng, F and Gilbert, Peter B},
  journal={The Canadian Journal of Statistics},
  volume={47},
  number={3},
  pages={352-373},
  url={DOI: 10.1002/cjs.11498. NIHMSID: NIHMS1022051.},
  year={2019}
}

@Article{Fangdissertation2018,
author =          {Fang, F},
title =          {IMPROVING SEMIPARAMETRIC ESTIMATION OF LONGITUDINAL DATA WITH COVARIANCE FUNCTION. {PhD dissertation (with Dr. Yanqing Sun), University of North Carolina at Charlotte}},
journal =          {},
year =          {2018},
volume =          {},
pages =          {}
}


@Article{Dengdissertation2019,
author =          {Deng, L},
title =          {ESTIMATION OF SEMIVARYING COEFFICIENT MODELS FOR COUNTING PROCESSES WITH APPLICATIONS. {PhD dissertation (with Dr. Yanqing Sun), University of North Carolina at Charlotte}},
journal =          {},
year =          {2019},
volume =          {},
pages =          {}
}


@Article{Hengdissertation2019,
author =          {Heng, F},
title =          {DYNAMIC MODELING OF INCOMPLETE EVENT HISTORY DATA. {PhD dissertation (with Dr. Yanqing Sun), University of North Carolina at Charlotte}},
journal =          {},
year =          {2019},
volume =          {},
pages =          {}
}


@Article{Chendissertation2019,
author =          {Chen, P},
title =          {STATISTICAL ESTIMATION AND INFERENCE FOR THE ASSOCIATIONS OF MULTIVARIATE RECURRENT EVENT PROCESSES. {PhD dissertation (with Dr. Yanqing Sun), University of North Carolina at Charlotte}},
journal =          {},
year =          {2019},
volume =          {},
pages =          {}
}


@article{barry_hansen_2016, title={Naturally acquired immunity to malaria}, volume={143}, DOI={10.1017/S0031182015001778}, number={2}, journal={Parasitology}, publisher={Cambridge University Press}, author={Barry, Alyssa and Hansen, Diana}, year={2016}, pages={125–128}}

@article{Sunetalsubmitted,
title={A hybrid approach for the stratified mark-specific proportional hazards models with missing covariates and missing marks, with applications to dengue vaccine efficacy trials},
author={Sun, Y and Qi, L and Fei, H and Gilbert, P B},
journal={},
note={Submitted}}


@article{ding2019decomposing,
  title={Decomposing treatment effect variation},
  author={Ding, Peng and Feller, Avi and Miratrix, Luke},
  journal={Journal of the American Statistical Association},
  volume={114},
  number={525},
  pages={304--317},
  year={2019},
  publisher={Taylor \& Francis}
}

@article{ding2016randomization,
  title={Randomization inference for treatment effect variation},
  author={Ding, Peng and Feller, Avi and Miratrix, Luke},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={78},
  number={3},
  pages={655--671},
  year={2016},
  publisher={Wiley Online Library}
}

@article{nolen2011randomization,
  title={Randomization-based inference within principal strata},
  author={Nolen, Tracy L and Hudgens, Michael G},
  journal={Journal of the American Statistical Association},
  volume={106},
  number={494},
  pages={581--593},
  year={2011},
  publisher={Taylor \& Francis}
}

@article{nolen2015analysis,
  title={Analysis of repeated low-dose challenge studies},
  author={Nolen, Tracy L and Hudgens, Michael G and Senb, Pranab K and Koch, Gary G},
  journal={Statistics in Medicine},
  volume={34},
  number={12},
  pages={1981--1992},
  year={2015},
  publisher={Wiley Online Library},
  note={PMCID: PMC4420691}
}

@article{kang2014discrete,
  title={A discrete-time survival model with random effects for designing and analyzing repeated low-dose challenge experiments},
  author={Kang, Chaeryon and Huang, Ying and Miller, Christopher J},
  journal={Biostatistics},
  volume={16},
  number={2},
  pages={295--310},
  year={2015},
  publisher={Oxford University Press},
  note={PMCID: PMC4786638}
}

@article{Neidichetal2019,
	Author = {Neidich, SD and Fong, Y and Li, S and Geraghty, D and Williamson, BD and Young, WC and Goodman, D and Seaton, KE and Shen, X and Sawant, S and Zhang, L and deCamp, A and Blette, BS and Shao, M and Yates, NL and Feely, F and Pyo, C-W and Ferrari, G and Frank, I and Karuna, ST and Swann, E and Mascola, JM and Graham, BS and Hammer, SM and Sobieszczyk, ME and Corey, L and Janes, HE and McElrath, MJ and Gottardo, R and Gilbert, PB and Tomaras, GD},  
	Journal = {Journal of Clinical Investigation},
	Pages = {},
	Title = {{Antibody Fc effector functions and IgG3 associate with decreased HIV-1 risk}},
	Volume = {in press},
	Year = {2019}}
	

@article{li2019fc,
  title={{Fc gamma receptor polymorphisms modulated the vaccine effect on HIV-1 risk in the HVTN 505 HIV vaccine trial}},
  author={Li, Shuying S and Gilbert, Peter B and Carpp, Lindsay N and Pyo, Chul-Woo and Janes, Holly and Fong, Youyi and Shen, Xiaoying and Neidich, Scott D and Goodman, Derrick and deCamp, Allan and Cohen, Kristen W and Ferrari, Guido and Hammer, Scott M and 
  Sobieszczyk, Magdalena E and Mulligan, Mark J and Buchbinder, Susan P and Keefer, Michael C and DeJesus, Edwin and Novak, Richard M and Frank, Ian and McElrath, M Juliana and Tomaras,  Georgia D and Geraghty, Daniel E and Peng, Xinxia},
  journal={Journal of Virology},
  pages={JVI--02041},
  year={2019},
  publisher={Am Soc Microbiol}
}

@article{Biswaletal2019,
  title={Efficacy of a tetravalent dengue vaccine in healthy children and adolescents},
  author={Biswal, Shibadas and Reynales, Humberto and Saez-Llorens, Xavier and Lopez, Pio and Borja-Tabora, Charissa and Kosalaraksa, Pope and Sirivichayakul, Chukiat and Watanaveeradej, Veerachai and Rivera, Luis and Espinoza, Felix and others},
  journal={New England Journal of Medicine},
  volume={381},
  number={21},
  pages={2009--2019},
  year={2019},
  publisher={Mass Medical Soc}
}

@Book{DaleyVereJones2003,
 author={Daley, D J and Vere-Jones, D},
  ALTeditor =          {},
  title ={An Introduction to the Theory of Point Processes},
  publisher =          {Springer },
  year =          {2003},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@Book{FanGijbels1996,
 author={Fan, J and Gijbels, I},
  ALTeditor =          {},
  title ={Local polynomial modelling and its applications},
  publisher =          {Chapman \& Hall Ltd },
  year =          {1996},
  OPTkey =          {},
  OPTvolume =          {},
 OPTnumber =          {},
 OPTseries =          {},
  address =          {London; New York},
  OPTedition =          {},
  OPTmonth =          {},
  OPTnote =          {},
  OPTannote =          {}
}


@article{LinWeiYangYing2000,
author={Lin, D Y and  Wei, L J and Yang, I and Ying, Z},
title ={Semiparametric regression for the mean and rate functions of recurrent events},
journal={Journal of the Royal Statistical Society, Series B},
year={2000},
volume={62},
number={},
pages={711--730},
note={}
}	  



@article{Scheike2002,
author={Scheike, Thomas H},
title ={The additive nonparametric and semiparametric {A}alen model as the rate function for a counting process},
journal={Lifetime Data Analysis},
year={2002},
volume={8},
number={},
pages={247--262},
note={}
}	  

@article{Grebe2019,
  doi = {10.1186/s12879-019-4543-9},
  
url = {https://doi.org/10.1186/s12879-019-4543-9},
  year = {2019},
  
month = oct,
  publisher = {Springer Science and Business Media {LLC}},
  
volume = {19},
  number = {1},
  pages={894},
  author = {Eduard Grebe and 
Shelley N. Facente and Jeremy Bingham and Christopher D. Pilcher and 
Andrew Powrie and Jarryd Gerber and Gareth Priede and Trust Chibawara 
and Michael P. Busch and Gary Murphy and Reshma Kassanjee and Alex Welte},
  
title = {Interpreting {HIV} diagnostic histories into infection time estimates: 
analytical framework and online tool},
  journal = {{BMC} Infectious Diseases},
  
note={PMCID: PMC6815418
}
}


@article{BakoyannisEtAl2017,
author = {Bakoyannis, Giorgos and Yu, Menggang and Yiannoutsos, Constantin T.},
title = {Semiparametric regression on cumulative incidence function with interval-censored competing risks data},
journal = {Statistics in Medicine},
volume = {36},
number = {23},
pages = {3683-3707},
keywords = {competing risks, cumulative incidence function, interval censoring, semiparametric efficiency, R function},
doi = {10.1002/sim.7350},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/sim.7350},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/sim.7350},
abstract = {},
year = {2017}
}
 
 
@article{HudgensEtAl2001,
author = {Hudgens, Michael G. and Satten, Glen A. and Longini Jr., Ira M.},
title = {Nonparametric Maximum Likelihood Estimation for Competing Risks Survival Data Subject to Interval Censoring and Truncation},
journal = {Biometrics},
volume = {57},
number = {1},
pages = {74-80},
keywords = {Competing risks, Cumulative incidence function, HIV subtypes, Interval censoring, Nonparametric maximum likelihood, Pseudolikelihood, Truncation},
doi = {10.1111/j.0006-341X.2001.00074.x},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/j.0006-341X.2001.00074.x},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/j.0006-341X.2001.00074.x},
abstract = {},
year = {2001}
}
 
 
@article{HudgensLiFine2014,
author = {Hudgens, Michael G. and Li, Chenxi and Fine, Jason P.},
title = {Parametric likelihood inference for interval censored competing risks data},
journal = {Biometrics},
volume = {70},
number = {1},
pages = {1-9},
keywords = {Competing risks, Cumulative incidence function, Gompertz, HIV/AIDS, Maximum likelihood},
doi = {10.1111/biom.12109},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1111/biom.12109},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1111/biom.12109},
abstract = {},
year = {2014}
}
 
 
@article{Li2015,
author = {Li, Chenxi},
year = {2015},
month = {11},
pages = {327-344},
title = {The Fine-Gray Model Under Interval Censored Competing Risks Data},
volume = {143},
journal = {Journal of multivariate analysis},
doi = {10.1016/j.jmva.2015.10.001}
}

@article{Halloranetal2020,
    author = {Halloran, M Elizabeth and Longini, Ira M and Gilbert, Peter B},
    title = "{Designing a Study of Correlates of Risk for Ebola Vaccination}",
    journal = {American Journal of Epidemiology},
    year = {2020},
    month = {01},
    abstract = "{The rVSV Ebola vaccine was shown to be very efficacious in a novel ring vaccination trial in Guinea. However, no correlates of vaccine protection have been established for Ebola vaccines. Several Ebola vaccine candidates are available, but conducting randomized trials of additional candidates in outbreaks is difficult. Establishing correlates of vaccine protection is essential. Here we explore power and sample size calculations to evaluate potential correlates of risk during an Ebola vaccination campaignin an outbreak. The method requires a blood draw be made at a predetermined time after vaccination. The statistical analysis estimates the relative risk of the Ebola endpoint occurring after the blood draw through to the end of follow-up, contrasting vaccine recipients with different values of the immune response marker. The analysis can be done assuming a trichotomous or continuous marker. Under certain assumptions, at an overall vaccine efficacy of 75\\%, 50 Ebola endpoints in the vaccinees provided good power. At an overall vaccine efficacy of 90\\%, 20 Ebola endpoints gave good power. Power was highest when more vaccinees were in the high and low responder groups versus the middle group and when vaccine efficacy differed the most between the high and low responder groups.}",
    issn = {0002-9262},
    doi = {10.1093/aje/kwaa001},
    url = {https://doi.org/10.1093/aje/kwaa001},
    note = {kwaa001},
    eprint = {https://academic.oup.com/aje/advance-article-pdf/doi/10.1093/aje/kwaa001/31945166/kwaa001.pdf},
}
 


